Deformations and second-order rigidity of polytopes

We study deformations of polytopes that preserve edge lengths and face coplanarities. This gives rise to a notion of rigidity, for which we develop a second-order theory together with an effective algorithm for testing second-order rigidity symbolically. The strength of these new tools is demonstrated on several polytope classes, including the previously intractable regular dodecahedron, which we find to be rigid. We also find that a single tested polytope evades our techniques and will therefore provide a simple test case for future developments of tools of even higher order. This paper also contains a study of so-called edge-length perturbations. We point out connections between rigidity and the ability to realize polytopes with slightly perturbed edge lengths. To explore these connections in practice, we dedicate a section to another case study of the regular dodecahedron. We investigate the local behavior of its realization space with a view towards edge-length perturbations, singularities and generic global rigidity.

==> sec/Introductio_-_copy_-_2026-06-23.tex <==

%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}


\vspace*{-1em}

\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities.
If such deformations exist, the polytope is said to be flexible, otherwise rigid.
Classical results in polyhedral rigidity (such as the rigidity theorems by Cauchy \cite{cauchy1813} or Dehn \cite{dehnstheorem}) enforce the stronger constraint of fixed face shapes, and then find that convexity generally implies rigidity.
This is in contrast to our setting, in which flexible convex polytopes do exist.
Still, only few techniques are known to construct such.


\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}
%
As a consequence, the sentiment arose that this sort of flexibility is still rather exceptional, not only among combinatorial types of polytopes, but also among~realizations of a fixed type.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that~in~dimension at least three, a \textit{generic} convex polytope of a given combinatorial type~is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques.
This already holds for polytopes with relatively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article, we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes a suitable second-order theory as~well as an effective algorithm for testing second-order rigidity of concrete examples.
For a demonstration, we analyze the rigidity properties of the Platonic, Archimedean and Catalan solids (see \cref{tab:comparison} and \cref{tab:catalan-comparison}). 
In particular, we decide the previously unknown rigidity properties of the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left).
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be determined by our techniques, but seems to require techniques of even higher order. It will thus serve as a simple test case for future theoretical and computational developments.
%
We find it remarkable that such varied rigidity behaviors can already be observed in classical examples.

This article is divided into theoretical, methodological, and experimental results,
of which we give an overview below.
%

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (10.25,-2) {Chapter 5};

\node[fill=white] (c6) at (12,2)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,2)  {Chapter 7};

\node[fill=white] (c9) at (20.2,0) {Chapter 9};
% Nodes
\node[
    draw=blue!30,
    fill=blue!20,
    rounded corners,
    fit=(c3)(c6)(c5),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=red!30,
    fill=red!20,
    rounded corners,
    fit=(c7)(c8),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=green!30,
    fill=green!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (intro) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{appendix:comp-data-dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (10.25,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,2)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,2)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.2,0) {\Cref{sec:dodecahedron}};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (c9);

\draw[->,dashed] (c10) to[bend left=-5] (intro);
\draw[->,dashed] (app) -- (c9);
\draw[->,dashed] (c9) -- (intro);
\end{tikzpicture}
\end{figure}
\vspace*{-1.65em}
}

\subsection{Theoretical results}
\label{sec:intro-theory}


In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics, and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions/flexes,\nls and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory}~we develop the second-order theory for polytope rigidity.
We provide analogues~for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cf\ \cref{res:sotest}).

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated by the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to rigidity and first-order rigidity.




\subsection{Methodological results}
\label{sec:intro-methods}
In \cref{section:second-order-rigidity-check}, we provide a concrete method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.

In \cref{sec:so_rigidity_dod} we give a step-by-step account of how to apply our second-order~rigidity certificate to the regular dodecahedron. We thereby verify that it is indeed rigid (\cf\ \cref{dodecahedronrig}), answering a question posed in \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

Analogous computations are performed for the other test polytopes and are~documented in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
We highlight two results: We show that, besides the dodecahedron, also the \textit{truncated icosahedron} (\cref{fig:Dod_TIco_TDod}, center) is not first- but second-order rigid. We also show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and thus its rigidity status remains open.
A detailed explanation of the tables and a discussion of the results follow in \cref{sec:experimental_results}.
Further theoretical background on the observed flexes and flex space dimensions is given in \cref{sec:dimension_estimates}.
All code and additional animations of the flexible polytopes are included in the Supplementary Material~\cite{zenodo_suppMaterial}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to~another case study of the regular dodecahedron.
We investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations and deformation paths using tools from Riemannian geometry and homotopy continuation (with more details given in \cref{sec:approx_continuous_motions}).
We also conclude that the dodecahedron is not generically globally rigid.





\tempnewpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article, let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is~a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and~a~\Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
For computational convenience, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}

\begin{align*}
\real(\mathcal P)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions, $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ does not allow facet hyperplanes to pass~through the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

The \Def{Lie group of Euclidean isometries} (\ie\ rotations and translations), denoted $\Iso$, acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
\end{align*}











% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.



    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, the Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
%
%
For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks.
Consequently, much of what we say here applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}







\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a geometric constraint system studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence~provides heuristics and criteria that can be efficiently checked in practice.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from the rigidity~matrix.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
\end{align}
%
%
Similar to the framework setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).


First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}


\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
\end{corollary}
%
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:


\begin{theorem}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}


This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible, then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends at $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms~of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a largest~integer $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    The converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}



\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second, and equally important, first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for the sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a Hookean spring with a spring constant given by the stress $\omega_{ij}$ at $ij\in E$. The spring constant determines the magnitude of the force with which the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign of $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be thought of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying signs from facet to facet.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}


Like first-order motions, stresses form a linear space -- the \Def{stress space}.
Stresses are particularly relevant in second-order theory (see \cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).


\begin{proposition}
    \label{res:flex_eq_stress}
    If $P \subset\RR^3$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}



The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.



\section{Second-order theory}
\label{sec:second_order}
\label{sec:second-order-theory}

Second-order rigidity theory investigates deformations that preserve constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
For that, we follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if $(\bsdot p,\bsdot a)$ forms a first-order motion and additionally the following equations hold:
%
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$},
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    \label{res:second-order-implies-rigid}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:first_order}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking the curve selection lemma \cite[Lemma 18.3]{algebraicapproximationcurves}, we obtain an analytic flex $P^t$.
    There is then a largest integer $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \,\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j),\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i,\, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,\,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:first_order}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system.
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently whether $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows us to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.




\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

\end{proof}


Following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 


\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}



\tempnewpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

For this section, we restrict ourselves to polyhedra, \ie\ 3-dimensional polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polyhedra, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization, the trivial first-order motions form a 6-dimensional subspace of the space of first-order motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$.  
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
In other words, all polyhedra have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. 
Since rigid realizations correspond to isolated points in $\mreal^*(\mathcal{P},P)$, the degrees of freedom in $\realR(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.
    
\begin{definition}
\label{def:edge-length-perturbations}
The
 \Def{edge length vector} of $P$ is given by
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

%
Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.

Let us first consider an example of the first-order rigid regular tetrahedron. For this polyhedron, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    As a polytope, it is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polyhedron is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$, as a bar-joint framework, meaning that the removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the corresponding value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polyhedron's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polyhedra concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid polyhedron $P$ has all edge length perturbations.
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). 
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of polyhedra are first-order rigid.  
This result requires a suitable definition of \emph{genericity}, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polyhedra to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 


\begin{corollary}
    Generic realizations of polyhedra have all edge length perturbations.
    \begin{proof}
        Take any polyhedron $P$. In \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polyhedron is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polyhedron in the following example. This example highlights that not all realizations of a polyhedron have all edge length perturbations.

\begin{example}
\label{ex:cube-edge-length-perturbations}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polyhedron, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    antipodal edges. 
\end{example}

We can turn the observation from this example, that not all polyhedra admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polyhedron's edge length vector to distinct polyhedra sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the polyhedron $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        Assume now that all of $P$'s edge length perturbations are realizable via 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. As a consequence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi=\varphi^{-1}\circ(\varphi\circ \psi)$ and $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        
        Consequently, there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ through the realization $P$ which preserves the edge lengths ${\bs\ell}(P)$, so $P$ is rigid. 
    \end{proof}
\end{theorem}
%
The assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets us continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. This restricts the family of admissible polyhedra.

Since \Cref{thm:rigidity-and-edge-length-perturbations} provides a sufficient condition for the rigidity of polyhedra, its contrapositive yields information about the reduced realization space $\realR(\mathcal{P})$. This observation is sufficiently useful to state explicitly as a corollary. Albeit, it is currently unclear whether checking the theorem's preconditions offers any advantage over directly verifying a polyhedron's rigidity or flexibility.

\begin{corollary}
    If a polyhedron $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}
%
Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample. 
\begin{remark}
\label{res:square_root_branching}
Consider $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.
\end{remark}

However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 

The correspondence between the edge length realization space of a polyhedron and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polyhedron is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polyhedron $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization~of a polyhedron have all edge length perturbations?
\end{question}







\pagebreak

\tempnewpage

\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}
\label{sec:so_certificate}

As laid out in \Cref{sec:second-order-theory}, any first-order flex of a polytope 
that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. 
That is, according to \Cref{res:sotest}, there exists a first-order flex $\dot P$ so that for all equilibrium stresses $\bs \xi$ we have $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$.
Conversely, if for each $\dot{P}$ there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$, then the polytope is 
%\notodo{\mwsays{In fact, PSS. Is this the proper converse that you want to state here?} \mhsays{Good catch, thanks.}}
second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the first-order flex space via a basis ${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ with variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ with variables $\mu=(\mu_1, \dots, \mu_s)$. 
This turns the second-order condition \eqref{block} into the cubic polynomial% of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, the homogeneous polynomial $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.
%
%
By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is non-zero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. 
Therefore, the first-order flexes that are not blocked by any stresses can be parametrized by the solutions of the %\mhsays{square}
polynomial system $Q_1=\dots= Q_s=0$, which form an algebraic set. %\todo{\mwsays{Is this clear?}}
This system can also be represented by the gradient of $E_{\dot{P},{\bs\xi}}$ with respect to $\mu$ to obtain $\nabla_\mu E_{\dot{P},{\bs\xi}}(\lambda)=0$.

We will later see that the zero-dimensionality of the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$ is sufficient for second-order rigidity. As a criterion for that, we formulate the following. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field 
        $\Bbbk$ and let $\mathcal{I}=\langle f_1,...,f_s\rangle$ be an ideal in $\Bbbk[x_1,..,x_r]$. Let $\mathcal{G}$ be a Gröbner basis of $\mathcal{I}$. Then, $\mathcal{I}$ is zero dimensional if and only if for every $i\in\{1,...,r\}$ some power of $x_i$ is the leading monomial of an element of $\mathcal{G}$.
    \end{lemma}

Of course, there are also other methods based on Gröbner bases to verify that an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic set $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homogeneous, it holds that \[\left(Q_1(c\cdot \lambda^*),\,\dots,\,Q_s(c\cdot \lambda^*)\right)=\left(c^2\cdot Q_1(\lambda^*),\,\dots,\,c^2\cdot Q_s(\lambda^*)\right)= 0\] 
for any $c\in \mathbb{C}$ and any $\lambda^*\in \mathcal{V}(\mathcal{I})$. In other words, all scalar multiples $c\cdot\lambda^*$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\{0\}$.
In our context, this translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system 
    $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ defined in \eqref{eqn:stress_polynomial_Qi} only has $\lambda_1=\dots=\lambda_r = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)=0$.
\end{proposition}

The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all polytopes tested in \cref{sec:experimental_results} (\cf\ \Cref{tab:comparison} and \ref{tab:catalan-comparison}). Still, 
our result using Gröbner bases is clearly not necessary for second-order rigidity, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})=\{0\}$ over the real numbers, even when we find non-trivial solutions over $\mathbb{C}$. A simple counterexample is given by the equation $x^2+y^2=0$, which only has $x=y=0$ as a real solution, but has the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solutions on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}). By appending the equation $\sum_{i=1}^r\lambda_i^2-1$ to the ideal $\mathcal{I}$ which describes the unit hypersphere, we guarantee that this approach only finds non-trivial solutions. We also do not lose any solutions beyond the origin due to the invariance of solutions under scalar multiplication.

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a $\mu\in \mathbb{R}^s$ defining a 
stress ${\bs\xi}=\sum_{j=1}^s \mu_j\cdot {\bs\xi}_j$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu_j$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix
%
$$\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_j\lambda_k}Q_j(\lambda)\right)_{j,k=1}^r$$
%
is positive definite for some choice of $\mu$. 






\tempnewpage

\section{Second-order rigidity of the regular dodecahedron}
\label{sec:so_rigidity_dod}

Among the Platonic solids, there is only one for which the question of rigidity is not answered immediately.
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid by Dehn's theorem \cite{dehnstheorem}. 
The cube is the classical example of~a~flexible polytope.
Solely the regular dodecahedron remains to be understood and initially eluded direct computation.

Symbolic computations reveal a 5-dimensional space of first-order flexes and a~5-dimensional space of stresses.\footnote{The specific embedding and orderings of vertices, edges and faces are provided in \cref{appendix:comp-data-dodecahedron}.}
%
Note that these dimensions must be identical~due~to \cref{res:flex_eq_stress}.
%
It is tempting to somehow relate the dimensions of the flex and stress spaces to the 5-fold symmetries of the dodecahedron.
We have no evidence~for such a relation, and instead found rather mild counter-evidence in the case of the truncated~dode\-cahedron (see \cref{sec:selected_rigidity}).


Since the regular dodecahedron is not first-order rigid, it is a promising test case for the second-order certificate from \cref{sec:so_certificate}.
Concretely, \cref{prop:stress-energy-condition} asserts that it suffices to compute the zeros of a certain polynomial system. 
We~proceed~as follows:
%
\begin{enumerate}
    \setlength{\itemsep}{0.7ex}
    \item 
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. 
    Using the~bases, we parametrize the spaces by variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$.
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadratic forms $Q_i$. % (see \cref{section:second-order-rigidity-check}).
    
    \item Use the equivalence in \cref{gbasis} to determine whether the system~has~fi\-nitely many (real) zeros.
    This is the case for the regular dodecahedron.
    
    \item Use \Cref{prop:stress-energy-condition} to infer second-order rigidity.
\end{enumerate}

    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}.
    For more specifics on the relevant \textsc{Mathematica} files, see \cref{appendix:comp-data-dodecahedron}.
    With the help of this Gröbner basis, we obtain the following results:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        The monomials $\lambda_1^2$, $\lambda_2^3$, $\lambda_3^3$, $\lambda_4^5$,  $\lambda_5^6$, appear as leading monomials in the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$.
        \Cref{gbasis} therefore implies that $\mathcal{I}$ is zero-dimensional. 
        %By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). 
        Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. 
        By \cref{prop:stress-energy-condition}, for any non-zero linear combination of the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. 
        By \Cref{res:sotest}, $P$ is second-order rigid. 
        By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

Having understood the rigidity properties of the Platonic solids, a natural move is to extend the search to the next best well-documented classes of polytopes -- the Archimedean and Catalan solids.
A detailed account of the findings is given~in~\cref{sec:archimedean} (see also \cref{tab:comparison} and \cref{tab:catalan-comparison}).

Among the 31 polytopes checked, only three are not first-order rigid, but also not predictably flexible (\cf\ \cref{sec:dimension_estimates}): the regular dodecahedron, the truncated icosahedron and the truncated dodecahedron (\cf\ \cref{fig:Dod_TIco_TDod}).
The procedure above was applied to all of them, and our findings are documented in \cref{sec:selected_results}.\todo{\mhsays{Should we also refer to Appendix C for the truncIco and truncDod?}}








\tempnewpage

\section{Computational results: Platonic, Archimedean and Catalan solids}
\label{sec:experimental_results}
\label{sec:archimedean}


We apply our techniques to the Platonic, Archimedean, and Catalan~solids.\nls
For these classes, combinatorial data and algebraic vertex and normal coordinates are readily available.%
%
\todo{\mhsays{Does the footnote contradict the previous footnote?}}
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}
%
The results are shown in \cref{tab:comparison} (for the Platonic and Archime\-dean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation of the content of the tables is given in \cref{sec:explain_table}.
%
%
A key takeaway is that even simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
See \cref{sec:selected_results}, \ref{sec:rigidity_comments} and \ref{sec:selected_flexibility}~for a discussion of the results.


\newpage
\vspace*{6mm}
\input{sec/table1}
\newpage

\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{1ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semidefinite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
    A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate for our setting.
    
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flex space} as introduced in \cref{sec:first_order}.
    In some cases we have a good understanding of how~the~dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension. 
    If further explanations are available, this is indicated by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and further theoretical background is provided in \cref{sec:dimension_estimates}.
\end{enumerate}
%
The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{1ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension of the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
\end{itemize}
%
Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
Again,\nls details are given in \cref{sec:dimension_estimates}.



\pagebreak

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding table cells are marked with \Star):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} have identical~rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes) nor prestress stable; yet, \emph{both are second-\mbox{order} rigid}. 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct concepts.
    Previous examples of this distinction were compa\-ratively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
 In fact, we verified symbolically that for all quadratic forms in~\eqref{eqn:stress_polynomial_Qi} we have $Q_i=0$. Second-order flexibility then followed via \cref{prop:stress-energy-condition}.
    %
    Since at this time no 
    methods exist to test rigidity beyond the second order, we do not know whether the truncated dodecahedron is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). 
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above is sensitive to small changes in their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.

\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty of non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priori.
We therefore formulate the following question:

\begin{question}
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps polytopes whose faces are triangles and 4-gons are simple enough for a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained by actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} match the values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.





\input{sec/table2}









% \tempnewpage

\pagebreak

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}

Due to its previous status as the guiding example,
%
we single out the dodecahedron once again for a closer inspection.
%
Exploring its realization space close to the regular dodecahedron helps us better understand the source of its exceptional behavior.
%
From that, we draw conclusions about the global rigidity of the polytope.






\subsection{Deformation paths}
\label{section:dodec-edge-length-perturbations}


%
By the Legendre-Steinitz theorem the reduced realization space $\realR(\mathcal{P})$ of the dodecahedron is a smooth $30$-dimensional manifold. 
The dodecahedron is rigid by \Cref{dodecahedronrig}, suggesting that these 30 degrees of freedom translate directly into changes in the lengths of its 30 edges.
Although we formulate the hope that all edge length perturbations of rigid polytopes are realizable in \Cref{conj:edge_length_perturbations}, even for the regular dodecahedron it is completely unclear whether this statement is true.

Due to dodecahedron's high symmetry (all edges are the same), one might suggest to deform a single edge and, if this is possible, to conclude that arbitrary perturbations are possible.
In this section, we investigate the deformations of the regular dodecahedron induced by shrinking or extending a single edge. 
By approximating such deformation paths using methods explained in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of this polytope $P$ in $\realR(\mathcal P)$. 
However, whether this implies that all edge length perturbations are possible must remain open.

For this experiment, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert~ < 1$. 
Sampling from the realization space intersected with the real algebraic set of prescribed edge lengths reveals \textit{six} distinct arcs starting at the regular dodecahedron corresponding to the shrinking of a single edge and \textit{two} corresponding to its expansion (see also \cite{deformationpaths}). 

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by perturbing a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge contractions, whereas gray curves correspond to edge expansions. On these curves, the eight corresponding realizations at $\ell^*(\pm 0.25)$ are depicted. Four realizations are connected by a nodal cubic (dark blue dashes).}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
 
%
%
In \Cref{fig:edge-contraction-deformation-space}, we depict a random projection of the deformations induced by edge contractions 
(blue) and expansions (gray), alongside eight realizations at $\ell^{\star}(\pm 0.25)$.
Remarkably, it appears that some of these arcs rejoin smoothly. 
For instance, the gray arcs corresponding to an edge expansion have the same tangent in the regular dodecahedron, and so do suitable pairs of arcs of the blue curves. 
Moreover, the arcs corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (dark blue dashed curve).
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron since there are multiple realizations with the same edge lengths arbitrarily close to the regular dodecahedron. Hence, it is possible that there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$ in this case (\cf\ \Cref{res:square_root_branching}). 
%

In total, three curves are passing through the regular dodecahedron that are induced by length changes of a single edge. 
Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective sum of the tangent vectors is sufficiently close to zero. 
We attach an animation of the smooth deformation passing through the regular dodecahedron on the solid blue path from $\ell^*(-0.25)$ via $\ell^*(0)$ to $\ell^*(-0.25)$ in the Supplementary Material \cite{zenodo_suppMaterial} of this article.

Additionally, we find that in the case of edge contractions there are two types of deformations: those that react to the edge contraction by flattening horizontally (see \Cref{fig:edge-contraction-deformation-space}, top) and those that flatten vertically (see \Cref{fig:edge-contraction-deformation-space}, bottom). Both types contain one realization with two reflection symmetries, and two realizations with only one reflection symmetry that are mutual mirror images of each other. 
        Intriguingly, not all dodecahedra persist until the edge collapses to length zero. 
        The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations below this particular edge length. 
        %
        %
        All of them persist until $\ell^*(-1)=0$. 


        Conversely, expanding an edge only produces two realizations with distinct reflection axes. 
        They are depicted on the left and right of \Cref{fig:edge-contraction-deformation-space}. 
        %
        Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.



\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytope is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore~globally rigid.
%
This leaves open the possibility of generic global rigidity. 

A polytope is called \Def{generically globally rigid} if every generic 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
First, we confirmed numerically that all of the equivalent realizations which are 
depicted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. 
Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently close generic realization of the dodecahedron.
Hence, generic realizations are also not necessarily globally rigid.
%
Notably, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}


It would be surprising, though also not absurd, if other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{12mm}
    \begin{minipage}[c]{0.32\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edge have the same length (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}





\tempnewpage % temporary new page

\section{Conclusion}
\label{sec:outlook}


In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 


\subsection{Main results}

We carefully develop a first-order and second-order theory for the rigidity of polytopes in \Cref{sec:first_order,sec:second-order-theory}. 
Using these tools, we demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. 
Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 
A well-developed second-order theory is important since it is right at the boundary of what is practically possible: analogous statements are no longer true for naive higher-order rigidity criteria (see \Cref{sec:higher_order_rigidity}). 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves induced by edge length modifications.


Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. 
%\notodo{\mwsays{Sec 9 has changed}\mhsays{Done.}}
In \Cref{sec:so_rigidity_dod}, we explicitly demonstrate a strategy for proving the second-order rigidity of the regular dodecahedron as a test case. Moreover, we investigate deformations induced by modifying the length of a single edge in \Cref{sec:dodecahedron}, which reveals a highly interesting local geometry and also serves as a counterexample to the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}


Among the 31 polytopes we considered, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is 4-dimensional, so it is not first-order rigid.
We also determine that it is not second-order rigid, since the associated system of homogeneous quadratic equations $Q_1=\dots=Q_4=0$ arising from \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. 
In fact, we 
find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish whether it is flexible or rigid.

In \Cref{fig:TDod_flex_conc}, we depict samples from a numerically generated deformation of the truncated dodecahedron.
It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances.
%
%\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}
%
However, when we apply a more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
\label{sec:higher_order_rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
This result would help explain why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which 
satisfies the edge length and facet planarity constraints with reasonably small numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, the authors observe that the energy landscape around an $N$-th order rigid realization locally looks like the 
polynomial curve $y=x^{2N}$. This implies that, for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

If the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity, and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 


==> sec/Introduction_-_copy_-_2026-06-17.tex <==

%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}

\todo{\mhsays{Abstract: Replace at least one of the ``we'' alliterations by a different beginning. Fix overful. \mwsays{Will do.} }}


\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities (\ie\ it is flexible) or not (\ie\ it is rigid).
%. The major difference to the classical setting of polyhedral rigidity is that these deformations are explicitly 
These assump\-tions are weak in comparison to classical polyhedral rigidity, which also enforces fixed face shapes. %\todo{\mhsays{I don't understand this sentence.}\mwsays{Sorry, what exactly is unclear?}\mhsays{I understand what you want to say here, but ``weak'' is always slightly confusing to me as a non-logician. Maybe ``are more restrictive'' or ``are implied by the flexibility in classical polyhedral rigidity''?}}%\todo{\mhsays{Should we highlight rigidity in the first sentence of the introduction, too? Currently it is only about flexibility.}}
While flexible polytopes exist in this setting, still only few techniques are known to construct such. %polytopes that admit such deformations.%\mhsays{and which polytopes do not admit continuous deformations? (to highlight rigidity and not just flexibility.)}.

\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}

As a consequence, the sentiment arose that this sort of flexibility is exceptional, not only among combinatorial types of polytopes, but also among realizations of a fixed type.
%Only few classes of flexible polytopes are known, constructed from a handful of techniques such as Minkowski sums and affine transformations.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that in dimension~at~least three, a \textit{generic} convex polytope of a given combinatorial type is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

%\mwsays{Add picture with Dod, TDod, TIco}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
%     \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically. \mhsays{Suggestion: Move to Conclusion and replace image by truncated dodecahedron, dodecahedron and truncated icosahedron, since they are special.}}
%     \label{fig:TDod_flex}
% \end{figure}

%\todo{\mhsays{I do not think anymore that the first page is a good place for a flex, for which we have strong evidence against being a true polyhedral flex. This may generate false expectations. I would prefer putting it in the conclusion/outlook as future work and focusing on the examples that we can actually solve.}}
Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
%The previous exploration therefore focused on first-order and generic rigidity.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques. %, such as a naive Gröbner basis approach. %, and so it remains unknown whether they are rigid or admit continuous deformations.
This already holds for polytopes with realtively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes the formulation of a suitable second-order theory, \todo{\mwsays{As I understand section 7, we do not develop new tracing tools here}\mhsays{Technically no, but also yes.}\mwsays{I will rewrite to: we use/generalize what exists.}}as well as computational tools for tracing deformation paths.
For a demonstration we apply these techniques to the Platonic, Archimedean and Catalan solids, deciding their rigidity in all but one case (see \cref{tab:comparison}). In particular,\nls we~decide the previously unknown rigidity properties of the regular dodecahedron.
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be characterized by our techniques. 
Solving this question  will require techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
%
We found it remarkable that such variety of rigidity behaviors can already be observed among classical examples.
%This is not for lack of computations resources, but rather 
%In particular the truncated dodecahedron can serve a surprisingly simple test case for future theoretical and computational developments.
%Merely the \emph{truncated dodecahedron} (see \cref{fig:TDod_flex}, left) evades our approaches. The reason though is interesting, and is of a technical nature rather than from computational limitations.


% \mwsays{The first article develops first- and generic theory. In this article we address notions of rigidity skipped over in the first part: second-order, continuous and global.}

This article divides into theoretical, methodological and experimental results,
of which we give an overview below.\todo{\mhsays{We can also leave the introduction out or replace it by Table 1/2. The structure of our paper may be slightly confusing and this is an attempt at making the structure clearer. I am \textit{very} open to suggestions here on how to organize the roadmap.}\mwsays{Let's decide this at the end.}}

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (10.25,-2) {Chapter 5};

\node[fill=white] (c6) at (12,2)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,2)  {Chapter 7};

\node[fill=white] (c9) at (20.2,0) {Chapter 9};
% Nodes
\node[
    draw=blue!30,
    fill=blue!20,
    rounded corners,
    fit=(c3)(c6)(c5),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=red!30,
    fill=red!20,
    rounded corners,
    fit=(c7)(c8),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=green!30,
    fill=green!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (intro) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{appendix:comp-data-dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (10.25,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,2)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,2)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.2,0) {\Cref{sec:dodecahedron}};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (c9);

\draw[->,dashed] (c10) to[bend left=-5] (intro);
\draw[->,dashed] (app) -- (c9);
\draw[->,dashed] (c9) -- (intro);
\end{tikzpicture}
\end{figure}
\vspace*{-1.65em}
}

\subsection{Theoretical results}
\label{sec:intro-theory}

% The main theoretical contributions are a careful deve\-lop\-ment of the first- and second-order theory of polytope rigidity, as well as %an~application of the former to so-called 
% the creation of dual certificates based on which perturbations of a 3-dimensional polytope's edge lengths can be realized.
% %edge length perturbations for 3-dimensional polytopes.

In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions/flexes,\nls and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory}~we develop the second-order theory for polytope rigidity.
We provide analogues~for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
%including notions of second-order motions and flexes.
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cref{res:sotest}).
%This allows us to define prestress stability for polytopes.
%
%\notodo{\mwsays{We need results to reference on the arrows.}}

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated from the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to rigidity and first-order rigidity.


% In \cref{section:edge-length-perturbations} we apply first-order theory to study polytope realization spaces, motivated from the following train of thought:
% the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo rigid motions is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
% This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.
% If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same edge lengths. 
% This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}.
%In \cref{section:edge-length-perturbations} we provide an interpretation of these degrees of freedom for first-order rigid polytopes by perturbing their edge lengths.



\iffalse % old text, maybe still useful

We subsequently apply the first-order theory to questions of realizability:
given a combinatorial type $\mathcal P$, one may ask whether there exists a realization $P\subset\RR^d$ with prescribed edge lengths $\ell_e$, $e\in E$.
In general, this question is very hard.
In \cref{section:edge-length-perturbations} we explore the connection between rigidity and the existence of so-called \emph{local edge length perturbations} (see \cref{prop:inf-rigidity-edge-perturbations} and
\cref{thm:rigidity-and-edge-length-perturbations}).\nls
In~\cref{sec:dodecahedron-global-rigidity} we use the results to show that some polytopes are \textit{not} generically globally rigid.

\mwsays{
Using this language, we demonstrate that the dodecahedron exhibits a highly interesting algebraic and topological behavior in \Cref{section:dodec-edge-length-perturbations}. We also compute deformation paths associated with perturbing a single edge length using techniques from \Cref{sec:approx_continuous_motions}.}

\mhsays{Add pictures for this section as well}

% We analyze the full realization space of a few examples where this is possible. This includes cubical zonotopes and generic Minkowski sums.

\fi



% We explore the connection between first-order rigidity and the existence of local edge-length perturbations for polytope realizations.


\subsection{Methodological results}
\label{sec:intro-methods}
%\mwsays{More details: numerical, symbolic, ...}
In \cref{section:second-order-rigidity-check}, we describe a method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.

\todo{\mwsays{This needs rephrasing so that it is clear that we just recall this theory. Or we move to appendix. \mhsays{I guess the novel part is that we can apply it to edge length perturbations. However, it holds in greater generality, which is why I describe it like that. I could make that more explicit in the section?}}\mwsays{This is now appendix. Incorporate it into the introduction differently.}}
%
{\color{lightgray}
In \cref{sec:approx_continuous_motions} we describe an algorithm for approximating continuous motions of flexible polytopes based on Riemannian geometry and homotopy continuation. It relies on numerically tracking the solution to the 
optimization problem that searches for the Euclidean closest point to the realization space. We can also apply this method to investigate edge length perturbations of polytopes. %(see \Cref{section:edge-length-perturbations}).% \mwsays{A bit more details?} 
%\mhsays{Mention generalization to realization spaces?}
}


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
%Our newly developed tools allow us to answer questions that have previously been intractable.
%The Archimedean and Catalan solids provided a convenient benchmark. 
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.
All results are displayed in \cref{tab:comparison} and \cref{tab:catalan-comparison} and discussed further in \cref{sec:experimental_results}.
We highlight two results: first, we show that the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left) is second-order rigid, answering the question from \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
Second, we show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and its rigidity status remains open.
Further theoretical background on the observed flex space~di\-mensions is given in \cref{sec:dimension_estimates}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to a case study of the regular dodecahedron.
We demonstrate how to apply our second-order rigidity certificate.
Subsequently we investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations, deformation paths and conclude that it is not generically globally rigid.


\iffalse % old computational results introduction

\newpage

Doing so already enables us to answer questions that were previously intractable.


The results for the five Platonic, 13 Archimedean and 13 Catalan solids are shown in \Cref{sec:archimedean} and reveal a wide range of interesting behaviors.
%The 13 Catalan solids have less surprising rigidity properties and can be found in \cref{tab:catalan-comparison} in \cref{appendix:catalan}.
%The structure of the tables cells is explained in \cref{sec:explain_table}.
We highlight the most noteworthy finding from these experiments here: 
\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and \Def{truncated icosahedron} have identical rigidity properties: they are neither first-order rigid (both have a 5-dimensional~space of first-order flexes), nor prestress stable; yet, \emph{both are second order rigid}.\nls 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct~concepts.
    Previous examples were comparatively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} (\Cref{fig:Dod_TIco_TDod}, right) is not first-order rigid (it has a 4-dimensional space of first-order flexes), not prestress stable and \emph{not second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order,\nls we do not know whether it is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system that demonstrates that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}
\mwsays{Maybe also list the cool fact that most of our lower bounds match the actual flex space dimensions?}\\
%
%\todo{\mwsays{Maybe I move this to dedicated section. Outlook maybe?}}
%\todo{\mhsays{Shorten Introduction to 3 pages?} \mwsays{I will try. Is there a specific reason? Is it bad if it is 3.2 pages?}\mhsays{Not necessarily, but ``in der K\"urze liegt die W\"urze. Just add whatever now you want now and then we shorten during editing.}}
{
\color{lightgray}
%Numerical experiments reveal that all these properties are very sensitive to small changes in the polytope's geometry.
%First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
%Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
%At this time it is unclear why exactly the realizations with uniform edge lengths show low-order flexibility. 
%In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.



%In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
%The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}}
%By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
%We find bifurcating deformation paths and construct from this a counterexample to generic global rigidity for polytopes.

}

\fi



\newpage

\iffalse
{
\color{gray}

Some polytopes turned out first-order rigid without us having an a priori explanation for this.
More remarkable however we found the rigidity properties of the three polytopes marked in \textcolor{orange}{orange} that are \emph{not} first-order rigid:
%
\begin{itemize}
    % \item For all but three Archimedean solids the first-order theory decides the rigidity.
    % If a polytope is first-order rigid, then it is rigid (see \cref{thm:first_order}. All Archimedean solids that were identified as flexible are so via a Minkowski flex and the dimension of the first-order flex space is as expected from this construction. 
    \item
    The \textit{regular dodecahedron} is rigid. This was previously unknown since it is first-order flexible. The second order tools developed in this article allowed to identify the dodecahedron as second-order rigid \emph{but not} prestress stable.
    The regular dodecahedron furthermore becomes first-order rigid after a generic linear transformation. This suggests that the regular realization of the dodecahedron is a singularity in the realization space.
    By computing deformation paths that shrink/extend a single edge of the regular dodecahedron, we probe the neighborhood of this singularity. We find that bifurcating deformation paths and thereby a counterexample to generic global rigidity for polytopes.
    \item 
    The truncated icosahedron (the football) is also first-order flexible yet second-order rigid.
    \item 
    The truncated dodecahedron is flexible in both first- and second order. At this time it is unknown whether it admits a deformation. If it admits a deformation it is the first example of a polytope flex that is no of Minkowski sum type. If it is rigid then it is the first example of a naturally occurring rigidity of order greater than two.
\end{itemize}


\hrulefill

\mwsays{I write ...}

We develop the second-order rigidity theory for polytopes with edge length and coplanarity constraints. 
In addition, we develop computational tools for checking the rigidity of polyhedral surfaces and for approximating continuous motions. 

\mwsays{Regarding caption \cref{tab:comparison}: we should write first-/second-order rigidity instead of the numeric variants, but if I change it the table vanishes completely. Not sure what is going on. Maybe the figure becomes too long for the page?}


% \footnotetext[1]{As a triangulated sphere, this polytope is first-order rigid by Cauchy's rigidity theorem \cite{cauchy1813}.}
% \footnotetext[2]{As a zonotope, this polytope is flexible according to Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.}
% \footnotetext[3]{As a ``generic'' Minkowski sum, this polytope is flexible (\cf\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}).}

\begin{enumerate}[label=\arabic*)]
    \item All Archimedean zonotopes (except for the cube) have 5 inf flexes because they are projectively unique as zonotopes and hence their only transformations come from the 9-dim general linear group minus rotations and global scale. The cube also loses scaling along axis, hence 3 less (but global scale is already contained in here).
    \item The first-order flex spaces of Rhombicuboctahedron and Rhombicosidodecahedron can be explained as the sum of the first-order flex spaces of their constituents + 3-dim rotations. 
\end{enumerate}

\subsection{Dodecahedron and Truncated Icosahedron}
\label{sec:dodecahedron}

The regular dodecahedron and the truncated icosahedron are interesting case studies. They are both first-order flexible and possess a 5-dimensional space of first-order flexes. Nevertheless, using techniques from computational algebra (\cf\ \Cref{section:second-order-rigidity-check}) we show that for each first-order flex there exists an equilibrium stress that \emph{blocks} the first-order flex from extending to a continuous motion. In other words, both polytopes are second-order rigid (see \Cref{section:rigidity-of-the-regdod}).

\mwsays{First-order rigid once we apply affine trafo or change the height of truncation.}

\subsection{Truncated Dodecahedron}
\label{sec:truncated_dodecahedron}

The truncated dodecahedron is both first-order and second-order flexible.
More precisely, it has a 4-dimensional space of first-order flexes, which is surprisingly different from the five dimensions that we usually associate with icosahedral symmetry (see \cref{sec:dodecahedron}). % that we found for both dodecahedron and truncated icosahedron.
For second-order rigidity it turns out that none of the first-order flexes is blocked by any stress, so all of them are potentially real. \mhsays{``real'' is not a good word in this context.}
%
Remarkably, we were able to construct a flex numerically!
So far we are not aware of an analytic way to obtain this flex.
Thus, whether this flex is actually real or not remains a mystery. 
In particular, if no such flex is real, there are currently no feasible techniques to prove the rigidity of this polytope.

Interestingly, all first-order flexes of the truncated dodecahedron vanish either on affine transformation or when changing the size of the triangles (keeping it vertex transitive).

The facts listed above suggest that the \emph{uniform} truncated dodecahedron is quite special.
In particular, it seems unlikely that the existence of its flex is a mere coincidence.
More likely, there exists a yet unknown construction, similar to Minkowski sums, that generates this flex.

If flexible, the truncated dodecahedron has some remarkable properties:
%
\begin{itemize}
    \item its flex is not reducible to a Minkowski sum
    \item its affine transformations are not (first-order) flexible.
\end{itemize}
%
In contrast, if it were rigid, this would be remarkable as well. 
It would then be the first example of a polyhedron that is second-order flexible, yet rigid.
The general consensus seems to be that rigidity beyond the second order only appears in contrived constructions specifically made for this purpose.
The truncated dodecahedron, being very natural, would then be an interesting counterexample.

\subsection{Outline}
This article is divided into three main parts: The theoretical foundation in \Cref{sec:combinatorics-of-polytopes,section:edge-length-perturbations}, followed by methods in \ref{section:second-order-rigidity-check,sec:approx_continuous_motions} and a case study on the regular dodecahedron in \Cref{sec:dodecahedron}.

}

\fi










\iffalse % paper roadmap

\newpage

{\color{lightgray}

\begin{itemize}
    \item Introduction (Martin)
    \item Theory part (Martin, fix notation and terminology, stay close to first paper)
    \begin{itemize}
        \item first-order theory
        \item second order theory (prestress stability) 
        \color{lightgray}
        \item construction of flexible polytopes (continuous motions)
        \begin{itemize}
            \item theorem for generic zonotopes
            \item counterexample for general zonotopes (hex prism)
            \item questio for generic Minkowski sums
        \end{itemize}
        \item Edge length perturbation (Matthias)
    \end{itemize}
    \item Methods part
    \begin{itemize}
        \item second-order rigidity check (Gröbner bases, ...) (Albert)
        \item Computing deformation paths (also works for changing edge lengths but we don't mention this here maybe???)  (Matthias)
    \end{itemize}
    \item Case studies (results)
    \begin{itemize}
        \item Dodecahedron
        \begin{itemize}
            \item not first-order rigid (five dim space)
            \item proof of second-order rigid (not prestress stable)
            \item numerical experiments on edge length perturbations and what they might entail (Matthias) 
            \item no global rigidity (Matthias)
        \end{itemize}
        \item Truncated Icosahedron (Matthias + Martin)
        \begin{itemize}
            \item Five first-order flexes
            \item Still second-order rigid
        \end{itemize}
        \item Truncated dodecahedron (Matthias + Martin)
        \begin{itemize}
            \item unclear rigidity
            \item NOT second-order rigid (evidence?)
            \item we believe it is flexible ???
            \item have potential deformation paths
        \end{itemize}
    \end{itemize}
    \item Outlook (Martin)
    \begin{itemize}
        \item (questions about edge-length perturbations -- maybe already in theory part)
        \item is there specific structure in the TDod that helps us to see it is rigid/flexible and construct the flex
        \item Are there general stronger methods for deciding rigidity and constructing deformations
    \end{itemize}
    \item Supplementary material
    \begin{itemize}
        \item computational output (Gröbner bases etc)
        \item Code, algorithms
        \item Animations
    \end{itemize}
\end{itemize}

\newpage % temporary new page

Main results:
\begin{itemize}
    \item carefully define first- and second-order rigidity and prestress stability for this setting.
    \item this gives a strong test for rigidity (resolves previously open cases).
    \begin{itemize}
        \item dodecahedron
        \item truncated icosahedron
        \item checked all Archimedean solids and duals (resolved all but one) 
    \end{itemize}
    \item very interesting special case: truncated dodecahedron (TDod)
    \begin{itemize}
        \item we believe it is flexible (for now)
    \end{itemize}
    \item something about edge length perturbation?
    \item edge length perturbations of the dodecahedron: we find there is a singularity in the ``dual space'' (rigidity transition region is algebraically singular)
    \item dodecahedron is an example that we don't have global rigidity
    \item maybe something about zonotope flexes
\end{itemize}

\hrulefill

\begin{itemize}
    \item many examples of rigidity
    \begin{itemize}
        \item short edges make rigid
        \item higher dimensions + first-order rigidity in higher dimensions
    \end{itemize}
    \item second-order rigidity
    \begin{itemize}
        \item second order rigid implies rigid
        \item Q: does second-order flexibility imply proper flexibility?
        \item $\#stresses=\#flexes$ trivial or worth mentioning?
    \end{itemize}
    \item the dodecahedron example
    \begin{itemize}
        \item affine trafos do not preserve first-order rigidity
        \item there is no global rigidity for polytopes in 3D
    \end{itemize}
    \item many other open questions
    \begin{itemize}
        \item Q: does flexibility need parallel edges?
    \end{itemize}
\end{itemize}

Notes on Archimedean solids:
\begin{itemize}
    \item the only Archimedean solids that are inf-flexible but not generic Minkowski sums are the dodecahedron, truncated dodecahedrona (4 flexes) and truncated icosahedron (5 flexes). Where do we lose the flex on the way from truncated dodecahedron to dodecahedron?
    \item Are they second-order rigid? Can the dimension of their flex spaces and their second-order rigidity be explained in some way using the known properties of the dodecahedron? (Limit argument?)
    \item Are there continuous motions between Archimedean/Catalan/Platonic solids thats preserve the planarity of facets and the edge lengths?
\end{itemize}

Other notes
\begin{itemize}
    \item A zonotope is highly flexible, but is there a zonotope that can flex in more ways than just deforming into other zonotopes, either real or infinitesimally?
    \item If $P$ and $Q$ have first-order flexes, then does $P+Q$ inherit them in some way?
\end{itemize}
\newpage % temporary new page


}

\fi








\newpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and a \Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
%Evidently, every convex polytope $P$ gives rise to such a structure, which we call the combinatorial type of $P$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
%If $\mathcal P$ is the combinatorial type of a convex polytope $P$, this notion agrees with the usual edge graph of $P$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
Convenient for computations, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}
%
% \begin{align*}
% \realSp(\mathcal P)
% %=\realSp(V,F,\sim)
% &:=\left\{\!\!
% \begin{array}{l}
%     \bs p\:V\to\RR^d
%     \\
%     \bs a\:F\to\RR^d
% \end{array}
% \Big\vert
%     \begin{array}{rcl}
%     % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
%     \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,
%     \end{array}
% \!\right\}.
% \end{align*}
%
%Analogously, the \Def{convex realization space} is defined as%\todo{\mhsays{Do we need the convex realization space?}}
%
%\todo{\mwsays{Do we really need both notations? I would like to ditch the one with the subscript c.}\mhsays{We should keep the convex realizations in our assumption right? Or do we build a second-order theory for arbitrary point-hyperplane structures?}\mwsays{I will keep the convex ones and delete the subscript-c.}\mhsays{Do we need convexity for anything in this article?}}
%
\begin{align*}
%\begin{align*}
\real(\mathcal P)
%=\realSp_{\mathrm c}(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
%
%We shall write $P\in\real(\mathcal P)$
%\notodo{\mhsays{What does this sentence add?} \mwsays{Nothing. Removed it.}}
Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ does not allow facet hyperplane to pass~though the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

%\mwsays{Maybe move the below to edge length perturbation section? I think this is the first (and only?) place it is used.}\mhsays{Sure, we can do that. Might even call it configuration space?}

% and the \Def{reduced convex realization space} is defined as
% \begin{align*}
% \realRCvx(\mathcal P)
% :=\realCvx(\mathcal{P})\,/\,\mathrm{Iso}
% \end{align*}
%
%where $\mathrm{Iso}$ is the Lie group of Euclidean isometries of $\mathbb{R}^d$.

%\mwsays{Define $\realR(P)$ reduced realization space?}

%As we show in \Cref{sec:first_order},
%\todo{\mhsays{This is absolutely not clear and we spend quite some time to show that.}\mwsays{I am not sure what you mean. This statement is either trivial or false by \cref{res:new_notion}}\mhsays{How the group action works on $\mathbf{a}$ is only explained in Section 4 and was subtle, so using ``clearly'' here is somewhat dishonest. I would suggest writing something like ``As we show in \Cref{sec:first_order}, the Lie group...}}
The \Def{Lie group of Euclidean isometries} (\ie\ rotations and translations), denoted $\Iso$, acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
%\qquad 
%\realRCvx(\mathcal P)
    %:=\realCvx(\mathcal%{P})\,/\,\mathrm{Iso}
\end{align*}

\iffalse % edge-length measurement map

\todo{\mwsays{This here is not the place for metric stuff. This is what the next section is for. I will move this later}}
\todo{\mhsays{If you want, we can call $\realR$ $\conf$ (the configuration space) instead and use something like $\textsc{M}\conf$ for $\mreal^*$, the metric configuration space.}}
Since in this article we are considering polytopes whose edge lengths are fixed, we also define the \Def{edge-length measurement map} as
\[m_E:\mathbb{R}^{dV}\rightarrow \mathbb{R}^E,\quad m_E(\bs p) = \left(\|p_i-p_j\|^2\right)_{ij\in E},\]
which lets us define the \Def{edge-length realization space}
\[\mreal(\mathcal{P},P)\,=\,\real(\mathcal{P})\,\cap\, m_E^{-1}\left(m_E(\bs p)\right),\]
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are fixed according to the realization $P$. The preimage of a given edge length vector is a real algebraic set, as its given by all realizations which satisfy a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}). \todo{\mhsays{Briefly talk about relation to $I$-rigidity?}}

\fi










% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

%\notodo{\mhsays{Maybe have this as section 2.1 instead? This section is quite short.}\mwsays{Yes, maybe. I think about it.}}
We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.


% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
% \label{def:continuous-rigidity}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
%\todo{\mhsays{Use $\mreal{\mathcal P}$ instead of ``equivalent'' to help distinguish the concepts?} \mwsays{This feels the wrong way around.}}
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, then Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
% \end{definition}

%\mwsays{Define configuration space $\conf$ and reduced configuration space $\conv^*$.}
%\mwsays{Define the \Def{metric realization space} $\mreal(P)$ (and reduced $\mreal^*(P)$) and replace below occurrences of $\conf(P)$ by it.}

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks.
Consequently, much of what we say applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}
%This also applies to the subsequent section, which develop a first- and second-order theory for polytopes, but are applicable more generally.

% Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% %
% A \Def{motion} of $(\bs p,\bs a)$ is a curve $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$;
% the motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% A non-trivial motion is called a \Def{flex}.
% If a realization $(\bs p,\bs a)$ has a flex, then we call it \Def{flexible}, and \Def{rigid} otherwise.

% {\color{lightgray}

% \begin{remark}
%     \mwsays{?? Simulating polytope rigidity via stacking prisms on faces.}
%     \mhsays{I'd say we leave it out.}
% \end{remark}

% }

For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.








\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a rigidity systems studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence provides heuristics and criteria that can be efficiently checked in practice.
%Investigating the first-order properties of a system comes down to the study of its \emph{rigidity matrix}.
%The first-order theory for polytopes is analogous to point-hyperplane frameworks, so the theory developed in this section applies verbatim to the more general case.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
    %\label{fig:placeholder}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from it.
%$p_i$ should be thought of as the coordinate of vertex $i$, and $a_\sigma$ the corresponding vertex of facet $\sigma$ in the polar dual of $P$.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    % \label{eq:flex_at_face}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    % \\
    % \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    % \label{eq:flex_at_face}
\end{align}
%
%\todo{\mwsays{Here we could say that $\bsdot a$ is determined by $\bsdot p$. Then it becomes clearer why trivial only needs to be specified on the $p$-part. This is however only true for our polytope setting and not general point-hyperplane frameworks. So we should be cautious claiming generality.}}
%
Like in the frameworks setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also, that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).

%\todo{\mwsays{Turn the lemma into a short remark, maybe without proof and point to the proof below.}}

\iffalse % lemma that adot determined by pdot

{\color{lightgray}\small
\begin{lemma}
    \label{res:p_determines_a}
    The $\bsdot p$ uniquely determine the $\bsdot a$.
\end{lemma}
%
\begin{proof}
    For fixed $\sigma$ choose a basis $p_{i_1},..., p_{i_d}$ among the $p_i,i\sim \sigma$ (we can always do this in our setup).
    Then $\dot a_\sigma$ is the unique solution of the linear system $\<\dot a_\sigma,p_{i_k}\>=-\<\dot p_{i_k},a_\sigma\>$ for all $k\in\{1,...,d\}$.
\end{proof}
}

\fi % lemma that adot determined by pdot

First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any vertex $i\in V$ and facet $\sigma\in F$}.
    % \label{eq:trivial_motion_facet}
    %\\
    %\<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any $i\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    %\\
    %\<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%\mhsays{Potentially we will need $i\sim \sigma$ in $(4.4)$ as well (analogous to (4.2)). The possible trivial inf motions are already restricted to the Lie algebra of the Euclidean isometries (i.e. infinitesimal rotations and translations) by $(4.3)$ and the normals move automatically in first order alongside the vertices. By restricting the flexes further, we may make the equation impossible to satisfy (see computation below). It should be sufficient to have a complete graph as the 1-skeleton and the normals are immediately determined in first order. I don't mind $(4.5)$, but I don't think it adds much. Also, I don't quite understand where (4.5) comes from.}
%\mwsays{Let's delete (4.4) and (4.5).}
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    %The trivial first-order motions of a $d$-dimensional polytope $P$ form a vector space $\mathcal T_P$ of dimension $\binom{d+1}{2}$. 
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    %By assumption $P$ has non-empty interior, so we can assume that $\bs p$ is affinely spanning.
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    % \mhsays{I think it is necessary to at least show that 4.4 and 4.5 are satisfied to complete the proof. For a trivial motion, it holds that \[\langle S p_i+t,a_\sigma\rangle+\langle p_i,S a_\sigma\rangle= \langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle + \langle a_\sigma,Sp_i\rangle=\langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle - \langle p_i, Sa_\sigma\rangle=\langle t,a_\sigma\rangle\]
    % (for (4.5) this works). Of course, this is an issue, because in general this is $\neq 0$. Instead, we take a diagonal matrix $F(t)\in \mathbb{R}^3$ with positive eigenvalues, which is responsible for scaling ${\bs a}$. We require $\bsdot{a}=F(t)\cdot S \cdot {\bs a}$ and compute according to $(4.4)$
    % \begin{eqnarray*}
    % &~&\langle S p_i+t,a_\sigma\rangle+\langle p_i,F(t)\cdot S\cdot a_\sigma\rangle= \langle t, a_\sigma\rangle + \langle p_i,(F(t)-I)\cdot S \cdot a_\sigma\rangle \overset{!}{=}0\\
    % &\Rightarrow & \left(t+(F(t)-I)\cdot S \cdot p_i\right)\T \cdot a_\sigma=0 \quad\left(\Rightarrow t+(F(t)-I)\cdot S \cdot p_i \perp a_\sigma \right)
    % \end{eqnarray*}
    % for arbitrary choices of $t$ and normals $a_\sigma$; since $P$ is affinely spanning, the normals $a_\sigma$ generate $\mathbb{R}^3$ as a vector space. Therefore, 
    % \begin{eqnarray*}
    % S\cdot F(t)\cdot p_i=S\cdot p_i+t~\Rightarrow ~\underbrace{(F(t)-I)}_{=G(t)}\cdot \left( S\cdot p_i \right) = t
    % \end{eqnarray*}
    % for each $i$, since $S$ is not invertible in odd dimensions. This equation essentially needs to be solved for all points $p$ on the hyperplane $\mathcal{H}_\sigma$ with normal $a_\sigma$ which is spanned by the points $p_i$ with $i\sim \sigma$ (here is the exact point where problems occur when we take into account $(4.4)$, since the hyperplane is not defined and we compute on $\mathbb{R}^3$ instead). This equation is overdetermined. The main question is: why does the result for a specific point on $\mathcal{H}_\sigma$ generalize to all points on $\mathcal{H}_\sigma$??? \\[2mm]
    % For $(4.5)$ it holds that 
    % \[\langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle + \langle a_\tau, F(t)\cdot S \cdot a_\sigma\rangle = \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle - \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle = 0\]
    % due to the skew-symmetry of $S$ and diagonality of $F(t)$.}
        %Hence, $\mathcal T\simeq\mathcal T_F$ and the claim follows.
    %\mhsays{Also, I think we should give an argument that this is indeed a linear space and not an affine-linear space or a union of such spaces; contrary to the bar-joint equations, (4.2) vaguely resembles $Ax=b$. Nevertheless, we now have variables $\dot{a}$ and $\dot{p}$, so we can rewrite Equation (4.2) as $\langle \dot{p}_i\times \dot{a}_\sigma,  a_\sigma\times p_i\rangle=0$, which implies that the space is indeed linear.} \mwsays{I don't understand. The equations are linear so the solution spaces are linear.}
    %\mwsays{We should choose $\dot a_\sigma$ as the solution of $\<\dot a_\sigma, p_i\> = \<Sp_i+t,a_\sigma\> = \<p_i, S a_\sigma\> + \<t,a_\sigma\>$ over all $i\sim\sigma$. Choose a basis among the $p_i,i\sim\sigma$ to get a candidate solution. Then use that all other $p_i$ are in the affine span of this basis and that the equations are affinely covariant and hence do indeed have a solution that works for all $i\sim\sigma$. Then it satisfies (4.2), and we delete (4.4) and (4.5).}
    %
    %It suffices to show that each $\bsdot p\in\mathcal T_F$ extends to a polytopal first-order motion $(\bsdot p,\bsdot a)$.
    %
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}

\iffalse

\todo{\mhsays{Prove that trivial flexes have the correct dimension? Clearly, space of inf flexes is contained in framework inf flexes by construction. Apply Asimow-Roth $\Rightarrow$ ``$\leq$''. Construct Inf flexes: skew-symmetric $Q$, translation $T$; on vertices: $Qp(i)+T$, on normals $Qa(\sigma)$.}}

{\color{lightgray}

\begin{observation}
    If a facet $\sigma\in F$ is a simplex, then the left hand side of \eqref{eq:stress_at_face} is a linear combination of $d$ linearly independent vectors in $\RR^d$. 
    This can be zero only if all coefficients are zero.
    Hence, $\eta_{i\sigma}=0$ for all $i\sim\sigma$.

    Thus, if the polytope is simplicial, then all facet stresses are zero and the stress is a pure classical framework stress. Due to a theorem of Dehn, convex simplicial polytopes cannot have a non-zero framework stress. \mwsays{True in $d\ge 4$?}\asays{the 16-cell (cross-polytope) has 8 vertices and 24 edges and hence has two self-stresses. In general, there are many stresses, I think}
\end{observation}
}

\fi

%Since $\mathcal T_P\subset\ker \mathcal R(P)$, it 

\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    %\asays{below we use infinitesimal rigidity. Let's choose one throughout} 
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
    %\mwsays{I prefer ``first-order rigid'' because it is more consistent with ``second-order rigid''. Using ``first-order rigid'' and ``corank'' would be consistent with the other paper.}
\end{corollary}
%
%\todo{\mhsays{First prove inf rigid $\Rightarrow$ regular point in realization space. Then use Riemannian geometry. (see also Asimow-Roth)}\mwsays{Why did we need this complicated stuff again?} \mhsays{Yeah, I agree that it doesn't seem to be necessary anymore. I think the ``complexity'' happens in 4.1.}}
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
    %
    %\qedhere
    
    %By \cref{res:trivial_dim} $\corank \mathcal (P)\ge \binom{d+1}{2}$.
    % If $P$ is first-order rigid, all its first-order flexes are trivial, that is, $\ker \mathcal R(P) \subseteq\mathcal T$. Hence $\ker \mathcal R(P)=\mahcal T$ and the claim follows from \cref{res:trivial_dim}.

    % \TODO\ \mwsays{Maybe not true if $P$ is not affinely spanning. But we are always spanning. Cite a paper by Bernd, Bill, Tony, ... for this}\asays{it's not formally proved there, but I think we can still reference it. I do agree we need spanning. If the joints are spanning, then this statement is pretty clear I think. We have a non-trivial first-order flex iff kernel has dimension larger than ${d+1}\choose 2$}
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:

% \mwsays{In the theorem below, should we go for the differential geometry proof?}
% \mhsays{I think it's fine. The proof technique is pretty standard in rigidity theory.}
% \mwsays{I try to formulate the differential geometry argument. See Matthias' paper.}

% \begin{theorem}
%     % \label{res:second-order-implies-rigid}
%     % \label{res:first_order}
%     If a polytope is first-order rigid, then it is rigid.
% \end{theorem}
% %
% \begin{proof}
%     Observe that $\mathcal R(P)$ is the Jacobi matrix of the constraint system. %If its rank is maximal, then this implies that $\real(\mathcal P)$ is smooth at $P$.
%     \mwsays{We currently have no name for the space of all realizations with prescribed edge lengths.}
% \end{proof}

\begin{theorem}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}

%\notodo{\mhsays{I would say we refer to the Corollary 6.6.}\mwsays{I added a reference. Though I also see educational value in seeing the first- and second-order theory proofs side by side and observing that they are so similar. I know I found this interesting.}}

This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends in $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms~of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a maximal~number $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    A converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}



% {\color{gray}
% \todo{\mwsays{I think this text would fit better in \cref{sec:selected_results}}\mhsays{I agree. Can you move it?}\mwsays{Okay, I will}}

% Dehn's theorem \cite{dehnstheorem} proves that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
% Later, we encounter plenty of non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
% Currently no theoretical tools are available that would identify these as rigid a priorily.
% We therefore formulate the following question:

% \begin{question}
%     %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
%     Can we extend Dehn's theorem to some classes of non-simplicial polytopes? 
%     That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
% \end{question}

% Natural candidates are polytopes whose faces are triangles and 4-gons.
% See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

% }



\iffalse % Albert's proof

{\color{lightgray}

\begin{proof}
    %\textcolor{red}{Add proof here}
    We prove the contrapositive: if $P$ is flexible, then it is first-order flexible. 
    Let $P^t$ be a flex. \todo{\mwsays{I think we need to invoke curve selection to get an analytic flex}} 
    Since $P^t$ is non-trivial, there is some minimal order $k$ for which truncating the Taylor expansion of $P^t$ at this order does not look like the truncation of a trivial motion.
    %we can truncate the Taylor expansion of $P^t$ at some order, say $k$, after which it cannot be completed to a trivial motion by adding higher order terms. 

    We expand the $k$-th derivative of the constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}\!(p_i^t-p_j^t)\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}\!(p_i^t-p_j^t)=0.
    \end{equation*}
    %
    For the coplanarity constraint \eqref{eq:flex_at_vertex_face} at $i\sim\sigma$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell} \!p_i^t\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell} \!\!a_\sigma^t=0.
    \end{equation*}

    Since $k$ was chosen minimal, we can add a suitable trivial motion to cancel all terms of order up to $k-1$. The two equations above become the following. 
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!(p_i^t-p_j^t)=0
    \end{equation*}
    and 
    \begin{equation*}
        p_i^t \cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!a_\sigma^t+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!p_i^t \cdot a_\sigma^t=0
    \end{equation*}
    The $k$-th derivative satisfies the same equation as a first-order flex does.\todo{\mwsays{I don't think this is clear from what we know so far.}} Therefore, $P$ is first-order flexible. 
\end{proof}

}

\fi

\iftrue % polyhedra rigidity stresses first-order theory

%\newpage

\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second and equally important first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
%(recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

% Stresses have no counterpart to ``trivial'' motions

Like first-order flexes, stresses form a linear space -- the \Def{stress space}.
Stresses~are particularly relevant in second-order theory (see \cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).

%One fact that makes 3-dimensional polytope rigidity tractable as compared to dimension $d\ge 4$ is that first-order rigidity can be expressed purely in terms of stresses.

\begin{proposition}
    \label{res:flex_eq_stress}
    If $P$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%
%\notodo{\mhsays{I think it would be cleaner to simply move this comment after the proof.} \mwsays{I like to comment on results before everybody got drained out by the proof. I consider the proof as a nice addendum but nothing crucial for reading. Matter of taste I guess.} \mhsays{This is not important to me. The way I read a paper is I usually skip the proof and read the comments first, but like you said, matter of taste. Why I wanted to move the text is so that before section 4 there is not such a weird gap anymore after the $\square$.}}

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]
    %We first show that for $\mathcal R(P)$ holds $(*)$ $\text{$\#$rows}=\text{$\#$columns}-6$.

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}

% \begin{corollary}
%     \label{res:rigid_eq_stress_free}
%     A polyhedron is first-order rigid if and only if it has no non-zero stress.
% \end{corollary}


The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.


\fi


\iffalse

\hrulefill

\begin{lemma}
    For $\mathcal R(P)$ holds $\text{$\#$columns}=\text{$\#$rows}+6$.
\end{lemma}
%
\begin{proof}
    Let $v,e$ and $f$ be the number of vertices, edges and faces of $P$ respectively.
    
    For each vertex, the number of incident faces equals the number of incident~edges. Thus, the total number of vertex-face incidences in $P$ is equal to the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we arrive at
    %
    \begin{align*}
        \text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
\end{proof}

\mhsays{Add the property that $\# flexes = \# stresses$ for polytopes?} \mwsays{Only true for $d=3$, and yes we should mention this.}

\fi


% \subsection{Flex space dimensions}
% \label{sec:flex_space_dim}

% \mwsays{Delete this section.}















% \tempnewpage % temporary new page

\section{Second-order theory}
% \section{Second-order rigidity and prestress stability}
\label{sec:second_order}
\label{sec:second-order-theory}

%\notodo{\mhsays{Segue from previous section. We now consider arbitrary polytopes again? Or exchange Sections 5 and 6.}}
Second-order rigidity theory investigates continuous flexes that preserve the constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
%Sometimes, the polyhedron can still be rigid even if it is not first-order rigid. 
%Rigidity beyond first order is often difficult to test even for bar frameworks. 
%
We follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if $(\bsdot p,\bsdot a)$ form a first-order motion and additionally it holds 
%
%\notodo{\mhsays{Don't we also need that $\dot{P}$ is a first-order flex?}\mwsays{Thanks! Fixed.}}
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$}
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
%Analogous to what was observed in \Cref{sec:first-order-theory}, the $\bsddot a$ are automatically determined by the $\bsddot p$ in this setting
%\todo{\mwsays{Is the sentence about $\bsddot a$ being determined by $\bsddot p$ necessary?}\mhsays{Not really. We can remove it.}}.
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

%\todo{\asays{I think we deleted what it means to be non-trivial in this case. An issue is that $(0,\bsdot p)$ would be non-trivial for a non-trivial first-order $\bsdot p$ if you are not careful, but it doesn't tell us anything other than the first order motion being non-trivial. A clear definition would be a second-order motion with nontrivial first-order terms.}\mwsays{Oops, true, this got deleted. Will fix.}}
%\mwsays{I previously introduced commands to render $\bs p, \bsdot p, \bsddot p$ (see TeX code for commands) in place of $\mathbf{\ddot{p}}$; again, this would be consistent with the first paper. In any way, I recommend to use the command, we can change its appearance later if desired.}

% Let $\dot P,\ddot{P}$ be the vectors $(\dot{p}_1,...,\dot{p}_{|V|},\dot{a}_1,...,\dot{a}_{|F|})$, $(\ddot{p}_1,...,\ddot{p}_{|V|}$ and $\ddot{a}_1,...,\ddot{a}_{|F|})$ correspondingly. We can now define the second-order flex:
%\mhsays{I suggest using textit and a pale color (\eg\ blue) for definitions instead of bold font. That makes it distinguishable from Definitions/Theorems} \mwsays{I imported the command \texttt{\textbackslash Def} for this. It renders \Def{like this}. Feel free to modify.} \mhsays{Looks good!}

% \begin{definition}\label{sorigid}
%     The pair $(\dot{P},\ddot{P})$ is a \Def{second-order flex} if equations \eqref{eq1} and \eqref{eq2} are satisfied. A second-order flex is \Def{non-trivial} if $\dot{P}$ is not a trivial first-order flex. The polyhedron $P$ is \Def{second order flexible} if there exists a non-trivial second-order flex. Otherwise, we say that it is \Def{second-order rigid}.
%     %\mwsays{Use eqref for referencing equations. Use cref for everything else.}
% \end{definition}

% \begin{remark}
%     Notice that we are not defining trivial second-order flexes as the first and second derivatives of trivial flexes. The reason is that while it is possible to build a non-trivial flex with a trivial first derivative, it is not interesting because $\ddot P$ is simply identical to a non-trivial first-order flex, as the proof of \cref{res:second-order-implies-rigid} shows. Therefore, we only need to look at the case where $\dot{p}$ is non-trivial. 
%     \todo{\mwsays{Not really clear}}
% \end{remark}

% \mhsays{We should fix a notation about the realization ${\bs p}, P, ({\bs p},{\bs a})...$ and keep it consistent throughout the article.}
% \asays{Since we defined $P=(\mathbf p,\mathbf a)$, I defined $\dot P$ and $\ddot P$ analogously.} \mwsays{I am fine with using $P$ and $(\bs p,\bs a)$ (and the dotted variants) almost interchangeably. But I also find it weird to use $\dot P$ as a vector.}

%\mhsays{Are the $\ddot{a}$ automatically determined by the $\ddot{p}$? $\Rightarrow$ write a lemma about it?} \mwsays{They are. We have no lemma for this in the first-order case, just a sentence. If it is not needed, let's keep it at the one-sentence-level, no?}\mhsays{ok.}

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    \label{res:second-order-implies-rigid}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking curve selection, we obtain an analytic flex $P^t$.
    There is then a maximal number $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:second-order-implies-rigid}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system.
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently whether $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.

\iffalse % stresses

% \subsection{Equilibrium Stresses}
% \label{sec:stresses}

%The test is based on the notion of equilibrium stresses, which we introduce next.

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system. 
We denote them by pairs $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$ (recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ sake of brevity and call it a \Def{polytope stress}.

\mwsays{Remark: first-order rigid iff no stress. (and then make this its own equilibrium stress subsection). Maybe move stresses to first-order theory.}\mhsays{Maybe as Proposition?}

%\begin{remark}
%\label{res:stress_eq_flex}    
%\end{remark}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

\fi





% Equations \eqref{eq1} and \eqref{eq2} can be compactly written as a single equation:
% % \begin{equation*}
% %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
% % \end{equation*}
% %
% \begin{equation}\label{eq:compact}
%     \mathcal R(P)\cdot \ddot{P}+\mathcal R(\dot{P})\cdot \dot{P}=0
%     % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
% \end{equation}
% %
% Recall that we use $P$ interchangeably with $(\bs p,\bs a)\in \RR^{dV}\oplus\RR^{dF}$, and analogously~with $\dot P$ and $\ddot P$.
% %
% Now, given a second-order motion $(\dot P,\ddot P)$ and any stress ${\bs \xi}$, we obtain
% %
% \begin{equation}
%     \label{eq:with_stress}
%     {\bs \xi}\T \left(\mathcal R(P)\cdot \ddot P+ \mathcal R(\dot P)\cdot \dot P\right)=0.
% \end{equation}
% %
% %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
% Since ${\bs \xi} \in \ker \mathcal R(P)\T$ by definition of stress, we have ${\bs \xi}\T \mathcal  R(P)\ddot P=0$.
% Equation \eqref{eq:with_stress} then becomes ${\bs \xi}\T \mathcal  R(\dot P)\dot P=0$. We say that a stress $\bs\xi$ \Def{blocks} a first-order motion $\bs P$ if
% %
% $${\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0$$
% %Next, we move on to the second-order duality which can be useful when we want to prove $\ddot{P}$ does not exist. 


\iffalse 
Before that, we first introduce the following equality form of Farkas' lemma:
    \begin{lemma}\label{farkaseq}
        \mwsays{Maybe just use it in the proof and don't list it as a separate lemmas.}\mhsays{I don't mind the Lemma here tbh. }
        Either $Ax=b$ has a solution, or $A^Ty=0$ has a solution with $b^T y\not =0$.
    \end{lemma}
    Intuitively, this Lemma says that either $b$ is in $A$'s column space, or there exists a hyperplane containing the column space of $A$ and $b$ is not in it. 

\begin{lemma}\label{lem2}
    Given a first-order flex $\dot P$, if and only if there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
        {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
    \end{equation}
    then there cannot be a $\ddot P$ such that $(\dot P,\ddot P)$ is a second-order flex. 
    ${\bs \xi}$ is called a \Def{blocking stress} for $\dot P$ if Inequality $\eqref{block}$ holds. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
\end{lemma}
\begin{proof}
    The ``if'' direction is already given in the discussion above. To show ``only if'', we use \cref{farkaseq}.
    %\mhsays{I don't like using the theorem environment in a proof} 
    Let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$. Then \cref{farkaseq} says that either there exists a $\ddot P$ or you can find a blocking stress. 
\end{proof}
\fi

%The following test is an elegant application of Farkas' lemma:

\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

% \begin{lemma}\label{lem2}
%     Let $\dot P$ denote a first-order flex of a polytope $P$. Then there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
%         {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
%     \end{equation}
%     if and only if there is no $\ddot P$ for which $(\dot P,\ddot P)$ is a second-order flex. If $\eqref{block}$ holds,
%     ${\bs \xi}$ is said to \Def{block} $\dot P$. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
% \end{lemma}
\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    % \begin{equation*}
    %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
    % \end{equation*}
    %
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

    
    % This system has the form $A\ddot P=b$ for $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$.
    % By Farkas' lemma, the non-existence of a solution for $\ddot P$ (and hence, second-order rigidity of $P$) is equivalent to the existence of a solution of the system $A\T \bs \xi=0$ for some $\bs\xi$ with $\bs\xi\T b=0$, that is,
    % %
    % $$\mathcal R(P)\T \xi=0,\qquad \bs\xi\T\mathcal R(\sot P)\dot P\not=0.$$
    
    % For an arbitrary stress ${\bs \xi}$ therefore holds
    % %
    % \begin{equation}
    %     \label{eq:with_stress}
    %     0 = {\bs \xi}\T \left(\mathcal R(P) \ddot P+ \mathcal R(\dot P) \dot P\right) = 
    %    \underbrace{ {\bs \xi}\T \mathcal R(P)}_{=0} \ddot P+ 
    %     {\bs \xi}\T\mathcal R(\dot P) \dot P={\bs \xi}\T\mathcal R(\dot P) \dot P.
    % \end{equation}
    % %
    % %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
    % where ${\bs \xi}\T \mathcal  R(P)=0$ follows from the definition of a stress as an element of $\ker \mathcal R(P)\T$.
    % We see that $\dot P$ cannot be blocked by any $\bs \xi$.
    
    % To show ``only if'', let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$ and consider the two linear systems $Ax=b$ and $A\T y = 0$. We apply a linearized version of Farkas' Lemma, which implies that either $Ax=b$ has a solution, or $A\T y=0$ has a solution with $b\T y\not =0$.
    % In other words, there either exists a second-order flex $\ddot P$ or it is possible to find a blocking stress. 
\end{proof}

    % By combining the definition of second-order rigidity and \cref{lem2}, we can obtain the following result:
    % \begin{theorem}\label{res:sotest}
    %     $P$ is second-order rigid if and only if every non-trivial first-order flex has a blocking stress. 
    % \end{theorem}%\mhsays{Formulate as a theorem? This seems to be what people are usually doing in second-order rigidity papers, right?} 

In following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 

% The following notion is often more convenient to use:

%\todo{\mhsays{Expand on the relevance of prestress stability and that it is connected to second-order rigidity by swapping quantifiers?}}

% \begin{definition}
% \label{def:prestress-stable}
%     If there exists a stress that blocks every non-trivial first-order flex, we say the polyhedron is \Def{prestress stable}.
% \end{definition}

\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}

\iffalse

{\color{lightgray}

\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    
    Let $k$ be the smallest integer such that the first $k$ derivatives of $P^t$ do not come from a trivial flex at $t=0$. The $2k$-th derivative of the constraints can be expanded as:
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(a_k^t)=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $k$ is the smallest integer, the first, second, all the way up to $k-1^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to the $k-1^{th}$ are all zeros. The two equations above become the following. 
    %
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t-p_j^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    and 
    %
    \begin{equation*}
        (p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(a_k)+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t)\cdot (a_k^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t)\cdot\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(a_k)=0
    \end{equation*}
    %
    Set $\dot P= \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}P^t\big|_{t=0}$ and $\ddot P=2/\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}P^t\big|_{t=0}$. The two above equations become Equations \eqref{eq1} and \eqref{eq2}. Therefore, if $P$ is flexible, it has a non-trivial second-order flex. 
    \mwsays{It remains to show that the motion is non-trivial.}
\end{proof}

}

\fi














\iffalse % previous first-order section

\newpage

\subsection{First-order theory}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.


A \Def{first-order motion} $(\bsdot p,\bsdot a)$ of $P$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$, %=(\dot p_i\in\RR^3:i \in V;\, \dot a_\sigma\in\RR^3 : \sigma \in F)$.
that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    %\label{eq:flex_at_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    %\label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    %\label{eq:flex_at_face}
\end{align}

A first-order motion is \Def{trivial} if in addition it satisfies
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    %\label{eq:trivial_motion_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
A non-trivial first-order motion is called a \Def{first-order flex}.
A framework is \Def{first-order rigid} if it has no first-order flexes; it is \Def{first-order flexible} otherwise.
Many results from the bar-joint framework setting transfer in the expected way. In particular, if a polytope is first-order rigid, then it is rigid. 

The first-order flex conditions \eqref{eq:flex_at_vertex} -- \eqref{eq:flex_at_face} can be collected in a corresponding \Def{rigidity matrix} $\mathcal R(P)$ % with dimensions $(E+\VF)\times(dV+dF)$. 
which satisfies $\mathcal R(P)(\dotbs p,\dotbs a)=0$ if and only if $(\dotbs p,\dotbs a)$ is a first-order motion.
%
Since we only consider polytopes with non-empty interior, they are in particular affinely spanning and
the rank condition of first-order rigidity applies: 

\begin{lemma}
    \label{res:rank_condition}
    We have
    %
    $$\corank \mathcal R(P) \ge \binom{d+1}{2},$$
    %
    with equality if and only if $P$ is first-order rigid.
\end{lemma}

\hrulefill

%\begin{definition}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
We write
%
\begin{align*}
    \realP{\mathcal P}P &= \realpa{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \real(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
    \\
    \realPCvx{\mathcal P}P &= \realpaCvx{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \realCvx(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
\end{align*}
%
for the (\Def{convex}) \Def{configuration space}, \ie\ the space of all (convex) realizations equivalent to a given (convex) realization $P=(\bs p,\bs a)$.

A \Def{motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\realpa{\mathcal P}{\bs p}{\bs a}$ for which $(\bs p^0,\bs a^0)=(\bs p,\bs a)$.
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all~$t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, we call it \Def{flexible}, and \Def{rigid} otherwise.
%\end{definition}

In general, understanding the full configuration space is intractable in all but the simplest cases. 
We mention here a few situations in which such a full understanding is possible due to various genericity assumptions.
In our language, Cauchy's classical rigidity theorem \cite{cauchy1813} states that $\realPCvx{\mathcal P}P$ is a single point whenever $\mathcal P$ is a simplicial polytope.
As a consequence of the main result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} we also obtain the following:

\begin{theorem}
    Let $\mathcal P$ be the combinatorial type of a 3-dimensional polytopes (\ie\ a polyhedral graph).
    Then for almost all convex (in fact, Zariski convex) realizations $P$ of $\mathcal P$ holds: $\realP{\mathcal P}P$ consists of finitely many isolated points.
\end{theorem}
%
Here, \emph{almost all} means that a dense open subset of the (Zariski closure of) the convex realization space has this property.
%
\begin{proof}
    \TODO \mhsays{$\real(\mathcal{P})$ may be irreducible, but that does not mean that $\real(\mathcal{P},P)$ is. The geometry of $\real(\mathcal{P},P)$ may be pretty complicated. We know that $P$ has generic coordinates; however, it seems like what we need to do is show that $P$ also has generic edge lengths. By going back to the edge length perturbation space and proving a stronger result than Proposition 5.2, we then may be able to prove this. The main issue is that we don't really understand the edge length measurement variety and much less the intersection of that variety with $\real(\mathcal{P})$. So I guess to conclude: I don't really have an easy idea how to approach this. You?} \mwsays{I cannot prove this at this moment. Maybe delete theorem?}
\end{proof}

We conjecture the same to be the case in higher dimensions.

Lastly, recall that a \Def{zonotope} is a polytope obtained as the Minkowski sum of finitely many line segments. A \Def{cubic zonotope} is a zonotope with all faces being combinatorial cubes. Cubical zonotopes are the zonotopal equivalent of simplicial polytopes, in the sense that they are generic in the class of zonotopes: they are generated from line segments in general position:

\begin{theorem}
If $P\subset\RR^d$ is a cubic zonotope generated from $k$ line segments, then %
$$\realP{\mathcal P}P = (\RR P^{d-1})^k.$$
\end{theorem}
%
\begin{proof}
    \TODO
\end{proof}

\fi








\iffalse % old flexible polytopes section by Martin

\newpage % temporary new page

{\color{lightgray}

\section{Constructing flexible polytopes}
\label{sec:flexible_polytopes}

% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
%     Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% A \Def{continuous motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that
% \begin{itemize}
% \item $(\bs p^t(0),\bs a^t(0))=(\bs p,\bs a)$ and 
% \item $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% \end{itemize}
% The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% If a realization $(\bs p,\bs a)$ has a motion, then we call it \Def{flexible}, and \Def{rigid} otherwise.
% \end{definition}
As defined in \Cref{sec:rigidity}, a polytopal realization is flexible if it admits a non-trivial continuous motion.

\subsection{Zonotopes}

A zonotope is \Def{generic} if all its faces are combinatorial cubes. We call it generic because it generated from line segments in generic position. Generic zonotopes are the zonotopal equivalent of simplicial polytopes. For the latter the rigidity theory is classical -- they are rigid, both in first order and globally (Chauchy's and Dehn's theorem).
Likewise, for generic zonotopes a complete theory can be given.

\begin{theorem}
    Let $P\subset\RR^d$ be a rhombic zonotope with $n$ generators. Then
    %
    \begin{myenumerate}
        \item 
        $\realR(P)$ is a connected smooth variety of dimension $(d-1)n-\binom{d}{2}$.
        In particular, each polytope $Q$ combinatorially equivalent to $P$ with the same edge lengths can be deformed into $P$.
        \item if $Q\in\real(P)$ then $Q$ is a zonotope.
        \item The first-order flex space of $P$ has dimension $(d-1)n-\binom{d}{2}$.
        \item Each first-order flex of $P$ corresponds to a real flex.
    \end{myenumerate}
\end{theorem}
%
\begin{proof} \mwsays{Work in progress, these are just ``mental'' notes.}
    Consider the space of all deformations of a zonotope that preserves only coplanarity and central symmetry of the facets (the latter is in combinatorial cubes also implied by edge length constraints).
    Note that for $n$ generators there are $2\binom{n}{d-1}$ facets, and that the central symmetry of each is guaranteed by $d(d-2)$ equations: each pair of opposite vertices (of which there are $d-1$) must have a centroid identical to the centroid of the first pair; this is a vector identity with $d$ components.
    Note that this preserves coplanarity automatically.
    Likewise for an first-order flex -- there $dV$ DOFs and $2d(d-2)\binom{n}{d-1}$ constraints. Removing translations but not rotations, we obtain $dV-2d(d-2)\binom{n}{d-1}-d$ final first-order DOFs.
    Observe that the realization space is a manifold of dimension $nd$, or $n(d-1)$ if we want to preserve lengths. It is also well known that $V=2\sum_{k=0}^{d-1} \binom{n-1}{k}$.
    It remains to check
    %
    $$dV-2d(d-2)\binom{n}{d-1}-d = nd.$$
    %
    This seems to yield too few remaining DOFs ($< dn$) and so some of the constraints are redundant. Which and how many is unclear?
    
    \mwsays{Check that the fact that all inf flexes extend follows already from some general theory about realization spaces of polytopes when the realization spaces are smooth manifolds.}
\end{proof}

\begin{remark}
    More general zonotopes have non-zonotopal flexes. 
    As soon as some face of a zonotope is not a rhombus, then it is the Minkowski sum of this face with the other generators. But a polygon with more than four sides has a non-trivial (\ie\ not symmetry preserving) flex. Hence the Minowski sum of this flex with the other generators yields a non-zonotope.
\end{remark}

\begin{question}
    Is the first-order flex space of zonotopes exactly the tangent space to the finite flexes?
\end{question}

We can ask analogous questions for general Minkowski sums.

\begin{question}
    Is it true that the generic Minkowski sum (where no two faces, edge or higher, share an affine span) of rigid polytopes only has Minkowski flexes? Same first-order. More generally Is the first-order flex space of a Minkowski sum just the sum of the first-order flex spaces of the individual polytopes?
\end{question}

\subsection{Minkowski sums}

% We previously explained how \emph{generic} Minkowski sums become flexible polytopes.
% We can be more precise here.

% \begin{theorem}
%     Given polytopes $P,Q$, let
%     Let $\mathcal U$ be the set of linear subspaces of 
% \end{theorem}

Let $\mathfrak F(P)$ be the first-order flex space of $P$.

\begin{theorem}
    For a generic Minkowski sum of dimension $d\ge 3$ holds $\mathfrak F(P+Q) = \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$.
\end{theorem}
%
\begin{proof}
    \mwsays{This theorem is wishful thinking. It could be that a Minkowski sum has more (first-order) flexes than the ones that come from the summands. I think we know enough to show that $\mathfrak F(P+Q) \subseteq \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$. Maybe the other direction can be proven using some limit argument.}
\end{proof}

\mwsays{Not true in $d=2$ or for non-generic Minkowski sums, consider two triangles that add up to a hexagon, or prisms over those.}

\subsection{Truncation}

If two frameworks on the same graph have the same edge directions, then they have the same first-order theory since the rows in the rigidity matrix are just multiples of each other.
The following would be a generalization to polytopes:

\begin{theorem}
    If $P$ and $Q$ are normally equivalent, then $\mathfrak F(P)\simeq \mathfrak F(Q)$.
\end{theorem}
%
\begin{proof}
    \TODO
    \mwsays{True?} \mwsays{WRONG! TIco and TDod}
\end{proof}

\mhsays{We lose all flexes when changing the truncation of the truncated dodecahedron. Therefore, the flexes are not a result of the polytopes' symmetry, but rather of the coordinates. }

\subsection{Truncation}
Questions:
\begin{itemize}
    \item Does there exist a truncation in (0,1) preserving the flexes of either of the truncated ends?
    \item Is rigidity/flexibility preserved under certain assumptions on the truncation? 
\end{itemize}

}

\fi













\newpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

%The convex realization space $\realCvx({\mathcal{P}})$ of 3-dimensional polytopes of combinatorial type $\mathcal{P}$ is a smooth $(E+6)$-dimensional manifold, on which the 6-dimensional Lie group of rigid motions acts smoothly. %In fact, the reduced realization space $\realRCvx(\mathcal{P})$ is homeomorphic to an open ball (\cf\ \cite[Thm.\ 13.3]{richter2006realization}). Intuitively, this claim \emph{has} to be true, simply by subtracting the appropriate dimensions. However, proving it is %\todo{\mwsays{Not only ``slightly more subtle'', but this is a big deal :D}}
%significantly more difficult than it seems, as we are working with manifolds and associated Lie groups instead of Euclidean space.

%\mwsays{We should start with emphasizing very clearly that this section will be $d=3$ only. This is the first place in the paper where we are not general-$d$.}
%\todo{\mhsays{I reference second-order rigidity in this section. Honestly, I would prefer to switch this section with the second-order rigidity; also, because we restrict ourselves to 3D here and later relax that assumption again.}\mwsays{I am torn. The current transition from ``second-order theory'' straight to ``certifying second-order theory'' is also nice. Where do you mention 2nd-order? Only in the question? Maybe move the question?} \mhsays{I don't think there is a place for the question other than here. I could write ``rigid, but not fo rigid'', which would fix the problem. However, my main issue is that we restrict to $\mathbb{R}^3$ and then revert the restriction in the coming section. That feels confusing and unnatural. But I also understand that second-order rigidity$\Rightarrow$ certifying is a nice order. Let's discuss!}}
For this section, we restrict ourselves to 3-dimensional convex polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
%\notodo{\mwsays{I still think it is a bad idea to say we study the complement. We don't really. The complement is a terrible object. It is not a variety. I would say we study $\real(\mathcal P)$ locally.}}
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polytopes, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to %\notodo{\mwsays{I am not sure I understand ``first-order flexes which only preserve the coplanarity constraints'', or if I do, I think this is misuse of terminology because flex has a well-defined meaning always fixing edge lengths. Otherwise it is a deformation, or a curve in $\real(\mathcal P)$, but not a flex. First-order terminology we don't have for this at all.}} 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization the trivial first-order motions form a 6-dimensional subspace of the space of infinitesimal motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$. %For that reason, $\Iso$ acts smoothly on $\real({\mathcal{P}})$ and since $\realR(\mathcal{P})$ is given by a quotient manifold of the form $\real(\mathcal{P})/\mathrm{Iso}$, 
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension%\todo{\mwsays{$\real^*$ is a smooth manifold, but the reason given here is incorrect:quotients by smooth actions can fail to be smooth.}\mhsays{Not if the group acts smoothly, freely, and properly (see citation). Feel free to rewrite the paragraph though.}} (\cf\ \cite[Thm.\ 21.10]{lee-smooth-manifolds})
%
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
%\notodo{\mwsays{You want to pin a vertex, constrain an edge to a 1-dim subspace and a face to a 2-dim subspace. Pinning the edge sounds like restricting its length.}\mhsays{Adjusted.}}%
In other words, all polytopes have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). %\todo{\mwsays{Not enough pinning. Maybe use Louis' paper? Or just pin an edge and an constraint a vertex to a plane that is in the same face as this edge.}} 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
%\todo{\mwsays{I would not call it a coincidence that $E$ is the number of edges}}
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. %\notodo{\mwsays{\emph{``This line of thought would imply that we can locally freely perturb the edge lengths around rigid realizations''} I think it is not clear why you mention ``rigid realizations'' in this sentence.} \mhsays{Changed the sentence.}} 
Since rigid realizations correspond to isolated points in $\mreal(\mathcal{P},P)$, the degrees of freedom in $\real(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.

%\notodo{\mwsays{Can't we just define existence of edge-length perturbations as that ``the map from realizations to edge length vectors is locally surjective at $P$?} \mhsays{I do not believe this avoids the invariance of domain theorem. ``continuous'' plus ``locally surjective'' just rewords what is already there and abstracts the meaning. I am not necessarily against this change, I just don't believe it is going to be impactful.}}
    
\begin{definition}
\label{def:edge-length-perturbations}
%Fix an ordering of the edges $E$ for a polytope $P$. We denote 
The
 %\todo{\mwsays{maybe ``edge length vector'', since then perturbations are a more natural thing?}}
 \Def{edge length vector} of $P$ is given by
 %\notodo{\mwsays{Should we use $(a|b)$ instead of $(a : b)$ for consistency with the other text? Or are vectors significantly different to justify different notation from sets?}}
 %
% \notodo{\mwsays{I want to suggest notation: $\bs\ell(P)$ for the edge length vector, since consistent with other indexed families like $\bs p$. Also I think it is not good to have both $\ell(e)$ and $\ell_e$. I think we should use only $\ell_e$ since we call it a vector, and $\bs\ell'$ or so if we need another vector like in the paragraph below. Next, $\mathcal L(\mathcal P)$ can now be used for the space of edge lengths vectors. Or something like $\text{\textsc{Len}}(\mathcal P)$, but I think it would be useful to have notation since we write the phrase so often}}
 %
 %\notodo{\mwsays{Why not just $\|p_i-p_j\|$?} \mhsays{So that the Jacobian is actually the rigidity matrix and we do not need the weird shenanigans with scaling.}\mwsays{A bit weird to call it the ``edge length'' vector then, but this was already weird because of the square ... so I guess this is fine :)}\mhsays{I get where you're coming from. At least it is heavily related to edge lengths. Unfortunately, I don't have a better name in mind (which does not completely ignore brevity).}}
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
% \ie\ if there are edge length perturbations arbitrarily close to ${\bs\ell}(P)$ that can not be realized as a polytope $Q$ sufficiently close to $P$, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

\iffalse 
More precisely, $P$ has all edge length perturbations if for some $C>0$ and every $\varepsilon\in (0,C]$ there exists a $\delta>0$ such that every edge length vector $\bs\ell'$ with 
%
\[\text{dist}({\bs\ell}(P),\,\bs\ell')<\delta\] 
%
there exists a polytope $Q=\psi(\bs\ell')$ of the same combinatorial type as $P$ that satisfies
%
\[\text{dist}(P,\,Q)<\varepsilon\] 
%
in the Euclidean metric on $\mathbb{R}^{d(V+F)}$. This definition implies that the edge length map $\bs\ell:\real(\mathcal{P})\rightarrow\mathbb{R}^E$ is locally surjective around $P$. \fi

Let us first consider an example of the first-order rigid regular tetrahedron. For this polytope, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    This polytope is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polytope is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$ as a bar-joint framework, meaning that removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polytope's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polytopes concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid convex polytope $P$ has all edge length perturbations.
    \iffalse
    \begin{proof}
    %\notodo{\mwsays{I find this confusing: we start talking about reduced non-metric realization space, but then continue with the Jacobian, which is the tangent space of the non-reduced metric realization space}}
    %The reduced realization space of a convex polytope $\realR(\mathcal{P})$ is a smooth $E$-dimensional manifold, where $E$ denotes the number of edges of $P$. 
    Assuming that $P$ is %\todo{\mwsays{First-order rigid}}
        first-order rigid, the rigidity matrix $\mathcal{R}(P)$ has the minimal corank $6$ (\cf\ \cref{res:corank_rigid}), so its rank is $dV+dF-6$. 
        %In particular, $P$ is a regular point of $\mreal(\mathcal P, P)$. 
        %This implies that all sufficiently close realizations of $P$ are also first-order rigid: the Jacobian matrix of a polynomial system drops rank in a proper algebraic subset of lower dimension, implying that around every \todo{\mwsays{Let's not talk abut regular points --  we did not introduce the relation between regular points and first-order rigidity (via generic rigidity). Since we only care about the rigidity, let's just reference \cref{res:corank_rigid}}\mhsays{But this doesn't give us that all sufficiently close realizations are first-order rigid, does it? We need something algebraic here.}}regular point of an algebraic variety there is an open neighborhood of regular points \cite[Thm.\ 5.3]{hartshorne}.
%This implies that $\mreal({\mathcal{P},P})$ locally forms a 6-dimensional manifold around the realization $P$ which is locally parametrized by $\mathrm{Iso}$.
Moreover, the realization space $\real(\mathcal{P})$ is a $(E+6)$-dimensional manifold according to the Legendre-Steinitz theorem, which implies that its tangent space $T_P(\real(\mathcal{P}))$ at the realization $P$ also has dimension $(E+6)$. Moreover $\real(\mathcal{P})\subset\mathbb{R}^{dV+dF}$, so that the dimension of the normal space of the realization space $\real(\mathcal{P})$ is equal to $dV+dF-(E+6)$. Since the rows of the rigidity matrix $\mathcal{R}(\mathcal{P})$ are exactly given by a basis of the normal space of $\real(\mathcal{P})$ (\cf\ \cite[Proposition 5.38 and Section 6]{lee-smooth-manifolds}) and the Jacobian %\todo{\mwsays{$d\bs\ell$? Not $J\bs\ell$? If you insist on $d$, can we do $\mathrm d\bs \ell$ or $\partial \bs \ell$ or $\delta\bs\ell$? $d$ is already the variable for the dimension.}}
$d\bs\ell$ of the edge length map $\bs\ell: \real(\mathcal{P})\rightarrow \mathbb{R}^E$, the rank of the rigidity matrix satisfies the inequality
%
\begin{eqnarray*}
    dF+dV-6=\rank(\mathcal{R}(P))&\leq& \rank(J\bs\ell(P))+\dim(T_P(\real(\mathcal{P}))^\perp)\\
    &=&\rank(J\bs\ell(P))+dV+dF-(E+6)\\[3mm]
    &\Rightarrow& \rank(J\bs\ell(P))\geq E
\end{eqnarray*}
%
    On the other hand, $\rank(J\bs\ell(P))\leq E$ by construction, which implies that the rank of $J\bs\ell(P))$ is equal to $E$. Thus, the Jacobian $J\bs\ell(P)$ has full rank. Consequently, $\bs\ell$ is locally a submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}), which implies that $\bs\ell$ is locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). Therefore, all sufficiently small edge length perturbations are realizable.
    \end{proof}
\fi
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    %\notodo{\mwsays{In the rest of the section your write $E$ instead of $E$ for cardinalities.}\mhsays{I reckon you prefer using $E$ for cardinalities? How do we call the set of edges then?}\mwsays{I prefer $E$ for the set and the number. I reckon you are not okay with this abuse of notation. And since we already do it differently everywhere else, lets just use $|E|$, no?}\mhsays{No, I am fine with it. We should just be consistent and say it once in Section 2 that we use them interchangeably.}}
    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). %\todo{\mhsays{There is a gap in the proof here, since the definition requires the existence of $\ell^{-1}$ (sort of), so we need to construct a continuous map from $\mathbb{R}^E\rightarrow \real(\mathcal{P})$} \mwsays{This is easy enough by quotienting by the Iso-action. But let's not touch this before we have figured out the definition problem}}
    %Therefore, all sufficiently small edge length perturbations of $P$ are realizable.
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of convex 3-polytopes are first-order rigid.  
This result requires a suitable definition of genericity, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polytopes to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 

%\mwsays{``For a suitable definition of generic, see \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}:''. Random Coordinates}


\begin{corollary}
    A generic realization of a convex polytope $P$ has all edge length perturbations.
    \begin{proof}
        In \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polytope is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polytope in the following example. This example highlights that that not all realizations of convex polytopes have all edge length perturbation.

%\notodo{\mwsays{Proposal: we bring the two examples as motivation; we take the locally surjective definition; we prove fo-rigid implies all perturbation exist; we discuss whether the cube example can be generalized; we give Theorem 5.6 as a question; we discuss the $z^2$ problem; we prove flexible implies not all perturbations exist under the additional example of continuous inverse (maybe constant fiber?).}}

\begin{example}
\label{ex:cube-edge-length-perturbations}
    %\todo{\mwsays{I think this example is very educational and should, together with a positive example, come in the beginning of this section}}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polytope, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    %\notodo{\mwsays{``antipodal edges'' better?} \mhsays{Sure}}antipodal edges. 
\end{example}

We can turn the observation from this example, that not all convex polytopes admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polytope's edge length vector to distinct polytopes sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the convex polytope $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        %\mwsays{I am skeptical of the conclusion of the second paragraph. We assume that $\real^*$ is smooth and $E$-dim, $\bs\ell\:\real^*\to\RR^E$ is polynomial and locally surjective. But from this alone we cannot conclude that $\bs\ell$ has a local inverse by a continuous map $\psi$. There are counterexamples in this general setting. Either you use more structure and I don't understand how, or there is a gap.}\mhsays{I do not use $\bs\ell$ in this proof 
        %\mwsays{I don't understand, you literally write $\psi(\bs\ell(P))=P$.} and the edge length realization space is also not reliant on $\bs\ell$. In fact, the definition goes the other way around: All edge length perturbations are realizable if there exists a local, well-defined, continuous map $\mathbb{R}^E\rightarrow \real(\mathcal{P})$; in other words, for all sufficiently small edge length perturbations $\bs\ell'$ of $\bs\ell(P)$ we can find a realization $Q$ sufficiently close to $P$ such that $\bs\ell(Q)=\bs\ell'$ (i.e., the map that I am describing above maps an open neighborhood of $\bs\ell(P)$ to some sort of set that contains $P$). At least that is what I intended to convey. If the definition does not convey this, we need to fix it. Nothing about local surjectivity whatsoever. Honestly, you confused me more with your comment about local surjectivity than it helped, so I'd prefer forgetting this term entirely. This map is trivially injective though. I reckon we should add a comment/remark after the definition to clarify either way. }
        %\mwsays{Here is what I just did to sanity check myself: I took a screenshot of your definition of edge length perturbation and put it into ChatGPT. I asked whether this gives me a local continuous inverse $\psi$ that you claim. It said no. It told me that this definition is a sort of ``local surjectivity'' of $\bs\ell$. I did not put this word in, it came back with it itself. So I think the definition is not unclear, but simply not what you want it to be. We need to either fix the definition or the result.}
        %\mhsays{ChatGPT customizes the chats to you by learning from past chats. If I ask ChatGPT \emph{anything} mathematical, I usually get rigidity theory as an example. This is not really an argument. Also, around 40\% of AI queries produce erronous answers. The definition is simply the $\varepsilon$-$\delta$ definition of local continuity of $\psi$. I am still convinced that the definition says exactly that. When I queried ChatGPT about local surjectivity, it often reversed the arrows. This may stem from the fact that suspensions mainly appear in differential geometry where they are used to show the existence of a locally surjective atlas (which reverses the arrows).}
        %\mwsays{Thinking some more I now believe that I understand where you are coming from. I simply had a different (weaker) notion of ``edge length perturbations exist'' in mind. Which one is better is unclear to me. The one where we can prove more, or the one that needs less assumptions. For example, I think with your definition, the answer to Question 5.9 is very likely No already for the dodecahedron. But I am very optimistic it has all perturbations under my definition (which equals your currently written down definition). Especially since all edges can be perturbed individually.}
        Assume now that all of $P$'s edge length perturbations are realizable via 
        % Then, in particular, we can locally extend and contract each of $P$'s edges individually. In fact, we can arbitrarily combine these edge length perturbations, %\todo{\mwsays{``Since we factored out Euclidean isometries'': how does this imply the second half of the sentence?}}Since we factored out Euclidean isometries, 
        %so that each combination of edges that we perturb gives rise to a \emph{distinct} continuous deformation of $P$. This implies that there is an open ${E}$-dimensional ball of realizable edge length perturbations containing ${\bs\ell}(P)$. Therefore, the map 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. As a consequence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi=\varphi^{-1}\circ(\varphi\circ \psi)$ and $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        
        Consequently, there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ that preserves the edge lengths ${\bs\ell}(P)$, so $P$ is rigid. 
        \iffalse
        \mhsays{To show:
        Conversely, if $P$ is rigid, then $P$ is a real-isolated solution of the polynomial system of edge length, facet planarity and pinning equations that factor out the rigid motions (see previous implication). Recall that the configuration space $\mathcal{C}_\mathcal{P}$ is a smooth manifold of dimension $E$. Therefore, intersecting $\mathcal{C}_P$ with the real algebraic set generated by the edge length equations
        \[\mathcal{E}_P~=~\left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||=\mathcal{L}_{(u,v)}~\forall uv\in E\right\}\]
        contains the isolated point $P$. Consequently, intersecting $\mathcal{C}_\mathcal{P}$ with the complement
        \[\mathcal{N}_P ~=~ \left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||\neq \mathcal{L}_{(u,v)}~\text{ for some } uv\in E\right\},\]
        which exactly characterizes the edge length perturbations of $P$, is equal to $\mathcal{C}_{\mathcal{P}}\setminus \{P\}$.
        We now show that for every sufficiently small perturbation of ${\bs\ell}(P)$, there is a convex polytope close to $P$. In other words, we need to show that $U({\bs\ell}(P)$ is open in $\mathbb{R}^{E}$ and not only in the realization space of edge length perturbations. \textcolor{red}{Also, we need to show well-definedness of $\psi$.}
        %Since $\mathcal{C}_\mathcal{P}$ is a smooth, $E$-dimensional manifold, it is locally diffeomorphic to $\mathbb{R}^{E}$ via $\varphi:\mathcal{C}_\mathcal{P}\rightarrow \mathbb{R}^{E}$. This property implies that there exists an open neighborhood $V\subset\mathbb{R}^{E}$ such that $\varphi:\varphi^{-1}(V)\rightarrow V$ is a diffeomorphism. Note that we can choose $V$ so that ${\bs\ell}(P)$ is contained in $\varphi^{-1}(V)$ since $\mathcal{C}_\mathcal{P}$ is a smooth manifold. By possibly shrinking the open sets, we obtain a continuous map $\varphi \circ \psi:U_{\bs\ell}(P\rightarrow V$. 
        The rigidity of $P$ implies that
        \[\mathcal{C}_\mathcal{P} ~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right)\,\cup\, \left(\mathcal{C}_\mathcal{P}\cap \mathcal{E}_P/\sim\right)~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right) \cup \{P\}.\]
        Since $\psi$ is injective and continuous by construction, the preimage of any open set around $P$ under $\psi$ is open again. Since all realizations come from edge length perturbations, $\psi$ is surjective; therefore, $\psi$ is a homeomorphism.}
        \fi
    \end{proof}
\end{theorem}

The contraposition of this theorem provides a sufficient condition for the rigidity of polytopes, which makes it worth to point it out as a corollary. Albeit, it is unclear whether checking that all edge length perturbations are realizable offers any advantage over directly verifying a polytope's rigidity.

\begin{corollary}
    If a convex polytope $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}

%\notodo{\mwsays{As written this is not correct. What you want to say is that the \emph{existence} of such $\psi$ is equivalent to the \emph{existence} of such other $\psi$.}\mhsays{You meant the Corollary, right? In that case: Fixed.}}
%
We also note that the assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. This restricts the admissible polytopes.

Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample: The map $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.


However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 
\iffalse
\begin{remark}
    %\todo{\mwsays{As written, it sounds as if we have an example of this, which we don't}}
    It is unclear, whether the converse of \Cref{thm:rigidity-and-edge-length-perturbations} is true: The space of edge length perturbations may be full-dimensional, even though the realization $P$ is rigid and only certain edge length perturbations which form a lower-dimensional algebraic subset are not realizable. 
\end{remark}
\fi

The correspondence between the edge length realization space of a polytope and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polytope is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

%\notodo{\mwsays{Can we make the first two questions into one with (i) and (ii) since they are just inverses of each other?} \mhsays{I was contemplating that, too. Fixed.}}

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polytope $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization of a convex polytope have all edge length perturbations?
\end{question}

%\notodo{\mwsays{In the question below, do you also want to ask that it is not first-order rigid? Otherwise the tetrahedron is a counterexample. And maybe move this question to the end of the so-theory section? Depends on if we move this section of course.} \mhsays{True. Thanks for pointing out this oversight. I chose to replace it by ``rigid, but not fo-rigid''.}}

% \begin{question}
% Assuming a convex polytope $P$ is rigid, but not first-order rigid, is ${\bs\ell}(P)$ then singular in the edge length realization space $\mathcal{L}(P)$ (see \cref{fig:edge-contraction-deformation-space})?
% \end{question}

%\todo{\mhsays{I might delete this question, since I find it confusing in the context of Legendre-Steinitz and it is not formulated precisely, since we only change the length of a single edge.}}

%While we do not understand the edge length realization space of polytopes nearly enough to provide answers to these questions, they provide interesting observations that should be investigated in future research.\todo{\mwsays{You essentially repeat the last sentence before the questions}}

%\todo{\mhsays{Technically, we could also move this section to the appendix if need be. Without \Cref{thm:rigidity-and-edge-length-perturbations}, this section is not what it used to be.}}


















\newpage
\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}
\label{sec:so_certificate}

%\todo{\mwsays{Use $\mathcal{R}$ for rigidity matrix}}

As laid out in \Cref{sec:second-order-theory}, any first-order flex of a polytope in the edge-length realization space \mbox{$\mreal(\mathcal{P},P)$} that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. This provides a convenient heuristic for finding non-blocked flexes: Essentially, for all equilibrium stresses $\bs \xi$ we need to find a flex $\dot{P}$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$ (\cf\ \Cref{res:sotest}). Conversely, if for each $\dot{P}$ there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$, then the polytope is 
%\notodo{\mwsays{In fact, PSS. Is this the proper converse that you want to state here?} \mhsays{Good catch, thanks.}}
second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the flex space via a basis ${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ and variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ and variables $\mu=(\mu_1, \dots, \mu_s)$. %\notodo{\mwsays{refer to \eqref{res:sotest} explicitly}\mhsays{done}}
This turns the second-order condition \eqref{block} into a cubic polynomial of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, the homogeneous polynomial $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.

By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is nonzero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. 
Therefore, the first-order flexes that are not blocked by any stresses can be parametrized by the solutions of the polynomial system $Q_1=\dots= Q_s=0$, which form an algebraic set. %\todo{\mwsays{Is this clear?}}
This system can also be represented by the gradient of $E_{\dot{P},{\bs\xi}}$ with respect to $\mu$ to obtain $\nabla_\mu E_{\dot{P},{\bs\xi}}(\lambda)=0$.

%\todo{\mwsays{Why does this suffice? Finitely many solutions are still solutions. Further below you explain that finite implies empty due to homogeneity. This should come here, no?} \mhsays{We are in projective space, so finitely many solutions implies positive-dimensional solution space.}\mwsays{I know. This is mentioned below because it is necessary for the argument. But it must be mentioned here because the argument is already used here.} \mhsays{Potentially I can just remove/replace this sentence here, since I explain it in the next paragraph anyway.}\mwsays{That is possible. Just without a comment this sentence is confusing}}
We will later see that the zero-dimensionality of the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$ is sufficient for second-order rigidity. As a criterion for that, we formulate the following. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field %\todo{\mwsays{Can we use $\Bbbk$ for the field?}}
        $\Bbbk$. Given an ideal $\mathcal{I}=\langle f_1,...,f_s\rangle$, where $f_i\in \Bbbk[x_1,..,x_r]$, and a Gröbner basis $\mathcal{G}$ of $\mathcal{I}$. Then, $\mathcal{I}$ is zero dimensional if and only if for every $i\in\{1,...,r\}$ some power of $x_i$ is the leading monomial of an element of $\mathcal{G}$.%\mhsays{Only for algebraically closed $k$? If so, replace $k$ by $\mathbb{C}$. Else, define what $k$ can be. }
    \end{lemma}

Of course, there are also other methods based on Gröbner bases to verify that an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proved to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic variety $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homogeneous, we can interpret $\mathcal{V}(\mathcal{I})$ as a projective algebraic set and it holds that $\mathcal{V}(\mathcal{I})\subset \mathbb{P}_\mathbb{C}^{r-1}$. Thus, for any solution $\lambda^*$ of the polynomial system $Q_1(\lambda)=\,\dots,\,=Q_s(\lambda)=0$, all scalar multiples $c\cdot\lambda^*$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\emptyset$, since $0\notin \mathbb{P}_\mathbb{C}^{r-1}$. In our context, the emptiness of $\mathcal{V}(\mathcal{I})$ translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system %\notodo{\mwsays{Since this proposition tries to be self-contained, one should repeat what is the \emph{finite} system. As written down I don't see a system but only one equations. What do we quantify over? Alternatively, refer to (6.1), but also name what finitely many indices we quantify over.}}
    \todo{\mwsays{I was confused for the wrong reasons, but I am still confused: where does nabla come from?} \mhsays{It's the gradient. This is standard notation. I added a line above to explain this.}\mwsays{My question should have been: where does the gradient come from? I agree the notation is standard. But I think I found the sentence where this is explained.}}
    $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ defined in \eqref{eqn:stress_polynomial_Qi} only has $\lambda_1=\dots=\lambda_r = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)=0$.
\end{proposition}

%\mhsays{Describe Test for prestress stability: Albert's code.}

\notodo{\mwsays{This paragraph reads to me like: we were lucky that our technique worked for the polytopes we tested it on, but there was no guarantee. If true, this is new to me and this is not how we sell it in other parts of the paper.} \mhsays{Why would there be a guarantee? I don't see how we could prove something like that. We use an established sufficient condition, which works over $\mathbb{C}$ and lets us certify second-order rigidity in the cases we consider. I don't believe it is necessary. We can easily tweak it though in case we ever need it by using the Euclidean distance degree, which has a significantly higher complexity, so I wouldn't worry too much about that (last sentence). }\mwsays{I think I understand now: even if the algorithm says ``no'', it might still be so-rigid.}}The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all Archimedean, Catalan and Platonic solids (\cf\ \Cref{tab:comparison} and \ref{tab:catalan-comparison}). Still, \notodo{\mwsays{I am stumbling with the sentence structure here: what is not necessary for what?} \mhsays{elaborated.}}our result using Gröbner bases is clearly not necessary for second-order rigidity, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})$ is empty over the real numbers, even when we find solutions over $\mathbb{C}$. The trivial counterexample is $x^2+y^2=0$, which only has $x=y=0$ as a real solution, yet the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solution on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}).

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a $\mu\in \mathbb{R}^s$ defining a \notodo{\mwsays{Why ``linear combination of stresses $\mu$'' instead of ``stress $\mu$?}}stress ${\bs\xi}=\sum_{j=1}^s \mu_j\cdot {\bs\xi}_j$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu_j$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix
%
$$\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_j\lambda_k}Q_j(\lambda)\right)_{j,k=1}^r$$
%
is positive definite for some choice of $\mu$. Our calculation shows that the regular dodecahedron and truncated icosahedron are not prestress stable using a numerical SDP solver. A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate in our case.

\mwsays{Some sentences in this section reach too deep into other sections, such as mentioning the exact test cases and the results for Dod and TIco.}


\newpage

\section{Second-order rigidity of the regular dodecahedron}

Among the Platonic solids, for only one of them the question of rigidity is not~immediately clear. 
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid by Dehn's theorem \cite{dehnstheorem}. 
The cube is the classical example~of~a~flexible polytope.
Solely the regular dodecahedron remains to be understood and initially eluded direct computation.

Symbolic computations reveal a 5-dimensional space of first-order flexes and a~5-dimensional space of stresses.\footnote{The specific embedding and orderings of vertices, edges and faces are provided in \cref{appendix:comp-data-dodecahedron}.}
%
Note that these dimensions must be identical~due~to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
%
It is tempting to somehow relate the dimensions of the flex and stress spaces to the 5-fold symmetries of the dodecahedron.
We have no evidence~for such a relation, and rather mild counter-evidence in the case of the truncated~dode\-cahedron (see \cref{sec:selected_rigidity}).


\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

% By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
% \footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
% Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
% %\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
% Consequently, the regular dodecahedron is not first-order rigid.

%We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. 

Since the regular dodecahedron is not first-order rigid it is a promising test case for the second-order certificate of \cref{sec:so_certificate}.
Concretely, \cref{prop:stress-energy-condition} asserts~that it suffices to compute the zeros of a certain polynomial system. 
We proceed~as~follows:
%
\begin{enumerate}
    \setlength{\itemsep}{0.7ex}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. 
    Using the~bases, we parametrize the spaces by variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$,\nls respecti\-vely. 
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadric forms $Q_i$. % (see \cref{section:second-order-rigidity-check}).
    
    \item Use the equivalence in \cref{gbasis} to determine whether the system~has~fi\-nitely many (real) zeros.
    This is the case for the regular dodecahedron.
    
    \item Use \Cref{prop:stress-energy-condition} to infer second-order rigidity.
\end{enumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. Then, $\mathcal{I}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}.
    For more specifics on the relevant \textsc{Mathematica} files, see \cref{appendix:comp-data-dodecahedron}.
    With the help of this Gröbner basis, we obtain the following results:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        The monomials $\lambda_1^2$, $\lambda_2^3$, $\lambda_3^3$, $\lambda_4^5$,  $\lambda_5^6$, appear as leading monomials in the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$.
        \Cref{gbasis} therefore implies that $\mathcal{I}$ is zero-dimensional. 
        %By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). 
        Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. 
        By \cref{prop:stress-energy-condition}, for any nonzero $\dot P$ generated by the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. 
        By \Cref{res:sotest}, $P$ is second-order rigid. 
        By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

\begin{remark}
    Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid}). The contraposition of \Cref{gbasis} can be used to show that the truncated dodecahedron is \emph{not} second-order rigid (see \Cref{res:TDod_not_Second_order_rigid} for details).
    % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
\end{remark}\todo{\mwsays{Incorporate TIco and TDod into Remark}\mhsays{I made an attempt. Feel free to change.}}











\newpage

\section{Computational results: Platonic, Archimedean and Catalan solids}
\label{sec:experimental_results}
\label{sec:archimedean}

\todo{\mwsays{Note to myself: add this footnote somewhere: The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}\mhsays{Is this footnote now part of Section 7?}}

\mwsays{TODO for me: rewrite section intro}

We demonstrate our techniques on the Platonic, Archimedean, and Catalan~solids -- classes of polyhedra for which combinatorial data and algebraic vertex and normal coordinates are readily available.
The results are shown in \cref{tab:comparison} (for the~Platonic and Archimedean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation~for the content of the tables is given in \cref{sec:explain_table}.
%
%A more detailed step-by-step~expla\-nation for how the second-order rigidity results were obtained is given in \cref{section:rigidity-of-the-regdod} on the example of the regular dodecahedron.
%
A key takeaway is that already simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a remarkably simple test case for future theoretical and computational developments.
See \cref{sec:selected_results} for a discussion of selected results from the tables.



\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{0.7ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    %{\color{gray} 
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semi-definite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
%\mwsays{Something about how the numerical computations are sufficiently stable and the results away from zero or whatever so that we can trust them.}\mhsays{Replace ``We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.'' by: The numerical results are based on an eigenvalue computation, for which \noBut\ indicates the existence of an eigenvalue close to machine precision ($\approx 0$), whereas \yesBut\ indicates the existence of an eigenvalue whose absolute value lies above $10^{-6}$, which is sufficiently far away from zero. We observe no intermediate eigenvalues. Since eigenvalue computation is numerically stable and the thresholds have been chosen conservatively, we have a high degree of confidence in these results.}\mwsays{Then we should probably only explain \noBut, because \yesBut\ is never used. And also: do we ever explain this eigenvalue stuff in the paper? I don't remember having done anything with eigenvalues in Mathematica when I checked prestress stability.}\mhsays{I guess you solved an SDP of the form $C=\lambda_1\cdot A_1+\dots+\lambda_4\cdot A_4$ to find an assignment of $\lambda_i$ that makes $C$ positive definite. However, we always found a zero eigenvalue I guess? I don't exactly recall.}
    %}\mwsays{Okay, let's look into Albert's code to see what can be said.}
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flexe space} as introduced in \cref{sec:first_order}.
    %\nls Heu\-ristically, it is the expected number of independent ways in which the polytope can deform in first order. 
    %If the number is zero, the polytope~is first-order rigid. 
    %If the polytope is a generic Minkowski sum, the dimension~decomposes as explained in \cref{sec:generic_Msum} (see also \SymThree\ below).
    In some cases we have a good understanding for how~the~dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension. 
    If further explanations are available, this is indicated by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and more theoretical background given in \cref{sec:dimension_estimates}.
    %
    %\todo{\mhsays{Maybe only refer to \SymTwo\ and \SymThree\ here? \ie\, ``see \SymTwo\ and \SymThree\ for an explanation of the number''? Otherwise we write it twice.}}
\end{enumerate}
%
The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{0.7ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension for the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
    %If~the zonotope is generic (\ie\ all faces are rhombi), the dimension of the first-order flex space is precisely $2\times\#\text{generators}-3$ (see \cref{res:generic_zonotope}).
    %For~general zonotopes a lower bound is given~by $\dim\GL(\RR^3)-4=5$ (with a few exceptions, see \cref{res:bound_zonotopes}).
    
    % The dimension of the flex space of a generic Minkowski sum is at least the sum of the dimensions of the flex spaces of the summands, plus the dimension of the Lie group that parametrizes the relative orientations of the summands.
    % For this class we write the flex space dimension in the table as a sum of these two contributions.
    
    % %show how this dimension decomposes into flexes coming from flexes of the Minkowski summands (left term) and flexes coming from the relative orientation changes of the Minkowski summands (right term). 
    % For example, the \emph{rhombicuboctahedron} (\cf\ \cref{tab:comparison}) is a Minkowski sum of a cube and an octahedron. The cube provides itself three dimensions~for the flex space, whereas the octahedron provides none. The remaining three dimensions come from $\mathrm{SO}(\RR^3)$, which encodes the relative orientation of~the cube and octahedron. We denote this by 3+3.
\end{itemize}
%
%These considerations are elaborated in \cref{sec:dimension_estimates}.
Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
Again,\nls details are given in \cref{sec:dimension_estimates}.

% \mwsays{In all cases our heuristic lower bounds match the actual dimension of the flex space. In some cases (permutahedra) this is especially remarkable since it suggests that the combinatorics and edge lengths constrains enforce a zonotopal realization.}


\iffalse
Numerical experiments reveal that all these properties are sensitive to small changes in the polytope's geometry.
First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
At this time it is unclear why exactly the realizations with uniform edge lengths are flexible in first- and second-order. 
In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.
\fi

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding table cells are marked by \Star):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} have identical~rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes), nor prestress stable; yet, \emph{both are second \mbox{order} rigid}. 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    %In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct concepts.
    Previous examples of this distinction were compa\-ratively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order, we do not know whether it is in fact rigid.
    If~it~is~rigid,\nls it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above are sensitive to small changes in the their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.

\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priorily.
We therefore formulate the following question:

\begin{question}
    %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps polytopes whose faces are triangles and 4-gons are simple enough for a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.


% \mwsays{Here would be a good place to put Question 3.5} \mhsays{I agree}

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained from actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} match the values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.





\input{sec/table1}
\input{sec/table2}










% \newpage

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}

Due to its previous status as the guiding example, %we dedicate \cref{sec:dodecahedron} to a case study of the regular dodecahedron.
%
% Among the Platonic solids, only for one of them the question of rigidity is not immediately clear. 
% The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid; the cube is a zonotope, hence flexible. 
% Only the regular dodecahedron remains to be understood, and initially eluded direct computation.
%
we single out the regular~dodecahedron once again for a closer inspection.
%We explain in more detail how we found it to be second-order rigid.
%
We share our results from exploring the realization space close to the regular configuration with the hope of better understanding its exceptional behavior.
We draw conclusions about global rigidity.

%Solving the system of first-order conditions, we find that there exists a 5-dimensional space of first-order flexes.






\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

\iffalse % old rigidity section

\subsection{Rigidity} 
\label{section:rigidity-of-the-regdod}

By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
Consequently, the regular dodecahedron is not first-order rigid.

We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. \Cref{prop:stress-energy-condition} asserts that computing the zeros of a certain polynomial system lets us certify this property. For that reason, we employ the following strategy:

\begin{myenumerate}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. We parametrize these bases via variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$, respectively. 
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadrics $Q_i$ (see \cref{section:second-order-rigidity-check}).
    
    \item Employ \Cref{gbasis} to show that this system has finitely many zeros.
    
    \item According to \Cref{prop:stress-energy-condition}, this implies that the regular dodecahedron is second-order rigid.
\end{myenumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. $\mathcal{G}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}. With the help of this Gröbner basis, we can prove the following theorem:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. As a result, for any nonzero $\dot P$ generated by the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. By \Cref{res:sotest}, $P$ is second-order rigid. By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

\begin{remark}
    Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid} for details).
    % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
\end{remark}

\fi







\subsection{Deformation paths}
\label{section:dodec-edge-length-perturbations}


\todo{\mwsays{Potentially incorporate: ``By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
We find bifurcating deformation paths and from this, we construct  a counterexample to generic global rigidity for polytopes.''}\mhsays{Done}}
%
Although \Cref{dodecahedronrig} shows that when fixing its edge lengths, the dodecahedron with combinatorial type $\mathcal{P}$ is rigid, its realization space $\real(\mathcal{P})$ is a smooth $36$-dimensional manifold due to the Legendre-Steinitz theorem. According to \Cref{section:edge-length-perturbations} we can say more: its reduced realization space $\realR(\mathcal{P})$ is a smooth $30$-dimensional manifold. In \Cref{conj:edge_length_perturbations} we formulate the hope that for rigid polytopes, all edge length perturbations are realizable (\cf\ \Cref{def:edge-length-perturbations}). It is completely unclear, whether this claim is true.

In this section, we investigate how deformations of the regular dodecahedron in $\realR(\mathcal{P})$ induced by shrinking or extending a single edge length behave. By approximating such deformation paths using the methods introduced in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of this polytope. 
With this approach, we describe bifurcating deformation paths, which lets us construct a counterexample to generic global rigidity for polytopes.

By the dodecahedron's regularity, all edges are combinatorially identical. It does not matter which edge is chosen. For this example, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert < 1$. Sampling from the realization space intersected with the real algebraic set generated by the edge length equations reveals that there are six distinct curves through the regular dodecahedron corresponding to the contraction of a single edge length (see also \cite{deformationpaths}) and two corresponding to its expansion. All eight configurations at $\ell^{\star}(\pm 0.25)$ are depicted in \Cref{fig:edge-contraction-deformation-space}.

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by perturbing a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge constractions, whereas gray curves correspond to edge expansions. On these curves, the eight corresponding realizations at $\ell^*(\pm 0.25)$ are depicted. Four realizations are connected by a nodal cubic (dark blue dashes).}
            %Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
        
\iffalse
     \begin{figure}[h!]
        \centering
        \includegraphics[width=0.25\linewidth]{Images/dodeca3.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca1.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca2.png}\\[2mm]

        \hspace*{7mm}
        \includegraphics[width=0.16\linewidth]{Images/dodeca5.png}
        \hfill
        \includegraphics[width=0.18\linewidth]{Images/dodeca4.png}
        \hfill
        \includegraphics[width=0.17\linewidth]{Images/dodeca6.png}\hspace*{7mm}
        \addtocounter{equation}{1}
        \caption{The six configurations obtained by contracting the blue edge. They can be split into two types that are organized in the top and bottom row. In the central column, the configurations have two reflection axes, while the left and right columns are mutual mirror images with only one reflection axis. }
        \label{fig:dodecahedron-configurations-contraction}
    \end{figure}
\fi

        It turns out that in the case of edge length contractions there are two types of configurations: Those mitigating the edge contraction by deforming vertically (see \Cref{fig:edge-contraction-deformation-space}, top) and those that deforming horizontally (see \Cref{fig:edge-contraction-deformation-space}, bottom). Both types contain one configuration with two mirror axes and two configurations with one reflection symmetry that are mutual mirror images. Intriguingly, not all dodecahedra persist until the edge collapses. The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations beyond this particular edge length. \todo{\mwsays{Discuss the fact that the orange branches meet again: the two branches of the loop have opposite symmetries, and must therefore pass through a common symmetrization to connect to each other}} All of them persist until $\ell^*(-1)=0$. 
\iffalse
        \begin{figure}[h!]
        \vspace*{2mm}
            \centering
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT1.png}
            \hfill
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT2.png}
                \addtocounter{equation}{1}
            \caption{The two configurations obtained by expanding the blue edge. Both admit two distinct reflection symmetries.}
            \label{fig:dodecahedron-configurations-expansion}
        \end{figure}
\fi

        Conversely, expanding an edge only produces two configurations that both have distinct distinct reflection axes. They are depicted on the sides of \Cref{fig:edge-contraction-deformation-space}. There is no indication that there exists a maximal edge length beyond which no realizations exist. Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.

        %What remains is a qualitative analysis of the eight deformation paths that emerge from contracting any of the dodecahedron's edges. By considering projections of the eight deformation paths onto random 2-dimensional subspaces and approximating the curves' derivatives, an understanding of the curves' tangents in the regular dodecahedron can be obtained. \Cref{fig:edge-contraction-deformation-space} visualizes these curves' behavior. 

        %\mhsays{Mention how the graphic was formed (see above text)}

        % \begin{figure}[h!]
        %     \centering
        %     %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation.jpg}
        %     %\hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom.jpg}
        %     %\\[4mm]
        %      %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation2.jpg}
        %     \hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom2.jpg}
        %     \addtocounter{equation}{1}
        %     \caption{Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths (\cf\ \Cref{fig:dodecahedron-configurations-contraction}) have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
        %     \label{fig:edge-contraction-deformation-space}
        % \end{figure}

         %\todo[inline]{\mwsays{Put little pictures of the deformations at the branches of the graphics.}}

%\mhsays{Picture looks good imo. I wonder if we can replace the pictures above by a bigger picture of the topological diagram (since it already contains all configurations)? It feels like Figures 3 and 4 do not add much anymore.}

In \Cref{fig:edge-contraction-deformation-space}, we also depict the deformation paths corresponding to these eight realizations, which are induced by edge contractions 
%\notodo{\mwsays{I am not sure this dashed line will be universally understood to be blue} \mhsays{Like this?}\mwsays{Much better!}}
(blue) and expansions (gray).
Remarkably, it appears that some of these curves can be matched smoothly. For instance, the gray curves corresponding to an edge expansion have the same tangent in the regular dodecahedron and so do the corresponding arcs of the blue curves. Moreover, the curves corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (see \Cref{fig:edge-contraction-deformation-space}, dark blue dashed curve).
%todo{\mwsays{Give a different color to nodal cubic so it is easier to refer to.}} %In particular, the regular dodecahedron is a singularity in the deformation space induced by all possible modifications of a single edge. 
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron due to the and that there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$.

%\todo{\mhsays{Is this even true?}\mwsays{Unclear. Depends on the singularity. It is likely but we don't know this.} \mhsays{How to rephrase?}}

Two symmetric deformations remain, which also share the same tangent in the regular dodecahedron. In total, four smooth curves are passing through the regular dodecahedron that are parametrized by edge perturbations. Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective tangents' sum is sufficiently close to zero. Finally, we attach an animation of a smooth deformation path passing through the regular dodecahedron induced by an edge expansion from $\ell^*(-0.25)$ to $\ell^*(0)$ followed by a compatible contraction from $\ell^*(0)$ to $\ell^*(-0.25)$ in the supplementary material \cite{zenodo_suppMaterial} of this article. 




\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytopes is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore globally rigid.

However, the regular dodecahedron is highly symmetric, which still leaves the global rigidity of generic realizations open. A polytope is called \Def{generically globally rigid} if every generic %\todo{\mwsays{Generic undefined. We mention it already earlier, but never define it I think.} \mhsays{We define it \emph{intuitively} on page 15}}\textit{generic} 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
%Let us consider a small generic perturbation $P'$ of one of the realizations shown in \cref{fig:edge-contraction-deformation-space}.
We first observe that all of the equivalent realizations which are highlighted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. This claim has been verified numerically. Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently small generic perturbation $P'$.
Hence, generic realizations are also not necessarily globally rigid.
Interestingly, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}

%\notodo{\mhsays{This is the opposite of global rigidity :D}}

It would be surprising, though also not absurd, that other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{13mm}
    \begin{minipage}[c]{0.32\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edge have the same lengths (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}

For bar-joint frameworks, generic global rigidity is often checked by computing the rank of a \Def{stress matrix} for a random equilibrium stress (\cf\ \cite{gortler-healy-thurston}). Since we demonstrate in this article, that many concepts from bar-joint framework rigidity theory carry over to the polytopal setting, it is possible that we can formulate a similar criterion for the generic global rigidity of polytopes. This provides an exciting direction for future research.

\begin{question}
    Can the rank of the stress matrix be used as a criterion for generic global rigidity?
\end{question}

% Still, that argument does not resolve whether the regular dodecahedron with combinatorial type $\mathcal{D}$ is globally rigid. Nevertheless, we know that there exists a realization of the dodecahedral graph in $\mathbb{R}^2$ that has equal edge lengths (\cf\ \Cref{fig:planar-dodec}). While this realization is not affinely spanning, it clearly has planar facets. If $0$ lies in the relative interior of this polytope, it is impossible to satisfy the equation $\langle p_i, a_\sigma\rangle=1$ for $i\sim \sigma$, as each facet normal must necessarily be normal to the embedded plane $\mathbb{R}^2$, so that $\langle p_i, a_\sigma\rangle=0$. For that reason, we put the plane at height $1$ so that each face has the same normal vector. With this modification, we find that the realization of $\mathcal{D}$ lies in $\real(\mathcal{D})$, implying that the regular dodecahedron is not globally rigid.






%\newpage % temporary new page

%\section{Case study: The truncated dodecahedron}
%\label{sec:truncated_dodecahedron}
%\label{sec:TDod}





\newpage % temporary new page

\section{Conclusion}
\label{sec:outlook}

\mwsays{I am not a fan of a conclusions section that just repeats introduction and main body for the third time. I liked the outlook we had in the last paper because it was just full of questions. If I see correctly, then the only new bit here is the TDod discussion, which might as well go into the results section. This section would be an easy place to shorten the paper.}
\mhsays{A conclusion/outlook is a formal requirement for any scientific paper. In it, the main arguments/results should be restated and it gives room for open problems and future research. Ideally, one uses the three questions ``what?'', ``so what?'' and ``now what?'' to guide the writing. The conclusion is an important place in the paper to state and summarize our most significant findings and results, why they are useful and what should happen next. We can keep it to 1 page, but it is an essential section.}


\todo{\mwsays{Like for title and abstract, I don't think we should reduce this article to second-order theory} \mhsays{Better? }}%
In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 

\notodo{\mwsays{I see ``a careful development of first- and second-order theory'' as a main result.}\mhsays{First-order theory was in the first paper, right? Added this sentence to Main Results.}\mwsays{First paper only contains claims, no development of the actual first-order theory. Developing first-order theory properly was one of the selling point of this paper here that we declared back then.}\mhsays{This was a question that a reviewer might ask. I have no problem adding this to the Conclusion (which I now did).}}

\subsection{Main results}

We carefully develop a first-order and second-order theory for the rigidity of polytopes in \Cref{sec:first_order,sec:second-order-theory}. Using these tools, we demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves induced by edge length modifications.

\iffalse\textcolor{gray}{
\todo{\mwsays{Saying this makes only sense if it would be in the main body, but it is in the appendix} \mhsays{The conclusion was written when this was not the case.} Feel free to remove.}%
Moreover, we extend our analysis to flexible polytopes. For zonotopes and generic Minkowski sums, we provide a lower bound on the dimension of the flex space. As of now, all flexible convex polytopes that we are able to find arise as zonotopes or generic Minkowski sums. To approximate the flexes of polytopes, we develop an algorithm in \Cref{sec:approx_continuous_motions}, which relies on Riemannian geometry and homotopy continuation, alongside several useful heuristics.}
\fi

Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. In \Cref{sec:dodecahedron}, we explicitly demonstrate a strategy for proving the second-order rigidity of the regular dodecahedron as a test case and we also investigate deformations induced by modifying the length of a single edge, which reveals a highly interesting local geometry and also serves as a counterexample for the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}

\iffalse
\begin{remark}
For the truncated dodecahedron, the system of homogeneous quadratic \todo{\mwsays{Reference these equations by number rather than words}}equations introduced in \Cref{section:second-order-rigidity-check} has a non-trivial solution. According to \Cref{res:sotest}, this implies that the truncated dodecahedron is not second-order rigid. In fact, we find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
\end{remark}
\fi

Among the 31 polytopes we consider, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is four-dimensional, so it is not first-order rigid, and we demonstrate that it is not second-order rigid, since the associated system of homogeneous quadratic equations $Q_1=\dots=Q_4=0$ arising from Equation \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. In fact, we \notodo{\mwsays{Say that we find this only numerically.}\mhsays{Apparently we know this symbolically! (Y)}}find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
In \Cref{fig:TDod_flex_conc}, we show samples from a deformation of the truncated dodecahedron.
It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances.
%which is \todo{\mwsays{``It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances''}} constructed using gradient descent with reasonable numerical tolerance.

\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}

However, when we apply a more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
%\todo{\mhsays{Discuss energy interpretation}}
This result would help explain, why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which has reasonably low numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, they observe that the energy landscape around an $N$-th order rigid realization locally looks like the parabola $y=x^{2N}$. This implies that for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

Unfortunately, if the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 

%\mhsays{Develop higher-order rigidity techniques.}

% \notodo{\mwsays{I would say we don't need this section. Move the problems to their sections or mention them in the introduction.} 
% \mhsays{Open problems only belong into the introduction if (a) we solve them or (b) they are guiding problems that motivate our article. Neither is the case. We should move them to the respective sections instead (which I did). }}

%\mhsays{Theoretical results for why some polytopes in special position are inf rigid, even though Cauchy-Dehn does not say this.}

%\mhsays{More constructions for flexible polytopes OR proof that Minkowski flexes are all.}

%\mhsays{Dodecahedron and truncated icosahedron have the same numer of first-order flexes; does this come from the symmetries? Counter point: the truncated dodecahedron only has 4 dimensions of first-order flexes even though it has the same symmetry. Where is the lost dimension? Is there a general way of predicting the first-order flexes from the symmetry group?}

%\mwsays{Is there special structure in the TDod that helps deciding the rigidity question?}

%\mhsays{Point out many interesting questions from \Cref{sec:dodecahedron}}



==> sec/introduction_-_copy_-_2026-01-11.tex <==

%For comments: \mhsays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}


\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and ask under what conditions a polytope admits a continuous deformation that preserves edge lengths and face coplanarities,
%. The major difference to the classical setting of polyhedral rigidity is that these deformations are explicitly 
but, in contrast to classical polyhedral rigidity, is allowed to change the shapes of the faces.
As a general outcome of their investigations the sentiment arose that flexibility in polytopes (\ie\ the existence of a deformation) is an exceptional property, not only among combinatorial types of polytopes, but also among realizations of a fixed type.
The authors conjecture that a generic convex realization of a combinatorial type admits no deformation, that is, is rigid. This was proven in dimension three.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex}
\end{figure}

Not unlike the classical setting of framework rigidity, deciding the rigidity properties of a given polytope is computationally hard once one moves beyond the first-order analysis. 
In fact, only few examples of flexible polytopes are known, constructed using a hand full of techniques such as Minkowski sums and affine flexes.
Conversely, already for polytopes with only a few faces it is unknown whether they are rigid or transformations.
The article \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} singles out the regular dodecahedron as a prime example of a small polytope with unclear rigidity properties.

In this article we develop new techniques for analyzing the rigidity of polytopes. 
This includes the formulation of a suitable second-order theory of polytope rigidity, as well as computational tools for probing the realization spaces and computing deformation paths.
We showcase these techniques by determining the rigidity properties of all but one of the Archimedean and Catalan solids, including the previously open regular dodecahedron.
As the only exception we identified the \emph{truncated dodecahedron} as a polytope with remarkable (thought not fully understood) rigidity properties that can serve as a future benchmark for computational tools.

\mwsays{In this article we address notions of rigidity skipped over in the first part: second-order, continuous and global.}

\subsection{Theoretical results}

In this article we provide a clean development of the necessary first- and second-order theory of polytope rigidity (or more generally, for point hyperplane frameworks).

We analyze the full realization space of a few examples where this is possible. This includes cubical zonotopes and generic Minkowski sums.

We explore the connection between first-order rigidity and the existence of local edge-length perturbations for polytope realizations.


\subsection{Methodological results}

...


\subsection{Computational results}

Our techniques apply to any polytope. The Archimedean and Catalan solids provided a convenient benchmark. The results are listed in \cref{tab:comparison}.

Our major finding include:
\begin{itemize}
    \item For all but three Archimedean solids the first-order theory decides the rigidity.
    If a polytope is first-order rigid, then it is rigid (see \cref{thm:first_order}. All Archimedean solids that were identified as flexible are so via a Minkowski flex and the dimension of the first-order flex space is as expected from this construction. 
    \item
    The regular dodecahedron is rigid. This was previously unknown since it is first-order flexible. The second order tools developed in this article allowed to identify the dodecahedron as second-order rigid \emph{but not} prestress stable.
    The regular dodecahedron furthermore becomes first-order rigid after a generic linear transformation. This suggests that the regular realization of the dodecahedron is a singularity in the realization space.
    By computing deformation paths that shrink/extend a single edge of the regular dodecahedron, we probe the neighborhood of this singularity. We find that bifurcating deformation paths and thereby a counterexample to generic global rigidity for polytopes.
    \item 
    The truncated icosahedron (the football) is also first-order flexible yet second-order rigid.
    \item 
    The truncated dodecahedron is flexible in both first- and second order. At this time it is unknown whether it admits a deformation. If it admits a deformation it is the first example of a polytope flex that is no of Minkowski sum type. If it is rigid then it is the first example of a naturally occurring rigidity of order greater than two.
\end{itemize}


\hrulefill

\mwsays{I write ...}

We develop the second-order rigidity theory for polytopes with edge length and coplanarity constraints. 
In addition, we develop computational tools for checking the rigidity of polyhedral surfaces and for approximating continuous motions. 

{
\def\arraystretch{1.5} 

\begin{table}[ht]
\centering
\begin{tabular}{|lc|c|lc|}
\cline{1-2}\cline{4-5}
\makecell{Tetrahedron\footnotemark\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/tetrahedron} & &
\makecell{Truncated Tetrahedron\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/truncatedTetrahedron.png} \\
\customdoubleline

\makecell{Cube\footnotemark\\[2.5mm](\no , \no , \no , 3)}&\cincludegraphics{Images/cube.png} & &
\makecell{Octahedron\addtocounter{footnote}{-2}\footnotemark\\[2.5mm](\yes , \yes , \yes , 0) } & \cincludegraphics{Images/octahedron.png} \\ \cline{1-2}\cline{4-5}

\makecell{Cuboctahedron\addtocounter{footnote}{1}\footnotemark\\[2.5mm](\no , \no , \no , 0+3)} &\cincludegraphics{Images/cuboctahedron.png} &  &
\makecell{Truncated Cube\\[2.5mm](\yes , \yes , \yes , 0) } & \cincludegraphics{Images/truncatedcube.png} \\ \cline{1-2}\cline{4-5}

\makecell{Truncated Octahedron\addtocounter{footnote}{-2}\footnotemark\\[2.5mm](\no , \no , \no , 5)} & \cincludegraphics{Images/truncatedOctahedron.png} & &
\makecell{Rhombicuboctahedron\footnotemark\\[2.5mm](\no , \no , \no , 3+3)} & \cincludegraphics{Images/SmallRhombiCuboctahedron.png}\\ \cline{1-2}\cline{4-5}

\makecell{Truncated Cuboctahedron\addtocounter{footnote}{-2}\footnotemark\\[2.5mm](\no , \no , \no , 5)} & \cincludegraphics{Images/greatRhombiCuboctahedron.png} & &
\makecell{Snub Cube\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/snubCube.png}\\ \customdoubleline

\makecell{Icosahedron\addtocounter{footnote}{-2}\footnotemark\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/icosahedron.png} & &
\makecell{\textcolor{DarkOrange}{Dodecahedron}\\[2.5mm](\no , \yes , \yes , 5)} & \cincludegraphics{Images/dodecahedron.png}\\ \cline{1-2}\cline{4-5}

\makecell{Icosidodecahedron\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/icosidodecahedron.png} & &
\makecell{\textcolor{DarkOrange}{Truncated Dodecahedron}\\[2.5mm](\no , \no , \Ques , 4)} & \cincludegraphics{Images/truncatedDodecahedron.png}\\ \cline{1-2}\cline{4-5}

\makecell{\textcolor{DarkOrange}{Truncated Icosahedron}\\[2.5mm](\no , \yes , \yes , 5)} & \cincludegraphics{Images/truncatedIcosahedron.png} & &
\makecell{Rhombicosidodecahedron\addtocounter{footnote}{1}\footnotemark\\[2.5mm](\no , \no , \no , 5+3)} & \cincludegraphics{Images/SmallRhombiIcosidodecahedron.png}\\ \cline{1-2}\cline{4-5}

\makecell{Truncated Icosidodecahedron\addtocounter{footnote}{-2}\footnotemark\\[2.5mm](\no , \no , \no , 5)} & \cincludegraphics{Images/greatRhombiIcosidodecahedron.png} & &
\makecell{Snub Dodecahedron\\[2.5mm](\yes , \yes , \yes , 0)} & \cincludegraphics{Images/snubDodecahedron.png}\\ \cline{1-2}\cline{4-5}

\end{tabular}
    \caption{\justifying The rigidity properties of the five Platonic solid and the 13 Archimedean solids sorted by the polytopes' symmetry classes. The 4-tuple below a polytope's name represents the following properties:\\ (1$^{\text{st}}$-order rigidity, 2$^{\text{nd}}$-order rigidity, rigidity, number of 1$^{\text{st}}$-order flexes).\\
    For all flexible polytopes, we provide an animation in the Supp. Mat.}
    \label{tab:comparison}
\end{table}
}

\mwsays{Regarding caption \cref{tab:comparison}: we should write first-/second-order rigidity instead of the numeric variants, but if I change it the table vanishes completely. Not sure what is going on. Maybe the figure becomes too long for the page?}


\footnotetext[1]{As a triangulated sphere, this polytope is infinitesimally rigid by Cauchy's Theorem \cite{cauchy1813}.}
\footnotetext[2]{As a zonotope, this polytope is flexible according to Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.}
\footnotetext[3]{As a ``generic'' Minkowski sum, this polytope is flexible (cf. \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}).}

\begin{enumerate}[label=\arabic*)]
    \item All Archimedean zonotopes (except for the cube) have 5 inf flexes because they are projectively unique as zonotopes and hence their only transformations come from the 9-dim general linear group minus rotations and global scale. The cube also loses scaling along axis, hence 3 less (but global scale is already contained in here).
    \item The first-order flex spaces of Rhombicuboctahedron and Rhombicosidodecahedron can be explained as the sum of the first-order flex spaces of their constituents + 3-dim rotations. 
\end{enumerate}

\subsection{Dodecahedron and Truncated Icosahedron}
\label{sec:dodecahedron}

The regular dodecahedron and the truncated icosahedron are interesting case studies. They are both first-order flexible and possess a 5-dimensional space of nontrivial infinitesimal flexes. Nevertheless, using techniques from computational algebra (cf. \Cref{section:second-order-rigidity-check}) we show that for each nontrivial flex there exists an equilibrium stress that \emph{blocks} the flex from extending to a continuous motion. In other words, both polytopes are second-order rigid (see \Cref{section:rigidity-of-the-regdod}).

The Legendre-Steinitz Theorem \cite{rastanawi2021dimensions} guarantees that any polytope $P$ in $\mathbb{R}^3$ lives in a smooth $(|E|+6)$-dimensional realization space. When factoring out the rigid motions, this leaves $|E|$ degrees of freedom. In \Cref{section:edge-length-perturbations}, we provide an interpretation of these degrees of freedom in terms of perturbations of the edge lengths: For rigid polytopes, the $|E|$ dimensions are necessarily associated with nearby realizations with different edge lengths from $P$. Using this language, we demonstrate that the dodecahedron exhibits a highly interesting algebraic and topological behavior in \Cref{section:dodec-edge-length-perturbations}. We also compute deformation paths associated with perturbing a single edge length using techniques from \Cref{sec:approx_continuous_motions}. \mhsays{Add pictures for this section as well}


\subsection{Truncated Dodecahedron}
\label{sec:truncated_dodecahedron}

The truncated dodecahedron is both first-order and second-order flexible.
More precisely, it has a 4-dimensional space of non-trivial first-order flexes, which is surprisingly different from the five dimensions that we usually associate with icosahedral symmetry (see \cref{sec:dodecahedron}). % that we found for both dodecahedron and truncated icosahedron.
For second-order rigidity it turns out that none of the first-order flexes is blocked by any stress, so all of them are potentially real. \mhsays{``real'' is not a good word in this context.}
%
Remarkably, we were able to construct a flex numerically!
So far we are not aware of an analytic way to obtain this flex.
Thus, whether this flex is actually real or not remains a mystery. 
In particular, if no such flex is real, there are currently no feasible techniques to prove the rigidity of this polytope.

Interestingly, all first-order flexes of the truncated dodecahedron vanish either on affine transformation or when changing the size of the triangles (keeping it vertex transitive).

The facts listed above suggest that the \emph{uniform} truncated dodecahedron is quite special.
In particular, it seems unlikely that the existence of its flex is a mere coincidence.
More likely, there exists a yet unknown construction, similar to Minkowski sums, that generates this flex.

If flexible, the truncated dodecahedron has some remarkable properties:
%
\begin{itemize}
    \item its flex is not reducible to a Minkowski sum
    \item its affine transformations are not (first-order) flexible.
\end{itemize}
%
In contrast, if it were rigid, this would be remarkable as well. 
It would then be the first example of a polyhedron that is second-order flexible, yet rigid.
The general consensus seems to be that rigidity beyond the second order only appears in contrived constructions specifically made for this purpose.
The truncated dodecahedron, being very natural, would then be an interesting counterexample.

\subsection{Outline}
This article is divided into three main parts: The theoretical foundation in Sections \ref{sec:combinatorics-of-polytopes}--\ref{section:edge-length-perturbations}, followed by methods in Sections \ref{section:second-order-rigidity-check}--\ref{sec:approx_continuous_motions} and a case study in \Cref{sec:dodecahedron}.












\newpage

\mwsays{Should we mention somewhere that polytope rigidity can be modeled using framework rigidity by stacking prisms?}

\begin{itemize}
    \item Introduction (Martin)
    \item Theory part (Martin, fix notation and termninology, stay close to first paper)
    \begin{itemize}
        \item first-order theory
        \item second order theory (prestress stability) 
        \item construction of flexible polytopes (continuous motions)
        \begin{itemize}
            \item theorem for generic zonotopes
            \item counterexample for general zonotopes (hex prism)
            \item questio for generic Minkowski sums
        \end{itemize}
        \item Edge length perturbation (Matthias)
    \end{itemize}
    \item Methods part
    \begin{itemize}
        \item second-order rigidity check (Gröbner bases, ...) (Albert)
        \item Computing deformation paths (also works for changing edge lengths but we don't mention this here maybe???)  (Matthias)
    \end{itemize}
    \item Case studies (results)
    \begin{itemize}
        \item Dodecahedron
        \begin{itemize}
            \item not first-order rigid (five dim space)
            \item proof of second-order rigid (not prestress stable)
            \item numerical experiments on edge length perturbations and what they might entail (Matthias) 
            \item no global rigidity (Matthias)
        \end{itemize}
        \item Truncated Icosahedron (Matthias + Martin)
        \begin{itemize}
            \item Five first-order flexes
            \item Still second-order rigid
        \end{itemize}
        \item Truncated dodecahedron (Matthias + Martin)
        \begin{itemize}
            \item unclear rigidity
            \item NOT second-order rigid (evidence?)
            \item we believe it is flexible ???
            \item have potential deformation paths
        \end{itemize}
    \end{itemize}
    \item Outlook (Martin)
    \begin{itemize}
        \item (questions about edge-length perturbations -- maybe already in theory part)
        \item is there specific structure in the TDod that helps us to see it is rigid/flexible and construct the flex
        \item Are there general stronger methods for deciding rigidity and constructing deformations
    \end{itemize}
    \item Supplementary material
    \begin{itemize}
        \item computational output (Gröbner bases etc)
        \item Code, algorithms
        \item Animations
    \end{itemize}
\end{itemize}

\newpage % temporary new page

Main results:
\begin{itemize}
    \item carefully define first- and second-order rigidity and prestress stability for this setting.
    \item this gives a strong test for rigidity (resolves previously open cases).
    \begin{itemize}
        \item dodecahedron
        \item truncated icosahedron
        \item checked all Archimedean solids and duals (resolved all but one) 
    \end{itemize}
    \item very interesting special case: truncated dodecahedron (TDod)
    \begin{itemize}
        \item we believe it is flexible (for now)
    \end{itemize}
    \item something about edge length perturbation?
    \item edge length perturbations of the dodecahedron: we find there is a singularity in the ``dual space'' (rigidity transition region is algebraically singular)
    \item dodecahedron is an example that we don't have global rigidity
    \item maybe something about zonotope flexes
\end{itemize}

\hrulefill

\begin{itemize}
    \item many examples of rigidity
    \begin{itemize}
        \item short edges make rigid
        \item higher dimensions + first order rigidity in higher dimensions
    \end{itemize}
    \item second-order rigidity
    \begin{itemize}
        \item second order rigid implies rigid
        \item Q: does second-order flexibility imply proper flexibility?
        \item $\#stresses=\#flexes$ trivial or worth mentioning?
    \end{itemize}
    \item the dodecahedron example
    \begin{itemize}
        \item affine trafos do not preserve first-order rigidity
        \item there is no global rigidity for polytopes in 3D
    \end{itemize}
    \item many other open questions
    \begin{itemize}
        \item Q: does flexibility need parallel edges?
    \end{itemize}
\end{itemize}

Notes on Archimedean solids:
\begin{itemize}
    \item the only Archimedean solids that are inf-flexible but not generic Minkowski sums are the dodecahedron, truncated dodecahedrona (4 flexes) and truncated icosahedron (5 flexes). Where do we lose the flex on the way from truncated dodecahedron to dodecahedron?
    \item Are they second-order rigid? Can the dimension of their flex spaces and their second-order rigidity be explained in some way using the known properties of the dodecahedron? (Limit argument?)
    \item Are there continuous motions between Archimedean/Catalan/Platonic solids thats preserve the planarity of facets and the edge lengths?
\end{itemize}

Other notes
\begin{itemize}
    \item A zonotope is highly flexible, but is there a zonotope that can flex in more ways than just deforming into other zonotopes, either real or infinitesimally?
    \item If $P$ and $Q$ have infinitesimal flexes, then does $P+Q$ inherit them in some way?
\end{itemize}
\newpage % temporary new page













\newpage

\section{Polytopes, combinatorial types and realizations}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 


Recall from Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} that the combinatorics of a polytope can be described using its~vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is a triple~consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and a \Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
%Evidently, every convex polytope $P$ gives rise to such a structure, which we call the combinatorial type of $P$.


To enforce edge length constraints we need to access the vertex adjacency information in $\mathcal P$: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.
This defines a graph structure on $V$ which we call the~\Def{edge graph} $G_{\mathcal P}=(V,E)$.
%If $\mathcal P$ is the combinatorial type of a convex polytope $P$, this notion agrees with the usual edge graph of $P$.
To emphasize the presence of this graph structure~we~also~de\-note a combinatorial type by $\mathcal P = (V,E,F,\sim)$.

The polytopes that have a given combinatorial type $\mathcal P$ form the \emph{polytopal~realizations} of $\mathcal P$.
More convenient for computations, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ we have $\|a_\sigma\|=1$ and~the~points~(or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane})~with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_j-p_i,a_\sigma\>=0,\quad\text{whenever $i,j\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_j-p_i,a_\sigma\><0,\quad\text{whenever $i\sim \sigma,j\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ gives rise to a convex realization in this sense with the facet normals pointing outwards.
We often identify a polytope with the corresponding realization~and use $P$ and $(\bs p,\bs a)$ interchangeably.





All realizations of $\mathcal P$ taken together form the \Def{realization space} of $\mathcal P$: % that can be concisely expressed as
%
\begin{align*}
\realSp(\mathcal P)
%=\realSp(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Big\vert
    \begin{array}{rcl}
    \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_j-p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 0\text{ whenever $i,j\sim \sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
Analogously, the \Def{convex realization space} is defined as
%
\begin{align*}
%\begin{align*}
\realSp_{\mathrm c}(\mathcal P)
%=\realSp_{\mathrm c}(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_j-p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 0\text{ whenever $i,j\sim \sigma$}\,\\
    \<p_j-p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 0\text{ whenever $i\sim \sigma, s\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
%Clearly $\real(\mathcal P)$ is a real algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!, and $\realCvx(\mathcal P)$ is a real semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.

\mwsays{Define $\realR(P)$ reduced realization space?}




\tempnewpage

\section{Polytope rigidity}
\label{sec:rigidity}

We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarity and the combinatorial type.

Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
A \Def{motion} of $(\bs p,\bs a)$ is a curve $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$;
the motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, then we call it \Def{flexible}, and \Def{rigid} otherwise.

\mwsays{Something about the examples we know and that it is hard to find examples.}

% Several examples of flexes in polytopes are shown in \cref{fig:flexes}.
% More examples and concrete constructions are provided in \cref{sec:examples}.
% The central question in this setting is:

% \begin{question}
%     Can one characterize the class of polytopes that are rigid or flexible? %Can one do so at least for polytopes of dimension $d=3$?
% \end{question}


% The reader familiar with \emph{point-hyperplane frameworks} (that is, bar-joint frameworks with additional coplanarity constraints) recognizes our construction as~a~special instance thereof.
% We refer to Eftekhari et al.\ \cite{EJNSTW} for a general introduction and also for further details on their first-order theory.
% %
% Our investigation can be seen as an attempt at understanding where the origin of such a framework from a polytope allows us to prove stronger results than in the more general setting.
% In particular convexity and sphericity are properties known for having strong implications in many contexts.












\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.

Let \Def{$\VF$} be the set of incident vertex-facet pairs. The \Def{rigidity matrix} $\mathcal R(P)$ of a polytope $P=(\bs p,\bs a)\subset\RR^d$ is a matrix of dimension $(|E|+|\VF|)\times(d|V|+d|F|)$ and has entries as follows:
%
\vspace{1ex}
\begin{center}
    \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
\end{center}
%
The shown entries are to be interpreted as $1\times d$ sub-matrices. 
%
The first-order~theory of rigidity is essentially the study of the linear algebra properties of the rigidity~matrix and the central first-order notions can be derived from $\mathcal R(P)$.
%$p_i$ should be thought of as the coordinate of vertex $i$, and $a_\sigma$ the corresponding vertex of facet $\sigma$ in the polar dual of $P$.

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We~denote them as pairs $\dot P=(\bsdot p,\bsdot a)$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    % \label{eq:flex_at_face}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    \label{eq:flex_at_face}
\end{align}
%
First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any vertex $i\in V$ and facet $\sigma\in F$}.
    % \label{eq:trivial_motion_facet}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    \label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    \label{eq:trivial_motion_facet}
\end{align}
%
Non-trivial first-order motions are called \Def{first-order flexes}. A polytope is \Def{first-order flexible} if it has first-order flexes, and is called \Def{first-order rigid} otherwise.


The elements of the cokernel (the kernel of the transpose $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system. 
We denote them by pairs~$(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following~two~\Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}

{\color{lightgray}

\begin{observation}
    If a facet $\sigma\in F$ is a simplex, then the left hand side of \eqref{eq:stress_at_face} is a linear combination of $d$ linearly independent vectors in $\RR^d$. 
    This can be zero only if all coefficients are zero.
    Hence, $\eta_{i\sigma}=0$ for all $i\sim\sigma$.

    Thus, if the polytope is simplicial, then all facet stresses are zero and the stress is a pure classical framework stress. Due to a theorem of Dehn, convex simplicial polytopes cannot have a non-zero framework stress. \mwsays{True in $d\ge 4$?}\asays{the 16-cell (cross-polytope) has 8 vertices and 24 edges and hence has two self-stresses. In general, there are many stresses, I think}
\end{observation}

\begin{lemma}
    \label{res:corank_rigid}
    A polytope is first-order
    %\asays{below we use infinitesimal rigidity. Let's choose one throughout} 
    rigid if and only if $\corank \mathcal R(P) = {{d+1}\choose 2}$
    %\mwsays{I prefer ``first-order rigid'' because it is more consistent with ``second-order rigid''. Using ``first-order rigid'' and ``corank'' would be consistent with the other paper.}
\end{lemma}
%
\begin{proof}
    \TODO\ \mwsays{Maybe not true if $P$ is not affinely spanning. But we are always spanning. Cite a paper by Bernd, Bill, Tony, ... for this}\asays{it's not formally proved there, but I think we can still reference it. I do agree we need spanning. If the joints are spanning, then this statement is pretty clear I think. We have a non-trivial infinitesimal motion iff kernel has dimension larger than ${d+1}\choose 2$}
\end{proof}

}

The reason we care about first-order rigidity is given by the following theorem:

\begin{theorem}\label{thm1}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}

\begin{proof}
    %\textcolor{red}{Add proof here}
    We prove the contrapositive: if $P$ is flexible, then it is first-order flexible. 
    Let $P^t$ be a flex. \todo{\mwsays{I think we need to invoke curve selection to get an analytic flex}} 
    If $P^t$ is not trivial, then we can truncate the Taylor expansion of $P^t$ at some order, say $k$, after which it cannot be completed to a trivial motion by adding higher order terms. 

    We expand the $k$-th derivative of the constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} we obtain
    %
    \begin{equation*}
        \sum_{i=0}^k\binom{k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i(t)-p_j(t))\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k-i}(p_i(t)-p_j(t))=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^k\binom{k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i(t))\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k-i}(a_k(t))=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $k$ is the smallest integer, the first, second, all the way up to $(k-1)^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to order $k-1$ are all zeros. The two equations above become the following. 
    \begin{equation*}
        2(p_i(t)-p_j(t))\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i(t)-p_j(t))=0
    \end{equation*}
    and 
    \begin{equation*}
        (p_i(t))\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(a_k)+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i(t))\cdot (a_k(t))=0
    \end{equation*}
    The $k$-th derivative satisfies the same equation as a non-trivial infinitesimal flex does. Therefore, $P$ is infinitesimally flexible. 
\end{proof}

\iffalse
\subsection{Equilibrium Stresses}
\label{sec:stresses}

\mhsays{Global rigidity definition? Stress-based global rigidity criterion?}
\fi



\subsection{3-dimensional polyhedra}

One fact that makes 3-dimensional polytope rigidity tractable as compared to dimension $d\ge 4$ is that first-order rigidity can be expressed purely in terms of stresses.

\begin{lemma}
    For $\mathcal R(P)$ holds $\text{$\#$columns}=\text{$\#$rows}+6$.
\end{lemma}
%
\begin{proof}
    Let $v,e$ and $f$ be the number of vertices, edges and faces of $P$ respectively.
    
    For each vertex, the number of incident faces equals the number of incident~edges. Thus, the total number of vertex-face incidences in $P$ is equal to the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2e$.
    Using Euler's polyhedral formula $v-e+f=2$, we arrive at
    %
    $$\text{\#rows}=|\VF|+e=2e+e=3e=3(v+f-2)=3v+3f-6=\text{\#columns}-6.$$
\end{proof}

\mhsays{Add the property that $\# flexes = \# stresses$ for polytopes?} \mwsays{Only true for $d=3$, and yes we should mention this.}

\begin{corollary}
    \label{res:rigid_eq_stress_free}
    A polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{corollary}












\tempnewpage % temporary new page

\section{Second-order theory}
% \section{Second-order rigidity and prestress stability}
\label{sec:second_order}
\label{sec:second-order-theory}

Sometimes, the polyhedron can still be rigid even if it is not first-order rigid. Rigidity beyond first order is often difficult to test even for bar frameworks. The technique of this section is motivated by Connelly and Whiteley \cite{connelly1996second}. Taking the second derivative of the edge length and planarity constraints, we have 
    \begin{equation}\label{eq1}
        \<p_i-p_j,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\dot{p}_i-\dot{p}_j\>=0
    \end{equation} for each edge $ij$ in $E$, and 

    \begin{equation}\label{eq2}
        \<p_i,\ddot{a}_k\>+2\< \dot{p}_i,\dot{a}_k\>+\<a_k,\ddot{p}_i\>=0
    \end{equation} for each vertex $i$ in facet $k$. 

%\mwsays{I previously introduced commands to render $\bs p, \bsdot p, \bsddot p$ (see TeX code for commands) in place of $\mathbf{\ddot{p}}$; again, this would be consistent with the first paper. In any way, I recommend to use the command, we can change its appearance later if desired.}

Let $\dot P,\ddot{P}$ be the vectors $(\dot{p}_1,...,\dot{p}_{|V|},\dot{a}_1,...,\dot{a}_{|F|})$, $(\ddot{p}_1,...,\ddot{p}_{|V|}$ and $\ddot{a}_1,...,\ddot{a}_{|F|})$ correspondingly. We can now define the second-order flex:
%\mhsays{I suggest using textit and a pale color (e.g. blue) for definitions instead of bold font. That makes it distinguishable from Definitions/Theorems} \mwsays{I imported the command \texttt{\textbackslash Def} for this. It renders \Def{like this}. Feel free to modify.} \mhsays{Looks good!}
\begin{definition}\label{sorigid}
    The pair $(\dot{P},\ddot{P})$ is a \Def{second-order flex} if equations \eqref{eq1} and \eqref{eq2} are satisfied. A second-order flex is \Def{nontrivial} if $\dot{P}$ is not a trivial first-order flex. The polyhedron $P$ is \Def{second order flexible} if there exists a non-trivial second-order flex. Otherwise, we say that it is \Def{second-order rigid}. \mhsays{Prestress stability?} 
    
    %\mwsays{Use eqref for referencing equations. Use cref for everything else.}
\end{definition}
\begin{remark}
    Notice here we are not defining trivial second-order flexes as first and second derivatives of trivial flexes. The reason is that while it is possible to build a nontrivial flex with a trivial first derivative, it is not interesting because we can ``push'' the lowest nontrivial derivative down to the first derivative. Therefore, we only need to look at the case where $\dot{p}$ is nontrivial. 
\end{remark}
\mhsays{We should fix a notation about the realization ${\bs p}, P, ({\bs p},{\bs a})...$ and keep it consistent throughout the article.}
\asays{Since we defined $P=(\mathbf p,\mathbf a)$, I defined $\dot P$ and $\ddot P$ analogously.}
In terms of matrices, equations $\eqref{eq1}$ and $\eqref{eq2}$ can be written as a matrix equation:
\begin{equation*}
    R(P)\ddot{P}+R(\dot P)\dot P=\mathbf{0}
\end{equation*}
For any non-trivial $\dot{P}$, if $\ddot{P}$ exists, then for any stress $\omega$ we have:
$$\omega (R(P)\ddot P+ R(\dot P)\dot P)=0$$ since the dot product of any vector with the $\mathbf{0}$ vector is 0.
%\mhsays{Use a different symbol for the all-zeros vector? E.g., $\overrightarrow{\rm 0}$ or $\mathbf{0}$.} 
Observe that if $\omega$ is a stress, then $\omega R(P)\ddot P=0$ because $\omega R(P)$ is the 0 vector. This forces $\omega R(\dot P)\dot P=0$ to hold.

Next, we move on to the second-order duality which can be useful when we want to prove $\ddot{P}$ does not exist. Before that, we first introduce the following equality form of Farkas' lemma:
    \begin{lemma}\label{farkaseq}
        Either $Ax=b$ has a solution, or $A^Ty=0$ has a solution with $b^T y\not =0$.
    \end{lemma}
    Intuitively, this Lemma says that either $b$ is in $A$'s column space, or there exists a hyperplane containing the column space of $A$ and $b$ is not in it. 

\begin{lemma}\label{lem2}
    Given an infinitesimal motion $\dot P$, if and only if there exists a stress $\omega$ such that \begin{equation}\label{block}
        \omega R(\dot P)\dot P\not=0
    \end{equation}
    then there cannot be a $\ddot P$ such that $(\dot P,\ddot P)$ is a second-order flex. 
    $\omega$ is called a \Def{blocking stress} for $\dot P$ if inequality $\eqref{block}$ holds. \mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.}
\end{lemma}

\begin{proof}
    The ``if'' direction is already given in the discussion above. To show ``only if'', we use \cref{farkaseq}.
    %\mhsays{I don't like using the theorem environment in a proof} 
    Let $A=R(P)$, $b=-R(\dot P)\dot P$, $x=\ddot P$, and $y=\omega$. Then \cref{farkaseq} says that either there exists a $\ddot P$ or you can find a blocking stress. 
\end{proof}

\begin{definition}
    If there exists a stress that blocks every non-trivial first-order flex, we say the polyhedron is \Def{prestress stable}.
\end{definition}

    By combining \cref{sorigid} and \cref{lem2}, we have the following result:
    \begin{theorem}\label{sotest}
        $P$ is second-order rigid if and only if every nontrivial first-order flex has a blocking stress. 
    \end{theorem}%\mhsays{Formulate as a theorem? This seems to be what people are usually doing in second-order rigidity papers, right?} 
Second-order rigidity is useful because of the following:

\begin{theorem}
    \label{thm3}
    \label{res:second_order_rigid_impl_rigid}
    Second-order rigidity implies rigidity. 
\end{theorem}

\begin{proof}
    The proof is almost identical to that of \cref{thm1}. Let $q$ be the smallest integer such that the first $q$ derivatives of $P(t)$ do not come from a trivial flex at $t=0$. The $2q^{th}$ derivative of the constraints can be expanded as:
    %
    \begin{equation*}
        \sum_{i=0}^{2q}\binom{2q}{i}\Bigl(\frac{d}{dt}\Bigr)^i(p_i(t)-p_j(t))\cdot \Bigl(\frac{d}{dt}\Bigr)^{2q-i}(p_i(t)-p_j(t))=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^{2q}\binom{2q}{i}\Bigl(\frac{d}{dt}\Bigr)^i(p_i(t))\cdot \Bigl(\frac{d}{dt}\Bigr)^{2q-i}(a_k(t))=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $q$ is the smallest integer, the first, second, all the way up to $q-1^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to the $q-1^{th}$ are all zeros. The two equations above become the following. 
    %
    \begin{equation*}
        2(p_i(t)-p_j(t))\cdot \Bigl(\frac{d}{dt}\Bigr)^{2q}(p_i(t)-p_j(t))+\binom{2q}{q}\Bigl(\frac{d}{dt}\Bigr)^{q}(p_i(t)-p_j(t))\cdot \Bigl(\frac{d}{dt}\Bigr)^{q}(p_i(t)-p_j(t))=0
    \end{equation*}
    %
    and 
    %
    \begin{equation*}
        (p_i(t))\cdot \Bigl(\frac{d}{dt}\Bigr)^{2q}(a_k)+\Bigl(\frac{d}{dt}\Bigr)^{2q}(p_i(t))\cdot (a_k(t))+\binom{2q}{q}\Bigl(\frac{d}{dt}\Bigr)^{q}(p_i(t))\cdot\Bigl(\frac{d}{dt}\Bigr)^{q}(a_k)=0
    \end{equation*}
    %
    Set $\dot P= \Bigl(\frac{d}{dt}\Bigr)^{q}P(t)\big|_{t=0}$ and $\ddot P=2/\binom{2q}{q}\Bigl(\frac{d}{dt}\Bigr)^{2q}P(t)\big|_{t=0}$. The two above equations become Equations \eqref{eq1} and \eqref{eq2}. Therefore, if $P$ is flexible, it has a non-trivial second-order flex. 
\end{proof}
















\newpage

\subsection{First-order theory}
\label{sec:first_order}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.


A \Def{first-order motion} $(\bsdot p,\bsdot a)$ of $P$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$, %=(\dot p_i\in\RR^3:i \in V;\, \dot a_\sigma\in\RR^3 : \sigma \in F)$.
that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    \label{eq:flex_at_face}
\end{align}

A first-order motion is \Def{trivial} if in addition it satisfies
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    \label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    \label{eq:trivial_motion_facet}
\end{align}
%
A non-trivial first-order motion is called a \Def{first-order flex}.
A framework is \Def{first-order rigid} if it has no first-order flexes; it is \Def{first-order flexible} otherwise.
Many results from the bar-joint framework setting transfer in the expected way. In particular, if a polytope is first-order rigid, then it is rigid. 

The first-order flex conditions \eqref{eq:flex_at_vertex} -- \eqref{eq:flex_at_face} can be collected in a corresponding \Def{rigidity matrix} $\mathcal R(P)$ % with dimensions $(E+\VF)\times(dV+dF)$. 
which satisfies $\mathcal R(P)(\dotbs p,\dotbs a)=0$ if and only if $(\dotbs p,\dotbs a)$ is a first-order motion.
%
Since we only consider polytopes with non-empty interior, they are in particular affinely spanning and
the rank condition of first-order rigidity applies: 

\begin{lemma}
    \label{res:rank_condition}
    We have
    %
    $$\corank \mathcal R(P) \ge \binom{d+1}{2},$$
    %
    with equality if and only if $P$ is first-order rigid.
\end{lemma}

\hrulefill

%\begin{definition}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
We write
%
\begin{align*}
    \realP{\mathcal P}P &= \realpa{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \real(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
    \\
    \realPCvx{\mathcal P}P &= \realpaCvx{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \realCvx(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
\end{align*}
%
for the (\Def{convex}) \Def{configuration space}, \ie\ the space of all (convex) realizations equivalent to a given (convex) realization $P=(\bs p,\bs a)$.

A \Def{motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\realpa{\mathcal P}{\bs p}{\bs a}$ for which $(\bs p^0,\bs a^0)=(\bs p,\bs a)$.
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all~$t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, we call it \Def{flexible}, and \Def{rigid} otherwise.
%\end{definition}

In general, understanding the full configuration space is intractable in all but the simplest cases. 
We mention here a few situations in which such a full understanding is possible due to various genericity assumptions.
In our language, Cauchy's classical rigidity theorem \cite{cauchy1813} states that $\realPCvx{\mathcal P}P$ is a single point whenever $\mathcal P$ is a simplicial polytope.
As a consequence of the main result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} we also obtain the following:

\begin{theorem}
    Let $\mathcal P$ be the combinatorial type of a 3-dimensional polytopes (\ie\ a polyhedral graph).
    Then for almost all convex (in fact, Zariski convex) realizations $P$ of $\mathcal P$ holds: $\realP{\mathcal P}P$ consists of finitely many isolated points.
\end{theorem}
%
Here, \emph{almost all} means that a dense open subset of the (Zariski closure of) the convex realization space has this property.
%
\begin{proof}
    \TODO \mhsays{$\real(\mathcal{P})$ may be irreducible, but that does not mean that $\real(\mathcal{P},P)$ is. The geometry of $\real(\mathcal{P},P)$ may be pretty complicated. We know that $P$ has generic coordinates; however, it seems like what we need to do is show that $P$ also has generic edge lengths. By going back to the edge length perturbation space and proving a stronger result than Proposition 5.2, we then may be able to prove this. The main issue is that we don't really understand the edge length measurement variety and much less the intersection of that variety with $\real(\mathcal{P})$. So I guess to conclude: I don't really have an easy idea how to approach this. You?}
\end{proof}

We conjecture the same to be the case in higher dimensions.

Lastly, recall that a \Def{zonotope} is a polytope obtained as the Minkowski sum of finitely many line segments. A \Def{cubic zonotope} is a zonotope with all faces being combinatorial cubes. Cubical zonotopes are the zonotopal equivalent of simplicial polytopes, in the sense that they are generic in the class of zonotopes: they are generated from line segments in general position:

\begin{theorem}
If $P\subset\RR^d$ is a cubic zonotope generated from $k$ line segments, then %
$$\realP{\mathcal P}P = (\RR P^{d-1})^k.$$
\end{theorem}
%
\begin{proof}
    \TODO
\end{proof}










\newpage % temporary new page

\section{Constructing flexible polytopes}
\label{sec:flexible_polytopes}

To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

\begin{definition}
    Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
A \Def{continuous motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that
\begin{itemize}
\item $(\bs p^t(0),\bs a^t(0))=(\bs p,\bs a)$ and 
\item $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
\end{itemize}
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If a realization $(\bs p,\bs a)$ has a motion, then we call it \Def{flexible}, and \Def{rigid} otherwise.
\end{definition}

\subsection{Zonotopes}

A zonotope is \Def{generic} if all its faces are combinatorial cubes. We call it generic because it generated from line segments in generic position. Generic zonotopes are the zonotopal equivalent of simplicial polytopes. For the latter the rigidity theory is classical -- they are rigid, both infinitesimally and globally (Chauchy's and Dehn's theorem).
Likewise, for generic zonotopes a complete theory can be given.

\begin{theorem}
    Let $P\subset\RR^d$ be a rhombic zonotope with $n$ generators. Then
    %
    \begin{myenumerate}
        \item 
        $\realR(P)$ is a connected smooth variety of dimension $(d-1)n-{d\choose 2}$.
        In particular, each polytope $Q$ combinatorially equivalent to $P$ with the same edge lengths can be deformed into $P$.
        \item if $Q\in\real(P)$ then $Q$ is a zonotope.
        \item The first-order flex space of $P$ has dimension $(d-1)n-{d\choose 2}$.
        \item Each first-order flex of $P$ corresponds to a real flex.
    \end{myenumerate}
\end{theorem}
%
\begin{proof} \mwsays{Work in progress, these are just ``mental'' notes.}
    Consider the space of all deformations of a zonotope that preserves only coplanarity and central symmetry of the facets (the latter is in combinatorial cubes also implied by edge length constraints).
    Note that for $n$ generators there are $2{n\choose d-1}$ facets, and that the central symmetry of each is guaranteed by $d(d-2)$ equations: each pair of opposite vertices (of which there are $d-1$) must have a centroid identical to the centroid of the first pair; this is a vector identity with $d$ components.
    Note that this preserves coplanarity automatically.
    Likewise for an infinitesimal flex -- there $dV$ DOFs and $2d(d-2){n\choose d-1}$ constraints. Removing translations but not rotations, we obtain $dV-2d(d-2){n\choose d-1}-d$ final infinitesimal DOFs.
    Observe that the realization space is a manifold of dimension $nd$, or $n(d-1)$ if we want to preserve lengths. It is also well known that $V=2\sum_{k=0}^{d-1} {n-1\choose k}$.
    It remains to check
    %
    $$dV-2d(d-2){n\choose d-1}-d = nd.$$
    %
    This seems to yield too few remaining DOFs ($< dn$) and so some of the constraints are redundant. Which and how many is unclear?
    
    \mwsays{Check that the fact that all inf flexes extend follows already from some general theory about realization spaces of polytopes when the realization spaces are smooth manifolds.}
\end{proof}

\begin{remark}
    More general zonotopes have non-zonotopal flexes. 
    As soon as some face of a zonotope is not a rhombus, then it is the Minkowski sum of this face with the other generators. But a polygon with more than four sides has a non-trivial (\ie\ not symmetry preserving) flex. Hence the Minowski sum of this flex with the other generators yields a non-zonotope.
\end{remark}

\begin{question}
    Is the first-order flex space of zonotopes exactly the tangent space to the finite flexes?
\end{question}

We can ask analogous questions for general Minkowski sums.

\begin{question}
    Is it true that the generic Minkowski sum (where no two faces, edge or higher, share an affine span) of rigid polytopes only has Minkowski flexes? Same first-order. More generally Is the first-order flex space of a Minkowski sum just the sum of the first-order flex spaces of the individual polytopes?
\end{question}

\subsection{Minkowski sums}

% We previously explained how \emph{generic} Minkowski sums become flexible polytopes.
% We can be more precise here.

% \begin{theorem}
%     Given polytopes $P,Q$, let
%     Let $\mathcal U$ be the set of linear subspaces of 
% \end{theorem}

Let $\mathfrak F(P)$ be the first-order flex space of $P$.

\begin{theorem}
    For a generic Minkowski sum of dimension $d\ge 3$ holds $\mathfrak F(P+Q) = \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$.
\end{theorem}
%
\begin{proof}
    \mwsays{This theorem is wishful thinking. It could be that a Minkowski sum has more (first-order) flexes than the ones that come from the summands. I think we know enough to show that $\mathfrak F(P+Q) \subseteq \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$. Maybe the other direction can be proven using some limit argument.}
\end{proof}

\mwsays{Not true in $d=2$ or for non-generic Minkowski sums, consider two triangles that add up to a hexagon, or prisms over those.}

\subsection{Truncation}

If two frameworks on the same graph have the same edge directions, then they have the same first-order theory since the rows in the rigidity matrix are just multiples of each other.
The following would be a generalization to polytopes:

\begin{theorem}
    If $P$ and $Q$ are normally equivalent, then $\mathfrak F(P)\simeq \mathfrak F(Q)$.
\end{theorem}
%
\begin{proof}
    \TODO
    \mwsays{True?} \mwsays{WRONG! TIco and TDod}
\end{proof}

\mhsays{We lose all flexes when changing the truncation of the truncated dodecahedron. Therefore, the flexes are not a result of the polytopes' symmetry, but rather of the coordinates. }

\subsection{Truncation}
Questions:
\begin{itemize}
    \item Does there exist a truncation in (0,1) preserving the flexes of either of the truncated ends?
    \item Is rigidity/flexibility preserved under certain assumptions on the truncation? 
\end{itemize}




























\newpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

The realization space $\real({\mathcal{P}})$ of 3-dimensional polytopes is a smooth $(|E|+6)$-dimensional manifold, on which the 6-dimensional Lie group of rigid motions acts smoothly. In fact, the configuration space $\realR(\mathcal{P})$ is homeomorphic to an open $|E|$-ball. Intuitively, this claim \emph{has} to be true, simply by subtracting the appropriate dimensions. However, proving it is \todo{\mwsays{Not only ``slightly more subtle'', but this is a big deal :D}}slightly more subtle than it seems, as we are working with manifolds and associated Lie groups instead of Euclidean space.

To prove the claim, we first note that according to Richter-Gebert \cite[Thm.\ 13.3.3]{richter2006realization} factoring out the $12$-dimensional group of affine transformations $\mathrm{Aff} $ from the realization space $\real({\mathcal{P}})$ produces a $(|E|-6)$-dimensional open ball. Now, $\realR(\mathcal{P})\cong \left(\real(\mathcal{P})/\mathrm{Aff}\right) \,\times\, \left(\mathrm{Aff}\,/\,\mathrm{Iso}\right)$ for the Euclidean isometries $\mathrm{Iso}$. Since $(\mathrm{Aff}\,/\,\mathrm{Iso})$ is a $6$-dimensional manifold, 
this implies that the product $\realR(\mathcal{P})$ is a smooth, 
$|E|$-dimensional manifold, since $|E|=(|E|-6)+6$
(cf. \cite[p.\ 7]{lee-smooth-manifolds}).

In other words, even rigid polytopes have $|E|$ degrees of freedom when constraining one of their facets to a hyperplane. \todo{\mwsays{I would not call it a coincidence that $|E|$ is the number of edges}}Coincidentally, this number is identical to the number of edges, suggesting that the degrees of freedom exactly correspond to perturbations of the edge lengths. This line of thought would imply that we can locally freely perturb the edge lengths around rigid realizations (see \Cref{conj:edge_length_perturbations}).  We formalize this intuition in the following definition.
    
\begin{definition}
\label{def:edge-length-perturbations}
 Denote the \todo{\mwsays{maybe ``edge length vector'', since then perturbations are a more natural thing?}}\Def{edge length list} of $P$ by 
 \[\mathcal L(P):=(\ell(e):e\in E(P)).\]
We say that a list $(\ell_e\in\RR : e\in E(P))$ is \Def{realized} by $P$ if $\ell(e)=\ell_e$ for all $e\in E(P)$. The \Def{edge length realization space of $P$} contains all possible lists of edge lengths corresponding to convex realizations of the combinatorial type of $P$.

Moreover, $P$ \Def{has all edge length perturbations} if every sufficiently small perturbation of its edge length list $\mathcal L(P)$ can be realized by a polytope $Q$ of the same combinatorial type that lies sufficiently close to $P$. More precisely, $P$ has all edge length perturbations if for some $C>0$ and every $C\geq\varepsilon>0$ there exists a $\delta>0$ such that every list of edge lengths $\mathcal{L}(Q)$ with 
\[\text{dist}(\mathcal{L}(P),\,\mathcal{L}(Q))<\delta\] 
can be realized by a polytope $Q$ of the same combinatorial type as $P$ that satisfies
\[\text{dist}(P,\,Q)<\varepsilon\] 
in the Euclidean metric. 

If that is not the case, \ie\ if there are edge length perturbations arbitrarily close to $\mathcal{L}(P)$ that can not be realized as a polytope close to $P$, we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

While this definition may seem rather technical, these concepts are helpful in formulating a relationship between a polytope's rigidity and topological properties of its edge length realization space. Using this language, we can show that first-order rigid polytopes concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    An first-order rigid realization of a convex polytope \todo{\mwsays{Of a combinatorial type $\mathcal P$}}$P$ has all edge length perturbations.
    \begin{proof}
        Fix the combinatorial type $\mathcal{P}$ of $P$. The configuration space of a convex polytope $\realR(\mathcal{P})$ is a smooth $|E|$-dimensional manifold, where $|E|$ denotes the number of edges of $P$. Assuming the realization of $P$ is \todo{\mwsays{First-order rigid}}infinitesimally rigid, there exists an open neighborhood where the rigidity matrix $R(P)$ has the minimal corank $6$, implying that all sufficiently close realizations of $P$ are also infinitesimally rigid when fixing edge lengths and the planarity of facets. This stems from the fact that a polynomial system's Jacobian matrix drops rank in a proper algebraic subset of lower dimension, implying that around every regular point of an algebraic variety there is an open neighborhood of regular points \cite[Thm.\ 5.3]{hartshorne}.
        
        This leaves $|E|$ dimensions when also allowing the edges to change their lengths. Since the realization space factored out by the rigid motions is locally diffeomorphic to an open ball in $\mathbb{R}^{|E|}$ and since the tangent space does not contain any vectors corresponding to continuous motions that preserve the edge lengths, this means that sufficiently small edge length perturbations are realizable.
    \end{proof}
\end{proposition}


\begin{corollary}
    A generic realization of a convex polytope $P$ has all edge length perturbations.
    \begin{proof}
        In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polytope is infinitesimally rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}

\todo{\mwsays{I think this example is very educational and should, together with a positive example, come in the beginning of this section}}Not all realizations of convex polytopes have all edge length perturbation. For instance, consider the regular cube, whose realization is given by the coordinates $\{1,-1\}^3$. It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two opposing edges. In this case, this property arises because the cube is flexible.
We can turn this simple observation into a general statement about flexible polytopes. 

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If a convex polytope $P$ is flexible, then some of its edge length perturbations are not realizable.
    \begin{proof}
        Denote the combinatorial type of $P$ by $\mathcal{P}$. Analogous to the proof of \Cref{prop:inf-rigidity-edge-perturbations}, the configuration space $\realR(\mathcal{P})$ of $\mathcal{P}$ is homeomorphic to a smooth $|E|$-dimensional manifold. \iffalse
        the Legendre-Steinitz theorem \cite{rastanawi2021dimensions} tells us that the realization space $\real(\mathcal{P})$ of convex polytopes in $\mathbb{R}^3$ is a smooth $(|E|+6)$-dimensional manifold. We factor the rigid motions out of $\real(\mathcal{P})$ by pinning the position of a first vertex ${\bs p}_1$, constraining a second vertex to lie on the line ${\bs p}_1+t\cdot (1,0,0)$ for $t\in \mathbb{R}$ and fixing the third vertex to the affine plane generated by the expression ${\bs p}_1+t\cdot (1,0,0)+s\cdot (0,1,0)$ for $s,t\in \mathbb{R}$. We denote the resulting configuration space by $\mathcal{C}_\mathcal{P}=\real (\mathcal{P})/\sim$. It is a smooth manifold of dimension $|E|$, since the Lie group of rigid motions acts freely (the vertices are labeled), smoothly (it is a Lie group) and properly (preimages of compact sets are compact under the group action) on the manifold $\real(\mathcal{P})$ \cite[Thm.\ 21.10]{lee-smooth-manifolds}. \mwsays{Find citation for $\real(P)/\sim \cong \RR^E$}
        \fi
        
        \iffalse
        Therefore, the nontrivial continuous flexes $\mathcal{F}$ and the continuous edge length perturbations $\mathcal{E}$ both necessarily live in $\mathbb{R}^{|E|}$. In particular, they can be written as the following semi-algebraic sets:
        \begin{eqnarray*}
            \mathcal{F} &=& \mathcal{C}_\mathcal{P}~\cap~\big\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u-{\bs p}_v|| = \mathcal{L}(P)_{(u,v)}\, \forall (u,v)\in E\big\}\quad\text{and}\\
            \mathcal{E}&=& \{P\}\,\cup\, \left(\mathcal{C}_\mathcal{P}\,\setminus \,\mathcal{F}\right).
        \end{eqnarray*}
        Since $P$ is flexible, we know that the dimension of $\mathcal{F}$'s tangent space at $P$ is at least $1$. Since $P$ is convex, all its edge lengths are positive.
    \fi

	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{|E|}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{\mathcal{L}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small$\mathcal{L}(P)$};
			\node (CP) [right=of R1] {$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{|E|}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] (UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} (R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        Assume now that all of $P$'s edge length perturbations are realizable. Then, in particular, we can locally extend and contract each of $P$'s edges individually. In fact, we can arbitrarily combine these edge length perturbations. Since we factored out rigid motions before, each combination of edges that we perturb gives rise to a \emph{distinct} continuous deformation of $P$. This implies that there is an open ${|E|}$-dimensional ball of realizable edge length perturbations containing $\mathcal{L}(P)$. The following topological arguments are summarized in \Cref{fig:proofhelper-invariance-of-domain}.
        
        By a previous argument, the map $\psi:\mathbb{R}^{|E|}\rightarrow \realR(\mathcal{P})$ taking a list of edge lengths and producing a realization of $\mathcal{P}$ is well-defined, injective and continuous in a sufficiently small open neighborhood $U_{\mathcal{L}(P)}\subset\mathbb{R}^{|E|}$ of $\mathcal{L}(P)$. Since the manifold $\realR(\mathcal{P})$ is $|E|$-dimensional, it is locally diffeomorphic to $\mathbb{R}^{|E|}$ via $\varphi:\realR(\mathcal{P})\rightarrow \mathbb{R}^{|E|}$. Now, take any open neighborhood $V$ of $\varphi(P)$ in $\mathbb{R}^{|E|}.$ By the Invariance of Domain Theorem \cite{invariance-of-domain}, the locally continuous injection $\varphi\circ \psi: U_{\mathcal{L}(P)}\rightarrow V\subset \mathbb{R}^{|E|}$ for \mbox{$V=\varphi\circ \psi (U_{\mathcal{L}(P)})$} is a homeomorphism on its domain and $V$ is open, so we can pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\mathcal{C}_\mathcal{P}$. As a consequence, $\psi:U_{\mathcal{L}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, as well. 
        This implies that there is an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no continuous motion that preserves the edge lengths in $\mathcal{L}(P)$, so $P$ is rigid. 
        \iffalse
        \mhsays{To show:
        Conversely, if $P$ is rigid, then $P$ is a real-isolated solution of the polynomial system of edge length, facet planarity and pinning equations that factor out the rigid motions (see previous implication). Recall that the configuration space $\mathcal{C}_\mathcal{P}$ is a smooth manifold of dimension $|E|$. Therefore, intersecting $\mathcal{C}_P$ with the real algebraic set generated by the edge length equations
        \[\mathcal{E}_P~=~\left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||=\mathcal{L}_{(u,v)}~\forall uv\in E\right\}\]
        contains the isolated point $P$. Consequently, intersecting $\mathcal{C}_\mathcal{P}$ with the complement
        \[\mathcal{N}_P ~=~ \left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||\neq \mathcal{L}_{(u,v)}~\text{ for some } uv\in E\right\},\]
        which exactly characterizes the edge length perturbations of $P$, is equal to $\mathcal{C}_{\mathcal{P}}\setminus \{P\}$.
        We now show that for every sufficiently small perturbation of $\mathcal{L}(P)$, there is a convex polytope close to $P$. In other words, we need to show that $U(\mathcal{L}(P))$ is open in $\mathbb{R}^{|E|}$ and not only in the realization space of edge length perturbations. \textcolor{red}{Also, we need to show well-definedness of $\psi$.}
        %Since $\mathcal{C}_\mathcal{P}$ is a smooth, $|E|$-dimensional manifold, it is locally diffeomorphic to $\mathbb{R}^{|E|}$ via $\varphi:\mathcal{C}_\mathcal{P}\rightarrow \mathbb{R}^{|E|}$. This property implies that there exists an open neighborhood $V\subset\mathbb{R}^{|E|}$ such that $\varphi:\varphi^{-1}(V)\rightarrow V$ is a diffeomorphism. Note that we can choose $V$ so that $\mathcal{L}(P)$ is contained in $\varphi^{-1}(V)$ since $\mathcal{C}_\mathcal{P}$ is a smooth manifold. By possibly shrinking the open sets, we obtain a continuous map $\varphi \circ \psi:U_\mathcal{L}(P)\rightarrow V$. 
        The rigidity of $P$ implies that
        \[\mathcal{C}_\mathcal{P} ~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right)\,\cup\, \left(\mathcal{C}_\mathcal{P}\cap \mathcal{E}_P/\sim\right)~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right) \cup \{P\}.\]
        Since $\psi$ is injective and continuous by construction, the preimage of any open set around $P$ under $\psi$ is open again. Since all realizations come from edge length perturbations, $\psi$ is surjective; therefore, $\psi$ is a homeomorphism.}
        \fi
    \end{proof}
\end{theorem}

The contraposition of this theorem provides a sufficient condition for the rigidity of polytopes, which makes it worth to point it out as a corollary. Albeit, it is still unclear whether checking that all edge length perturbations are realizable offers any advantage over verifying a polytope's rigidity.

\begin{corollary}
    If all edge length perturbations of a convex polytope are realizable, then it is rigid.
\end{corollary}

\begin{remark}
    \todo{\mwsays{As written, it sounds as if we have an example of this, which we don't}}The converse of \Cref{thm:rigidity-and-edge-length-perturbations} is not necessarily true: The space of edge length perturbations may be full-dimensional, even though the realization $P$ is rigid and only edge length perturbations forming a proper algebraic subset are not realizable. This constitutes the main difficulty in proving meaningful results in this scenario.
\end{remark}

The correspondence between the edge length realization space of a polytope and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polytope is continuously rigid. In our experiments (cf. \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

\begin{question}
\label{conj:edge_length_perturbations}
\todo{\mwsays{Let's not phrase it as a conjecture/statement}}Every rigid realization of a convex polytope has all edge length perturbations.
\end{question}

\begin{question}
If a convex polytope is higher-order rigid (cf.\ \cite{higher-order-rigidity}), then $\mathcal{L}(P)$ is singular in the edge length realization space (cf. \cref{fig:edge-contraction-deformation-space}).
\end{question}

While we do not understand the edge length realization space of polytopes nearly enough to provide answers to these questions, they provide interesting observations that 
















\newpage
\section{Second-order rigidity check}
\label{section:second-order-rigidity-check}

As laid out in \Cref{sec:second-order-theory}, any nontrivial infinitesimal flex of a polytope \mbox{$P\in \real(\mathcal{P})$} of combinatorial type $\mathcal{P}$ that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. This provides a convenient heuristic for finding nonblocked flexes: Essentially, we need to find a nontrivial flex $\dot{P}$ such that $(\omega,\eta)\cdot R(\bsdot P)\cdot \bsdot q=0$ for all equilibrium stresses $\bs \xi$ (cf. \Cref{lem2}). This is accomplished by parametrizing the flex space via a basis ${\bsdot q}=({\bsdot q}_1,\dots,{\bsdot q}_r)$ and variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ and variables $\mu=(\mu_1, \dots, \mu_s)$. This turns the second-order condition from \Cref{lem2} into a cubic polynomial of the form 

\[E_{{\bsdot q},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot R\left(\sum_{i=1}^r \lambda_i{\bsdot q}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\bsdot q}_i\right).\]

More precisely, $E_{\bsdot q,\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. By \cref{lem2}, to assert second-order rigidity, it suffices to show that every nontrivial infinitesimal motion has a blocking stress. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\bsdot q},\,\bs \xi}(\lambda,\mu)\neq 0$.

By expanding $E_{\dot{P},\,\Xi}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
$$E_{{\bsdot q},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$$ 
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is nonzero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i{\bsdot q}_i$. Therefore, the infinitesimal motions corresponding to a $\lambda$ that are not blocked by any stresses must live in the algebraic set given by the intersection of the zeros of $Q_1,\dots, Q_s$. 

Since the polynomials $Q_1,\dots, Q_s$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$. The following lemma lets us certify the zero-dimensionality of an algebraic variety and it proves useful to us in practice. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[x_1,..,x_m]$, and a set of Gröbner bases $G$. $I$ is zero dimensional if and only if some power of $x_i$ is the leading monomial of an element of $G$ for every $i\in\{1,...,m\}$.
    \end{lemma}

There are also other methods based on Gröbner bases to verify than an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic variety $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Prop.\ 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homgeneous, $\mathcal{V}(\mathcal{I})\subset \mathbb{P}_\mathbb{C}^{r-1}$, so for any solution $\lambda^\star$ of the polynomial system $Q_1(\lambda)=0,\,\dots,\,Q_s(\lambda)=0$, all scalar multiples $c\lambda$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\{0\}$. In our context, this translated to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system $\nabla_\mu E_{\bsdot q, \bs \xi} (\lambda) = 0$ only has $\lambda = 0$ as a solution, then all infinitesimal flexes are blocked by equilibrium stresses. Any flex that is not blocked by an equilibrium stress corresponds to a nontrivial, real zero of $\nabla_\mu E_{\bsdot q, \bs \xi} (\lambda)$.
\end{proposition}


\section{Approximating Continuous Motions}
\label{sec:approx_continuous_motions}


Determining the flexibility of a bar-and-joint framework is NP-hard \cite{abbott2008NPhard}, so there is little hope that our more complicated setting will be any easier. Instead, we shift our attention to numerically approximating deformation paths of this geometric constraint system.

In this article, we use a technique that relies on following solution paths along a given initial direction that continually satisfy the constraints.
Assume we are given a nontrivial infinitesimal motion $(\bsdot p, \bsdot a)$ that extends to a continuous motion. In other words, $(\bs p,\bs a)+(\bsdot p, \bsdot a)$ lies in the linearization of the underlying constraint set. In Heaton and Himmelmann \cite{heaton2025euclideandistanceretraction}, a method for approximating the corresponding deformation path based on Riemannian optimization is implemented as a combination of the metric projection to the closest point and homotopy continuation. It is called the \Def{Euclidean distance retraction} as it projects $(\bs p,\bs a)+(\bsdot p, \bsdot a)$ to its closest point on the constraint set.

The closest point problem can be described by a constrained polynomial optimization problem, so we can reformulate it as a (polynomial) Lagrange multiplier system whose zeros characterize the optimization problem's critical points (cf. \cite{Nocedal2006}). Since we already know a solution to this polynomial system in $u=(\bs p, \bs a)$ -- namely, the point $(\bs p, \bs a)$ itself -- we can apply homotopy continuation methods consisting of a predictor step (e.g.\ Euler's method) and a corrector step (e.g.\ Newton's method). Such schemes are often applied for solving polynomial systems \cite{sommese2005numericalsolutionpolynomial}. 

In general, a direct application of the Newton corrector method may diverge or converge to the wrong point. Nevertheless, for the problem of computing the Euclidean distance retraction, the convergence of the predictor-corrector scheme to the closest point to $(\bs p,\bs a)+(\bsdot p, \bsdot a)$ can be shown, as long as the linear step $(\bs p, \bs a)+(\bsdot p, \bsdot a)$ stays sufficiently close to the underlying constraint set \cite{heaton2025euclideandistanceretraction}.

Nevertheless, three questions remain:
\begin{myenumerate}
    \item how to ensure that an initial flex extends to a continuous motion,
    \item how to compute the subsequent flex in the case where the linear space of nontrivial infinitesimal flexes has a dimension greater than 1 and
    \item how to traverse singularities?
\end{myenumerate}

If we assume that there exists an infinitesimal flex that extends to a continuous motion (e.g.\ by assuming that the polytope $P$ is flexible), this flex necessarily needs to be a non-blocked flex. For this reason, assume we know a basis of nontrivial infinitesimal flexes $\bsdot q =({\bsdot q}_1, \dots, {\bsdot q}_r)$ and a basis of equilibrium stresses $\bs \xi = (\bs\xi _1,\dots, \bs\xi_s)$. Following \Cref{section:second-order-rigidity-check}, we solve the homogeneous polynomial system $\nabla_\mu E_{\bsdot q,\,\bs \xi}(\lambda) = 0$
over $\mathbb{R}\mathbb{P}^{r-1}$ for $\lambda_1^*,\dots,\lambda_r^*$ we can obtain a nontrivial flex $\dot{P}=\sum_{i=1}^r \lambda_i^*{\bsdot q}_i$ that is not blocked by any equilibrium stress (cf \Cref{prop:stress-energy-condition}). We take it as our initial flex, as it heuristically has a good chance of providing a flex that extends to a continuous motion, since we have no examples of second-order flexible polytopes that are rigid. 


For the second question, we return to Riemannian geometry: On a smooth manifold, the \Def{parallel transport} \cite[§10.3]{boumal2020intromanifolds} is a means to compare vectors that live in distinct tangent spaces. This inspires our approach: Given the previous flex $\dot{P}_\text{old}$ corresponding to the realization ${P}_\text{old}$ for which ${P}_\text{old}+\dot{P}_\text{old}$ has been projected to obtain the current realization $P$, we first compute a basis of the space of nontrivial infinitesimal flexes that we collect as the rows of a matrix $A$. To find the closest analogue to the flex $\dot{P}_\text{old}$ in the new realization $P$, we compute a solution to the minimization problem 
\[\min_{x\in \mathbb{R}^{d(|V|+|F|)}}||Ax-\dot{P}_\text{old}||^2,\]
which can, for instance, be solved by computing the Moore-Penrose pseudoinverse of $A$, which provides a minimum norm least squares solution \cite[Prop.\
7.2.1]{allaire2008numericallinearalgebra}. This approach guarantees that we pick the closest subsequent nontrivial infinitesimal flex and that our deformation path will be as smooth as possible.

Finally, algebraic constraint sets are distinct from smooth manifolds by having the potential to contain singularities. In our setting, such points can be characterized by the rigidity matrix dropping rank. They notoriously pose issues for smooth approximation approaches. Nevertheless, homotopy continuation schemes come with techniques such as the \Def{singular endgame} to approach singular solutions (cf. \cite[§10]{sommese2005numericalsolutionpolynomial}). Conversely, escaping singularities poses issues even for such schemes, although this ability is essential for our purposes. To tackle this problem, we take inspiration from Holmes-Cerfon, Theran and Gortler \cite{Holmes-Cerfon2021AlmostRigidity}, in which they describe an acceleration-based method to escape singularities by keeping track of a local, orthogonal frame along the deformation path. This information allows us to reliably traverse nodal-like singularities and to change direction in cusp-like singularities. 

All of these individual techniques for approximating deformation paths has been implemented in the Julia package \texttt{DeformationPaths.jl}\footnote{\url{https://github.com/matthiashimmelmann/DeformationPaths.jl}}, where all Archimedean and Catalan solids that are discussed in this article are provided as test sets. The corresponding animations of the flexible polytopes are provided as supplementary material to this article.


\section{Case study: The regular dodecahedron}
\label{sec:dodecahedron}

In this section we show what tools are available to move beyond statements about generic rigidity.
Among the classically best known polyhedra, the Platonic~solids, only for one of them the question of rigidity is not immediately clear. The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid; the cube is a zonotope, hence flexible. 
It remains to check the regular dodecahedron.

Solving the system of first order conditions, we find that there exists a 5-dimensional space of non-trivial infinitesimal flexes.

\iffalse
    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi


\subsection{Rigidity of the Regular Dodecahedron} 
\label{section:rigidity-of-the-regdod}

By symbolically computing the space of nontrivial infinitesimal flexes and stresses associated with the regular dodecahedron, we find that their dimension is $5$. The specific embedding, computations, ordering of vertices, edges, and facets are all provided as \texttt{Mathematica} code in the Supplementary Material. Consequently, the regular dodecahedron is not first-order rigid.

We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. \Cref{prop:stress-energy-condition} asserts that computing the zeros of a certain polynomial system lets us certify this property. For that reason, we employ the following strategy:

\begin{myenumerate}
    \item Compute a basis of the space of nontrivial infinitesimal flexes $(\bsdot q_1,\dots,q_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. We parametrize these basis via variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$, respectively.
    \item From the stress energy $E_{\bsdot q,\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\bsdot q,\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadrics $Q_i$ (see \cref{section:second-order-rigidity-check}).
    \item Employ \Cref{gbasis} to show that this system has finitely many zeros.
    \item According to \Cref{prop:stress-energy-condition}, this implies that the regular dodecahedron is second-order rigid.
\end{myenumerate}

\iffalse

    Expand $\omega R(\dot P)\dot P$ in terms of $y_i$, we have $$\omega R(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the infinitesimal motions corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $G$. $I$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $G$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the supplementary material. 
    \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
    The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\bsdot{q}_1,\dots, \bsdot{q}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        By \cref{gbasis}, the set of polynomials $\{Q_1,\,\dots,\, Q_5\}$ only has finitely many common zeros. Since the system is homogeneous, the only solution is $y_1=y_2=...=y_5=0$. As a result, for any nonzero $\dot P$ generated by the five nontrivial infinitesimal motions, we can find a stress so that inequality \eqref{block} holds. By \cref{lem2}, $P$ is second-order rigid. By \cref{thm3}, $P$ is rigid. 
    \end{proof}

\begin{remark}
    Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (cf. \cref{tab:comparison}).
\end{remark}


\subsection{Edge Length Perturbations of the Regular Dodecahedron}
\label{section:dodec-edge-length-perturbations}
Although \Cref{dodecahedronrig} shows that when fixing its edge lengths, the dodecahedron with combinatorial type $\mathcal{P}$ is rigid, its realization space $\real(\mathcal{P})$ is a smooth $36$-dimensional manifold according to the Legendre-Steinitz Theorem (cf. \cite{rastanawi2021dimensions}). According to \Cref{section:edge-length-perturbations} we can even say more: Its configuration space $\realR(\mathcal{P})$ is a smooth $30$-dimensional manifold. In \Cref{conj:edge_length_perturbations} we formulate the hope that for rigid polytopes, all edge length perturbations are realizable (cf. \Cref{def:edge-length-perturbations}). It is completely unclear, whether this claim is true.

To gain a better understanding of what the claim means, we are going to investigate in this section how deformations of the regular dodecahedron induced by altering a single edge length behave. By the polytope's regularity, all edges are combinatorially identical. It does not matter which edge is chosen. For this example, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^\star(t) = 1-t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$. Sampling from the realization space intersected with the real algebraic set generated by the edge length equations reveals that there are 6 distinct curves through the regular dodecahedron corresponding to the contraction of a single edge length and 2 corresponding to its expansion. The 6 configurations at $\ell^{\star}(-0.25)$ are depicted in \Cref{fig:dodecahedron-configurations-contraction}.

     \begin{figure}[h!]
        \centering
        \includegraphics[width=0.25\linewidth]{Images/dodeca3.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca1.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca2.png}\\[2mm]

        \hspace*{8mm}
        \includegraphics[width=0.16\linewidth]{Images/dodeca5.png}
        \hfill
        \includegraphics[width=0.18\linewidth]{Images/dodeca4.png}
        \hfill
        \includegraphics[width=0.17\linewidth]{Images/dodeca6.png}\hspace*{8mm}
        \addtocounter{equation}{1}
        \caption{The 6 configurations obtained by contracting the blue edge. They can be split into two types that are organized in the top and bottom row. In the central column, the configurations have 2 reflection axes, while the left and right columns are mutual mirror images with only 1 reflection axis. }
        \label{fig:dodecahedron-configurations-contraction}
    \end{figure}

        It turns out that there are two types of configurations: Those mitigating the edge contraction by contracting vertically and those that contract horizontally. Both types contain one configuration with two mirror axes and two configurations with one reflection symmetry that are mutual enantiomers. Intriguingly, not all dodecahedra persist until the edge collapses. The configurations in the top left and top right are confluent with the configuration in the top center at $\approx\ell^{\star}(-0.37194)$, leaving only 4 configurations beyond this point. All of them persist until $\ell^\star(-1)=0$. 

        \begin{figure}[h!]
        \vspace*{2mm}
            \centering
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT1.png}
            \hfill
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT2.png}
                \addtocounter{equation}{1}
            \caption{The 2 configurations are obtained by expanding the blue edge. They both admit to 2 distinct reflection axes.}
            \label{fig:dodecahedron-configurations-expansion}
        \end{figure}

        Conversely, expanding an edge only produces two configurations that both have 2 distinct reflection axes. They are depicted for the edge length $\ell^\star(0.25)$ in \Cref{fig:dodecahedron-configurations-expansion}. Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigations.

        What remains is a qualitative analysis of the eight deformation paths that emerge from contracting any of the dodecahedron's edges. By considering projections of the eight deformation paths onto random 2-dimensional subspaces and approximating the curves' derivatives, an understanding of the curves' tangents in the regular dodecahedron can be obtained. \Cref{fig:edge-contraction-deformation-space} visualizes the curves' behavior. 

            \begin{figure}[h!]
            \centering
            %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation.jpg}
            %\hspace*{8mm}
            \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom.jpg}
            %\\[4mm]
             %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation2.jpg}
            \hspace*{8mm}
            \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom2.jpg}
            \addtocounter{equation}{1}
            \caption{Both figures depict distinct random projections of the 8 deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths (cf. \Cref{fig:dodecahedron-configurations-contraction}) have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}

         


        Remarkably, it appears that the curves can be smoothly matched. As the grey curves correspond to an edge expansion, they seem to have the same tangent in the regular dodecahedron. The two asymmetric green and red deformation paths can be matched as well. Two symmetric deformations remain, which also share the same tangent in the regular dodecahedron. In total, 4 smooth curves are passing through the regular dodecahedron that are parametrized by edge perturbations. Numerically computing the derivative in the regular dodecahedron confirms this observation: Though naturally, we expect that our numerical calculations are not exact, the respective tangents' sum is sufficiently close to 0. Finally, we attached an animation of a smooth deformation path passing through the singularity (see \Cref{fig:edge-contraction-deformation-space}) induced by an edge expansion from $\ell^\star(-0.25)$ to $\ell^\star(0)$ followed by a compatible contraction from $\ell^\star(0)$ to $\ell^\star(-0.25)$ in the supplementary material of this article. 


\begin{remark}
    Since we find multiple configurations corresponding to both, edge-length contractions and expansions, we conclude that the dodecahedron is not generically globally rigid (cf. \cite{Connelly2005}). 
\end{remark}








\newpage % temporary new page

\section{Case study: The truncated dodecahedron}
\label{sec:truncated_dodecahedron}
\label{sec:TDod}






\newpage % temporary new page

\section{Outlook}
\label{sec:outlook}

\mwsays{Questions here ...}



==> sec/introduction_-_copy_-_2026-05-28.tex <==
Add MSC for the polynomial/computational aspects of the paper ✓MH: Howeer, I only
found computational aspects. I added a few algebraic geometry MSC codes that we might
add later.
Find good title: global rigidity must go; something with realization spaces ✓
Use R for rigidity matrix ✓
Replace infinitesimal by first-order ✓
Use commands for e.g. and i.e. and cf. ✓
Numbers up to twelve as words (when used for counting)
Use abbreviations for references inside of citations? Figure⇒ Fig. MW: We should do this
only if the source does it MH: I am not sure I understand correctly? I think we should rather
be consistent and choose one of the two options throughout.
Mention somewhere that all symbolic results were double-checked numerically?
Make sure all realc and conf are gone.
Check all occurences of mreal ✓
Once everything is done:
Remove all \todo
1
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF
POLYTOPES WITH EDGE LENGTH AND COPLANARITY
CONSTRAINTS
MATTHIAS ADRIAN-HIMMELMANN, MARTIN WINTER, AND ZHEN ZHANG
Abstract. We develop a second-order rigidity theory for polytopes, for which
both edge lengths and the planarity of faces are required to be preserved.
Alongside the theory, we implement an effective algorithm for checking second-
order rigidity. Using these tools, we are able to characterize the rigidity prop-
erties of the Platonic, Archimedean and Catalan solids. Only the truncated
dodecahedron, which is not second-order rigid but likely also not flexible, does
not fit into this theory.
Alongside this characterization, we also provide a lower bound on the di-
mension of the space of flexes for certain polytopes and provide an algorithm
for approximating such deformations.
We also study the geometry of the polytopal realization space by investi-
gating the complement of the metric realization space, where the edge lengths
are fixed. We call this complement the edge length perturbation space. This
reveals an intricate relationship between the rigidity of polytopes and the local
topology of the edge length perturbation space.
1. Introduction
In [4] the authors initiated the study of convex polytopes as point-hyperplane
frameworks and asked under what conditions a polytope admits a continuous defor-
mation that preserves both its edge lengths and face coplanarities. These assump-
tions are weak in comparison to classical polyhedral rigidity, which also enforces
fixed face shapes. Still, only few techniques are known to construct polytopes that
admit such deformations MH: and which polytopes do not admit continuous deformations?
(to highlight rigidity and not just flexibility.). As a consequence, the general sentiment is
that flexibility in polytopes (i.e., the existence of such deformations) is an excep-
tional property, not only among combinatorial types, but also among realizations
of a fixed type. In [4, Conjecture 1.1] the authors conjecture that for polytopes in
dimension at least 3, a generic convex realization of a combinatorial type admits
no deformations, i.e., is rigid. This claim was shown to hold in dimension three
[4, Theorem 1.2].MH: I do not think
anymore that the
first page is a good
place for a flex, for
which we have strong
evidence against be-
ing a true polyhedral
flex. This may gen-
erate false expecta-
tions. I would pre-
fer putting it in the
conclusion/outlook
as future work and
focusing on the ex-
amples that we can
actually solve.
Like in the classical setting of frameworks, deciding rigidity for a given polytope
is computationally hard. Once a polytope is not first-order rigid, and even if it has
few vertices and faces, the question about rigidity is often out of reach for direct
techniques. For example, in [4, Section 6.2] the authors singled out the regular
Date: May 28, 2026.
2010 Mathematics Subject Classification. 51M20, 52C25, 52B11, 14Q30, 65H14.
Key words and phrases. convex polytopes, rigidity and flexibility, point hyperplane frame-
works, second-order rigidity, realization spaces.
2
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 3
Figure 1. The Archimedean truncated dodecahedron (left) and two of
its potential flexes (middle and right) constructed numerically. MH:
Suggestion: Move to Conclusion and replace image by truncated dodecahe-
dron, dodecahedron and truncated icosahedron, since they are special.
dodecahedron (20 vertices, 30 edges and 12 faces) as a primary example of a small
polytope with unclear rigidity status.
In this article we develop tools for the analysis of realization spaces and rigidity
properties of polytopes. This includes the formulation of a suitable second-order
theory, as well as computational tools for tracing deformation paths. For a demon-
stration we apply these techniques to the Platonic, Archimedean and Catalan solids,
deciding their rigidity in all but one case (see Table 1). In particular, we decide
the rigidity of the previously open regular dodecahedron. Solely the rigidity of the
truncated dodecahedron (Figure 1, left) cannot be decided by our techniques. It ap-
pears to require techniques of even higher order and can thus serve as a remarkably
simple test case for future theoretical and computational developments. We found
it quite surprising that such variety of rigidity behaviors can already be observed
among such classical examples.
This article divides into theoretical, methodological and experimental results, of
which we give an overview below. MH: I decided to
add a roadmap to
explain the article
structure (since we
have many pages and
sections whose rela-
tions are somewhat
difficult to under-
stand).MW: I like
the graphics, but
I wonder wether it
might be confusing.
For example, why is
the introduction at
the end?MH: We
can also leave the in-
troduction out or re-
place it by Table 1/2.
The structure of our
paper may be slightly
confusing and this is
an attempt at making
the structure clearer.
I am very open to
suggestions here on
how to organize the
roadmap.
Introduction
Appendix
Section 10
Section 2
Chapter 3
Chapter 4
Chapter 5
Chapter 6
Chapter 8
Chapter 7
Chapter 9
Theory (cf. Section 1.1) Methods (cf. Section 1.2) Results (cf. Section 1.3)
Introduction
Section 10
Appendix A and BSection 2
Section 3
Section 4
Section 5
Section 6
Section 8
Section 7
Section 9
Figure 2. Roadmap for the article.
1.1. Theoretical results. The main theoretical contributions are a careful deve-
lopment of the first- and second-order theory of polytope rigidity, as well as the
creation of dual certificates based on which perturbations of a 3-dimensional poly-
tope’s edge lengths can be realized.
4 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
In Section 2 and Section 3 we recall the basic of polytope geometry, combinatorics
and rigidity from [4]. In Section 4 we present the first-order theory. This includes
definitions for the rigidity matrix as well as first-order motions and flexes. We prove
that first-order rigidity implies rigidity.
Subsequently we apply the ideas of first-order theory to edge-length perturba-
tions, motivated from the following train of thought: The classical Legendre-Steinitz
theorem states that the realization space of a 3-dimensional polytope modulo rigid
motions is homeomorphic to RE , where E is the number of edges of P [23]. This
suggests that the shape of a 3-polytope can be controlled by one free and indepen-
dent parameter per edge. In Section 5 we provide an interpretation of these degrees
of freedom for first-order rigid polytopes by perturbing their edge lengths.
In Section 6 we develop the second-order theory for polytope rigidity, includ-
ing notions of second-order motions and flexes. Subsequently we define equilibrium
stresses and generalize the second-order stress test by Connelly and Whiteley [10]
to polytopes. We provide polytope-analogues for the following notions and impli-
cations from framework rigidity:
first-order rigid 6.4
==⇒ prestress stable 6.4
==⇒ second-order rigid 6.1
==⇒ rigid.
1.2. Methodological results. In Section 6.2 we describe a method for certifying
second-order rigidity of polytopes which are based on real algebraic geometry. It
relies on transforming the blocking inequality (6.5) into a polynomial system of
homogeneous equations, which can be symbolically solved using Gröbner bases. If
this system has no non-trivial solutions, then the polytope is second-order rigid.
In Section 8 we describe an algorithm for approximating continuous motions of
flexible polytopes based on Riemannian geometry and homotopy continuation. It
relies on numerically tracking the solution to the optimization problem that searches
for the Euclidean closest point to the realization space. We also use this method to
investigate the realization space of polytopes in Section 9.
1.3. Computational results. Our newly developed first- and second-order rigid-
ity certificates apply to any polytope. For demonstration purposes, we benchmark
them on the Platonic, Archimedean and Catalan solids for which combinatorial data
and exact vertex and normal coordinates are readily available. Doing so already
enables us to answer questions that were previously intractable.
The results for the five Platonic and 13 Archimedean solids are shown in Table 1
below and reveal a wide range of interesting behaviors. The 13 Catalan solids have
less surprising rigidity behavior and can be found in Table 2 in Appendix A. The
structure of the tables cells is explained in Section 1.4. Still, we highlight the most
noteworthy finding from these experiments here:
• The regular dodecahedron and truncated icosahedron have identical rigidity
properties: they are not first-order rigid (both have a 5-dimensional space
of first-order flexes) nor prestress stable; but, both are second order rigid. In
particular, they are rigid. This was previously stated as an open question
for the regular dodecahedron in [4, Section 6.2]. With these properties they
are remarkably natural geometric constraint systems that demonstrate that
prestress stability and second-order rigidity are distinct concepts. Previous
examples of this distinction have been comparatively ad hoc (e.g. [10, Fig.
9b and 17a]).
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 5
• The truncated dodecahedron is not first-order rigid (it has a 4-dimensional
space of first-order flexes), not prestress stable and not second-order rigid.
Since at this time no methods exist to test rigidity beyond the second or-
der, we do not know whether it is in fact rigid. If it is rigid, it would provide
a remarkably natural geometric constraint system that demonstrates that
rigidity does not imply second-order rigidityPrevious examples of this dis-
tinction have been comparatively ad hoc (e.g. [10, Figure 22]). If it is
flexible, its flex would be fundamentally different from all polytope flexes
encountered before (cf. [4, Question 4.2]). Some potential flexes that pre-
serve many symmetries have been computed numerically (see Figure 1). MH: This sentence
again raises hope
that the truncDod
is flexible (and that
we have evidence for
that). I suggest re-
moving it, since the
discussion on what
the flex looks like is
too lengthy. Would
fit the outlook nicely
though.MW: We can
remove it here. But
it would be good to
mention somewhere
in the introduction
what the figure is
about. Any idea
where?MH: I would
like to move the fig-
ure, too.
MW: Maybe also list the cool fact that most of our lower bounds match the actual flex space
dimensions?
Numerical experiments reveal that all these properties are very sensitive to small
MW: Maybe I move
this to dedicated
section. Outlook
maybe?
changes in the polytope’s geometry. First, applying a generic linear transformation
resulted in a first-order rigid polytope. This is in contrast to how all known flexible
polytopes preserve their flexibility under linear transformations (cf. [4, Question
4.3]). Second, changing the height of truncation in the truncated variants resulted
in a first-order rigid polytope. At this time it is unclear why exactly the realizations
with uniform edge lengths show low-order flexibility. In particular, we see that these
properties are not a consequence of the polytope’s symmetry alone.
In Section 9 we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (i.e., maximally symmetric) realization
of the dodecahedron is a singularity in its realization space. By computing defor-
MH: This is impos-
sible according to
Legendre-Steinitz.
Rephrase!
mation paths that shrink or extend a single edge of the regular dodecahedron we
probe the neighborhood of this singularity. We find bifurcating deformation paths
and construct from this a counterexample to generic global rigidity for polytopes.
1.4. Explanation of Table 1. Each table cell contains the name and a visualiza-
tion for the polytope in question. The parentheses contain the following data from
left to right:
(1) Whether the polytope is first-order rigid (✓) or first-order flexible (✗). This
is computed symbolically based on the description in Section 4.
(2) Whether the polytope is prestress stable (✓) or not (✗). If not implied by
other symbolic first- or second-order computations, this is computed numer-
ically based on the description in Section 6 and using our new techniques
developed in Section 7, in this case reducing to a semi-definite program. We
use ✓/✗ to indicate numerical results.
(3) Whether the polytope is second-order rigid (✓) or second-order flexible (✗).
This is computed symbolically based on the description in Section 6 and
using our new techniques developed in Section 7.
(4) Whether the polytope is rigid (✓) or flexible (✗). This is inferred from the
previous symbolic computations or indicated as unknown (?).
(5) The dimension of the space of first-order flexes. This is a notion from the
first-order theory explained in Section 4. Heuristically, it is the expected
number of independent ways in which the polytope can deform. If the
number is 0, the polytope is MH: (first-order)? rigid. If the polytope is a
6 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
▲
Tetrahedron
(✓, ✓, ✓, ✓, 0)
Truncated Tetrahedron
(✓, ✓, ✓, ✓, 0)
✣ ✿
Cube
(✗, ✗, ✗, ✗, 3) ▲
Octahedron
(✓, ✓, ✓, ✓, 0)
✿
Cuboctahedron
(✗, ✗, ✗, ✗, 0+3)
Truncated Cube
(✓, ✓, ✓, ✓, 0)
✣
Truncated Octahedron
(✗, ✗, ✗, ✗, 5) ✿
Rhombicuboctahedron
(✗, ✗, ✗, ✗, 3+3)
✣
Truncated Cuboctahedron
(✗, ✗, ✗, ✗, 5)
Snub Cube
(✓, ✓, ✓, ✓, 0)
▲
Icosahedron
(✓, ✓, ✓, ✓, 0)
Dodecahedron
(✗, ✗, ✓, ✓, 5)
Icosidodecahedron
(✓, ✓, ✓, ✓, 0)
Truncated Dodecahedron
(✗, ✗, ✗, ?, 4)
Truncated Icosahedron
(✗, ✗, ✓, ✓, 5) ✿
Rhombicosidodecahedron
(✗, ✗, ✗, ✗, 5+3)
✣
Truncated Icosidodecahedron
(✗, ✗, ✗, ✗, 5)
Snub Dodecahedron
(✓, ✓, ✓, ✓, 0)
Table 1. The rigidity properties of the five Platonic solid and the 13
Archimedean solids sorted by the polytopes’ symmetry. The 5-tuple be-
low a polytope’s name represents the following properties: (first-order
rigidity, prestress stability, second-order rigidity, rigidity, number of
first-order flexes).
generic Minkowski sum, the table shows the dimension as a sum explained
in Section 10 (see also ✿ below).MH: Maybe only re-
fer to ▲ and ✿ here?
i.e., “see ▲ and ✿ for
an explanation of the
number”? Otherwise
we write it twice.
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 7
In some cases we have a good understanding for how the dimension of the flex space
comes about. In other cases we can provide at least lower bounds on the dimension,
which, remarkably, are always matched exactly in the examples tested here. These
explanations are indicated by the following symbols in the table cells:
▲ This is a simplicial polytope (i.e., all faces are triangles). Hence the polytope
is first-order rigid by Dehn’s rigidity theorem, as well as globally rigid by
Cauchy’s rigidity theorem (for details on the classical rigidity theorems see
[4, Remark 1.3] or [22, Chapter 26+]).
✿ This polytope is a generic Minkowski sum, and hence flexible according
to [4, Section 4.1]. The dimension of the first-order flex space decomposes
according to the two types of flexes that exist for such polytopes – sum-
mand flexes and reorientation flexes (see Section 10.1 for details).
✣ This is a zonotope, and therefore flexible according to [4, Section 4.2]. See
Section 10.2 for an explanation of the observed flex space dimensions. If the
zonotope is generic (marked by ✣ ✿), the exact dimension for the first-order
flex space can be computed (cf. Theorem 10.2).
8 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
2. Polytopes, combinatorial types and realizations
Throughout this article let P ⊂ Rd denote a d-dimensional convex polytope with
non-empty interior and vertices p1, ..., pn, i.e., P is the convex hull conv{p1, ..., pn}.
We often focus on polytopes in dimension three, which we call polyhedra. Below we
recall the relevant facts about polytopes; for a general introduction we refer to [26].
The combinatorics of a polytope can be described using its vertex-facet incidence
structure: a combinatorial type P = (V, F, ∼) is a triple consisting of an (abstract)
vertex set V , an (abstract) facet set F and a vertex-facet incidence relation ∼ ⊆
V × F . To each convex polytope P ⊂ Rd we can assign such a combinatorial type
in the obvious way. Note that the edge graph is encoded within P too: we say that
vertices i, j ∈ V are adjacent in P, and denote this by i ∼ j, if there are facets
σ1, ..., σr ∈ F so that i and j are the only two vertices incident to all of them. This
defines a graph structure on V which we call the edge graph GP = (V, E). To
emphasize the presence of this graph structure we also denote a combinatorial type
as the quadruple P = (V, E, F, ∼). MH: Depending on the context, we also use V , E and
F to represent the number of vertices, edges and facets.
The polytopes that share a combinatorial type P form the polytopal realizations
of P. More convenient for computations, for us a d-dimensional polytopal realization
of P will be given as a pair (p, a) consisting of a vertex map p : V → Rd and a facet
normal map a : F → Rd, so that for each σ ∈ F the points (or vertices) {pi | i ∼ σ}
lie on a common affine hyperplane (the facet hyperplane) with normal vector aσ (the
facet normal ). This can be expressed as
⟨pi, aσ ⟩ = 1, whenever i ∼ σ.
We say that a realization is strictly convex (or just convex for short) if additionally
⟨pi, aσ ⟩ < 1, whenever i̸ ∼ σ.
Each convex polytope P with combinatorial type P and 0 ∈ int(P ) gives rise to a
convex realization in this sense with the facet normals pointing outwards. We often
identify a polytope with the corresponding realization and use P and (p, a) inter-
changeably.
All realizations of P taken together form the (convex) realization space of P:
real(P) :=
(
p : V → Rd
a : F → Rd
⟨pi, aσ ⟩ = 1 whenever i ∼ σ
⟨pi, aσ ⟩ < 1 whenever i̸ ∼ σ
)
,
With these definitions real(P) is a semi-algebraic set in RdV ⊕ RdF.
Remark 2.1. The realization spaces defined in [4, Section 2] are slightly different.
Our constraint ⟨pi, aσ ⟩ = 1 for i ∼ σ does not allow facet hyperplane to pass though
the origin. This formulation is more convenient for our purpose. The corresponding
constraint from [4] is ⟨pi −pj , aσ ⟩ = 0 for i, j ∼ σ and does not entail this restriction.
Both definitions lead to spaces that are birationally equivalent in a neighborhood of
each convex realization that has the origin in its interior. Since our analysis will be
primarily local and since every affinely-spanning convex polytope can be translated
so that it contains the origin in its interior, this distinction can be ignored.
The Lie group of Euclidean isometries (i.e., rotations and translations), denoted
Iso, acts on real(P). Factoring it out yields the reduced realization space:
real∗(P) := real(P) / Iso .
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 9
3. Polytope rigidity
We examine continuous deformations of P that preserve edge lengths, analogous
to bar-joint framework rigidity. Unlike in the framework setting, these motions must
also preserve the polytope’s structure, that is, facet planarity and the combinatorial
type. Below we make this precise.
Two realizations (p, a), (˜p, ˜a) ∈ real(P) are
equivalent if ∥pj − pi∥ = ∥˜pj − ˜pi∥ for each edge ij ∈ E,
congruent if ∥pj − pi∥ = ∥˜pj − ˜pi∥ for each pair i, j ∈ V .
A (continuous) motion of (p, a) is a continuous map (pt, at) : [0, 1] → real(P) so
that (p0, a0) = (p, a) and (pt, at) is equivalent to (p, a) for all t ∈ [0, 1]. Let us de-
fine the metric realization space
mreal(P, P ) := (p, a) ∈ real(P) | (p, a) is equivalent to P ,
which contains all realizations of the polytope P, whose edge lengths are prescribed
according to the realization P . The equivalence of edge lengths can be expressed
as ∥pi − pj ∥2 = ∥˜pi − ˜pj ∥2, that is, by a system of quadratic polynomial equations.
Therefore, mreal(P, P ) too is a semi-algebraic set in RdV ⊕RdF . A motion can also
be understood as a continuous curve pt : [0, 1] → mreal(P, P ).
A motion is trivial if (pt, at) is congruent to (p, a) for all t ∈ [0, 1]. If non-trivial,
we call it a flex of P . If a polytope has a flex, we call it flexible, otherwise rigid .
As before, then Lie group of Euclidean isometries Iso acts on mreal(P, P ) and can
be factored out to obtain the reduced metric realization space
mreal∗(P, P ) = mreal(P, P )/ Iso .
A flex can be understood as a non-constant curve pt : [0, 1] → mreal∗(P, P ).
Remark 3.1. Evidently, these definitions apply verbatim to the more general class
of point-hyperplane frameworks. Consequently, much of what we say applies more
generally. Caution is necessary when we assume certain sub-configurations to be
affinely spanning, which is natural in the polytope setting, but does not apply to
general point-hyperplane frameworks.
Remark 3.2. MW: ?? Simulating polytope rigidity via stacking prisms on faces. MH: I’d
say we leave it out.
For examples of flexible polytopes, see Section 10 or [4, Section 4].
10 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
4. First-order theory of polytope rigidity
The first-order theory of a rigidity systems studies the deformations that preserve
the constraints up to first order. It is a linear theory and hence provides practical
heuristics and criteria that can be efficiently checked in practice.
Given a polytope P = (p, a) ⊂ Rd, its rigidity matrix R(P ) = R(p, a) has the
following structure:
All displayed entries are to be interpreted as 1 × d sub-matrices. The dimensions of
R(P ) are therefore (E + VF ) × (dV + dF ), where VF denotes the set of incident
vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled version of) the
Jacobian corresponding to the polynomial system of equations that define the metric
realization space mreal(P, P ).
The first-order theory of rigidity is essentially the study of the linear algebra pro-
perties of R(P ). All first-order notions can be derived from it.
4.1. First-order rigidity. The elements of the kernel of R(P ) are called first-order
motions of P . We denote them as pairs ˙P = ( ˙p, ˙a) consisting of maps ˙p : V → Rd
and ˙a : F → Rd that satisfy the following equations:
⟨pi − pj , ˙pi − ˙pj ⟩ = 0, whenever ij ∈ E,(4.1)
⟨pi, ˙aσ ⟩ + ⟨ ˙pi, aσ ⟩ = 0, whenever i ∼ σ.(4.2)
Like in the frameworks setting, the interpretation is that ˙p and ˙a are infinitesimal
changes in the values of p and a. In particular, (4.1) and (4.2) can be obtained by
differentiating the equations for edge length and coplanarity constraints. Note also,
that ˙a is already determined by ˙p via (4.2) (for details see the proof of Lemma 4.1).
First-order motions are called trivial if they satisfy
⟨pi − pj , ˙pi − ˙pj ⟩ = 0, for any i, j ∈ V ,(4.3)
Separate constraints on ˙a are not necessary since they are already determined via
(4.2). Non-trivial first-order motions are called first-order flexes. If a first-order flex
exists, the polytope is called first-order flexible, otherwise first-order rigid .
The trivial first-order motions of P form a linear subspace TP ⊆ ker R(P ). The
first-order flexes do not form a linear space, though for matters of dimension count-
ing we can consider the quotient ker R(P )/TP . We shall call it the first-order flex
space of P . This space is trivial if and only if P is first-order rigid. The dimensions
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 11
of the first-order flex space for the Archimedean and Catalan solids are included in
Table 1 and Table 2.
Lemma 4.1. dim TP = d+1
2
. In particular, corank R(P ) ≥ d+1
2
.
Proof. Constraints (4.3) are precisely the constraints of trivial first-order motions
for bar-joint frameworks. In this setting, trivial first-order motions have the form
˙p = Sp + t for a skew-symmetric matrix S ∈ Rd×d and t ∈ Rd, forming a vector
space T ′
P of dimension d+1
2
 [6]. Note that this assumes that p is affinely spanning,
which follows from our assumption that P has nonempty interior.
It remains to verify that each ˙p ∈ T ′
P extends to a polytopal first-order motion
of P . For this, fix σ ∈ F and choose a basis pi1 , ..., pik among the pi, i ∼ σ. This is
possible because the face spans a (d − 1)-dimensional affine subspace. Let ˙aσ be the
unique solution of the full-rank linear system ⟨ ˙aσ , pik ⟩ = −⟨aσ , ˙pik ⟩ where k ranges
over {1, ..., d}. This ensures (4.2) for the pik , and it remains to verify (4.2) for a
general pi, i ∼ σ. Since the pi, i ∼ σ are coplanar, we can write pi = P
k αkpik for
coefficients αk that satisfy P
k αk = 1. Using ˙pi = Spi + t, we obtain
⟨ ˙aσ , pi⟩ =
D
˙aσ , X
k
αkpik
E
= X
k
αk⟨ ˙aσ , pik ⟩ = − X
k
αk⟨aσ , ˙pik ⟩
= − X
k
αk⟨aσ , Spik + t⟩ = −
D
aσ , S X
k
αkpik + t X
k
αk
E
= −⟨aσ , Spi + t⟩ = −⟨aσ , ˙pi⟩.
We conclude TP ≃ T ′
P , and the claim follows. □
Corollary 4.2. A polytope is first-order rigid if and only if corank R(P ) = d+1
2

Proof. Let TP ⊆ ker R(P ) be the space of trivial first-order motions of P . Then
P is first-order rigid def
⇐⇒ ker R(P ) = TP
4.1
⇐⇒ corank R(P ) = d+1
2
. □
First-order rigidity provides an efficiently computable certificate for rigidity:
Theorem 4.3. If a polytope is first-order rigid, then it is rigid.
This is a consequence of the second-order results Theorem 6.1 and Corollary 6.4.
Below we give an independent proof to highlight the similarities between the first-
and second-order theory (in particular, compare to the proof of Theorem 6.1).
Proof of Theorem 4.3. We prove the contrapositive: we assume that P is flexible,
and show that it is first-order flexible. For this, consider the algebraic subset
M ⊆ mreal(P, P ) where we restrict sufficiently many vertices of P to subspaces
so as to precisely cancel the trivial motions. If P is flexible then P is not an isolated
point of M . Hence, using the curve selection lemma (see e.g. [25, Lemma 18.3]) we
obtain a non-constant analytic path P t in M that ends in P . In other words, P t is
a flex of P that has a Taylor series expansion that converges to P t.
By adding trivial motions to P t we can cancel some of the lower order terms
of the series expansion. Since P t is non-trivial and analytic, there is a maximal
number k so that we can simultaneously cancel all orders 1, ..., k − 1.
We now consider the k-th derivatives of the first-order motion constraints. We
write ( d
dt )m
t=0 for the operator that takes the m-th derivative and evaluates at t = 0.
12 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
For the edge length constraint (4.1) at ij ∈ E we obtain
0 =
 d
dt
k
t=0
∥pi − pj ∥2 =
kX
ℓ=0
k
ℓ
D d
dt
ℓ
t=0
(pi − pj ),
 d
dt
k−ℓ
t=0
(pi − pj )
E
(∗)
= 2
D
pi − pj ,
 d
dt
k
t=0
(pi − pj )
E
,
where in (∗) we use that most terms are zero by the choice of k. Analogously, for
the vertex-facet incidence constraint (4.2) at i ∼ σ we obtain
0 =
 d
dt
k
t=0
⟨pi, aσ ⟩ =
kX
ℓ=0
k
ℓ
D d
dt
ℓ
t=0
pi,
 d
dt
k−ℓ
t=0
aσ
E
=
D
pi,
 d
dt
k
t=0
aσ
E
+
D d
dt
k
t=0
pi, aσ
E
.
Observe that these two identities precisely express that ˙P := ( d
dt )k
t=0P satisfies the
equations of a first-order motion. It remains to show that ˙P is non-trivial. In fact,
if ˙P were trivial, then ˙P = d
dt Q for some trivial motion Qt. One can check that
then the reparameterization ˆQt := Qtk /k! is still trivial and cancels the k-th order
term of P t, in contradiction to the choice of k. □
Remark 4.4. A converse of Theorem 4.3 does not hold in general. For example,
the regular dodecahedron is first-order flexible (it has a 5-dimensional space of first-
order flexes), but is second-order rigid, and hence rigid (cf. Table 1).
While Dehn’s theorem already implies the first-order rigidity of various polytopes
whose faces are triangles, not all first-order rigid examples that we encounter here
satisfy this assunption. We therefore formulate the following question:
Question 4.5. It is not possible to certify the first-order rigidity of all polytopes
from Table 1 and Table 2 by only using Dehn’s theorem [12]. For instance, the
truncated tetrahedron and the rhombic dodecahedron are first-order rigid, even
though they are not simplicial. Is it possible to construct a combinatorial criterion
for the first-order rigidity of polytopes are not covered by Dehn’s theorem?
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 13
5. Edge Length Perturbations
For this section, we restrict ourselves to 3-dimensional convex polytopes, which
come with various theoretical advantages over the general case (see e.g. [4]). Here,
we investigate the complement of mreal(P, P ) in real(P), i.e., the space of all
realizations that arise from perturbing some of the edge lengths of P . We establish
topological techniques that provide novel conditions for the rigidity and flexibility of
polytopes, but also provide insights into the geometry of mreal(P, P ) by providing
an intuition for how first-order flexes are related to first-order flexes which only
preserve the coplanarity constraints.
According to the Legendre-Steinitz Theorem [23] the convex realization space
real(P) is a (E + 6)-dimensional manifold. At every polytopal realization the
trivial first-order motions form a 6-dimensional subspace of the space of infinitesimal
motions (cf. Lemma 4.1) which is completely determined by the 6-dimensional Lie
group of Euclidean isometries Iso. This turns real∗(P) into a smooth manifold of
dimension
dim (real∗(P)) = dim(real(P)) − dim(Iso) = (E + 6) − 6 = E.
In other words, all polytopes have E degrees of freedom when pinning a vertex, MW: You want to
pin a vertex, con-
strain an edge to
a 1-dim subspace
and a face to a 2-
dim subspace. Pin-
ning the edge sounds
like restricting its
length.MH: Ad-
justed.
constraining an edge to a one-dimensional subspace and a face to a hyperplane (cf.
[14]). This modification factors out the trivial motions of polytopes. As a matter
of fact, dim(real(P)) being exactly equal to the number of edges of P suggests
that the degrees of freedom correspond exactly to perturbations of the edge lengths.
Since rigid realizations correspond to isolated points in mreal(P, P ), the degrees
MW: “This line of
thought would imply
that we can locally
freely perturb the
edge lengths around
rigid realizations” I
think it is not clear
why you mention
“rigid realizations” in
this sentence. MH:
Changed the sen-
tence.
of freedom in real(P) must concentrate on the flexes that change the edge lengths.
This line of thought would imply that we can freely perturb the edge lengths locally
around rigid realizations (see Question 5.9). We formalize this intuition in the
following definition.
MW: Can’t we just
define existence of
edge-length pertur-
bations as that “the
map from realiza-
tions to edge length
vectors is locally sur-
jective at P ? MH:
I do not believe this
avoids the invariance
of domain theorem.
“continuous” plus “lo-
cally surjective” just
rewords what is al-
ready there and ab-
stracts the meaning.
I am not necessarily
against this change,
I just don’t believe it
is going to be impact-
ful.
Definition 5.1. The edge length vector of P is given by
ℓ(P ) :=
 1
2 ∥pi − pj ∥2 ij ∈ E

.
This gives rise to the edge length map ℓ : real(P) → RE with P 7 → ℓ(P ). We say
that a vector ℓ′ ∈ RE is realized by P if ℓ′ = ℓ(P ). The edge length realization
space L(P) of P consists of all possible vectors of edge lengths corresponding to
convex realizations of P. Moreover, P has all edge length perturbations if every
sufficiently small perturbation of its edge length vector ℓ(P ) can be realized via a
locally continuous map ψ : RE → real(P) with ψ(ℓ(P )) = P . If that is not the
case, i.e., if there are edge length perturbations arbitrarily close to ℓ(P ) that can
not be realized via ψ as a polytope Q sufficiently close to P , we say that some of
P ’s edge length perturbations are not realizable.
More precisely, P has all edge length perturbations if for some C > 0 and every
ε ∈ (0, C] there exists a δ > 0 such that every edge length vector ℓ′ with
dist(ℓ(P ), ℓ′) < δ
there exists a polytope Q = ψ(ℓ′) of the same combinatorial type as P that satisfies
dist(P, Q) < ε
14 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
in the Euclidean metric on Rd(V +F ). This definition implies that the edge length
map ℓ : real(P) → RE is locally surjective around P . However, the local surjec-
tivity of ℓ is a strictly weaker condition than the local continuity of ψ.
To explain that the condition is strictly weaker, let us consider a counterexample.
The map f : R2 → R2 with (x, y) 7 → (x2 − y2, 2xy). This mimics the holomorphic
map C → C with z 7 → z2 over R. The map f is continuous and around the
point (0, 0), it is locally surjective, since square roots over C exist. However, the
square root function is set-valued, so there exists no (locally) continuous square
root function on C due to the branching problem.
Having obtained a better understanding for the subleties of Definition 5.1, let
us now examine two examples. These examples elucidate which classes of poly-
topes admit all edge-length perturbations and for which classes certain edge-length
perturbations are not realizable.
Example 5.2. Consider the regular tetrahedron with realization P . This polytope
is first-order rigid according to Dehn’s Theorem [12]. The facet planarity constraints
are superfluous in this case, as all facets are triangles. As the edge graph of the
tetrahedron is the complete graph K4, this polytope is even minimally first-order
rigid in R3, implying that the removal of any edge renders the corresponding bar-
joint framework flexible. Given any sufficiently small perturbation ℓ′ ∈ RE of ℓ(P ),
we can thus iteratively remove each edge to make the tetrahedron flexible, deform
it until that particular edge length is correct, and then put the edge back. We can
iteratively repeat this process until we find a tetrahedral realization Q sufficiently
close to P which satisfies ℓ′ = ℓ(Q).
Example 5.3. Not all realizations of convex polytopes may have all edge length
perturbation. For instance, consider the regular cube, whose vertices are realized by
the elements from {1, −1}3. It is not possible to continuously perturb a single edge
without violating the planarity of the facets; the minimum requirement for realizing
an edge length perturbation is to simultaneously adjust two opposing edges. In this
case, this property arises because the cube is flexible (see Theorem 5.6 below).
While Definition 5.1 may seem rather technical, it is helpful in formulating a
relationship between a polytope’s rigidity and topological properties of its edge
length realization space. Using this language, we can show that first-order rigid
polytopes concentrate their degrees of freedom on deformations induced by edge
length perturbations.
Proposition 5.4. A first-order rigid convex polytope P has all edge length pertur-
bations.
Proof. Consider the following commutative diagram:
RdV ⊕ RdF RE ⊕ RVF
real(P) RE
f
ı
ℓ
ȷ
The vertical arrows ı and ȷ are the canonical embeddings. The arrow ℓ is the edge
length vector map. The arrow f maps an arbitrary pair (p, a) to 1
2 ∥pi − pj ∥2 for
ij ∈ E, and ⟨pi, aσ ⟩ for i ∼ σ.MW: In the rest of
the section your write
E instead of E for
cardinalities.MH:
I reckon you prefer
using E for cardi-
nalities? How do we
call the set of edges
then?MW: I prefer
E for the set and the
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 15
We observe that the Jacobian of f at the realization P is (up to scaling of rows)
equal to the rigidity matrix R(P ), and since P is first-order rigid, Corollary 4.2
yields that
rank f = rank R(P ) = dV + dF − corank R(P ) = dV + dF − 6,
where by rank of a map we mean the rank of its Jacobian at the realization P . The
map ı has rank E + 6 by the Legendre-Steinitz Theorem. From the commutative
diagram and basic results about the rank of matrix products, we obtain
rank(ℓ) ≥ rank(ȷ ◦ ℓ) = rank(f ◦ ı)
≥ rank(f ) + rank(ı) − dim(RdV ⊕ RdF )
= (dV + dF − 6) + (E + 6) − (dV + dF )
= E.
Since ℓ maps into RE , it follows that the map has the maximal rank(ℓ) = E. Finally,
ℓ is smooth, so we conclude that ℓ is a local submersion (cf. [19, Proposition 4.1])
and hence locally surjective (cf. [18, Proposition 2.2]). Therefore, all sufficiently MH: There is a gap
in the proof here,
since the definition
requires the existence
of ℓ−1 (sort of), so
we need to construct
a continuous map
from RE → real(P)
MW: This is easy
enough by quotient-
ing by the Iso-action.
But let’s not touch
this before we have
figured out the defini-
tion problem
small edge length perturbations of P are realizable. □
A major result of [4] is that almost all realizations of convex 3-polytopes are
infinitesimally rigid. This result requires a suitable definition of genericity, which
is omitted here for the sake of brevity (see [4, Definition 5.3.] for details). Intu-
itively, we can obtain a generic realization by drawing a random convex realization
realization from real(P). We can apply the statement about the generic rigidity
of polytopes to Proposition 5.4 in order to obtain a result about the edge length
perturbation space of generic realizations.
Corollary 5.5. A generic realization of a convex polytope P has all edge length
perturbations.
Proof. In [4] it is shown that any generic realization of a polytope is first-order
rigid. Hence, Proposition 5.4 is applicable, showing that P has all edge length
perturbations. □
In Example 5.3, we have seen that flexible polytopes do not necessarily permit
all edge length perturbations. We can turn this simple observation into a general
statement about flexible polytopes.
MW: Proposal: we bring the two examples as motivation; we take the locally surjective
definition; we prove fo-rigid implies all perturbation exist; we discuss whether the cube example
can be generalized; we give Theorem 5.6 as a question; we discuss the z2 problem; we prove
flexible implies not all perturbations exist under the additional example of continuous inverse
(maybe constant fiber?).
Theorem 5.6. If a convex polytope P is flexible, then some of its edge length
perturbations are not realizable.
Proof. Denote the combinatorial type of P by P. By a previous observation, the
reduced realization space real∗(P) of P is a smooth E-dimensional manifold via
the homeomorphism φ : real∗(P) → RE .
MW: I am skeptical of the conclusion of the second paragraph. We assume that real∗ is
smooth and E-dim, ℓ : real∗ → RE is polynomial and locally surjective. But from this alone we
cannot conclude that ℓ has a local inverse by a continuous map ψ. There are counterexamples
16 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
in this general setting. Either you use more structure and I don’t understand how, or there is a
gap.MH: I do not use ℓ in this proof and the edge length realization space is also not reliant on
ℓ. In fact, the definition goes the other way around: All edge length perturbations are realizable
if there exists a local, well-defined, continuous map RE → real(P); in other words, for all
sufficiently small edge length perturbations ℓ′ of ℓ(P ) we can find a realization Q sufficiently close
to P such that ℓ(Q) = ℓ′ (i.e., the map that I am describing above maps an open neighborhood
of ℓ(P ) to some sort of set that contains P ). At least that is what I intended to convey. If the
definition does not convey this, we need to fix it. Nothing about local surjectivity whatsoever.
Honestly, you confused me more with your comment about local surjectivity than it helped, so
I’d prefer forgetting this term entirely. This map is trivially injective though. I reckon we should
add a comment/remark after the definition to clarify either way. MW: Here is what I just
did to sanity check myself: I took a screenshot of your definition of edge length perturbation
and put it into ChatGPT. I asked whether this gives me a local continuous inverse ψ that you
claim. It said no. It told me that this definition is a sort of “local surjectivity” of ℓ. I did
not put this word in, it came back with it itself. So I think the definition is not unclear, but
simply not what you want it to be. We need to either fix the definition or the result. MH:
ChatGPT customizes the chats to you by learning from past chats. If I ask ChatGPT anything
mathematical, I usually get rigidity theory as an example. This is not really an argument. Also,
around 40% of AI queries produce erronous answers. The definition is simply the ε-δ definition of
local continuity of ψ. I am still convinced that the definition says exactly that. When I queried
ChatGPT about local surjectivity, it often reversed the arrows. This may stem from the fact that
suspensions mainly appear in differential geometry where they are used to show the existence of
a locally surjective atlas (which reverses the arrows). MW: Thinking some more I now believe
that I understand where you are coming from. I simply had a different (weaker) notion of “edge
length perturbations exist” in mind. Which one is better is unclear to me. The one where we can
prove more, or the one that needs less assumptions. For example, I think with your definition, the
answer to Question 5.9 is very likely No already for the dodecahedron. But I am very optimistic it
has all perturbations under my definition (which equals your currently written down definition).
Especially since all edges can be perturbed individually. Assume now that all of P ’s edge
length perturbations are realizable. Then, in particular, we can locally extend
and contract each of P ’s edges individually. In fact, we can arbitrarily combine
these edge length perturbations, so that each combination of edges that we perturb
gives rise to a distinct continuous deformation of P . This implies that there is an
open E-dimensional ball of realizable edge length perturbations containing ℓ(P ).
Therefore, the map ψ : RE → real∗(P) taking a list of edge lengths and producing
a realization of P with ψ(ℓ(P )) = P is well-defined, injective and continuous in a
sufficiently small open neighborhood Uℓ(P ) ⊂ RE of ℓ(P ).
RE ⊃ Uℓ(P )
∈
ℓ(P )
real∗(P) RE
ψ φ
Legendre-Steinitz
Invariance of Domain
Figure 3. A diagram for the topological argument used in this proof
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 17
We visualize the following topological arguments in Figure 3. By the Invariance
of Domain Theorem [8], the locally continuous injection φ ◦ ψ : Uℓ(P ) → V ⊂ RE
for V = φ ◦ ψ(Uℓ(P )) is a homeomorphism on its domain and V is open. This lets
us pull back the open set V to the open set φ−1(V ) in real∗(P), since φ is a local
homeomorphism. As a consequence, ψ : Uℓ(P ) → φ−1(V ) is a homeomorphism,
since ψ = φ−1 ◦ (φ ◦ ψ) and φ−1 and φ ◦ ψ are both homeomorphisms.
This implies that there exists an open neighborhood around P in the manifold
real∗(P), in which all realizations come from edge length perturbations. In other
words, there is no nontrivial continuous motion that preserves the edge lengths in
ℓ(P ), so P is rigid. □
The contraposition of this theorem provides a sufficient condition for the rigidity
of polytopes, which makes it worth to point it out as a corollary. Albeit, it is still
unclear whether checking that all edge length perturbations are realizable offers
any advantage over directly verifying a polytope’s rigidity.
Corollary 5.7. If all edge length perturbations of a convex polytope are realizable,
then it is rigid.
Remark 5.8. It is unclear, whether the converse of Theorem 5.6 is true: The space
of edge length perturbations may be full-dimensional, even though the realization P
is rigid and only certain edge length perturbations which form a lower-dimensional
algebraic subset are not realizable.
The correspondence between the edge length realization space of a polytope and
its rigidity properties is fascinating. Even though Proposition 5.4 and Theorem 5.6
almost paint a complete picture of this correspondence, we were unable to resolve
the case where the polytope is continuously rigid. In our experiments (cf. Sec-
tion 9.2), we find that this case seems to have particularly interesting algebraic and
topological properties. For that reason, we formulate the following two questions,
which we hope will inspire future research in this topic.
Question 5.9. Does every rigid realization of a convex polytope have all edge
length perturbations?
Question 5.10. Assuming a convex polytope P is second-order rigid (cf. Section 6),
is ℓ(P ) then singular in the edge length realization space L(P ) (see Figure 5)?
While we do not understand the edge length realization space of polytopes nearly
enough to provide answers to these questions, they provide interesting observations
that should be investigated in future research.
18 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
6. Second-order theory
Second-order rigidity theory investigates continuous flexes that preserve the con-
straints up to second order. It is mainly employed for the analysis of systems that
fail the first-order rigidity test. We follow the work of Connelly and Whiteley [10].
6.1. Second-order rigidity. A tuple ( ˙P, ¨P ) = ( ˙p, ˙a; ¨p, ¨a) of maps ˙p, ¨p : V → Rd
and ˙a, ¨a : F → Rd is called a second-order motion of P if it satisfies
⟨pi − pj , ¨pi − ¨pj ⟩ + ⟨ ˙pi − ˙pj , ˙pi − ˙pj ⟩ = 0, whenever ij ∈ E(6.1)
⟨pi, ¨aσ ⟩ + 2⟨ ˙pi, ˙aσ ⟩ + ⟨¨pi, aσ ⟩ = 0, whenever i ∼ σ.(6.2)
Analogous to what was observed in Section 4.1, the ¨a are automatically determined
by the ¨p in this setting. We call a second-order motion trivial if ( ˙p, ˙a) is trivial as aMW: Is the sentence
about ¨a being deter-
mined by ¨p neces-
sary?MH: Not really.
We can remove it.
first-order motion. A non-trivial second-order motion is called a second-order flex .
If P has a second-order flex, then it is called second-order flexible, and second-order
rigid otherwise.
Second-order rigidity provides a certificate for rigidity:
Theorem 6.1. If a polytope is second-order rigid, then it is rigid.
Proof. The proof is largely analogous to the proof of Theorem 4.3. As before, we
prove the contrapositive: we assume that P is flexible; and show that it is second-
order flexible. Through restricting vertices to suitable subspaces and invoking curve
selection, we obtain an analytic flex P t. There is then a maximal number k so that
adding a suitably chosen trivial motion simultaneously cancels all terms of order
1, ..., k − 1 in the Taylor expansion of P t.
This time we consider the 2k-th derivatives of the first-order motion constraints.
For the edge length constraint (4.1) at ij ∈ E we obtain
0 =
 d
dt
2k
t=0
∥pi − pj ∥2 =
2kX
ℓ=0
2k
ℓ
D d
dt
ℓ
t=0
(pi − pj ),
 d
dt
2k−ℓ
t=0
(pi − pj )
E
(∗)
= 2
D
pi − pj ,
 d
dt
2k
t=0(pi − pj )
E
+
2k
k
D d
dt
k
t=0(pi − pj ),
 d
dt
k
t=0(pi − pj )
E
where in (∗) we use that most terms are zero. Analogously, for the vertex-facet in-
cidence constraint (4.2) at i ∼ σ we obtain
0 =
 d
dt
2k
t=0
⟨pi, aσ ⟩ =
2kX
ℓ=0
2k
ℓ
D d
dt
ℓ
t=0
pi,
 d
dt
2k−ℓ
t=0
aσ
E
=
D
pi,
 d
dt
2k
ak
E
+
D d
dt
2k
t=0 pi, ak
E
+
2k
k
D d
dt
k
t=0 pi,
 d
dt
k
t=0ak
E
.
Observe that these two identities express that
˙P :=
 d
dt
k
t=0
P and ¨P := 2
2k
k
−1 d
dt
2k
t=0
P
together form a second-order motion of P . It remains to show that ˙P is non-trivial.
Analogously to the proof of Theorem 4.3, this follows from the choice of k. □
The notion of a second-order flex is not easy to apply directly. In contrast to first-
order theory, the defining equations (6.1) and (6.2) form a quadratic rather than
linear system. Given a candidate first-order flex ( ˙p, ˙a), the system becomes linear
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 19
in (¨p, ¨a) and we can check efficiently whether ( ˙p, ˙a) extends to a second-order flex.
This allows to check second-order rigidity at least for systems whose space of first-
order flexes is 1-dimension. If the dimension is higher, there is no obvious way to
choose the candidate first-order flexes from which to start.
In [10, Section 1.4] Connelly and Whiteley developed a second-order rigidity test
that reinterprets second-order rigidity as the study of the bilinear pairing of first-
order motions and equilibrium stresses. We adapt this technique to our setting.
6.2. The second-order stress test. The elements of the cokernel of the rigidity
matrix R(P ) (i.e., the kernel of R(P )⊤) are called the equilibrium stresses (or just
stresses) of a system. We denote them by pairs (ω, η) consisting of maps ω : E → R
and η : VF → R (recall that VF denotes the set of incident vertex-facet pairs). They
satisfy the following two stress equilibrium conditions:
X
j:ij∈E
ωij (pi − pj ) + X
σ:i∼σ
ηiσ aσ = 0, for all i ∈ V ,(6.3)
X
i:i∼σ
ηiσ pi = 0, for all σ ∈ F .(6.4)
We write ξ = (ω, η) sake of brevity and call it a polytope stress.
Figure 4. Visualization of a polytope stress (ω, η).
Remark 6.2. Stresses in frameworks can be given a physical interpretation: each
edge of a framework is thought of as a spring with a strength given by the stress ωij
at ij ∈ E. The strength determines how strongly the edge pushes or pulls on its end
vertices along the direction of the edge. Whether it pulls or pushes is determined
by the sign on ωij . The stress equilibrium condition (the first term of (6.3)) states
the forces that act on a vertex i ∈ V cancel each other out.
The spring constant interpretation persists for the ω-part of the polytope stress
(ω, η), but now they do not need to cancel out at the vertices on their own. Instead,
they need to add up to be equal and opposite to the second term – the η-part of
the stress. This is complicated by the fact that η contributes to two equilibrium
conditions, (6.3) and (6.4), for which we try to provide interpretations below.
First, the right term in (6.3) can be though of as forces pushing a vertex along
the normals of its incident facets (see Figure 4, left). One may think of this term
as a force resulting from pressure from within the polytope, though this analogy is
mostly non-physical: the forces are not proportional to the volume of the facet and
may even have varying sign from facet to facet.
Second, the stress condition (6.4) for a facet σ ∈ F can be interpreted as a force
equilibrium at the origin: each vertex i ∼ σ pushes or pulls the origin along their
connecting line (cf. Figure 4, right).
20 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
The following test is an elegant application of Farkas’ lemma:
Theorem 6.3 (Stress test). A polytope is second-order rigid if and only if for every
first-order flex ˙P there is a blocking stress, that is, a stress ξ with
ξ⊤R( ˙P ) ˙P̸ = 0.(6.5)
Proof. Fix a first-order flex ˙P = ( ˙p, ˙a). We shall show that it can be extended to a
second-order flex if and only if there is no blocking stress.
Recall that, after fixing ˙P , the equations (6.1) and (6.2) become linear in ¨P =
(¨p, ¨a). The linear system can be compactly expressed as
(6.6) R(P ) ¨P = −R( ˙P ) ˙P
This system has a solution in ¨P if and only if ˙P extends to a second-order flex.
The existence of a blocking stress ξ for ˙P can be expressed by the system
(6.7) R(P )⊤ξ = 0, ξ⊤R( ˙P ) ˙P̸ = 0.
It remains to observe that the systems (6.6) and (6.7) are dual in the sense of
Farkas’ lemma: if we set A := R(P ) and b := −R( ˙P ) ˙P , then either there is a ¨P with
A ¨P = b, or there is a ξ with A⊤ξ = 0 and ξ⊤b̸ = 0. □
In following [10], we also introduce the notion of prestress stability: a polytope
is prestress stable if there is a single stress ξ that blocks every first-order flex ˙P . By
reversing the quantifiers from the criterion for second-order rigidity in Theorem 6.3,
this creates a stronger sufficient condition for rigidity. In Remark 6.2, we provide
an interpretation of the stresses that gives rise to a nonlinear optimization problem,
whose strict equilibria correspond to prestress stable realizations.
Corollary 6.4. first-order rigid =⇒ prestress stable =⇒ second-order rigid.
Proof. If P is first-order rigid, then there are no first-order flexes, and the condition
of prestress stability is trivially satisfied. The second implication is clear from
Theorem 6.3 and the definition of prestress stability. □
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 21
7. Certifying Second-order rigidity
As laid out in Section 6, any non-trivial first-order flex of a polytope in the edge-
length realization space mreal(P, P ) that has the chance to extend to a continuous
motion must necessarily not be blocked by an equilibrium stress. This provides
a convenient heuristic for finding nonblocked flexes: Essentially, we need to find
a non-trivial flex ˙P such that ξ⊤R( ˙P ) ˙P = 0 for all equilibrium stresses ξ (cf.
Theorem 6.3). Conversely, if there exists a ξ such that ξ⊤R( ˙P ) ˙P̸ = 0 for all ˙P , then
the polytope is second-order rigid, which guarantees that it is rigid (cf. Theorem 6.1
and 6.3). This criterion can be checked by parameterizing the flex space via a basis
˙P = ( ˙P 1, . . . , ˙P r ) and variables λ = (λ1, . . . , λr ) and the equilibrium stress space
via a basis ξ = (ξ1, . . . , ξs) and variables μ = (μ1, . . . , μs). This turns the second-
order condition from Theorem 6.3 into a cubic polynomial of the form
E ˙P , ξ(λ, μ) =


sX
j=1
μj ξj

 · R
rX
i=1
λi ˙P i
!
·
rX
i=1
λi ˙P i
!
.
More precisely, E ˙P, ξ is linear in the variables μ and quadratic in the variables
λ. For asserting second-order rigidity, it suffices to show that every non-trivial
first-order flex has a blocking stress according to Theorem 6.3. In other words,
second-order rigidity can be checked by finding μ for each λ so that E ˙P , ξ(λ, μ)̸ = 0.
By expanding E ˙P, ξ(λ, μ) in terms of μj , we obtain
E ˙P , ξ(λ, μ) =
sX
j=1
μj · Qj (λ)
for quadratic forms Qj ∈ R2[λ1, . . . , λr ].
The crucial observation is the following: If any of the Qj is nonzero for a given
λ, then we can find μ such that Ps
j=1 μj · ξj blocks Pr
i=1 λi · ˙P i. Therefore, the
first-order flexes corresponding to a λ that are not blocked by any stresses must
live in the algebraic set given by the intersection of the zeros of Q1, . . . , Qs.
Since the polynomials Q1, . . . , Qs are homogeneous, it is sufficient to show that
there are only finitely many elements in the algebraic set V(Q1, . . . , Qs). The
following lemma lets us certify the zero-dimensionality of an algebraic variety and
it proves useful to us in practice. It is a standard result in computational algebraic
geometry and can be found in textbooks such as [11, Thm. 5.3.6].
Lemma 7.1. Fix a field k. Given an ideal I = ⟨f1, ..., fn⟩, where fi ∈ k[x1, .., xm],
and a Gröbner basis G. I is zero dimensional if and only if some power of xi is the
leading monomial of an element of G for every i ∈ {1, ..., m}.
There are also other methods based on Gröbner bases to verify than an ideal
is zero-dimensional; however, for our purposes, Lemma 7.1 proves to be sufficient.
If the ideal I = ⟨Q1, . . . , Qs⟩ is zero-dimensional, then the algebraic variety V(I)
contains only finitely many points [15, Prop. 1.7]. Since the quadratic forms Qi
are homgeneous, V(I) ⊂ Pr−1
C , so for any solution λ∗ of the polynomial system
Q1(λ) = 0, . . . , Qs(λ) = 0, all scalar multiples c · λ must also lie in V(I). The
zero-dimensionality of V(I) is therefore equivalent to V(I) = ∅. In our context,
this translated to the non-existence of non-blocked flexes. We summarize our ob-
servations in the following:
22 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
Proposition 7.2. If the homogeneous polynomial system ∇μE ˙P,ξ(λ) = 0 only has
λ = 0 as a real solution, then all first-order flexes are blocked by equilibrium stresses.
Conversely, any flex that is not blocked by an equilibrium stress corresponds to a
non-trivial, real zero of ∇μE ˙P,ξ(λ).
The approach based on Gröbner bases which is described in this section is suffi-
cient for all Archimedean solids (cf. Section 9). Still, it clearly is not necessary, as
we only determine the emptiness of V(I) over C. Therefore, it is possible that V(I)
is empty over the real numbers, even when we find solutions over C. The trivial
counterexample is x2 + y2 = 0, which only has x = y = 0 as a real solution, yet the
line x = iy as a complex solution. A weaker certificate is given by the Euclidean
distance degree problem [13] for a generic point p ∈ Rr , which guarantees finitely
many solution on all connected components of VR(I) (cf. [2]).
Analogous to second-order rigidity, we can decide prestress stability (cf. Corol-
lary 6.4). For that, we need to decide if there exists a linear combination of stresses
μ such that E ˙P, ξ(λ, μ)̸ = 0 for all λ. This is a standard semidefinite programming
(SDP) problem: we need to show that Ps
j=1 μj · Qj (λ) is positive definite for some
choice of μj . As this is a homogeneous quadratic form, we can alternatively check
whether the matrix Ps
j=1 μj ·
 ∂2
∂λj λk Qj (λ)
r
j,k=1
is positive definite for some choice
of μ. Our calculation shows that the regular dodecahedron and truncated icosa-
hedron are not prestress stable using a numerical SDP solver. A dual symbolic
approach is described in [20, Lemma 6.3.2], but we do not currently have a way to
produce such a certificate in our case.
8. Approximating Continuous Motions
Determining the flexibility of a bar-and-joint framework is NP-hard [1], so there
is little hope that our more complicated setting will be any easier. Instead, we shift
our attention to numerically approximating deformation paths of this geometric
constraint system.
In this article, we use a technique that relies on following solution paths along
a given initial direction that continually satisfy the constraints. Assume we are
given a non-trivial first-order flex ˙P that extends to a continuous motion. In other
words, P + ˙P lies in the linearization of the underlying constraint set. In Heaton
and Himmelmann [16], a method for approximating the corresponding deformation
path based on Riemannian optimization is implemented as a combination of the
metric projection to the closest point and homotopy continuation. It is called
the Euclidean distance retraction as it projects P + ˙P to its closest point on the
constraint set.
The closest point problem can be described by a constrained polynomial opti-
mization problem, so we can reformulate it as a (polynomial) Lagrange multiplier
system whose zeros characterize the optimization problem’s critical points (cf. [21]).
Since we already know a solution to this polynomial system in u = P – namely, the
realization P itself – we can apply homotopy continuation methods consisting of a
predictor step (e.g. Euler’s method) and a corrector step (e.g. Newton’s method).
Such schemes are often applied for solving polynomial systems [24].
In general, a direct application of the Newton corrector method may diverge
or converge to the wrong point. Nevertheless, for the problem of computing the
Euclidean distance retraction, the convergence of the predictor-corrector scheme to
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 23
the closest point to P + ˙P can be shown, as long as the linear step P + ˙P stays
sufficiently close to the underlying constraint set [16].
Nevertheless, three questions remain:
(i) how to ensure that an initial flex extends to a continuous motion,
(ii) how to compute the subsequent flex in the case where the linear space of
non-trivial first-order flexes has a dimension greater than 1 and
(iii) how to traverse singularities?
The Euclidean distance retraction has been refined for geometric constraint sys-
tems in Adrian-Himmelmann [2], where all of these questions are addressed using
heuristics and theoretical tools. If we assume that there exists a first-order flex
that extends to a continuous motion (e.g. by assuming that the polytope P is flex-
ible), this flex necessarily needs to be a non-blocked flex. For this reason, assume
we know a basis of non-trivial first-order flexes ˙P = ( ˙P1, . . . , ˙Pr ) and a basis of
equilibrium stresses ξ = (ξ1, . . . , ξs). Following Section 7, we solve the homoge-
neous polynomial system ∇μE ˙P, ξ(λ) = 0 over Pr−1
R for λ∗
1, . . . , λ∗
r we can obtain
a non-trivial flex ˙P = Pr
i=1 λ∗
i ˙P i that is not blocked by any equilibrium stress (cf
Proposition 7.2). We take it as our initial flex, as it heuristically has a good chance
of providing a flex that extends to a continuous motion, since we have no examples
of second-order flexible polytopes that are rigid.
For the second question, we return to Riemannian geometry: On a smooth
manifold, the parallel transport [7, §10.3] is a means to compare vectors that live in
distinct tangent spaces. This inspires our approach: Given the previous flex ˙Pold
corresponding to the realization Pold for which Pold + ˙Pold has been projected to
obtain the current realization P , we first compute a basis of the space of non-trivial
first-order flexes that we collect as the rows of a matrix A. To find the closest
analogue to the flex ˙Pold in the new realization P , we compute a solution to the
minimization problem
min
x∈Rd(V +F )
||Ax − ˙Pold||2,
which can, for instance, be solved by computing the Moore-Penrose pseudoinverse
of A, which provides a minimum norm least squares solution [5, Prop. 7.2.1]. This
approach guarantees that we pick the closest subsequent non-trivial first-order flex
and that our deformation path will be as smooth as possible.
Finally, algebraic constraint sets are distinct from smooth manifolds by having
the potential to contain singularities. In our setting, such points can be charac-
terized by the rigidity matrix dropping rank. They notoriously pose issues for
smooth approximation approaches. Nevertheless, homotopy continuation schemes
come with techniques such as the singular endgame to approach singular solutions
(cf. [24, §10]). Conversely, escaping singularities poses issues even for such schemes,
although this ability is essential for our purposes. To tackle this problem, we take
inspiration from Holmes-Cerfon, Theran and Gortler [17], in which they describe
an acceleration-based method to escape singularities by keeping track of a local, or-
thogonal frame along the deformation path. This information allows us to reliably
traverse nodal-like singularities and to change direction in cusp-like singularities.
All of these individual techniques for approximating deformation paths has been
implemented in the Julia package DeformationPaths.jl [3], where all Archi- MW: Can we put
the footnote in the
references? MH:
Done.
medean and Catalan solids that are discussed in this article are provided as test
24 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
sets. The corresponding animations of the flexible polytopes are provided as sup-
plementary material to this article.
MW: What is missing here is a transition to the results sections. I have no place to put general
thoughts about the tables but the introduction. And it could also explain the place of Section 10.
I don’t know what to do right now. MH: Maybe we can use Table 1 as a hook for the results
section? Either way, I would write the segue that you are asking for in the beginning of Section 9.
9. Results: The regular dodecahedron
In this section we show what tools are available to move beyond statements about
generic rigidity. Among the classically best known polyhedra, the Platonic solids,
only for one of them the question of rigidity is not immediately clear. The regular
tetrahedron, octahedron and icosahedron are simplicial, hence rigid; the cube is a
zonotope, hence flexible. It remains to check the regular dodecahedron. SolvingMH: Refer to Table
1 the system of first-order conditions, we find that there exists a 5-dimensional space
of non-trivial first-order flexes.
9.1. Rigidity. By symbolically computing the space of non-trivial first-order flexes
and stresses associated with the regular dodecahedron, we find that their dimension
is five.1 Consequently, the regular dodecahedron is not first-order rigid.
We still intend to show that the regular dodecahedron is rigid through an alge-
braic computation reliant on Gröbner bases. In Section 6, we introduce a sufficient
condition for the rigidity of a polytope called second-order rigidity. Proposition 7.2
asserts that computing the zeros of a certain polynomial system lets us certify this
property. For that reason, we employ the following strategy:
(i) Compute a basis of the space of non-trivial first-order flexes ( ˙P1, . . . , ˙P5)MW: Here it be-
comes visible that
there are equally
many fo-flexes and
stresses. Do we want
to leave this uncom-
mented? Because
the section that ex-
plained this was just
removed.MH: Do
we comment on this
in the last paper? I
think this is a nice
property. I don’t
think this is the place
to mention it though.
and a basis of the space of equilibrium stresses (ξ1, . . . , ξ5). We parametrize
these basis via variables λ1, . . . , λ5 and μ1, . . . , μ5, respectively.
(ii) From the stress energy E ˙P,ξ(λ, μ), we extract the polynomial system
∇μE ˙P,ξ(λ) = (Q1(λ), . . . , Q5(λ)) = 0
consisting of quadrics Qi (see Section 7).
(iii) Employ Lemma 7.1 to show that this system has finitely many zeros.
(iv ) According to Proposition 7.2, this implies that the regular dodecahedron is
second-order rigid.
The Gröbner basis for the ideal I = ⟨Q1, . . . , Q5⟩ in the lexicographic order-
ing consists of 31 polynomials and is provided in the supplementary material.
Lemma 7.1 implies that V(I) has only finitely many complex roots and, there-
fore, finitely many real roots. The ideal is generated by homogeneous polynomials,
so the only real solution is λ1 = λ2 = · · · = λ5 = 0. As a result, every possi-
ble non-zero linear combination of the generators ˙P1, . . . , ˙P5 has a blocking stress.
Consequently, the regular dodecahedron is second-order rigid and therefore rigid.
We have proved the following theorem:
Theorem 9.1. The regular dodecahedron is rigid.
Proof. By Lemma 7.1, the set of polynomials {Q1, . . . , Q5} only has finitely many
common zeros (see Appendix B). Since the system is homogeneous, the only solution
1The specific embedding, computations, ordering of vertices, edges, and facets are all provided
as Mathematica code in the Supplementary Material.
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 25
is y1 = y2 = ... = y5 = 0. As a result, for any nonzero ˙P generated by the five
non-trivial first-order flexes, we can find a stress so that inequality (6.5) holds. By
Theorem 6.3, P is second-order rigid. By Theorem 4.3, P then is rigid. □
Remark 9.2. Using analogous techniques to Theorem 9.1, we can show that the
truncated icosahedron is also second-order rigid (cf. Table 1).
Remark 9.3. For the truncated dodecahedron, the system of homogeneous qua-
dratic equations introduced in Section 7 has a non-trivial solution. According to
Theorem 6.3, this implies that the Truncated dodecahedron is not second-order
rigid. In fact, we find that almost no first-order flex is blocked by an equilibrium
stress in this polytope. Still, with our current tools we are not able to distinguish,
whether it is flexible or rigid. MW: The section
below does not re-
ally “perturb” edge
lengths in the sense
how we used the
word before, but
changes them system-
atically and globally.
Do we have a better
name for the section
... I am still thinking
...
9.2. Systematic modification of edge lengths. Although Theorem 9.1 shows
that when fixing its edge lengths, the dodecahedron with combinatorial type P is
rigid, its realization space real(P) is a smooth 36-dimensional manifold due to the
Legendre-Steinitz Theorem. According to Section 5 we can say more: Its reduced
realization space real∗(P) is a smooth 30-dimensional manifold. In Question 5.9
we formulate the hope that for rigid polytopes, all edge length perturbations are
realizable (cf. Definition 5.1). It is completely unclear, whether this claim is true.
To gain a better understanding of what the claim means, we are going to in-
vestigate in this section how deformations of the regular dodecahedron induced by
altering a single edge length behave. By the polytope’s regularity, all edges are
combinatorially identical. It does not matter which edge is chosen. For this exam-
ple, we keep all but one edge length constant at ℓ = 1 throughout the deformation.
Denote the non-constant edge length by ℓ∗(t) = 1 + t with t ∈ (−δ, +δ) for some
δ > 0 such that |δ|< 1. Sampling from the realization space intersected with the
real algebraic set generated by the edge length equations reveals that there are six
distinct curves through the regular dodecahedron corresponding to the contraction
of a single edge length (see also [2]) and two corresponding to its expansion. All
eight configurations at ℓ⋆(±0.25) are depicted in Figure 5.
It turns out that in the case of edge length contractions there are two types
of configurations: Those mitigating the edge contraction by deforming vertically
(see Figure 5 (top)) and those that deforming horizontally (see Figure 5 (bottom)).
Both types contain one configuration with two mirror axes and two configurations
with one reflection symmetry that are mutual mirror images. Intriguingly, not all
dodecahedra persist until the edge collapses. The configurations in the bottom
left and bottom right are confluent with the configuration in the bottom center at
≈ ℓ⋆(−0.37194 . . . ), leaving only four configurations beyond this particular edge
length. All of them persist until ℓ∗(−1) = 0. MW: Discuss the
fact that the orange
branches meet again:
the two branches of
the loop have oppo-
site symmetries, and
must therefore pass
through a common
symmetrization to
connect to each other
Conversely, expanding an edge only produces two configurations that both have
distinct distinct reflection axes. They are depicted on the sides of Figure 5. There is
no indication that there exists a maximal edge length beyond which no realizations
exist. Despite the dodecahedron’s high level of regularity and symmetry, there
are more deformation paths for contracting an edge than for expanding it. This
behavior is surprising and should be the object of further investigation.
In Figure 5, we also depict the deformation paths corresponding to these eight
realizations, which are induced by edge contractions (blue) and expansions (gray).
Remarkably, it appears that some of these curves can be matched smoothly. As
26 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
Figure 5. Realizations obtained by perturbing a single edge of the reg-
ular dodecahedron (the central blue circle). Blue curves correspond to
edge constractions, whereas gray curves correspond to edge expansions.
On the curves, the eight corresponding realizations at ℓ∗(±0.25) are de-
picted.
the gray curves correspond to an edge expansion, they have the same tangent in
the regular dodecahedron. The deformation paths corresponding to the four low-
symmetry realizations can be combined to form a nodal cubic curve. In particular,
the regular dodecahedron is a singularity in the corresponding edge length realiza-
tion space. Two symmetric deformations remain, which also share the same tangent
in the regular dodecahedron. In total, four smooth curves are passing through the
regular dodecahedron that are parametrized by edge perturbations. Numerically
computing the derivative in the regular dodecahedron confirms this observation:
though naturally, we expect that our numerical calculations are not exact, the re-
spective tangents’ sum is sufficiently close to zero. Finally, we attach an animation
of a smooth deformation path passing through the regular dodecahedron induced
by an edge expansion from ℓ∗(−0.25) to ℓ∗(0) followed by a compatible contraction
from ℓ∗(0) to ℓ∗(−0.25) in the supplementary material of this article.
9.3. Global rigidity. The results of Section 9.2 give us insight into the concept
of global rigidity for convex polytopes. Recall that a polytopes is called globally
rigid if there exists no other realization of the polytope with the same edge lengths.
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 27
Clearly, the realizations shown in Figure 5 (say, on the blue curve) are equivalent,
that is, have identical edge lengths. None of them is therefore globally rigid.
One may therefore ponder the escape of generic global rigidity [9]: a polytope is
called generically globally rigid if at least every generic realization is globally rigid. MW: Generic un-
defined. We men-
tion it already earlier,
but never define it I
think. MH: We de-
fine it intuitively on
page 15
However, consider a small generic perturbation P ′ of one of the realizations shown
in Figure 5. Since all the shown equivalent realizations are first-order rigid (verified
numerically), they can be perturbed to attain the same edge lengths as P ′ (using
Proposition 5.4). Hence, also generic realizations are not necessarily globally rigid.
Interestingly, the most concrete case remains open:
Question 9.4. Is the regular dodecahedron globally rigid? That is, does there
exist a convex realization of the dodecahedron with all edges of the same length,
besides the regular dodecahedron?
It would be surprising, though also not absurd, that other realizations with equal
edge lengths exist. Consider, for example, the near miss shown in Figure 6, whose
edge lengths are almost all equal. Or consider the “flat dodecahedron” shown in
Figure 7.
Figure 6. The regular dodecahedron (left) and another realization,
known as “Pyritohedron”, with all edges almost of the same length
(right). The colored edges have a slightly different length from the black
edges.
Figure 7. A 2-dimensional straight-line drawing of the dodecahedral
graph with all edge of the same lengths. The figure is a reproduction of
a result by, and is courtesy to, Bob Connelly and Simon Guest.
28 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
10. Dimension of first-order flex-spaces
The goal of this section is to explain some of the experimentally observed dimen-
sion values of the first-order flex space in Table 1 and 2 and draw conclusions from
their values. For this we revisit the constructions for flexible polytopes introduced
in [4, Section 4].
Recall that mreal∗(P, P ) is a semi-algebraic set. At regular points (i.e., where
the space is smooth), the first-order flex space can be understood as the tangent
space to mreal∗(P, P ), and hence, their (local) dimensions agree. At non-regular
points the relation is more complicated. The strategy in this section is to derive
lower bounds on the dimension of the first-order flex space by constructing sub-
manifolds M ⊆ mreal∗(P, P ).
10.1. Generic Minkowski sums. Given polytopes P1, ..., Pm ⊂ Rd, m ≥ 2 in
general orientation relative to each other, their Minkowski sum
P := P1 + · · · + Pm
is a flexible polytope for which we can distinguish two types of flexes:
(i) summand flexes result from one of the summands Pi being flexible.
(ii) reorientation flexes result from a relative reorientation of the summands.
These exist even if all summands are rigid.
Both types of flexes are called Minkowski flexes (as introduced in [4, Section 4.1]).
The assumption that the summands are in general position is necessary, since co-
incidental coplanarities of faces between the summands can prevent both types of
flexes to exist. As a consequence, mreal∗(P, P ) contains a copy of
mreal∗(P1, P1) × · · · × mreal∗(Pm, Pm) × RelO,
where RelO is a smooth open manifold that parametrizes the generic relative orien-
tations of the summands whose Minkowski sum is combinatorially equivalent to P .
Several polytopes in Table 1 and 2 are generic Minkowski sums (marked with ✿).
This includes
• the cuboctahedron, which is the generic Minkowski sum of two simplices,
each of which is rigid.
• the rhombicuboctahedron, which is the generic Minkowski sum of a cube
and an octahedron. The octahedron is (first-order) rigid. The cube has a
3-dimensional space of first-order flexes, all of which get inherited by the
Minkowski sum as summand flexes.
• the rhombicosidodecahedron, which is the generic Minkowski sum of a do-
decahedron and an icosahedron. Both summands are rigid, but the do-
decahedron has a 5-dimensional space of first-order flexes, which too get
inherited by the Minkowski sum (cf. Section 4).
The polytopes marked with ✣ ✿ are further examples. They are generic zonotopes
and will be discussed separately in Section 10.3.
All of the above polytopes are generic Minkowski sums of two full-dimensional
polytope. Hence, the relative orientations of their summands can be parametrized
by orthogonal transformations. That is, RelO is an open subset of O(R3) and pro-
vides three dimensions of reorientation flexes. Remarkably, in all three cases the
dimension of the first-order flex space matches the lower bound we get from the
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 29
above discussion. As a consequence we find that, locally at their respective realiza-
tions, the Minkowski flexes are the only flexes for these polytopes.
10.2. Zonotopes. A zonotope Z ⊂ Rd is a Minkowski sum of finitely many line seg-
ment. A flex of Z that consists of zonotopes throughout is called a zonotope flex .
Such are entirely described by a continuous reorientation of the generating line seg-
ments. Note that such a reorientation needs to respect the linear dependencies
between the segments in order to preserve the combinatorial type of the zonotope.
It was proven in [4, Section 4.2] that zonotope flexes do always exist: the group
GL(Rd) can be thought of as acting on mreal(Z, Z) by changing the orientations
of the generating line segments, while preserving linear dependencies and the line
segments’ lengths. Since GL(Rd) is a Lie group, this action is smooth and generates
flexes that we call linear zonotope flexes.
Let Con(Rd) ⊂ GL(Rd) be the subgroup of conformal transformations, i.e., scalar
multiples of orthogonal transformations. Suppose that the line arrangement of Z
is essential , i.e., there are no proper subspaces U1, ..., Ur ⊂ Rd with dim U1 + · · · +
dim Ur = d that contain all line segments. One can check that Con(Rd) is precisely
the stabilizer of Z in mreal∗(Z, Z). In consequence, the action of GL(Rd) generates
a submanifold M ⊆ mreal∗(Z, Z) of dimension
dim GL(Rd) − dim Con(Rd) = d2 − d
2
 + 1 = d+1
2
 − 1.
For d = 3 this implies that mreal∗(Z, Z) contains a submanifold of dimension4
2
−1 = 5. The zonotopes in Table 1 and 2 are marked with ✣. With the exception
of the cube, all of them have essential arrangement, and hence have a space of first-
order flexes of dimension at least five. Remarkably, four of them also attain the
bound with equality:
• the rhombic dodecahedron (from Table 2)
• the truncated octahedron (aka the permutahedron)
• the truncated cuboctahedron
• the truncated icosidodecahedron
As a consequence, locally at their respective realizations, the linear zonotope flexes
are the only flexes of these polytopes.
The rhombic dodecahedron is a generic zonotope (marked with ✣ ✿) and its di-
mension match will be explained in Section 10.3. The other three zonotopes also
share a property that is potentially relevant: let Z be any of these zonotopes, then
the matroid M(Z) of its line arrangement is linearly unique. This means that M(Z)
has a unique linear realization up to linear transformation (and scalar multiplication
of the vectors). This already implies that all zonotope flexes are necessarily linear
zonotope flexes. But we currently have no understanding for why all flexes of these
zonotopes should (locally) be zonotope flexes in the first place. This is not neces-
sary: for example, the hexagonal prism is a zonotope with a non-zonotopal flex.
Question 10.1. Given a zonotope Z, when are all its flexes zonotope flexes? Is this
true if M(Z) is linearly unique? More precisely, if M(Z) is linearly unique and es-
sential, do we have mreal∗(Z, Z) ≃ GL(Rd)/ Con(Rd) ≃ SPD∗(Rd)?
Here SPD∗(Rd) is the space of symmetric positive definite matrices with deter-
minant one. The isomorphism is obtain via GL(Rd) ∋ M 7 → M ⊤M .
30 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
10.3. Generic zonotopes. A generic zonotope is a generic Minkowski sum of line
segments. It is both a zonotope (Section 10.2) and a generic Minkowski sum (Sec-
tion 10.1). Table 1 and 2 contain three of them marked with ✣ ✿. These are the
following (m being the number of line segments):
• the cube (m = 3),
• the rhombic dodecahedron (m = 4) (Table 2), and
• the rhombic triacontahedron (m = 6) (Table 2).
Their Minkowski summands, i.e., the line segments, are clearly rigid and there are
no summand flexes. Moreover, the dimension of RelO can be computed exactly
by constraining the line segments so as to get rid of all isometries: restrict each line
segment to be centered at the origin, and for k ∈ {1, ..., d − 1} (assuming m ≥ d),
restrict the k-th line segment to lie in a fixed k-dimensional subspace. It has then
k degrees of freedom. Summing up the degrees of freedom, we obtain
dim RelO = 0 + 1 + · · · + (d − 1) +
m−d
z }| {
(d − 1) + · · · + (d − 1)
= (d − 1)m −
d
2

.
For d = 3 we obtain dim RelO = 2(m − 2) − 1 = 2m − 3. This matches the di-
mensions of the first-order flex spaces listed in the tables. This can be explained:
Theorem 10.2. If Z ⊂ Rd is a generic zonotope, then mreal∗(Z, Z) ≃ RelO
and all Q ∈ mreal(Z, Z) are zonotopes.
Proof. The case d = 1 is trivial.
If d = 2 then Z is a parallelogram, and the proof is straight-forward as well.
If d > 2, and since Z is generic, all 2-dimensional faces of Z are parallelograms.
If Q ∈ mreal∗(Z, Z), all 2-faces of Q are realizations of 2-faces of Z with the same
edge lengths as in Z. By the case d = 2, they are still parallelograms. Since all
2-faces of Q are parallelograms, Q is itself a generic zonotope.
Since the elements of mreal∗(Z, Z) that are generic zonotopes are exactly
parametrized by RelO, it necessarily covers the entire configuration space. □
Question 10.3. As of now, all flexible convex polytopes that we know are either
zonotopes or generic Minkowski sums. Are these all options or does there exist
another construction for flexible polytopes?
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 31
11. Conclusion
In this article, we develop a second-order rigidity theory for polytopes. We
demonstrate in Theorem 6.1 that this criterion is sufficient for the rigidity of poly-
topes. Using equilibrium stresses, we develop an effective algorithm for checking
second-order rigidity in Section 7.
For 3-dimensional polytopes, we also investigate the topological properties of the
realization space real(P) by considering the complement of the metric realization
space mreal(P, P ) inside real(P), which we call the edge length perturbation
space. This lets us generate novel conditions for rigidity (e.g. Proposition 5.4 and
Theorem 5.6).
Moreover, we extend our analysis to flexible polytopes. For zonotopes and
generic Minkowski sums, we provide a lower bound on the dimension of the flex
space. As of now, all flexible convex polytopes that we are able to find arise as
zonotopes or generic Minkowski sums. To approximate the flexes of polytopes,
we develop an algorithm in Section 8, which relies on Riemannian geometry and
homotopy continuation, alongside several useful heuristics.
Using these tools, we characterize the rigidity properties of the five Platonic and
13 Archimedean Solids in Table 1, and of the 13 Catalan Solids in Table 2. Notably,
we demonstrate that the regular dodecahedron and the truncated icosahedron are
second-order rigid, even though they are neither first-order rigid, nor prestress
stable. Therefore, they represent examples of rigid polytopes, for which the first-
order theory is insufficient.
Among these 31 polytopes, the truncated dodecahedron is the only one whose
rigidity we are unable to determine. We are able to show that this polytope’s
space of first-order flexes is four-dimensional, so it is not first-order rigid, and we
demonstrate that it is not second-order rigid. In Figure 8, we show samples from
a flex of the truncated dodecahedron which is constructed using gradient descent
with a reasonable numerical tolerance.
Figure 8. The Archimedean truncated dodecahedron (left) and two of
its potential flexes (middle and right) constructed numerically.
However, when we applied more robust numerical scheme (cf. Section 8) with a
tolerance close to machine precision, all of the realizations from the flex visualized
in Figure 8 converge back to the maximally symmetric truncated dodecahedron.
Therefore, this symmetric flex is likely not a true flex.
Initial experiments using the energy-based approach for higher-order rigidity of
Gortler, Holmes-Cerfon and Theran [14] suggest that the truncated dodecahedron
is instead third-order rigid. However, if the dimension of the space of first-order
32 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
flexes is greater than one, there currently exists no effective algorithm for checking
higher-order rigidity and we would have to solve infinitely many polynomial opti-
mization problems. It is a problem for future research to apply hierarchies from the
polynomial optimization literature (e.g. Lasserre hierarchy) to limit the number
of cases that need to be checked. Solving this issue would lead to an algorith-
mic framework which would be applicable to various geometric constraint systems
across rigidity theory, and not just polytopes.MW: I would say we
don’t need this sec-
tion. Move the prob-
lems to their sections
or mention them in
the introduction.
MH: Open prob-
lems only belong into
the introduction if
(a) we solve them or
(b) they are guiding
problems that moti-
vate our article. Nei-
ther is the case. We
should move them to
the respective sec-
tions instead (which I
did).
MW: Universality ...
?
Funding. Martin Winter was supported as Dirichlet Fellow by the Berlin Mathe-
matics Research Center MATH+ and the Berlin Mathematical School, funded by
the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under
Germany’s Excellence Strategy (EXC-2046/1, project ID 390685689), and further-
more by the SPP 2458 “Combinatorial Synergies” (project ID 539851419), funded
by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation).
Acknowledgements. Louis Theran, Bob Connelly, Simon Guest, Bernd Schulze...
TODO
References
[1] T. G. Abbott. Generalizations of Kempe’s Universality Theorem. Master’s thesis, Mas-
sachusetts Institute of Technology, 2008.
[2] M. Adrian-Himmelmann. Approximating continuous motions of geometric constraint systems,
2026.
[3] M. Adrian-Himmelmann. matthiashimmelmann/deformationpaths.jl: Release 1.1.0. Zenodo,
2026. https://doi.org/10.5281/zenodo.19830468.
[4] M. Adrian-Himmelmann, B. Schulze, and M. Winter. Rigidity of polytopes with edge length
and coplanarity constraints. International Mathematics Research Notices, 2026(7), 2026.
[5] G. Allaire and S. M. Kaber. Numerical Linear Algebra. Texts in Applied Mathematics Vol.
55. Springer Science & Business Media, 2008.
[6] L. Asimow and B. Roth. The Rigidity of Graphs I. Transactions of the American Mathemat-
ical Society, 245:279–289, 1978.
[7] N. Boumal. An Introduction to Optimization on Smooth Manifolds. Cambridge University
Press, 2023.
[8] L. E. Brouwer. Beweis der invarianz des n-dimensionalen gebiets. Mathematische Annalen,
71:305–313, 1912.
[9] R. Connelly. Generic global rigidity. Discrete & Computational Geometry, 33, 2005.
[10] R. Connelly and W. Whiteley. Second-order rigidity and prestress stability for tensegrity
frameworks. SIAM Journal on Discrete Mathematics, 9(3):453–491, 1996.
[11] D. Cox, J. Little, and D. O’Shea. Ideals, varieties, and algorithms. An introduction to compu-
tational algebraic geometry and commutative algebra. Undergraduate Texts in Mathematics.
Springer, 4th edition, 2015.
[12] M. Dehn. Über die Starrheit konvexer Polyeder. Mathematische Annalen, 77, 1916.
[13] J. Draisma, E. Horobeţ, G. Ottaviani, B. Sturmfels, and R. R. Thomas. The euclidean dis-
tance degree of an algebraic variety. Foundations of Computational Mathematics, 16(1), 2016.
[14] S. J. Gortler, M. Holmes-Cerfon, and L. Theran. Higher order rigidity and energy, 2025.
[15] R. Hartshorne. Algebraic Geometry, volume 52 of Springer Graduate Texts in Mathematics.
Springer Science & Business Media, 1 edition, 1977.
[16] A. Heaton and M. Himmelmann. Computing Euclidean distance and maximum likelihood
retraction maps for constrained optimization. Computational Geometry, 126, 2025.
[17] M. Holmes-Cerfon, L. Theran, and S. J. Gortler. Almost-rigidity of frameworks. Communi-
cations on Pure and Applied Mathematics, 74(10):2185–2247, 2021.
[18] S. Lang. Fundamentals of Differential Geometry. Graduate Texts in Mathematics. Springer,
1999.
[19] J. M. Lee. Introduction to Smooth Manifolds, volume 218 of Graduate Texts in Mathematics.
Springer New York, 2 edition, 2012.
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 33
[20] L. Lovász. Semidefinite Programs and Combinatorial Optimization, pages 137–194. Springer
New York, New York, NY, 2003.
[21] J. Nocedal and S. Wright. Numerical Optimization. Springer Series in Operations Research
and Financial Engineering. Springer New York, 2nd edition, 2006.
[22] I. Pak. Lectures on discrete and polyhedral geometry, 2010. Manuscript. http://www.math.
ucla.edu/~pak/book.htm.
[23] L. Rastanawi, R. Sinn, and G. M. Ziegler. On the dimensions of the realization spaces of
polytopes. Mathematika, 67(2):342–365, 2021.
[24] A. Sommese and C. Wampler. The Numerical Solution of Systems of Polynomials Arising
in Engineering and Science. World Scientific, 2005.
[25] A. H. Wallace. Algebraic approximation of curves. Canadian Journal of Mathematics, 10:242–
278, 1958.
[26] G. M. Ziegler. Lectures on polytopes, volume 152. Springer Science & Business Media, 2012.
34 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
Appendix A. Rigidity Properties of the Catalan Solids
▲
Triakis Tetrahedron
(✓, ✓, ✓, ✓, 0)
✣ ✿
Rhombic Dodecahedron
(✗, ✗, ✗, ✗, 5) ▲
Triakis Octahedron
(✓, ✓, ✓, ✓, 0)
▲
Tetrakis Hexahedron
(✓, ✓, ✓, ✓, 0)
Deltoidal Icositetrahedron
(✓, ✓, ✓, ✓, 0)
▲
Disdyakis Dodecahedron
(✓, ✓, ✓, ✓, 0)
Pentagonal Icositetrahedron
(✓, ✓, ✓, ✓, 0)
✣ ✿
Rhombic Triacontahedron
(✗, ✗, ✗, ✗, 9) ▲
Triakis Icosahedron
(✓, ✓, ✓, ✓, 0)
▲
Pentakis Dodecahedron
(✓, ✓, ✓, ✓, 0)
Deltoidal Hexecontahedron
(✓, ✓, ✓, ✓, 0)
▲
Disdyakis Triacontahedron
(✓, ✓, ✓, ✓, 0)
Pentagonal Hexecontahedron
(✓, ✓, ✓, ✓, 0)
Table 2. The rigidity properties of the 13 Catalan solids grouped by the
polytopes’ symmetry. In addition, the polytopes are sorted according
to the position of their dual Archimedean solid in Table 1. The 5-
tuple in each cell represents the following properties: (first-order rigidity,
prestress stability, second-order rigidity, rigidity, number of flexes).
SECOND-ORDER RIGIDITY AND REALIZATION SPACES OF POLYTOPES 35
Appendix B. Computational data for dodecahedron
Let ϕ be the golden ratio, 1
2 (1 + √5). We use the following coordinates for the
20 vertices:
p1 = (1, 1, 1) p2 = (1, 1, −1) p3 = (1, −1, 1) p4 = (1, −1, −1)
p5 = (−1, 1, 1) p6 = (−1, 1, −1) p7 = (−1, −1, 1) p8 = (−1, −1, −1)
p9 = (0, ϕ, 1
ϕ ) p10 = ( 1
ϕ , 0, ϕ) p11 = (ϕ, 1
ϕ , 0) p12 = (0, ϕ, −1
ϕ )
p13 = ( −1
ϕ , 0, ϕ) p14 = (ϕ, −1
ϕ , 0) p15 = (0, −ϕ, 1
ϕ ) p16 = ( 1
ϕ , 0, −ϕ)
p17 = (−ϕ, 1
ϕ , 0) p18 = (0, −ϕ, −1
ϕ ) p19 = ( −1
ϕ , 0, −ϕ) p20 = (−ϕ, −1
ϕ , 0)
The edge set E is given by the following pairs of vertices:
(1, 9) (1, 11) (2, 11) (2, 12) (9, 12) (1, 10)
(5, 9) (5, 13) (10, 13) (8, 20) (17, 20) (6, 17)
(6, 19) (8, 19) (7, 13) (5, 17) (7, 20) (4, 18)
(4, 14) (3, 14) (3, 15) (15, 18) (6, 12) (16, 19)
(2, 16) (4, 16) (11, 14) (3, 10) (7, 15) (8, 18)
From this information, one can recover the facets and the coordinates of the
normal vectors. Our specific computation uses the following vertex ordering for the
12 facets:
f1 : (1, 9, 5, 13, 10) f2 : (1, 9, 12, 2, 11) f3 : (1, 10, 3, 14, 11)
f4 : (2, 11, 14, 4, 16) f5 : (2, 12, 6, 19, 16) f6 : (3, 10, 13, 7, 15)
f7 : (3, 14, 4, 18, 15) f8 : (4, 16, 19, 8, 18) f9 : (5, 9, 12, 6, 17)
f10 : (5, 13, 7, 20, 17) f11 : (6, 17, 20, 8, 19) f12 : (7, 15, 18, 8, 20)
Symbolic expressions for a basis ( ˙P1, . . . , ˙P5) of nontrivial infinitessimal flexes
are provided in the supplementary file Dodecahedron/symbolicInfVFMatrix.mx,
whereas symbolic expressions for a basis (ξ1, . . . , ξ5) of the corresponding equilib-
rium stresses are provided in Dodecahedron/symbolicStrVFMatrix.mx. By ex-
ecuting the Mathematica notebook Dodecahedron/DodecahedronRigidity.nb,
one can first check that the dodecahedron is not prestress stable. Subsequently,
the polynomials Qi from the stress energy E ˙P,ξ are computed from parametrized
expressions for the nontrivial first-order flexes and equilibrium stresses (see Sec-
tion 7). The Gröbner basis G of the homogeneous ideal I = ⟨Q1, . . . , Q5⟩ for the
lexicographic monomial order has 31 elements. As y6
5 , y5
4 , y3
3 , y3
2 , y2
1 appear as
leading monomials in G, Lemma 7.1 implies that I is zero-dimensional. Since the
ideal I is also homogeneous, Proposition 7.2 thus implies that the dodecahedron is
second-order rigid, as asserted in Theorem 9.1.
Remark B.1. Analogously, we show that the truncated icosahedron is second-
order rigid. The corresponding computation is performed in the Mathematica
notebook TruncIco/TICORigidity.nb. For the truncated dodecahedron, we can
show that it is not second-order rigid using similar techniques. It has a four-
dimensional space of first-order flexes and equilibrium stresses. In the Mathe-
matica notebook TruncDod/TDODRigidity.nb, we show that the polynomial ideal
⟨Q1, Q2, Q3, Q4⟩ is positive-dimensional, as it is homogeneous and has nontrivial
solutions.
36 M. ADRIAN-HIMMELMANN, M. WINTER, AND Z. ZHANG
Institut für Analysis und Algebra, Technische Universität Braunschweig, Univer-
sitätsplatz 2, Germany
Email address: matthias.himmelmann@tu-braunschweig.de
Nonlinear Algebra Group, Max-Planck-Institute for Mathematics in the Sci-
ences, Leipzig, Germany
Email address: martin.winter@mis.mpg.de
Yau Mathematical Sciences Center, Tsinghua University, University, Haidian Dis-
trict, Beijing, China
Email address: zz628@tsinghua.edu.cn

==> sec/introduction_-_copy_-_2026-06-11.tex <==

%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}

\todo{\mhsays{Abstract: Replace at least one of the ``we'' alliterations by a different beginning. Fix overful. \mwsays{Will do.} }}


\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities (\ie\ it is flexible) or not (\ie\ it is rigid).
%. The major difference to the classical setting of polyhedral rigidity is that these deformations are explicitly 
These assump\-tions are weak in comparison to classical polyhedral rigidity, which also enforces fixed face shapes. %\todo{\mhsays{I don't understand this sentence.}\mwsays{Sorry, what exactly is unclear?}\mhsays{I understand what you want to say here, but ``weak'' is always slightly confusing to me as a non-logician. Maybe ``are more restrictive'' or ``are implied by the flexibility in classical polyhedral rigidity''?}}%\todo{\mhsays{Should we highlight rigidity in the first sentence of the introduction, too? Currently it is only about flexibility.}}
While flexible polytopes exist in this setting, still only few techniques are known to construct such. %polytopes that admit such deformations.%\mhsays{and which polytopes do not admit continuous deformations? (to highlight rigidity and not just flexibility.)}.

\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}

As a consequence, the sentiment arose that this sort of flexibility is exceptional, not only among combinatorial types of polytopes, but also among realizations of a fixed type.
%Only few classes of flexible polytopes are known, constructed from a handful of techniques such as Minkowski sums and affine transformations.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that in dimension~at~least three, a \textit{generic} convex polytope of a given combinatorial type is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

%\mwsays{Add picture with Dod, TDod, TIco}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
%     \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically. \mhsays{Suggestion: Move to Conclusion and replace image by truncated dodecahedron, dodecahedron and truncated icosahedron, since they are special.}}
%     \label{fig:TDod_flex}
% \end{figure}

%\todo{\mhsays{I do not think anymore that the first page is a good place for a flex, for which we have strong evidence against being a true polyhedral flex. This may generate false expectations. I would prefer putting it in the conclusion/outlook as future work and focusing on the examples that we can actually solve.}}
Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
%The previous exploration therefore focused on first-order and generic rigidity.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques. %, such as a naive Gröbner basis approach. %, and so it remains unknown whether they are rigid or admit continuous deformations.
This already holds for polytopes with realtively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes the formulation of a suitable second-order theory, \todo{\mwsays{As I understand section 7, we do not develop new tracing tools here}\mhsays{Technically no, but also yes.}\mwsays{I write: we use/generalize what exists.}}as well as computational tools for tracing deformation paths.
For a demonstration we apply these techniques to the Platonic, Archimedean and Catalan solids, deciding their rigidity in all but one case (see \cref{tab:comparison}). In particular,\nls we~decide the previously unknown rigidity properties of the regular dodecahedron.
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be characterized by our techniques. 
Solving this question  will require techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
%
We found it remarkable that such variety of rigidity behaviors can already be observed among classical examples.
%This is not for lack of computations resources, but rather 
%In particular the truncated dodecahedron can serve a surprisingly simple test case for future theoretical and computational developments.
%Merely the \emph{truncated dodecahedron} (see \cref{fig:TDod_flex}, left) evades our approaches. The reason though is interesting, and is of a technical nature rather than from computational limitations.


% \mwsays{The first article develops first- and generic theory. In this article we address notions of rigidity skipped over in the first part: second-order, continuous and global.}

This article divides into theoretical, methodological and experimental results,
of which we give an overview below.\todo{\mhsays{We can also leave the introduction out or replace it by Table 1/2. The structure of our paper may be slightly confusing and this is an attempt at making the structure clearer. I am \textit{very} open to suggestions here on how to organize the roadmap.}\mwsays{Let's decide this at the end.}}

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (10.25,-2) {Chapter 5};

\node[fill=white] (c6) at (12,2)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,2)  {Chapter 7};

\node[fill=white] (c9) at (20.2,0) {Chapter 9};
% Nodes
\node[
    draw=blue!30,
    fill=blue!20,
    rounded corners,
    fit=(c3)(c6)(c5),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=red!30,
    fill=red!20,
    rounded corners,
    fit=(c7)(c8),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=green!30,
    fill=green!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (intro) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{appendix:comp-data-dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (10.25,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,2)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,2)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.2,0) {\Cref{sec:dodecahedron}};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (c9);

\draw[->,dashed] (c10) to[bend left=-5] (intro);
\draw[->,dashed] (app) -- (c9);
\draw[->,dashed] (c9) -- (intro);
\end{tikzpicture}
\end{figure}
\vspace*{-1.65em}
}

\subsection{Theoretical results}
\label{sec:intro-theory}

% The main theoretical contributions are a careful deve\-lop\-ment of the first- and second-order theory of polytope rigidity, as well as %an~application of the former to so-called 
% the creation of dual certificates based on which perturbations of a 3-dimensional polytope's edge lengths can be realized.
% %edge length perturbations for 3-dimensional polytopes.

In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions/flexes,\nls and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory}~we develop the second-order theory for polytope rigidity.
We provide analogues~for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
%including notions of second-order motions and flexes.
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cref{res:sotest}).
%This allows us to define prestress stability for polytopes.
%
%\notodo{\mwsays{We need results to reference on the arrows.}}

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated from the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to rigidity and first-order rigidity.


% In \cref{section:edge-length-perturbations} we apply first-order theory to study polytope realization spaces, motivated from the following train of thought:
% the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo rigid motions is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
% This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.
% If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same edge lengths. 
% This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}.
%In \cref{section:edge-length-perturbations} we provide an interpretation of these degrees of freedom for first-order rigid polytopes by perturbing their edge lengths.



\iffalse % old text, maybe still useful

We subsequently apply the first-order theory to questions of realizability:
given a combinatorial type $\mathcal P$, one may ask whether there exists a realization $P\subset\RR^d$ with prescribed edge lengths $\ell_e$, $e\in E$.
In general, this question is very hard.
In \cref{section:edge-length-perturbations} we explore the connection between rigidity and the existence of so-called \emph{local edge length perturbations} (see \cref{prop:inf-rigidity-edge-perturbations} and
\cref{thm:rigidity-and-edge-length-perturbations}).\nls
In~\cref{sec:dodecahedron-global-rigidity} we use the results to show that some polytopes are \textit{not} generically globally rigid.

\mwsays{
Using this language, we demonstrate that the dodecahedron exhibits a highly interesting algebraic and topological behavior in \Cref{section:dodec-edge-length-perturbations}. We also compute deformation paths associated with perturbing a single edge length using techniques from \Cref{sec:approx_continuous_motions}.}

\mhsays{Add pictures for this section as well}

% We analyze the full realization space of a few examples where this is possible. This includes cubical zonotopes and generic Minkowski sums.

\fi



% We explore the connection between first-order rigidity and the existence of local edge-length perturbations for polytope realizations.


\subsection{Methodological results}
\label{sec:intro-methods}
%\mwsays{More details: numerical, symbolic, ...}
In \cref{section:second-order-rigidity-check}, we describe a method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.% \mwsays{A bit more details? Positivity check ... or something?} 
%
% \mwsays{What about prestress stable?}
% \mhsays{We don't have an effective check for this, so we shouldn't mention it. The PSS method is barely a paragraph in the entire document}

\todo{\mwsays{This needs rephrasing so that it is clear that we just recall this theory. Or we move to appendix. \mhsays{I guess the novel part is that we can apply it to edge length perturbations. However, it holds in greater generality, which is why I describe it like that. I could make that more explicit in the section?}}\mwsays{This is now appendix. Incorporate it into the introduction differently.}}
%
{\color{lightgray}
In \cref{sec:approx_continuous_motions} we describe an algorithm for approximating continuous motions of flexible polytopes based on Riemannian geometry and homotopy continuation. It relies on numerically tracking the solution to the 
optimization problem that searches for the Euclidean closest point to the realization space. We can also apply this method to investigate edge length perturbations of polytopes. %(see \Cref{section:edge-length-perturbations}).% \mwsays{A bit more details?} 
%\mhsays{Mention generalization to realization spaces?}
}


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
%Our newly developed tools allow us to answer questions that have previously been intractable.
%The Archimedean and Catalan solids provided a convenient benchmark. 
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.
All results are displayed in \cref{tab:comparison} and \cref{tab:catalan-comparison} and discussed further in \cref{sec:experimental_results}.
We highlight two results: first, we show that the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left) is second-order rigid, answering the question from \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
Second, we show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and its rigidity status remains open.
Further theoretical background on the observed flex space~di\-mensions is given in \cref{sec:dimension_estimates}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to a case study of the regular dodecahedron.
We demonstrate how to apply our second-order rigidity certificate.
Subsequently we investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations, deformation paths and conclude that it is not generically globally rigid.


\iffalse % old computational results introduction

\newpage

Doing so already enables us to answer questions that were previously intractable.


The results for the five Platonic, 13 Archimedean and 13 Catalan solids are shown in \Cref{sec:archimedean} and reveal a wide range of interesting behaviors.
%The 13 Catalan solids have less surprising rigidity properties and can be found in \cref{tab:catalan-comparison} in \cref{appendix:catalan}.
%The structure of the tables cells is explained in \cref{sec:explain_table}.
We highlight the most noteworthy finding from these experiments here: 
\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and \Def{truncated icosahedron} have identical rigidity properties: they are neither first-order rigid (both have a 5-dimensional~space of first-order flexes), nor prestress stable; yet, \emph{both are second order rigid}.\nls 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct~concepts.
    Previous examples were comparatively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} (\Cref{fig:Dod_TIco_TDod}, right) is not first-order rigid (it has a 4-dimensional space of first-order flexes), not prestress stable and \emph{not second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order,\nls we do not know whether it is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system that demonstrates that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}
\mwsays{Maybe also list the cool fact that most of our lower bounds match the actual flex space dimensions?}\\
%
%\todo{\mwsays{Maybe I move this to dedicated section. Outlook maybe?}}
%\todo{\mhsays{Shorten Introduction to 3 pages?} \mwsays{I will try. Is there a specific reason? Is it bad if it is 3.2 pages?}\mhsays{Not necessarily, but ``in der K\"urze liegt die W\"urze. Just add whatever now you want now and then we shorten during editing.}}
{
\color{lightgray}
%Numerical experiments reveal that all these properties are very sensitive to small changes in the polytope's geometry.
%First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
%Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
%At this time it is unclear why exactly the realizations with uniform edge lengths show low-order flexibility. 
%In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.



%In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
%The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}}
%By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
%We find bifurcating deformation paths and construct from this a counterexample to generic global rigidity for polytopes.

}

\fi



\newpage

\iffalse
{
\color{gray}

Some polytopes turned out first-order rigid without us having an a priori explanation for this.
More remarkable however we found the rigidity properties of the three polytopes marked in \textcolor{orange}{orange} that are \emph{not} first-order rigid:
%
\begin{itemize}
    % \item For all but three Archimedean solids the first-order theory decides the rigidity.
    % If a polytope is first-order rigid, then it is rigid (see \cref{thm:first_order}. All Archimedean solids that were identified as flexible are so via a Minkowski flex and the dimension of the first-order flex space is as expected from this construction. 
    \item
    The \textit{regular dodecahedron} is rigid. This was previously unknown since it is first-order flexible. The second order tools developed in this article allowed to identify the dodecahedron as second-order rigid \emph{but not} prestress stable.
    The regular dodecahedron furthermore becomes first-order rigid after a generic linear transformation. This suggests that the regular realization of the dodecahedron is a singularity in the realization space.
    By computing deformation paths that shrink/extend a single edge of the regular dodecahedron, we probe the neighborhood of this singularity. We find that bifurcating deformation paths and thereby a counterexample to generic global rigidity for polytopes.
    \item 
    The truncated icosahedron (the football) is also first-order flexible yet second-order rigid.
    \item 
    The truncated dodecahedron is flexible in both first- and second order. At this time it is unknown whether it admits a deformation. If it admits a deformation it is the first example of a polytope flex that is no of Minkowski sum type. If it is rigid then it is the first example of a naturally occurring rigidity of order greater than two.
\end{itemize}


\hrulefill

\mwsays{I write ...}

We develop the second-order rigidity theory for polytopes with edge length and coplanarity constraints. 
In addition, we develop computational tools for checking the rigidity of polyhedral surfaces and for approximating continuous motions. 

\mwsays{Regarding caption \cref{tab:comparison}: we should write first-/second-order rigidity instead of the numeric variants, but if I change it the table vanishes completely. Not sure what is going on. Maybe the figure becomes too long for the page?}


% \footnotetext[1]{As a triangulated sphere, this polytope is first-order rigid by Cauchy's rigidity theorem \cite{cauchy1813}.}
% \footnotetext[2]{As a zonotope, this polytope is flexible according to Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.}
% \footnotetext[3]{As a ``generic'' Minkowski sum, this polytope is flexible (\cf\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}).}

\begin{enumerate}[label=\arabic*)]
    \item All Archimedean zonotopes (except for the cube) have 5 inf flexes because they are projectively unique as zonotopes and hence their only transformations come from the 9-dim general linear group minus rotations and global scale. The cube also loses scaling along axis, hence 3 less (but global scale is already contained in here).
    \item The first-order flex spaces of Rhombicuboctahedron and Rhombicosidodecahedron can be explained as the sum of the first-order flex spaces of their constituents + 3-dim rotations. 
\end{enumerate}

\subsection{Dodecahedron and Truncated Icosahedron}
\label{sec:dodecahedron}

The regular dodecahedron and the truncated icosahedron are interesting case studies. They are both first-order flexible and possess a 5-dimensional space of first-order flexes. Nevertheless, using techniques from computational algebra (\cf\ \Cref{section:second-order-rigidity-check}) we show that for each non-trivial flex there exists an equilibrium stress that \emph{blocks} the flex from extending to a continuous motion. In other words, both polytopes are second-order rigid (see \Cref{section:rigidity-of-the-regdod}).

\mwsays{First-order rigid once we apply affine trafo or change the height of truncation.}

\subsection{Truncated Dodecahedron}
\label{sec:truncated_dodecahedron}

The truncated dodecahedron is both first-order and second-order flexible.
More precisely, it has a 4-dimensional space of first-order flexes, which is surprisingly different from the five dimensions that we usually associate with icosahedral symmetry (see \cref{sec:dodecahedron}). % that we found for both dodecahedron and truncated icosahedron.
For second-order rigidity it turns out that none of the first-order flexes is blocked by any stress, so all of them are potentially real. \mhsays{``real'' is not a good word in this context.}
%
Remarkably, we were able to construct a flex numerically!
So far we are not aware of an analytic way to obtain this flex.
Thus, whether this flex is actually real or not remains a mystery. 
In particular, if no such flex is real, there are currently no feasible techniques to prove the rigidity of this polytope.

Interestingly, all first-order flexes of the truncated dodecahedron vanish either on affine transformation or when changing the size of the triangles (keeping it vertex transitive).

The facts listed above suggest that the \emph{uniform} truncated dodecahedron is quite special.
In particular, it seems unlikely that the existence of its flex is a mere coincidence.
More likely, there exists a yet unknown construction, similar to Minkowski sums, that generates this flex.

If flexible, the truncated dodecahedron has some remarkable properties:
%
\begin{itemize}
    \item its flex is not reducible to a Minkowski sum
    \item its affine transformations are not (first-order) flexible.
\end{itemize}
%
In contrast, if it were rigid, this would be remarkable as well. 
It would then be the first example of a polyhedron that is second-order flexible, yet rigid.
The general consensus seems to be that rigidity beyond the second order only appears in contrived constructions specifically made for this purpose.
The truncated dodecahedron, being very natural, would then be an interesting counterexample.

\subsection{Outline}
This article is divided into three main parts: The theoretical foundation in Sections \ref{sec:combinatorics-of-polytopes}--\ref{section:edge-length-perturbations}, followed by methods in Sections \ref{section:second-order-rigidity-check}--\ref{sec:approx_continuous_motions} and a case study on the regular dodecahedron in \Cref{sec:dodecahedron}.

}

\fi










\iffalse % paper roadmap

\newpage

{\color{lightgray}

\begin{itemize}
    \item Introduction (Martin)
    \item Theory part (Martin, fix notation and terminology, stay close to first paper)
    \begin{itemize}
        \item first-order theory
        \item second order theory (prestress stability) 
        \color{lightgray}
        \item construction of flexible polytopes (continuous motions)
        \begin{itemize}
            \item theorem for generic zonotopes
            \item counterexample for general zonotopes (hex prism)
            \item questio for generic Minkowski sums
        \end{itemize}
        \item Edge length perturbation (Matthias)
    \end{itemize}
    \item Methods part
    \begin{itemize}
        \item second-order rigidity check (Gröbner bases, ...) (Albert)
        \item Computing deformation paths (also works for changing edge lengths but we don't mention this here maybe???)  (Matthias)
    \end{itemize}
    \item Case studies (results)
    \begin{itemize}
        \item Dodecahedron
        \begin{itemize}
            \item not first-order rigid (five dim space)
            \item proof of second-order rigid (not prestress stable)
            \item numerical experiments on edge length perturbations and what they might entail (Matthias) 
            \item no global rigidity (Matthias)
        \end{itemize}
        \item Truncated Icosahedron (Matthias + Martin)
        \begin{itemize}
            \item Five first-order flexes
            \item Still second-order rigid
        \end{itemize}
        \item Truncated dodecahedron (Matthias + Martin)
        \begin{itemize}
            \item unclear rigidity
            \item NOT second-order rigid (evidence?)
            \item we believe it is flexible ???
            \item have potential deformation paths
        \end{itemize}
    \end{itemize}
    \item Outlook (Martin)
    \begin{itemize}
        \item (questions about edge-length perturbations -- maybe already in theory part)
        \item is there specific structure in the TDod that helps us to see it is rigid/flexible and construct the flex
        \item Are there general stronger methods for deciding rigidity and constructing deformations
    \end{itemize}
    \item Supplementary material
    \begin{itemize}
        \item computational output (Gröbner bases etc)
        \item Code, algorithms
        \item Animations
    \end{itemize}
\end{itemize}

\newpage % temporary new page

Main results:
\begin{itemize}
    \item carefully define first- and second-order rigidity and prestress stability for this setting.
    \item this gives a strong test for rigidity (resolves previously open cases).
    \begin{itemize}
        \item dodecahedron
        \item truncated icosahedron
        \item checked all Archimedean solids and duals (resolved all but one) 
    \end{itemize}
    \item very interesting special case: truncated dodecahedron (TDod)
    \begin{itemize}
        \item we believe it is flexible (for now)
    \end{itemize}
    \item something about edge length perturbation?
    \item edge length perturbations of the dodecahedron: we find there is a singularity in the ``dual space'' (rigidity transition region is algebraically singular)
    \item dodecahedron is an example that we don't have global rigidity
    \item maybe something about zonotope flexes
\end{itemize}

\hrulefill

\begin{itemize}
    \item many examples of rigidity
    \begin{itemize}
        \item short edges make rigid
        \item higher dimensions + first-order rigidity in higher dimensions
    \end{itemize}
    \item second-order rigidity
    \begin{itemize}
        \item second order rigid implies rigid
        \item Q: does second-order flexibility imply proper flexibility?
        \item $\#stresses=\#flexes$ trivial or worth mentioning?
    \end{itemize}
    \item the dodecahedron example
    \begin{itemize}
        \item affine trafos do not preserve first-order rigidity
        \item there is no global rigidity for polytopes in 3D
    \end{itemize}
    \item many other open questions
    \begin{itemize}
        \item Q: does flexibility need parallel edges?
    \end{itemize}
\end{itemize}

Notes on Archimedean solids:
\begin{itemize}
    \item the only Archimedean solids that are inf-flexible but not generic Minkowski sums are the dodecahedron, truncated dodecahedrona (4 flexes) and truncated icosahedron (5 flexes). Where do we lose the flex on the way from truncated dodecahedron to dodecahedron?
    \item Are they second-order rigid? Can the dimension of their flex spaces and their second-order rigidity be explained in some way using the known properties of the dodecahedron? (Limit argument?)
    \item Are there continuous motions between Archimedean/Catalan/Platonic solids thats preserve the planarity of facets and the edge lengths?
\end{itemize}

Other notes
\begin{itemize}
    \item A zonotope is highly flexible, but is there a zonotope that can flex in more ways than just deforming into other zonotopes, either real or infinitesimally?
    \item If $P$ and $Q$ have first-order flexes, then does $P+Q$ inherit them in some way?
\end{itemize}
\newpage % temporary new page


}

\fi








\newpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and a \Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
%Evidently, every convex polytope $P$ gives rise to such a structure, which we call the combinatorial type of $P$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
%If $\mathcal P$ is the combinatorial type of a convex polytope $P$, this notion agrees with the usual edge graph of $P$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
Convenient for computations, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}
%
% \begin{align*}
% \realSp(\mathcal P)
% %=\realSp(V,F,\sim)
% &:=\left\{\!\!
% \begin{array}{l}
%     \bs p\:V\to\RR^d
%     \\
%     \bs a\:F\to\RR^d
% \end{array}
% \Big\vert
%     \begin{array}{rcl}
%     % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
%     \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,
%     \end{array}
% \!\right\}.
% \end{align*}
%
%Analogously, the \Def{convex realization space} is defined as%\todo{\mhsays{Do we need the convex realization space?}}
%
%\todo{\mwsays{Do we really need both notations? I would like to ditch the one with the subscript c.}\mhsays{We should keep the convex realizations in our assumption right? Or do we build a second-order theory for arbitrary point-hyperplane structures?}\mwsays{I will keep the convex ones and delete the subscript-c.}\mhsays{Do we need convexity for anything in this article?}}
%
\begin{align*}
%\begin{align*}
\real(\mathcal P)
%=\realSp_{\mathrm c}(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
%
%We shall write $P\in\real(\mathcal P)$
%\notodo{\mhsays{What does this sentence add?} \mwsays{Nothing. Removed it.}}
Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ does not allow facet hyperplane to pass~though the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

%\mwsays{Maybe move the below to edge length perturbation section? I think this is the first (and only?) place it is used.}\mhsays{Sure, we can do that. Might even call it configuration space?}

% and the \Def{reduced convex realization space} is defined as
% \begin{align*}
% \realRCvx(\mathcal P)
% :=\realCvx(\mathcal{P})\,/\,\mathrm{Iso}
% \end{align*}
%
%where $\mathrm{Iso}$ is the Lie group of Euclidean isometries of $\mathbb{R}^d$.

%\mwsays{Define $\realR(P)$ reduced realization space?}

%As we show in \Cref{sec:first_order},
%\todo{\mhsays{This is absolutely not clear and we spend quite some time to show that.}\mwsays{I am not sure what you mean. This statement is either trivial or false by \cref{res:new_notion}}\mhsays{How the group action works on $\mathbf{a}$ is only explained in Section 4 and was subtle, so using ``clearly'' here is somewhat dishonest. I would suggest writing something like ``As we show in \Cref{sec:first_order}, the Lie group...}}
The \Def{Lie group of Euclidean isometries} (\ie\ rotations and translations), denoted $\Iso$, acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
%\qquad 
%\realRCvx(\mathcal P)
    %:=\realCvx(\mathcal%{P})\,/\,\mathrm{Iso}
\end{align*}

\iffalse % edge-length measurement map

\todo{\mwsays{This here is not the place for metric stuff. This is what the next section is for. I will move this later}}
\todo{\mhsays{If you want, we can call $\realR$ $\conf$ (the configuration space) instead and use something like $\textsc{M}\conf$ for $\mreal^*$, the metric configuration space.}}
Since in this article we are considering polytopes whose edge lengths are fixed, we also define the \Def{edge-length measurement map} as
\[m_E:\mathbb{R}^{dV}\rightarrow \mathbb{R}^E,\quad m_E(\bs p) = \left(\|p_i-p_j\|^2\right)_{ij\in E},\]
which lets us define the \Def{edge-length realization space}
\[\mreal(\mathcal{P},P)\,=\,\real(\mathcal{P})\,\cap\, m_E^{-1}\left(m_E(\bs p)\right),\]
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are fixed according to the realization $P$. The preimage of a given edge length vector is a real algebraic set, as its given by all realizations which satisfy a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}). \todo{\mhsays{Briefly talk about relation to $g$-rigidity?}}

\fi










% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

%\notodo{\mhsays{Maybe have this as section 2.1 instead? This section is quite short.}\mwsays{Yes, maybe. I think about it.}}
We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.


% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
% \label{def:continuous-rigidity}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
%\todo{\mhsays{Use $\mreal{\mathcal P}$ instead of ``equivalent'' to help distinguish the concepts?} \mwsays{This feels the wrong way around.}}
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, then Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
% \end{definition}

%\mwsays{Define configuration space $\conf$ and reduced configuration space $\conv^*$.}
%\mwsays{Define the \Def{metric realization space} $\mreal(P)$ (and reduced $\mreal^*(P)$) and replace below occurrences of $\conf(P)$ by it.}

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks.
Consequently, much of what we say applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}
%This also applies to the subsequent section, which develop a first- and second-order theory for polytopes, but are applicable more generally.

% Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% %
% A \Def{motion} of $(\bs p,\bs a)$ is a curve $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$;
% the motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% A non-trivial motion is called a \Def{flex}.
% If a realization $(\bs p,\bs a)$ has a flex, then we call it \Def{flexible}, and \Def{rigid} otherwise.

% {\color{lightgray}

% \begin{remark}
%     \mwsays{?? Simulating polytope rigidity via stacking prisms on faces.}
%     \mhsays{I'd say we leave it out.}
% \end{remark}

% }

For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.








\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a rigidity systems studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence provides heuristics and criteria that can be efficiently checked in practice.
%Investigating the first-order properties of a system comes down to the study of its \emph{rigidity matrix}.
%The first-order theory for polytopes is analogous to point-hyperplane frameworks, so the theory developed in this section applies verbatim to the more general case.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
    %\label{fig:placeholder}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from it.
%$p_i$ should be thought of as the coordinate of vertex $i$, and $a_\sigma$ the corresponding vertex of facet $\sigma$ in the polar dual of $P$.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    % \label{eq:flex_at_face}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    % \\
    % \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    % \label{eq:flex_at_face}
\end{align}
%
%\todo{\mwsays{Here we could say that $\bsdot a$ is determined by $\bsdot p$. Then it becomes clearer why trivial only needs to be specified on the $p$-part. This is however only true for our polytope setting and not general point-hyperplane frameworks. So we should be cautious claiming generality.}}
%
Like in the frameworks setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also, that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).

%\todo{\mwsays{Turn the lemma into a short remark, maybe without proof and point to the proof below.}}

\iffalse % lemma that adot determined by pdot

{\color{lightgray}\small
\begin{lemma}
    \label{res:p_determines_a}
    The $\bsdot p$ uniquely determine the $\bsdot a$.
\end{lemma}
%
\begin{proof}
    For fixed $\sigma$ choose a basis $p_{i_1},..., p_{i_d}$ among the $p_i,i\sim \sigma$ (we can always do this in our setup).
    Then $\dot a_\sigma$ is the unique solution of the linear system $\<\dot a_\sigma,p_{i_k}\>=-\<\dot p_{i_k},a_\sigma\>$ for all $k\in\{1,...,d\}$.
\end{proof}
}

\fi % lemma that adot determined by pdot

First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any vertex $i\in V$ and facet $\sigma\in F$}.
    % \label{eq:trivial_motion_facet}
    %\\
    %\<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any $i\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    %\\
    %\<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%\mhsays{Potentially we will need $i\sim \sigma$ in $(4.4)$ as well (analogous to (4.2)). The possible trivial inf motions are already restricted to the Lie algebra of the Euclidean isometries (i.e. infinitesimal rotations and translations) by $(4.3)$ and the normals move automatically in first order alongside the vertices. By restricting the flexes further, we may make the equation impossible to satisfy (see computation below). It should be sufficient to have a complete graph as the 1-skeleton and the normals are immediately determined in first order. I don't mind $(4.5)$, but I don't think it adds much. Also, I don't quite understand where (4.5) comes from.}
%\mwsays{Let's delete (4.4) and (4.5).}
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    %The trivial first-order motions of a $d$-dimensional polytope $P$ form a vector space $\mathcal T_P$ of dimension $\binom{d+1}{2}$. 
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    %By assumption $P$ has non-empty interior, so we can assume that $\bs p$ is affinely spanning.
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    % \mhsays{I think it is necessary to at least show that 4.4 and 4.5 are satisfied to complete the proof. For a trivial motion, it holds that \[\langle S p_i+t,a_\sigma\rangle+\langle p_i,S a_\sigma\rangle= \langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle + \langle a_\sigma,Sp_i\rangle=\langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle - \langle p_i, Sa_\sigma\rangle=\langle t,a_\sigma\rangle\]
    % (for (4.5) this works). Of course, this is an issue, because in general this is $\neq 0$. Instead, we take a diagonal matrix $F(t)\in \mathbb{R}^3$ with positive eigenvalues, which is responsible for scaling ${\bs a}$. We require $\bsdot{a}=F(t)\cdot S \cdot {\bs a}$ and compute according to $(4.4)$
    % \begin{eqnarray*}
    % &~&\langle S p_i+t,a_\sigma\rangle+\langle p_i,F(t)\cdot S\cdot a_\sigma\rangle= \langle t, a_\sigma\rangle + \langle p_i,(F(t)-I)\cdot S \cdot a_\sigma\rangle \overset{!}{=}0\\
    % &\Rightarrow & \left(t+(F(t)-I)\cdot S \cdot p_i\right)\T \cdot a_\sigma=0 \quad\left(\Rightarrow t+(F(t)-I)\cdot S \cdot p_i \perp a_\sigma \right)
    % \end{eqnarray*}
    % for arbitrary choices of $t$ and normals $a_\sigma$; since $P$ is affinely spanning, the normals $a_\sigma$ generate $\mathbb{R}^3$ as a vector space. Therefore, 
    % \begin{eqnarray*}
    % S\cdot F(t)\cdot p_i=S\cdot p_i+t~\Rightarrow ~\underbrace{(F(t)-I)}_{=G(t)}\cdot \left( S\cdot p_i \right) = t
    % \end{eqnarray*}
    % for each $i$, since $S$ is not invertible in odd dimensions. This equation essentially needs to be solved for all points $p$ on the hyperplane $\mathcal{H}_\sigma$ with normal $a_\sigma$ which is spanned by the points $p_i$ with $i\sim \sigma$ (here is the exact point where problems occur when we take into account $(4.4)$, since the hyperplane is not defined and we compute on $\mathbb{R}^3$ instead). This equation is overdetermined. The main question is: why does the result for a specific point on $\mathcal{H}_\sigma$ generalize to all points on $\mathcal{H}_\sigma$??? \\[2mm]
    % For $(4.5)$ it holds that 
    % \[\langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle + \langle a_\tau, F(t)\cdot S \cdot a_\sigma\rangle = \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle - \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle = 0\]
    % due to the skew-symmetry of $S$ and diagonality of $F(t)$.}
        %Hence, $\mathcal T\simeq\mathcal T_F$ and the claim follows.
    %\mhsays{Also, I think we should give an argument that this is indeed a linear space and not an affine-linear space or a union of such spaces; contrary to the bar-joint equations, (4.2) vaguely resembles $Ax=b$. Nevertheless, we now have variables $\dot{a}$ and $\dot{p}$, so we can rewrite Equation (4.2) as $\langle \dot{p}_i\times \dot{a}_\sigma,  a_\sigma\times p_i\rangle=0$, which implies that the space is indeed linear.} \mwsays{I don't understand. The equations are linear so the solution spaces are linear.}
    %\mwsays{We should choose $\dot a_\sigma$ as the solution of $\<\dot a_\sigma, p_i\> = \<Sp_i+t,a_\sigma\> = \<p_i, S a_\sigma\> + \<t,a_\sigma\>$ over all $i\sim\sigma$. Choose a basis among the $p_i,i\sim\sigma$ to get a candidate solution. Then use that all other $p_i$ are in the affine span of this basis and that the equations are affinely covariant and hence do indeed have a solution that works for all $i\sim\sigma$. Then it satisfies (4.2), and we delete (4.4) and (4.5).}
    %
    %It suffices to show that each $\bsdot p\in\mathcal T_F$ extends to a polytopal first-order motion $(\bsdot p,\bsdot a)$.
    %
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}

\iffalse

\todo{\mhsays{Prove that trivial flexes have the correct dimension? Clearly, space of inf flexes is contained in framework inf flexes by construction. Apply Asimow-Roth $\Rightarrow$ ``$\leq$''. Construct Inf flexes: skew-symmetric $Q$, translation $T$; on vertices: $Qp(i)+T$, on normals $Qa(\sigma)$.}}

{\color{lightgray}

\begin{observation}
    If a facet $\sigma\in F$ is a simplex, then the left hand side of \eqref{eq:stress_at_face} is a linear combination of $d$ linearly independent vectors in $\RR^d$. 
    This can be zero only if all coefficients are zero.
    Hence, $\eta_{i\sigma}=0$ for all $i\sim\sigma$.

    Thus, if the polytope is simplicial, then all facet stresses are zero and the stress is a pure classical framework stress. Due to a theorem of Dehn, convex simplicial polytopes cannot have a non-zero framework stress. \mwsays{True in $d\ge 4$?}\asays{the 16-cell (cross-polytope) has 8 vertices and 24 edges and hence has two self-stresses. In general, there are many stresses, I think}
\end{observation}
}

\fi

%Since $\mathcal T_P\subset\ker \mathcal R(P)$, it 

\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    %\asays{below we use infinitesimal rigidity. Let's choose one throughout} 
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
    %\mwsays{I prefer ``first-order rigid'' because it is more consistent with ``second-order rigid''. Using ``first-order rigid'' and ``corank'' would be consistent with the other paper.}
\end{corollary}
%
%\todo{\mhsays{First prove inf rigid $\Rightarrow$ regular point in realization space. Then use Riemannian geometry. (see also Asimow-Roth)}\mwsays{Why did we need this complicated stuff again?} \mhsays{Yeah, I agree that it doesn't seem to be necessary anymore. I think the ``complexity'' happens in 4.1.}}
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
    %
    %\qedhere
    
    %By \cref{res:trivial_dim} $\corank \mathcal (P)\ge \binom{d+1}{2}$.
    % If $P$ is first-order rigid, all its first-order flexes are trivial, that is, $\ker \mathcal R(P) \subseteq\mathcal T$. Hence $\ker \mathcal R(P)=\mahcal T$ and the claim follows from \cref{res:trivial_dim}.

    % \TODO\ \mwsays{Maybe not true if $P$ is not affinely spanning. But we are always spanning. Cite a paper by Bernd, Bill, Tony, ... for this}\asays{it's not formally proved there, but I think we can still reference it. I do agree we need spanning. If the joints are spanning, then this statement is pretty clear I think. We have a non-trivial first-order flex iff kernel has dimension larger than ${d+1}\choose 2$}
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:

% \mwsays{In the theorem below, should we go for the differential geometry proof?}
% \mhsays{I think it's fine. The proof technique is pretty standard in rigidity theory.}
% \mwsays{I try to formulate the differential geometry argument. See Matthias' paper.}

% \begin{theorem}
%     % \label{res:second-order-implies-rigid}
%     % \label{res:first_order}
%     If a polytope is first-order rigid, then it is rigid.
% \end{theorem}
% %
% \begin{proof}
%     Observe that $\mathcal R(P)$ is the Jacobi matrix of the constraint system. %If its rank is maximal, then this implies that $\real(\mathcal P)$ is smooth at $P$.
%     \mwsays{We currently have no name for the space of all realizations with prescribed edge lengths.}
% \end{proof}

\begin{theorem}
    \label{res:second-order-implies-rigid}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}

%\notodo{\mhsays{I would say we refer to the Corollary 6.6.}\mwsays{I added a reference. Though I also see educational value in seeing the first- and second-order theory proofs side by side and observing that they are so similar. I know I found this interesting.}}

This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends in $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a maximal number $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    A converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}

{\color{gray}
\todo{\mwsays{I think this text would fit better in \cref{sec:selected_results}}\mhsays{I agree. Can you move it?}\mwsays{Okay, I will}}

Dehn's theorem \cite{dehnstheorem} proves that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
Later, we encounter plenty of non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priorily.
We therefore formulate the following question:

\begin{question}
    %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
    Can we extend Dehn's theorem to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Natural candidates are polytopes whose faces are triangles and 4-gons.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

}

\iffalse % Albert's proof

{\color{lightgray}

\begin{proof}
    %\textcolor{red}{Add proof here}
    We prove the contrapositive: if $P$ is flexible, then it is first-order flexible. 
    Let $P^t$ be a flex. \todo{\mwsays{I think we need to invoke curve selection to get an analytic flex}} 
    Since $P^t$ is non-trivial, there is some minimal order $k$ for which truncating the Taylor expansion of $P^t$ at this order does not look like the truncation of a trivial motion.
    %we can truncate the Taylor expansion of $P^t$ at some order, say $k$, after which it cannot be completed to a trivial motion by adding higher order terms. 

    We expand the $k$-th derivative of the constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}\!(p_i^t-p_j^t)\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}\!(p_i^t-p_j^t)=0.
    \end{equation*}
    %
    For the coplanarity constraint \eqref{eq:flex_at_vertex_face} at $i\sim\sigma$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell} \!p_i^t\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell} \!\!a_\sigma^t=0.
    \end{equation*}

    Since $k$ was chosen minimal, we can add a suitable trivial motion to cancel all terms of order up to $k-1$. The two equations above become the following. 
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!(p_i^t-p_j^t)=0
    \end{equation*}
    and 
    \begin{equation*}
        p_i^t \cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!a_\sigma^t+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!p_i^t \cdot a_\sigma^t=0
    \end{equation*}
    The $k$-th derivative satisfies the same equation as a non-trivial first-order flex does.\todo{\mwsays{I don't think this is clear from what we know so far.}} Therefore, $P$ is first-order flexible. 
\end{proof}

}

\fi

\iftrue % polyhedra rigidity stresses first-order theory

%\newpage

\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second and equally important first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
%(recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

% Stresses have no counterpart to ``trivial'' motions

Like first-order flexes, stresses form a linear space -- the \Def{stress space}.
Stresses~are particularly relevant in second-order theory (\cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).

%One fact that makes 3-dimensional polytope rigidity tractable as compared to dimension $d\ge 4$ is that first-order rigidity can be expressed purely in terms of stresses.

\begin{proposition}
    \label{res:flex_eq_stress}
    If $P$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%
\notodo{\mhsays{I think it would be cleaner to simply move this comment after the proof.} \mwsays{I like to comment on results before everybody got drained out by the proof. I consider the proof as a nice addendum but nothing crucial for reading. Matter of taste I guess.} \mhsays{This is not important to me. The way I read a paper is I usually skip the proof and read the comments first, but like you said, matter of taste. Why I wanted to move the text is so that before section 4 there is not such a weird gap anymore after the $\square$.}}

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]
    %We first show that for $\mathcal R(P)$ holds $(*)$ $\text{$\#$rows}=\text{$\#$columns}-6$.

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}

% \begin{corollary}
%     \label{res:rigid_eq_stress_free}
%     A polyhedron is first-order rigid if and only if it has no non-zero stress.
% \end{corollary}


The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.


\fi


\iffalse

\hrulefill

\begin{lemma}
    For $\mathcal R(P)$ holds $\text{$\#$columns}=\text{$\#$rows}+6$.
\end{lemma}
%
\begin{proof}
    Let $v,e$ and $f$ be the number of vertices, edges and faces of $P$ respectively.
    
    For each vertex, the number of incident faces equals the number of incident~edges. Thus, the total number of vertex-face incidences in $P$ is equal to the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we arrive at
    %
    \begin{align*}
        \text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
\end{proof}

\mhsays{Add the property that $\# flexes = \# stresses$ for polytopes?} \mwsays{Only true for $d=3$, and yes we should mention this.}

\fi


% \subsection{Flex space dimensions}
% \label{sec:flex_space_dim}

% \mwsays{Delete this section.}















% \tempnewpage % temporary new page

\section{Second-order theory}
% \section{Second-order rigidity and prestress stability}
\label{sec:second_order}
\label{sec:second-order-theory}

%\notodo{\mhsays{Segue from previous section. We now consider arbitrary polytopes again? Or exchange Sections 5 and 6.}}
Second-order rigidity theory investigates continuous flexes that preserve the constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
%Sometimes, the polyhedron can still be rigid even if it is not first-order rigid. 
%Rigidity beyond first order is often difficult to test even for bar frameworks. 
%
We follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if it satisfies \todo{\mhsays{Don't we also need that $\dot{P}$ is a first-order flex?}}
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$}
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
%Analogous to what was observed in \Cref{sec:first-order-theory}, the $\bsddot a$ are automatically determined by the $\bsddot p$ in this setting
%\todo{\mwsays{Is the sentence about $\bsddot a$ being determined by $\bsddot p$ necessary?}\mhsays{Not really. We can remove it.}}.
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

%\todo{\asays{I think we deleted what it means to be non-trivial in this case. An issue is that $(0,\bsdot p)$ would be non-trivial for a non-trivial first-order $\bsdot p$ if you are not careful, but it doesn't tell us anything other than the first order motion being non-trivial. A clear definition would be a second-order motion with nontrivial first-order terms.}\mwsays{Oops, true, this got deleted. Will fix.}}
%\mwsays{I previously introduced commands to render $\bs p, \bsdot p, \bsddot p$ (see TeX code for commands) in place of $\mathbf{\ddot{p}}$; again, this would be consistent with the first paper. In any way, I recommend to use the command, we can change its appearance later if desired.}

% Let $\dot P,\ddot{P}$ be the vectors $(\dot{p}_1,...,\dot{p}_{|V|},\dot{a}_1,...,\dot{a}_{|F|})$, $(\ddot{p}_1,...,\ddot{p}_{|V|}$ and $\ddot{a}_1,...,\ddot{a}_{|F|})$ correspondingly. We can now define the second-order flex:
%\mhsays{I suggest using textit and a pale color (\eg\ blue) for definitions instead of bold font. That makes it distinguishable from Definitions/Theorems} \mwsays{I imported the command \texttt{\textbackslash Def} for this. It renders \Def{like this}. Feel free to modify.} \mhsays{Looks good!}

% \begin{definition}\label{sorigid}
%     The pair $(\dot{P},\ddot{P})$ is a \Def{second-order flex} if equations \eqref{eq1} and \eqref{eq2} are satisfied. A second-order flex is \Def{non-trivial} if $\dot{P}$ is not a trivial first-order flex. The polyhedron $P$ is \Def{second order flexible} if there exists a non-trivial second-order flex. Otherwise, we say that it is \Def{second-order rigid}.
%     %\mwsays{Use eqref for referencing equations. Use cref for everything else.}
% \end{definition}

% \begin{remark}
%     Notice that we are not defining trivial second-order flexes as the first and second derivatives of trivial flexes. The reason is that while it is possible to build a non-trivial flex with a trivial first derivative, it is not interesting because $\ddot P$ is simply identical to a non-trivial first-order flex, as the proof of \cref{res:second-order-implies-rigid} shows. Therefore, we only need to look at the case where $\dot{p}$ is non-trivial. 
%     \todo{\mwsays{Not really clear}}
% \end{remark}

% \mhsays{We should fix a notation about the realization ${\bs p}, P, ({\bs p},{\bs a})...$ and keep it consistent throughout the article.}
% \asays{Since we defined $P=(\mathbf p,\mathbf a)$, I defined $\dot P$ and $\ddot P$ analogously.} \mwsays{I am fine with using $P$ and $(\bs p,\bs a)$ (and the dotted variants) almost interchangeably. But I also find it weird to use $\dot P$ as a vector.}

%\mhsays{Are the $\ddot{a}$ automatically determined by the $\ddot{p}$? $\Rightarrow$ write a lemma about it?} \mwsays{They are. We have no lemma for this in the first-order case, just a sentence. If it is not needed, let's keep it at the one-sentence-level, no?}\mhsays{ok.}

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking curve selection, we obtain an analytic flex $P^t$.
    There is then a maximal number $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:second-order-implies-rigid}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system.
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently whether $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.

\iffalse % stresses

% \subsection{Equilibrium Stresses}
% \label{sec:stresses}

%The test is based on the notion of equilibrium stresses, which we introduce next.

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system. 
We denote them by pairs $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$ (recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ sake of brevity and call it a \Def{polytope stress}.

\mwsays{Remark: first-order rigid iff no stress. (and then make this its own equilibrium stress subsection). Maybe move stresses to first-order theory.}\mhsays{Maybe as Proposition?}

%\begin{remark}
%\label{res:stress_eq_flex}    
%\end{remark}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

\fi





% Equations \eqref{eq1} and \eqref{eq2} can be compactly written as a single equation:
% % \begin{equation*}
% %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
% % \end{equation*}
% %
% \begin{equation}\label{eq:compact}
%     \mathcal R(P)\cdot \ddot{P}+\mathcal R(\dot{P})\cdot \dot{P}=0
%     % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
% \end{equation}
% %
% Recall that we use $P$ interchangeably with $(\bs p,\bs a)\in \RR^{dV}\oplus\RR^{dF}$, and analogously~with $\dot P$ and $\ddot P$.
% %
% Now, given a second-order motion $(\dot P,\ddot P)$ and any stress ${\bs \xi}$, we obtain
% %
% \begin{equation}
%     \label{eq:with_stress}
%     {\bs \xi}\T \left(\mathcal R(P)\cdot \ddot P+ \mathcal R(\dot P)\cdot \dot P\right)=0.
% \end{equation}
% %
% %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
% Since ${\bs \xi} \in \ker \mathcal R(P)\T$ by definition of stress, we have ${\bs \xi}\T \mathcal  R(P)\ddot P=0$.
% Equation \eqref{eq:with_stress} then becomes ${\bs \xi}\T \mathcal  R(\dot P)\dot P=0$. We say that a stress $\bs\xi$ \Def{blocks} a first-order motion $\bs P$ if
% %
% $${\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0$$
% %Next, we move on to the second-order duality which can be useful when we want to prove $\ddot{P}$ does not exist. 


\iffalse 
Before that, we first introduce the following equality form of Farkas' lemma:
    \begin{lemma}\label{farkaseq}
        \mwsays{Maybe just use it in the proof and don't list it as a separate lemmas.}\mhsays{I don't mind the Lemma here tbh. }
        Either $Ax=b$ has a solution, or $A^Ty=0$ has a solution with $b^T y\not =0$.
    \end{lemma}
    Intuitively, this Lemma says that either $b$ is in $A$'s column space, or there exists a hyperplane containing the column space of $A$ and $b$ is not in it. 

\begin{lemma}\label{lem2}
    Given a first-order flex $\dot P$, if and only if there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
        {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
    \end{equation}
    then there cannot be a $\ddot P$ such that $(\dot P,\ddot P)$ is a second-order flex. 
    ${\bs \xi}$ is called a \Def{blocking stress} for $\dot P$ if Inequality $\eqref{block}$ holds. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
\end{lemma}
\begin{proof}
    The ``if'' direction is already given in the discussion above. To show ``only if'', we use \cref{farkaseq}.
    %\mhsays{I don't like using the theorem environment in a proof} 
    Let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$. Then \cref{farkaseq} says that either there exists a $\ddot P$ or you can find a blocking stress. 
\end{proof}
\fi

%The following test is an elegant application of Farkas' lemma:

\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

% \begin{lemma}\label{lem2}
%     Let $\dot P$ denote a first-order flex of a polytope $P$. Then there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
%         {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
%     \end{equation}
%     if and only if there is no $\ddot P$ for which $(\dot P,\ddot P)$ is a second-order flex. If $\eqref{block}$ holds,
%     ${\bs \xi}$ is said to \Def{block} $\dot P$. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
% \end{lemma}
\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    % \begin{equation*}
    %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
    % \end{equation*}
    %
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

    
    % This system has the form $A\ddot P=b$ for $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$.
    % By Farkas' lemma, the non-existence of a solution for $\ddot P$ (and hence, second-order rigidity of $P$) is equivalent to the existence of a solution of the system $A\T \bs \xi=0$ for some $\bs\xi$ with $\bs\xi\T b=0$, that is,
    % %
    % $$\mathcal R(P)\T \xi=0,\qquad \bs\xi\T\mathcal R(\sot P)\dot P\not=0.$$
    
    % For an arbitrary stress ${\bs \xi}$ therefore holds
    % %
    % \begin{equation}
    %     \label{eq:with_stress}
    %     0 = {\bs \xi}\T \left(\mathcal R(P) \ddot P+ \mathcal R(\dot P) \dot P\right) = 
    %    \underbrace{ {\bs \xi}\T \mathcal R(P)}_{=0} \ddot P+ 
    %     {\bs \xi}\T\mathcal R(\dot P) \dot P={\bs \xi}\T\mathcal R(\dot P) \dot P.
    % \end{equation}
    % %
    % %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
    % where ${\bs \xi}\T \mathcal  R(P)=0$ follows from the definition of a stress as an element of $\ker \mathcal R(P)\T$.
    % We see that $\dot P$ cannot be blocked by any $\bs \xi$.
    
    % To show ``only if'', let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$ and consider the two linear systems $Ax=b$ and $A\T y = 0$. We apply a linearized version of Farkas' Lemma, which implies that either $Ax=b$ has a solution, or $A\T y=0$ has a solution with $b\T y\not =0$.
    % In other words, there either exists a second-order flex $\ddot P$ or it is possible to find a blocking stress. 
\end{proof}

    % By combining the definition of second-order rigidity and \cref{lem2}, we can obtain the following result:
    % \begin{theorem}\label{res:sotest}
    %     $P$ is second-order rigid if and only if every non-trivial first-order flex has a blocking stress. 
    % \end{theorem}%\mhsays{Formulate as a theorem? This seems to be what people are usually doing in second-order rigidity papers, right?} 

In following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 

% The following notion is often more convenient to use:

%\todo{\mhsays{Expand on the relevance of prestress stability and that it is connected to second-order rigidity by swapping quantifiers?}}

% \begin{definition}
% \label{def:prestress-stable}
%     If there exists a stress that blocks every non-trivial first-order flex, we say the polyhedron is \Def{prestress stable}.
% \end{definition}

\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}

\iffalse

{\color{lightgray}

\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    
    Let $k$ be the smallest integer such that the first $k$ derivatives of $P^t$ do not come from a trivial flex at $t=0$. The $2k$-th derivative of the constraints can be expanded as:
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(a_k^t)=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $k$ is the smallest integer, the first, second, all the way up to $k-1^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to the $k-1^{th}$ are all zeros. The two equations above become the following. 
    %
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t-p_j^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    and 
    %
    \begin{equation*}
        (p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(a_k)+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t)\cdot (a_k^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t)\cdot\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(a_k)=0
    \end{equation*}
    %
    Set $\dot P= \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}P^t\big|_{t=0}$ and $\ddot P=2/\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}P^t\big|_{t=0}$. The two above equations become Equations \eqref{eq1} and \eqref{eq2}. Therefore, if $P$ is flexible, it has a non-trivial second-order flex. 
    \mwsays{It remains to show that the motion is non-trivial.}
\end{proof}

}

\fi














\iffalse % previous first-order section

\newpage

\subsection{First-order theory}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.


A \Def{first-order motion} $(\bsdot p,\bsdot a)$ of $P$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$, %=(\dot p_i\in\RR^3:i \in V;\, \dot a_\sigma\in\RR^3 : \sigma \in F)$.
that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    %\label{eq:flex_at_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    %\label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    %\label{eq:flex_at_face}
\end{align}

A first-order motion is \Def{trivial} if in addition it satisfies
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    %\label{eq:trivial_motion_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
A non-trivial first-order motion is called a \Def{first-order flex}.
A framework is \Def{first-order rigid} if it has no first-order flexes; it is \Def{first-order flexible} otherwise.
Many results from the bar-joint framework setting transfer in the expected way. In particular, if a polytope is first-order rigid, then it is rigid. 

The first-order flex conditions \eqref{eq:flex_at_vertex} -- \eqref{eq:flex_at_face} can be collected in a corresponding \Def{rigidity matrix} $\mathcal R(P)$ % with dimensions $(E+\VF)\times(dV+dF)$. 
which satisfies $\mathcal R(P)(\dotbs p,\dotbs a)=0$ if and only if $(\dotbs p,\dotbs a)$ is a first-order motion.
%
Since we only consider polytopes with non-empty interior, they are in particular affinely spanning and
the rank condition of first-order rigidity applies: 

\begin{lemma}
    \label{res:rank_condition}
    We have
    %
    $$\corank \mathcal R(P) \ge \binom{d+1}{2},$$
    %
    with equality if and only if $P$ is first-order rigid.
\end{lemma}

\hrulefill

%\begin{definition}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
We write
%
\begin{align*}
    \realP{\mathcal P}P &= \realpa{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \real(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
    \\
    \realPCvx{\mathcal P}P &= \realpaCvx{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \realCvx(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
\end{align*}
%
for the (\Def{convex}) \Def{configuration space}, \ie\ the space of all (convex) realizations equivalent to a given (convex) realization $P=(\bs p,\bs a)$.

A \Def{motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\realpa{\mathcal P}{\bs p}{\bs a}$ for which $(\bs p^0,\bs a^0)=(\bs p,\bs a)$.
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all~$t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, we call it \Def{flexible}, and \Def{rigid} otherwise.
%\end{definition}

In general, understanding the full configuration space is intractable in all but the simplest cases. 
We mention here a few situations in which such a full understanding is possible due to various genericity assumptions.
In our language, Cauchy's classical rigidity theorem \cite{cauchy1813} states that $\realPCvx{\mathcal P}P$ is a single point whenever $\mathcal P$ is a simplicial polytope.
As a consequence of the main result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} we also obtain the following:

\begin{theorem}
    Let $\mathcal P$ be the combinatorial type of a 3-dimensional polytopes (\ie\ a polyhedral graph).
    Then for almost all convex (in fact, Zariski convex) realizations $P$ of $\mathcal P$ holds: $\realP{\mathcal P}P$ consists of finitely many isolated points.
\end{theorem}
%
Here, \emph{almost all} means that a dense open subset of the (Zariski closure of) the convex realization space has this property.
%
\begin{proof}
    \TODO \mhsays{$\real(\mathcal{P})$ may be irreducible, but that does not mean that $\real(\mathcal{P},P)$ is. The geometry of $\real(\mathcal{P},P)$ may be pretty complicated. We know that $P$ has generic coordinates; however, it seems like what we need to do is show that $P$ also has generic edge lengths. By going back to the edge length perturbation space and proving a stronger result than Proposition 5.2, we then may be able to prove this. The main issue is that we don't really understand the edge length measurement variety and much less the intersection of that variety with $\real(\mathcal{P})$. So I guess to conclude: I don't really have an easy idea how to approach this. You?} \mwsays{I cannot prove this at this moment. Maybe delete theorem?}
\end{proof}

We conjecture the same to be the case in higher dimensions.

Lastly, recall that a \Def{zonotope} is a polytope obtained as the Minkowski sum of finitely many line segments. A \Def{cubic zonotope} is a zonotope with all faces being combinatorial cubes. Cubical zonotopes are the zonotopal equivalent of simplicial polytopes, in the sense that they are generic in the class of zonotopes: they are generated from line segments in general position:

\begin{theorem}
If $P\subset\RR^d$ is a cubic zonotope generated from $k$ line segments, then %
$$\realP{\mathcal P}P = (\RR P^{d-1})^k.$$
\end{theorem}
%
\begin{proof}
    \TODO
\end{proof}

\fi








\iffalse % old flexible polytopes section by Martin

\newpage % temporary new page

{\color{lightgray}

\section{Constructing flexible polytopes}
\label{sec:flexible_polytopes}

% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
%     Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% A \Def{continuous motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that
% \begin{itemize}
% \item $(\bs p^t(0),\bs a^t(0))=(\bs p,\bs a)$ and 
% \item $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% \end{itemize}
% The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% If a realization $(\bs p,\bs a)$ has a motion, then we call it \Def{flexible}, and \Def{rigid} otherwise.
% \end{definition}
As defined in \Cref{sec:rigidity}, a polytopal realization is flexible if it admits a non-trivial continuous realization.

\subsection{Zonotopes}

A zonotope is \Def{generic} if all its faces are combinatorial cubes. We call it generic because it generated from line segments in generic position. Generic zonotopes are the zonotopal equivalent of simplicial polytopes. For the latter the rigidity theory is classical -- they are rigid, both in first order and globally (Chauchy's and Dehn's theorem).
Likewise, for generic zonotopes a complete theory can be given.

\begin{theorem}
    Let $P\subset\RR^d$ be a rhombic zonotope with $n$ generators. Then
    %
    \begin{myenumerate}
        \item 
        $\realR(P)$ is a connected smooth variety of dimension $(d-1)n-\binom{d}{2}$.
        In particular, each polytope $Q$ combinatorially equivalent to $P$ with the same edge lengths can be deformed into $P$.
        \item if $Q\in\real(P)$ then $Q$ is a zonotope.
        \item The first-order flex space of $P$ has dimension $(d-1)n-\binom{d}{2}$.
        \item Each first-order flex of $P$ corresponds to a real flex.
    \end{myenumerate}
\end{theorem}
%
\begin{proof} \mwsays{Work in progress, these are just ``mental'' notes.}
    Consider the space of all deformations of a zonotope that preserves only coplanarity and central symmetry of the facets (the latter is in combinatorial cubes also implied by edge length constraints).
    Note that for $n$ generators there are $2\binom{n}{d-1}$ facets, and that the central symmetry of each is guaranteed by $d(d-2)$ equations: each pair of opposite vertices (of which there are $d-1$) must have a centroid identical to the centroid of the first pair; this is a vector identity with $d$ components.
    Note that this preserves coplanarity automatically.
    Likewise for an first-order flex -- there $dV$ DOFs and $2d(d-2)\binom{n}{d-1}$ constraints. Removing translations but not rotations, we obtain $dV-2d(d-2)\binom{n}{d-1}-d$ final first-order DOFs.
    Observe that the realization space is a manifold of dimension $nd$, or $n(d-1)$ if we want to preserve lengths. It is also well known that $V=2\sum_{k=0}^{d-1} \binom{n-1}{k}$.
    It remains to check
    %
    $$dV-2d(d-2)\binom{n}{d-1}-d = nd.$$
    %
    This seems to yield too few remaining DOFs ($< dn$) and so some of the constraints are redundant. Which and how many is unclear?
    
    \mwsays{Check that the fact that all inf flexes extend follows already from some general theory about realization spaces of polytopes when the realization spaces are smooth manifolds.}
\end{proof}

\begin{remark}
    More general zonotopes have non-zonotopal flexes. 
    As soon as some face of a zonotope is not a rhombus, then it is the Minkowski sum of this face with the other generators. But a polygon with more than four sides has a non-trivial (\ie\ not symmetry preserving) flex. Hence the Minowski sum of this flex with the other generators yields a non-zonotope.
\end{remark}

\begin{question}
    Is the first-order flex space of zonotopes exactly the tangent space to the finite flexes?
\end{question}

We can ask analogous questions for general Minkowski sums.

\begin{question}
    Is it true that the generic Minkowski sum (where no two faces, edge or higher, share an affine span) of rigid polytopes only has Minkowski flexes? Same first-order. More generally Is the first-order flex space of a Minkowski sum just the sum of the first-order flex spaces of the individual polytopes?
\end{question}

\subsection{Minkowski sums}

% We previously explained how \emph{generic} Minkowski sums become flexible polytopes.
% We can be more precise here.

% \begin{theorem}
%     Given polytopes $P,Q$, let
%     Let $\mathcal U$ be the set of linear subspaces of 
% \end{theorem}

Let $\mathfrak F(P)$ be the first-order flex space of $P$.

\begin{theorem}
    For a generic Minkowski sum of dimension $d\ge 3$ holds $\mathfrak F(P+Q) = \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$.
\end{theorem}
%
\begin{proof}
    \mwsays{This theorem is wishful thinking. It could be that a Minkowski sum has more (first-order) flexes than the ones that come from the summands. I think we know enough to show that $\mathfrak F(P+Q) \subseteq \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$. Maybe the other direction can be proven using some limit argument.}
\end{proof}

\mwsays{Not true in $d=2$ or for non-generic Minkowski sums, consider two triangles that add up to a hexagon, or prisms over those.}

\subsection{Truncation}

If two frameworks on the same graph have the same edge directions, then they have the same first-order theory since the rows in the rigidity matrix are just multiples of each other.
The following would be a generalization to polytopes:

\begin{theorem}
    If $P$ and $Q$ are normally equivalent, then $\mathfrak F(P)\simeq \mathfrak F(Q)$.
\end{theorem}
%
\begin{proof}
    \TODO
    \mwsays{True?} \mwsays{WRONG! TIco and TDod}
\end{proof}

\mhsays{We lose all flexes when changing the truncation of the truncated dodecahedron. Therefore, the flexes are not a result of the polytopes' symmetry, but rather of the coordinates. }

\subsection{Truncation}
Questions:
\begin{itemize}
    \item Does there exist a truncation in (0,1) preserving the flexes of either of the truncated ends?
    \item Is rigidity/flexibility preserved under certain assumptions on the truncation? 
\end{itemize}

}

\fi













\newpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

%The convex realization space $\realCvx({\mathcal{P}})$ of 3-dimensional polytopes of combinatorial type $\mathcal{P}$ is a smooth $(E+6)$-dimensional manifold, on which the 6-dimensional Lie group of rigid motions acts smoothly. %In fact, the reduced realization space $\realRCvx(\mathcal{P})$ is homeomorphic to an open ball (\cf\ \cite[Thm.\ 13.3]{richter2006realization}). Intuitively, this claim \emph{has} to be true, simply by subtracting the appropriate dimensions. However, proving it is %\todo{\mwsays{Not only ``slightly more subtle'', but this is a big deal :D}}
%significantly more difficult than it seems, as we are working with manifolds and associated Lie groups instead of Euclidean space.

%\mwsays{We should start with emphasizing very clearly that this section will be $d=3$ only. This is the first place in the paper where we are not general-$d$.}
%\todo{\mhsays{I reference second-order rigidity in this section. Honestly, I would prefer to switch this section with the second-order rigidity; also, because we restrict ourselves to 3D here and later relax that assumption again.}\mwsays{I am torn. The current transition from ``second-order theory'' straight to ``certifying second-order theory'' is also nice. Where do you mention 2nd-order? Only in the question? Maybe move the question?} \mhsays{I don't think there is a place for the question other than here. I could write ``rigid, but not fo rigid'', which would fix the problem. However, my main issue is that we restrict to $\mathbb{R}^3$ and then revert the restriction in the coming section. That feels confusing and unnatural. But I also understand that second-order rigidity$\Rightarrow$ certifying is a nice order. Let's discuss!}}
For this section, we restrict ourselves to 3-dimensional convex polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
%\notodo{\mwsays{I still think it is a bad idea to say we study the complement. We don't really. The complement is a terrible object. It is not a variety. I would say we study $\real(\mathcal P)$ locally.}}
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polytopes, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to %\notodo{\mwsays{I am not sure I understand ``first-order flexes which only preserve the coplanarity constraints'', or if I do, I think this is misuse of terminology because flex has a well-defined meaning always fixing edge lengths. Otherwise it is a deformation, or a curve in $\real(\mathcal P)$, but not a flex. First-order terminology we don't have for this at all.}} 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization the trivial first-order motions form a 6-dimensional subspace of the space of infinitesimal motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$. %For that reason, $\Iso$ acts smoothly on $\real({\mathcal{P}})$ and since $\realR(\mathcal{P})$ is given by a quotient manifold of the form $\real(\mathcal{P})/\mathrm{Iso}$, 
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension%\todo{\mwsays{$\real^*$ is a smooth manifold, but the reason given here is incorrect:quotients by smooth actions can fail to be smooth.}\mhsays{Not if the group acts smoothly, freely, and properly (see citation). Feel free to rewrite the paragraph though.}} (\cf\ \cite[Thm.\ 21.10]{lee-smooth-manifolds})
%
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
%\notodo{\mwsays{You want to pin a vertex, constrain an edge to a 1-dim subspace and a face to a 2-dim subspace. Pinning the edge sounds like restricting its length.}\mhsays{Adjusted.}}%
In other words, all polytopes have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). %\todo{\mwsays{Not enough pinning. Maybe use Louis' paper? Or just pin an edge and an constraint a vertex to a plane that is in the same face as this edge.}} 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
%\todo{\mwsays{I would not call it a coincidence that $E$ is the number of edges}}
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. %\notodo{\mwsays{\emph{``This line of thought would imply that we can locally freely perturb the edge lengths around rigid realizations''} I think it is not clear why you mention ``rigid realizations'' in this sentence.} \mhsays{Changed the sentence.}} 
Since rigid realizations correspond to isolated points in $\mreal(\mathcal{P},P)$, the degrees of freedom in $\real(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.

%\notodo{\mwsays{Can't we just define existence of edge-length perturbations as that ``the map from realizations to edge length vectors is locally surjective at $P$?} \mhsays{I do not believe this avoids the invariance of domain theorem. ``continuous'' plus ``locally surjective'' just rewords what is already there and abstracts the meaning. I am not necessarily against this change, I just don't believe it is going to be impactful.}}
    
\begin{definition}
\label{def:edge-length-perturbations}
%Fix an ordering of the edges $E$ for a polytope $P$. We denote 
The
 %\todo{\mwsays{maybe ``edge length vector'', since then perturbations are a more natural thing?}}
 \Def{edge length vector} of $P$ is given by
 %\notodo{\mwsays{Should we use $(a|b)$ instead of $(a : b)$ for consistency with the other text? Or are vectors significantly different to justify different notation from sets?}}
 %
% \notodo{\mwsays{I want to suggest notation: $\bs\ell(P)$ for the edge length vector, since consistent with other indexed families like $\bs p$. Also I think it is not good to have both $\ell(e)$ and $\ell_e$. I think we should use only $\ell_e$ since we call it a vector, and $\bs\ell'$ or so if we need another vector like in the paragraph below. Next, $\mathcal L(\mathcal P)$ can now be used for the space of edge lengths vectors. Or something like $\text{\textsc{Len}}(\mathcal P)$, but I think it would be useful to have notation since we write the phrase so often}}
 %
 %\notodo{\mwsays{Why not just $\|p_i-p_j\|$?} \mhsays{So that the Jacobian is actually the rigidity matrix and we do not need the weird shenanigans with scaling.}\mwsays{A bit weird to call it the ``edge length'' vector then, but this was already weird because of the square ... so I guess this is fine :)}\mhsays{I get where you're coming from. At least it is heavily related to edge lengths. Unfortunately, I don't have a better name in mind (which does not completely ignore brevity).}}
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
% \ie\ if there are edge length perturbations arbitrarily close to ${\bs\ell}(P)$ that can not be realized as a polytope $Q$ sufficiently close to $P$, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

\iffalse 
More precisely, $P$ has all edge length perturbations if for some $C>0$ and every $\varepsilon\in (0,C]$ there exists a $\delta>0$ such that every edge length vector $\bs\ell'$ with 
%
\[\text{dist}({\bs\ell}(P),\,\bs\ell')<\delta\] 
%
there exists a polytope $Q=\psi(\bs\ell')$ of the same combinatorial type as $P$ that satisfies
%
\[\text{dist}(P,\,Q)<\varepsilon\] 
%
in the Euclidean metric on $\mathbb{R}^{d(V+F)}$. This definition implies that the edge length map $\bs\ell:\real(\mathcal{P})\rightarrow\mathbb{R}^E$ is locally surjective around $P$. \fi

Let us first consider an example of the first-order rigid regular tetrahedron. For this polytope, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    This polytope is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polytope is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$ as a bar-joint framework, meaning that removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polytope's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polytopes concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid convex polytope $P$ has all edge length perturbations.
    \iffalse
    \begin{proof}
    %\notodo{\mwsays{I find this confusing: we start talking about reduced non-metric realization space, but then continue with the Jacobian, which is the tangent space of the non-reduced metric realization space}}
    %The reduced realization space of a convex polytope $\realR(\mathcal{P})$ is a smooth $E$-dimensional manifold, where $E$ denotes the number of edges of $P$. 
    Assuming that $P$ is %\todo{\mwsays{First-order rigid}}
        first-order rigid, the rigidity matrix $\mathcal{R}(P)$ has the minimal corank $6$ (\cf\ \cref{res:corank_rigid}), so its rank is $dV+dF-6$. 
        %In particular, $P$ is a regular point of $\mreal(\mathcal P, P)$. 
        %This implies that all sufficiently close realizations of $P$ are also first-order rigid: the Jacobian matrix of a polynomial system drops rank in a proper algebraic subset of lower dimension, implying that around every \todo{\mwsays{Let's not talk abut regular points --  we did not introduce the relation between regular points and first-order rigidity (via generic rigidity). Since we only care about the rigidity, let's just reference \cref{res:corank_rigid}}\mhsays{But this doesn't give us that all sufficiently close realizations are first-order rigid, does it? We need something algebraic here.}}regular point of an algebraic variety there is an open neighborhood of regular points \cite[Thm.\ 5.3]{hartshorne}.
%This implies that $\mreal({\mathcal{P},P})$ locally forms a 6-dimensional manifold around the realization $P$ which is locally parametrized by $\mathrm{Iso}$.
Moreover, the realization space $\real(\mathcal{P})$ is a $(E+6)$-dimensional manifold according to the Legendre-Steinitz theorem, which implies that its tangent space $T_P(\real(\mathcal{P}))$ at the realization $P$ also has dimension $(E+6)$. Moreover $\real(\mathcal{P})\subset\mathbb{R}^{dV+dF}$, so that the dimension of the normal space of the realization space $\real(\mathcal{P})$ is equal to $dV+dF-(E+6)$. Since the rows of the rigidity matrix $\mathcal{R}(\mathcal{P})$ are exactly given by a basis of the normal space of $\real(\mathcal{P})$ (\cf\ \cite[Proposition 5.38 and Section 6]{lee-smooth-manifolds}) and the Jacobian %\todo{\mwsays{$d\bs\ell$? Not $J\bs\ell$? If you insist on $d$, can we do $\mathrm d\bs \ell$ or $\partial \bs \ell$ or $\delta\bs\ell$? $d$ is already the variable for the dimension.}}
$d\bs\ell$ of the edge length map $\bs\ell: \real(\mathcal{P})\rightarrow \mathbb{R}^E$, the rank of the rigidity matrix satisfies the inequality
%
\begin{eqnarray*}
    dF+dV-6=\rank(\mathcal{R}(P))&\leq& \rank(J\bs\ell(P))+\dim(T_P(\real(\mathcal{P}))^\perp)\\
    &=&\rank(J\bs\ell(P))+dV+dF-(E+6)\\[3mm]
    &\Rightarrow& \rank(J\bs\ell(P))\geq E
\end{eqnarray*}
%
    On the other hand, $\rank(J\bs\ell(P))\leq E$ by construction, which implies that the rank of $J\bs\ell(P))$ is equal to $E$. Thus, the Jacobian $J\bs\ell(P)$ has full rank. Consequently, $\bs\ell$ is locally a submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}), which implies that $\bs\ell$ is locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). Therefore, all sufficiently small edge length perturbations are realizable.
    \end{proof}
\fi
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    %\notodo{\mwsays{In the rest of the section your write $E$ instead of $E$ for cardinalities.}\mhsays{I reckon you prefer using $E$ for cardinalities? How do we call the set of edges then?}\mwsays{I prefer $E$ for the set and the number. I reckon you are not okay with this abuse of notation. And since we already do it differently everywhere else, lets just use $|E|$, no?}\mhsays{No, I am fine with it. We should just be consistent and say it once in Section 2 that we use them interchangeably.}}
    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). %\todo{\mhsays{There is a gap in the proof here, since the definition requires the existence of $\ell^{-1}$ (sort of), so we need to construct a continuous map from $\mathbb{R}^E\rightarrow \real(\mathcal{P})$} \mwsays{This is easy enough by quotienting by the Iso-action. But let's not touch this before we have figured out the definition problem}}
    %Therefore, all sufficiently small edge length perturbations of $P$ are realizable.
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of convex 3-polytopes are first-order rigid.  
This result requires a suitable definition of genericity, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polytopes to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 

%\mwsays{``For a suitable definition of generic, see \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}:''. Random Coordinates}


\begin{corollary}
    A generic realization of a convex polytope $P$ has all edge length perturbations.
    \begin{proof}
        In \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polytope is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polytope in the following example. This example highlights that that not all realizations of convex polytopes have all edge length perturbation.

%\notodo{\mwsays{Proposal: we bring the two examples as motivation; we take the locally surjective definition; we prove fo-rigid implies all perturbation exist; we discuss whether the cube example can be generalized; we give Theorem 5.6 as a question; we discuss the $z^2$ problem; we prove flexible implies not all perturbations exist under the additional example of continuous inverse (maybe constant fiber?).}}

\begin{example}
\label{ex:cube-edge-length-perturbations}
    %\todo{\mwsays{I think this example is very educational and should, together with a positive example, come in the beginning of this section}}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polytope, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    %\notodo{\mwsays{``antipodal edges'' better?} \mhsays{Sure}}antipodal edges. 
\end{example}

We can turn the observation from this example, that not all convex polytopes admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polytope's edge length vector to distinct polytopes sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the convex polytope $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        %\mwsays{I am skeptical of the conclusion of the second paragraph. We assume that $\real^*$ is smooth and $E$-dim, $\bs\ell\:\real^*\to\RR^E$ is polynomial and locally surjective. But from this alone we cannot conclude that $\bs\ell$ has a local inverse by a continuous map $\psi$. There are counterexamples in this general setting. Either you use more structure and I don't understand how, or there is a gap.}\mhsays{I do not use $\bs\ell$ in this proof 
        %\mwsays{I don't understand, you literally write $\psi(\bs\ell(P))=P$.} and the edge length realization space is also not reliant on $\bs\ell$. In fact, the definition goes the other way around: All edge length perturbations are realizable if there exists a local, well-defined, continuous map $\mathbb{R}^E\rightarrow \real(\mathcal{P})$; in other words, for all sufficiently small edge length perturbations $\bs\ell'$ of $\bs\ell(P)$ we can find a realization $Q$ sufficiently close to $P$ such that $\bs\ell(Q)=\bs\ell'$ (i.e., the map that I am describing above maps an open neighborhood of $\bs\ell(P)$ to some sort of set that contains $P$). At least that is what I intended to convey. If the definition does not convey this, we need to fix it. Nothing about local surjectivity whatsoever. Honestly, you confused me more with your comment about local surjectivity than it helped, so I'd prefer forgetting this term entirely. This map is trivially injective though. I reckon we should add a comment/remark after the definition to clarify either way. }
        %\mwsays{Here is what I just did to sanity check myself: I took a screenshot of your definition of edge length perturbation and put it into ChatGPT. I asked whether this gives me a local continuous inverse $\psi$ that you claim. It said no. It told me that this definition is a sort of ``local surjectivity'' of $\bs\ell$. I did not put this word in, it came back with it itself. So I think the definition is not unclear, but simply not what you want it to be. We need to either fix the definition or the result.}
        %\mhsays{ChatGPT customizes the chats to you by learning from past chats. If I ask ChatGPT \emph{anything} mathematical, I usually get rigidity theory as an example. This is not really an argument. Also, around 40\% of AI queries produce erronous answers. The definition is simply the $\varepsilon$-$\delta$ definition of local continuity of $\psi$. I am still convinced that the definition says exactly that. When I queried ChatGPT about local surjectivity, it often reversed the arrows. This may stem from the fact that suspensions mainly appear in differential geometry where they are used to show the existence of a locally surjective atlas (which reverses the arrows).}
        %\mwsays{Thinking some more I now believe that I understand where you are coming from. I simply had a different (weaker) notion of ``edge length perturbations exist'' in mind. Which one is better is unclear to me. The one where we can prove more, or the one that needs less assumptions. For example, I think with your definition, the answer to Question 5.9 is very likely No already for the dodecahedron. But I am very optimistic it has all perturbations under my definition (which equals your currently written down definition). Especially since all edges can be perturbed individually.}
        Assume now that all of $P$'s edge length perturbations are realizable via 
        % Then, in particular, we can locally extend and contract each of $P$'s edges individually. In fact, we can arbitrarily combine these edge length perturbations, %\todo{\mwsays{``Since we factored out Euclidean isometries'': how does this imply the second half of the sentence?}}Since we factored out Euclidean isometries, 
        %so that each combination of edges that we perturb gives rise to a \emph{distinct} continuous deformation of $P$. This implies that there is an open ${E}$-dimensional ball of realizable edge length perturbations containing ${\bs\ell}(P)$. Therefore, the map 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. As a consequence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi=\varphi^{-1}\circ(\varphi\circ \psi)$ and $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        
        This implies that there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ that preserves the edge lengths in ${\bs\ell}(P)$, so $P$ is rigid. 
        \iffalse
        \mhsays{To show:
        Conversely, if $P$ is rigid, then $P$ is a real-isolated solution of the polynomial system of edge length, facet planarity and pinning equations that factor out the rigid motions (see previous implication). Recall that the configuration space $\mathcal{C}_\mathcal{P}$ is a smooth manifold of dimension $E$. Therefore, intersecting $\mathcal{C}_P$ with the real algebraic set generated by the edge length equations
        \[\mathcal{E}_P~=~\left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||=\mathcal{L}_{(u,v)}~\forall uv\in E\right\}\]
        contains the isolated point $P$. Consequently, intersecting $\mathcal{C}_\mathcal{P}$ with the complement
        \[\mathcal{N}_P ~=~ \left\{({\bs p},\,{\bs a})\,:\,||{\bs p}_u - {\bs p}_v||\neq \mathcal{L}_{(u,v)}~\text{ for some } uv\in E\right\},\]
        which exactly characterizes the edge length perturbations of $P$, is equal to $\mathcal{C}_{\mathcal{P}}\setminus \{P\}$.
        We now show that for every sufficiently small perturbation of ${\bs\ell}(P)$, there is a convex polytope close to $P$. In other words, we need to show that $U({\bs\ell}(P)$ is open in $\mathbb{R}^{E}$ and not only in the realization space of edge length perturbations. \textcolor{red}{Also, we need to show well-definedness of $\psi$.}
        %Since $\mathcal{C}_\mathcal{P}$ is a smooth, $E$-dimensional manifold, it is locally diffeomorphic to $\mathbb{R}^{E}$ via $\varphi:\mathcal{C}_\mathcal{P}\rightarrow \mathbb{R}^{E}$. This property implies that there exists an open neighborhood $V\subset\mathbb{R}^{E}$ such that $\varphi:\varphi^{-1}(V)\rightarrow V$ is a diffeomorphism. Note that we can choose $V$ so that ${\bs\ell}(P)$ is contained in $\varphi^{-1}(V)$ since $\mathcal{C}_\mathcal{P}$ is a smooth manifold. By possibly shrinking the open sets, we obtain a continuous map $\varphi \circ \psi:U_{\bs\ell}(P\rightarrow V$. 
        The rigidity of $P$ implies that
        \[\mathcal{C}_\mathcal{P} ~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right)\,\cup\, \left(\mathcal{C}_\mathcal{P}\cap \mathcal{E}_P/\sim\right)~=~\left(\mathcal{C}_\mathcal{P}\cap \mathcal{N}_P/\sim\right) \cup \{P\}.\]
        Since $\psi$ is injective and continuous by construction, the preimage of any open set around $P$ under $\psi$ is open again. Since all realizations come from edge length perturbations, $\psi$ is surjective; therefore, $\psi$ is a homeomorphism.}
        \fi
    \end{proof}
\end{theorem}

The contraposition of this theorem provides a sufficient condition for the rigidity of polytopes, which makes it worth to point it out as a corollary. Albeit, it is unclear whether checking that all edge length perturbations are realizable offers any advantage over directly verifying a polytope's rigidity.

\begin{corollary}
    If a convex polytope $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}

%\notodo{\mwsays{As written this is not correct. What you want to say is that the \emph{existence} of such $\psi$ is equivalent to the \emph{existence} of such other $\psi$.}\mhsays{You meant the Corollary, right? In that case: Fixed.}}
%
We also note that the assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. This restricts the admissible polytopes.

Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample: The map $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.


However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 
\iffalse
\begin{remark}
    %\todo{\mwsays{As written, it sounds as if we have an example of this, which we don't}}
    It is unclear, whether the converse of \Cref{thm:rigidity-and-edge-length-perturbations} is true: The space of edge length perturbations may be full-dimensional, even though the realization $P$ is rigid and only certain edge length perturbations which form a lower-dimensional algebraic subset are not realizable. 
\end{remark}
\fi

The correspondence between the edge length realization space of a polytope and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polytope is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

%\notodo{\mwsays{Can we make the first two questions into one with (i) and (ii) since they are just inverses of each other?} \mhsays{I was contemplating that, too. Fixed.}}

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polytope $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization of a convex polytope have all edge length perturbations?
\end{question}

%\notodo{\mwsays{In the question below, do you also want to ask that it is not first-order rigid? Otherwise the tetrahedron is a counterexample. And maybe move this question to the end of the so-theory section? Depends on if we move this section of course.} \mhsays{True. Thanks for pointing out this oversight. I chose to replace it by ``rigid, but not fo-rigid''.}}

% \begin{question}
% Assuming a convex polytope $P$ is rigid, but not first-order rigid, is ${\bs\ell}(P)$ then singular in the edge length realization space $\mathcal{L}(P)$ (see \cref{fig:edge-contraction-deformation-space})?
% \end{question}

%\todo{\mhsays{I might delete this question, since I find it confusing in the context of Legendre-Steinitz and it is not formulated precisely, since we only change the length of a single edge.}}

%While we do not understand the edge length realization space of polytopes nearly enough to provide answers to these questions, they provide interesting observations that should be investigated in future research.\todo{\mwsays{You essentially repeat the last sentence before the questions}}

%\todo{\mhsays{Technically, we could also move this section to the appendix if need be. Without \Cref{thm:rigidity-and-edge-length-perturbations}, this section is not what it used to be.}}


















\newpage
\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}

%\todo{\mwsays{Use $\mathcal{R}$ for rigidity matrix}}

As laid out in \Cref{sec:second-order-theory}, any non-trivial first-order flex of a polytope in the edge-length realization space \mbox{$\mreal(\mathcal{P},P)$} that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. This provides a convenient heuristic for finding nonblocked flexes: Essentially, we need to find a non-trivial flex $\dot{P}$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$ for all equilibrium stresses $\bs \xi$ (\cf\ \Cref{res:sotest}). Conversely, if there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$ for all $\dot{P}$, then the polytope is second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the flex space via a basis ${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ and variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ and variables $\mu=(\mu_1, \dots, \mu_s)$. This turns the second-order condition from \Cref{res:sotest} into a cubic polynomial of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every non-trivial first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.

By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is nonzero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. Therefore, the first-order flexes corresponding to a $\lambda$ that are not blocked by any stresses must live in the algebraic set given by the intersection of the zeros of $Q_1,\dots, Q_s$. 

Since the polynomials $Q_1,\dots, Q_s$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$. The following lemma lets us certify the zero-dimensionality of an algebraic variety and it proves useful to us in practice. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field %\todo{\mwsays{Can we use $\Bbbk$ for the field?}}
        $\Bbbk$. Given an ideal $I=\langle f_1,...,f_s\rangle$, where $f_i\in \Bbbk[x_1,..,x_r]$, and a Gröbner basis $G$. $I$ is zero dimensional if and only if some power of $x_i$ is the leading monomial of an element of $G$ for every $i\in\{1,...,m\}$.%\mhsays{Only for algebraically closed $k$? If so, replace $k$ by $\mathbb{C}$. Else, define what $k$ can be. }
    \end{lemma}

There are also other methods based on Gröbner bases to verify than an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic variety $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homgeneous, it holds that $\mathcal{V}(\mathcal{I})\subset \mathbb{P}_\mathbb{C}^{r-1}$. Thus, for any solution $\lambda^*$ of the polynomial system $Q_1(\lambda)=0,\,\dots,\,Q_s(\lambda)=0$, all scalar multiples $c\cdot\lambda$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\emptyset$. In our context, this translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ only has $\lambda = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)$.
\end{proposition}

%\mhsays{Describe Test for prestress stability: Albert's code.}

The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all Archimedean, Catalan and Platonic solids (\cf\ \Cref{tab:comparison} and \ref{tab:catalan-comparison}). Still, it clearly is not necessary, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})$ is empty over the real numbers, even when we find solutions over $\mathbb{C}$. The trivial counterexample is $x^2+y^2=0$, which only has $x=y=0$ as a real solution, yet the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solution on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}).

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a linear combination of stresses $\mu$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu_j$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix  $\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_j\lambda_k}Q_j(\lambda)\right)_{j,k=1}^r$ is positive definite for some choice of $\mu$. Our calculation shows that the regular dodecahedron and truncated icosahedron are not prestress stable using a numerical SDP solver. A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate in our case.




\newpage

\section{Computational results}
\label{sec:experimental_results}
\label{sec:archimedean}


We demonstrate our techniques on the Platonic, Archimedean, and Catalan~solids -- classes of polyhedra for which combinatorial data and algebraic vertex and normal coordinates are readily available.
The results are shown in \cref{tab:comparison} (for the~Platonic and Archimedean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation~for the content of the tables is given in \cref{sec:explain_table}.
%
A more detailed step-by-step~expla\-nation for how the second-order rigidity results were obtained is given in \cref{section:rigidity-of-the-regdod} on the example of the regular dodecahedron.
%
A key takeaway is that already simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a remarkably simple test case for future theoretical and computational developments.
See \cref{sec:selected_results} for a discussion of selected results from the tables.



\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{0.7ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    %{\color{gray} 
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semi-definite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
%\mwsays{Something about how the numerical computations are sufficiently stable and the results away from zero or whatever so that we can trust them.}\mhsays{Replace ``We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.'' by: The numerical results are based on an eigenvalue computation, for which \noBut\ indicates the existence of an eigenvalue close to machine precision ($\approx 0$), whereas \yesBut\ indicates the existence of an eigenvalue whose absolute value lies above $10^{-6}$, which is sufficiently far away from zero. We observe no intermediate eigenvalues. Since eigenvalue computation is numerically stable and the thresholds have been chosen conservatively, we have a high degree of confidence in these results.}\mwsays{Then we should probably only explain \noBut, because \yesBut\ is never used. And also: do we ever explain this eigenvalue stuff in the paper? I don't remember having done anything with eigenvalues in Mathematica when I checked prestress stability.}\mhsays{I guess you solved an SDP of the form $C=\lambda_1\cdot A_1+\dots+\lambda_4\cdot A_4$ to find an assignment of $\lambda_i$ that makes $C$ positive definite. However, we always found a zero eigenvalue I guess? I don't exactly recall.}
    %}\mwsays{Okay, let's look into Albert's code to see what can be said.}
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flexe space} as introduced in \cref{sec:first_order}.
    %\nls Heu\-ristically, it is the expected number of independent ways in which the polytope can deform in first order. 
    %If the number is zero, the polytope~is first-order rigid. 
    %If the polytope is a generic Minkowski sum, the dimension~decomposes as explained in \cref{sec:generic_Msum} (see also \SymThree\ below).
    In some cases we have a good understanding for how~the~dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension. 
    If further explanations are available, this is indicated by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and more theoretical background given in \cref{sec:dimension_estimates}.
    %
    %\todo{\mhsays{Maybe only refer to \SymTwo\ and \SymThree\ here? \ie\, ``see \SymTwo\ and \SymThree\ for an explanation of the number''? Otherwise we write it twice.}}
\end{enumerate}
%
The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{0.7ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension for the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
    %If~the zonotope is generic (\ie\ all faces are rhombi), the dimension of the first-order flex space is precisely $2\times\#\text{generators}-3$ (see \cref{res:generic_zonotope}).
    %For~general zonotopes a lower bound is given~by $\dim\GL(\RR^3)-4=5$ (with a few exceptions, see \cref{res:bound_zonotopes}).
    
    % The dimension of the flex space of a generic Minkowski sum is at least the sum of the dimensions of the flex spaces of the summands, plus the dimension of the Lie group that parametrizes the relative orientations of the summands.
    % For this class we write the flex space dimension in the table as a sum of these two contributions.
    
    % %show how this dimension decomposes into flexes coming from flexes of the Minkowski summands (left term) and flexes coming from the relative orientation changes of the Minkowski summands (right term). 
    % For example, the \emph{rhombicuboctahedron} (\cf\ \cref{tab:comparison}) is a Minkowski sum of a cube and an octahedron. The cube provides itself three dimensions~for the flex space, whereas the octahedron provides none. The remaining three dimensions come from $\mathrm{SO}(\RR^3)$, which encodes the relative orientation of~the cube and octahedron. We denote this by 3+3.
\end{itemize}
%
%These considerations are elaborated in \cref{sec:dimension_estimates}.
Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
Again,\nls details are given in \cref{sec:dimension_estimates}.

% \mwsays{In all cases our heuristic lower bounds match the actual dimension of the flex space. In some cases (permutahedra) this is especially remarkable since it suggests that the combinatorics and edge lengths constrains enforce a zonotopal realization.}


\iffalse
Numerical experiments reveal that all these properties are sensitive to small changes in the polytope's geometry.
First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
At this time it is unclear why exactly the realizations with uniform edge lengths are flexible in first- and second-order. 
In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.
\fi

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding polytope names in the table are highlighted in \textcolor{orange}{orange}):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} (\Cref{fig:Dod_TIco_TDod}, right~and center) have identical rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes), nor prestress stable; yet, \emph{both are second order rigid}.\nls 
    In particular, they are rigid. 
    This~was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    %In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are \mbox{remarkably na}\-tural geometric constraint systems which demonstrate that prestress stabi\-lity and second-order rigidity are distinct concepts.
    Previous examples of this distinction were comparatively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} (\Cref{fig:Dod_TIco_TDod}, right) is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order, we do not know whether it is in fact rigid.
    If~it~is~rigid,\nls it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above are sensitive to small changes in the their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.

\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priorily.
We therefore formulate the following question:

\begin{question}
    %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps polytopes whose faces are triangles and 4-gons are simple enough for a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.


% \mwsays{Here would be a good place to put Question 3.5} \mhsays{I agree}

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained from actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} do match the values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.





\input{sec/table1}
\input{sec/table2}










% \newpage

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}

Among the Platonic solids, only for one of them the question of rigidity is not immediately clear. 
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid; the cube is a zonotope, hence flexible. 
Only the regular dodecahedron remains to be understood, and initially eluded direct computation.

In this section we single out the regular dodecahedron for a closer inspection.
We explain in more detail how we found it to be second-order rigid.
Subsequently we share what we found while exploring the realization space close to the regular configuration with the hope of better understanding its exceptional behavior.

%Solving the system of first-order conditions, we find that there exists a 5-dimensional space of first-order flexes.






\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi


\subsection{Rigidity} 
\label{section:rigidity-of-the-regdod}

By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
Consequently, the regular dodecahedron is not first-order rigid.

We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. \Cref{prop:stress-energy-condition} asserts that computing the zeros of a certain polynomial system lets us certify this property. For that reason, we employ the following strategy:

\begin{myenumerate}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. We parametrize these bases via variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$, respectively. 
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadrics $Q_i$ (see \cref{section:second-order-rigidity-check}).
    
    \item Employ \Cref{gbasis} to show that this system has finitely many zeros.
    
    \item According to \Cref{prop:stress-energy-condition}, this implies that the regular dodecahedron is second-order rigid.
\end{myenumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $G$. $I$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $G$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}. With the help of this Gröbner basis, we can prove the following theorem:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. As a result, for any nonzero $\dot P$ generated by the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. By \Cref{res:sotest}, $P$ is second-order rigid. By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

\begin{remark}
    Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid} for details).
    % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
\end{remark}


\subsection{Modifying edge lengths}
\label{section:dodec-edge-length-perturbations}


\todo{\mwsays{Potentially incorporate: ``By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
We find bifurcating deformation paths and from this, we construct  a counterexample to generic global rigidity for polytopes.''}\mhsays{Done}}
%
Although \Cref{dodecahedronrig} shows that when fixing its edge lengths, the dodecahedron with combinatorial type $\mathcal{P}$ is rigid, its realization space $\real(\mathcal{P})$ is a smooth $36$-dimensional manifold due to the Legendre-Steinitz theorem. According to \Cref{section:edge-length-perturbations} we can say more: Its reduced realization space $\realR(\mathcal{P})$ is a smooth $30$-dimensional manifold. In \Cref{conj:edge_length_perturbations} we formulate the hope that for rigid polytopes, all edge length perturbations are realizable (\cf\ \Cref{def:edge-length-perturbations}). It is completely unclear, whether this claim is true.

In this section, we investigate how deformations of the regular dodecahedron in $\realR(\mathcal{P})$ induced by shrinking or extending a single edge length behave. By approximating such deformation paths using the methods introduced in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of this polytope. 
With this approach, we describe bifurcating deformation paths, which lets us construct a counterexample to generic global rigidity for polytopes.

By the dodecahedron's regularity, all edges are combinatorially identical. It does not matter which edge is chosen. For this example, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert < 1$. Sampling from the realization space intersected with the real algebraic set generated by the edge length equations reveals that there are six distinct curves through the regular dodecahedron corresponding to the contraction of a single edge length (see also \cite{deformationpaths}) and two corresponding to its expansion. All eight configurations at $\ell^{\star}(\pm 0.25)$ are depicted in \Cref{fig:edge-contraction-deformation-space}.

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by perturbing a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge constractions, whereas gray curves correspond to edge expansions. On these curves, the eight corresponding realizations at $\ell^*(\pm 0.25)$ are depicted. Four realizations are connected by a nodal cubic (dark blue dashes).}
            %Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
        
\iffalse
     \begin{figure}[h!]
        \centering
        \includegraphics[width=0.25\linewidth]{Images/dodeca3.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca1.png}
        \hfill
        \includegraphics[width=0.25\linewidth]{Images/dodeca2.png}\\[2mm]

        \hspace*{7mm}
        \includegraphics[width=0.16\linewidth]{Images/dodeca5.png}
        \hfill
        \includegraphics[width=0.18\linewidth]{Images/dodeca4.png}
        \hfill
        \includegraphics[width=0.17\linewidth]{Images/dodeca6.png}\hspace*{7mm}
        \addtocounter{equation}{1}
        \caption{The six configurations obtained by contracting the blue edge. They can be split into two types that are organized in the top and bottom row. In the central column, the configurations have two reflection axes, while the left and right columns are mutual mirror images with only one reflection axis. }
        \label{fig:dodecahedron-configurations-contraction}
    \end{figure}
\fi

        It turns out that in the case of edge length contractions there are two types of configurations: Those mitigating the edge contraction by deforming vertically (see \Cref{fig:edge-contraction-deformation-space} (top)) and those that deforming horizontally (see \Cref{fig:edge-contraction-deformation-space} (bottom)). Both types contain one configuration with two mirror axes and two configurations with one reflection symmetry that are mutual mirror images. Intriguingly, not all dodecahedra persist until the edge collapses. The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations beyond this particular edge length. \todo{\mwsays{Discuss the fact that the orange branches meet again: the two branches of the loop have opposite symmetries, and must therefore pass through a common symmetrization to connect to each other}} All of them persist until $\ell^*(-1)=0$. 
\iffalse
        \begin{figure}[h!]
        \vspace*{2mm}
            \centering
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT1.png}
            \hfill
            \includegraphics[width=0.425\linewidth]{Images/dodecaEXT2.png}
                \addtocounter{equation}{1}
            \caption{The two configurations obtained by expanding the blue edge. Both admit two distinct reflection symmetries.}
            \label{fig:dodecahedron-configurations-expansion}
        \end{figure}
\fi

        Conversely, expanding an edge only produces two configurations that both have distinct distinct reflection axes. They are depicted on the sides of \Cref{fig:edge-contraction-deformation-space}. There is no indication that there exists a maximal edge length beyond which no realizations exist. Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.

        %What remains is a qualitative analysis of the eight deformation paths that emerge from contracting any of the dodecahedron's edges. By considering projections of the eight deformation paths onto random 2-dimensional subspaces and approximating the curves' derivatives, an understanding of the curves' tangents in the regular dodecahedron can be obtained. \Cref{fig:edge-contraction-deformation-space} visualizes these curves' behavior. 

        %\mhsays{Mention how the graphic was formed (see above text)}

        % \begin{figure}[h!]
        %     \centering
        %     %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation.jpg}
        %     %\hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom.jpg}
        %     %\\[4mm]
        %      %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation2.jpg}
        %     \hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom2.jpg}
        %     \addtocounter{equation}{1}
        %     \caption{Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths (\cf\ \Cref{fig:dodecahedron-configurations-contraction}) have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
        %     \label{fig:edge-contraction-deformation-space}
        % \end{figure}

         %\todo[inline]{\mwsays{Put little pictures of the deformations at the branches of the graphics.}}

%\mhsays{Picture looks good imo. I wonder if we can replace the pictures above by a bigger picture of the topological diagram (since it already contains all configurations)? It feels like Figures 3 and 4 do not add much anymore.}

In \Cref{fig:edge-contraction-deformation-space}, we also depict the deformation paths corresponding to these eight realizations, which are induced by edge contractions \notodo{\mwsays{I am not sure this dashed line will be universally understood to be blue} \mhsays{Like this?}\mwsays{Much better!}}(blue) and expansions (gray).
Remarkably, it appears that some of these curves can be matched smoothly. For instance, the gray curves corresponding to an edge expansion have the same tangent in the regular dodecahedron and so do the corresponding arcs of the blue curves. Moreover, the curves corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (see \Cref{fig:edge-contraction-deformation-space}, dark blue dashed curve).
%todo{\mwsays{Give a different color to nodal cubic so it is easier to refer to.}} %In particular, the regular dodecahedron is a singularity in the deformation space induced by all possible modifications of a single edge. 
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron due to the and that there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$.

%\todo{\mhsays{Is this even true?}\mwsays{Unclear. Depends on the singularity. It is likely but we don't know this.} \mhsays{How to rephrase?}}

Two symmetric deformations remain, which also share the same tangent in the regular dodecahedron. In total, four smooth curves are passing through the regular dodecahedron that are parametrized by edge perturbations. Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective tangents' sum is sufficiently close to zero. Finally, we attach an animation of a smooth deformation path passing through the regular dodecahedron induced by an edge expansion from $\ell^*(-0.25)$ to $\ell^*(0)$ followed by a compatible contraction from $\ell^*(0)$ to $\ell^*(-0.25)$ in the supplementary material \cite{zenodo_suppMaterial} of this article. 




\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytopes is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore globally rigid.

However, the regular dodecahedron is highly symmetric, which still leaves the global rigidity of generic realizations open. A polytope is called \Def{generically globally rigid} if every generic %\todo{\mwsays{Generic undefined. We mention it already earlier, but never define it I think.} \mhsays{We define it \emph{intuitively} on page 15}}\textit{generic} 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
%Let us consider a small generic perturbation $P'$ of one of the realizations shown in \cref{fig:edge-contraction-deformation-space}.
We first observe that all of the equivalent realizations which are highlighted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. This claim has been verified numerically. Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently small generic perturbation $P'$.
Hence, generic realizations are also not necessarily globally rigid.
Interestingly, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}

%\notodo{\mhsays{This is the opposite of global rigidity :D}}

It would be surprising, though also not absurd, that other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{13mm}
    \begin{minipage}[c]{0.31\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edge have the same lengths (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}

For bar-joint frameworks, generic global rigidity is often checked by computing the rank of a \Def{stress matrix} for a random equilibrium stress (\cf\ \cite{gortler-healy-thurston}). Since we demonstrate in this article, that many concepts from bar-joint framework rigidity theory carry over to the polytopal setting, it is possible that we can formulate a similar criterion for the generic global rigidity of polytopes. This provides an exciting direction for future research.

\begin{question}
    Can the rank of the stress matrix be used as a criterion for generic global rigidity?
\end{question}

% Still, that argument does not resolve whether the regular dodecahedron with combinatorial type $\mathcal{D}$ is globally rigid. Nevertheless, we know that there exists a realization of the dodecahedral graph in $\mathbb{R}^2$ that has equal edge lengths (\cf\ \Cref{fig:planar-dodec}). While this realization is not affinely spanning, it clearly has planar facets. If $0$ lies in the relative interior of this polytope, it is impossible to satisfy the equation $\langle p_i, a_\sigma\rangle=1$ for $i\sim \sigma$, as each facet normal must necessarily be normal to the embedded plane $\mathbb{R}^2$, so that $\langle p_i, a_\sigma\rangle=0$. For that reason, we put the plane at height $1$ so that each face has the same normal vector. With this modification, we find that the realization of $\mathcal{D}$ lies in $\real(\mathcal{D})$, implying that the regular dodecahedron is not globally rigid.






%\newpage % temporary new page

%\section{Case study: The truncated dodecahedron}
%\label{sec:truncated_dodecahedron}
%\label{sec:TDod}





\newpage % temporary new page

\section{Conclusion}
\label{sec:outlook}

\mwsays{I am not a fan of a conclusions section that just repeats introduction and main body for the third time. I liked the outlook we had in the last paper because it was just full of questions. If I see correctly, then the only new bit here is the TDod discussion, which might as well go into the results section. This section would be an easy place to shorten the paper.}
\mhsays{A conclusion/outlook is a formal requirement for any scientific paper. In it, the main arguments/results should be restated and it gives room for open problems and future research. Ideally, one uses the three questions ``what?'', ``so what?'' and ``now what?'' to guide the writing. The conclusion is an important place in the paper to state and summarize our most significant findings and results, why they are useful and what should happen next. We can keep it to 1 page, but it is an essential section.}


\todo{\mwsays{Like for title and abstract, I don't think we should reduce this article to second-order theory} \mhsays{Better? First paragraph needs work.}}%
In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 

\subsection{Main results}

We demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves arising from edge length modifications.

\iffalse\textcolor{gray}{
\todo{\mwsays{Saying this makes only sense if it would be in the main body, but it is in the appendix} \mhsays{The conclusion was written when this was not the case.} Feel free to remove.}%
Moreover, we extend our analysis to flexible polytopes. For zonotopes and generic Minkowski sums, we provide a lower bound on the dimension of the flex space. As of now, all flexible convex polytopes that we are able to find arise as zonotopes or generic Minkowski sums. To approximate the flexes of polytopes, we develop an algorithm in \Cref{sec:approx_continuous_motions}, which relies on Riemannian geometry and homotopy continuation, alongside several useful heuristics.}
\fi

Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. In \Cref{sec:dodecahedron}, we explicitly demonstrate a strategy for proving the second-order rigidity of the regular dodecahedron as a test case and we also investigate deformations induced by modifying the length of a single edge, which reveals a highly interesting local geometry and also serves as a counterexample for the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}

\iffalse
\begin{remark}
For the truncated dodecahedron, the system of homogeneous quadratic \todo{\mwsays{Reference these equations by number rather than words}}equations introduced in \Cref{section:second-order-rigidity-check} has a non-trivial solution. According to \Cref{res:sotest}, this implies that the truncated dodecahedron is not second-order rigid. In fact, we find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
\end{remark}
\fi

Among the 31 polytopes we consider, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is four-dimensional, so it is not first-order rigid, and we demonstrate that it is not second-order rigid, since the associated system of homogeneous quadratic \notodo{\mwsays{Reference these equations by number rather than words}\mhsays{Done.}}equations $Q_1=\dots=Q_4=0$ arising from Equation \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. In fact, we find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
In \Cref{fig:TDod_flex_conc}, we show samples from a deformation of the truncated dodecahedron which is constructed using gradient descent with reasonable numerical tolerance.

\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}

However, when we apply more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
%\todo{\mhsays{Discuss energy interpretation}}
This result would help explain, why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which has reasonably low numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, they observe that the energy landscape around an $N$-th order rigid realization locally looks like the parabola $y=x^{2N}$. This implies that for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

Unfortunately, if the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 

%\mhsays{Develop higher-order rigidity techniques.}

% \notodo{\mwsays{I would say we don't need this section. Move the problems to their sections or mention them in the introduction.} 
% \mhsays{Open problems only belong into the introduction if (a) we solve them or (b) they are guiding problems that motivate our article. Neither is the case. We should move them to the respective sections instead (which I did). }}

%\mhsays{Theoretical results for why some polytopes in special position are inf rigid, even though Cauchy-Dehn does not say this.}

%\mhsays{More constructions for flexible polytopes OR proof that Minkowski flexes are all.}

%\mhsays{Dodecahedron and truncated icosahedron have the same numer of first-order flexes; does this come from the symmetries? Counter point: the truncated dodecahedron only has 4 dimensions of first-order flexes even though it has the same symmetry. Where is the lost dimension? Is there a general way of predicting the first-order flexes from the symmetry group?}

%\mwsays{Is there special structure in the TDod that helps deciding the rigidity question?}

%\mhsays{Point out many interesting questions from \Cref{sec:dodecahedron}}



==> sec/introduction_-_copy_-_2026-06-18.tex <==

%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}

%\notodo{\mhsays{Abstract: Replace at least one of the ``we'' alliterations by a different beginning. Fix overful. \mwsays{Will do.} }}

\vspace*{-1em}

\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities.
If such deformations exist, the polytopes is said to be flexible, otherwise rigid.
%. The major difference to the classical setting of polyhedral rigidity is that these deformations are explicitly 
%
Classical results in polyhedral rigidity (such as the rigidity theorems by Cauchy \cite{cauchy1813} or Dehn \cite{dehnstheorem}) enforce the stronger constraint of fixed face shapes, and then find that convexity generally implies rigidity.
This is in contrast to our setting, in which flexible convex polytopes do exist.
Still, only few techniques are known to construct such.

%
%These assumptions are weak in comparison to classical polyhedral rigidity, which also enforces fixed face shapes. 
%
%\todo{\mhsays{I don't understand this sentence.}\mwsays{Sorry, what exactly is unclear?}\mhsays{I understand what you want to say here, but ``weak'' is always slightly confusing to me as a non-logician. Maybe ``are more restrictive'' or ``are implied by the flexibility in classical polyhedral rigidity''?}}%\todo{\mhsays{Should we highlight rigidity in the first sentence of the introduction, too? Currently it is only about flexibility.}}
% \notodo{\mwsays{This sentence sounds like we are in the classical setting}}
%
%Due to In contrast to the classical setting, our setting admits flexibility, even when the polytopes are convex.
%
%While~in~our~setting~even~convex polytopes may be flexible
%Still, only few techniques are known to construct such. %polytopes that admit such deformations.%\mhsays{and which polytopes do not admit continuous deformations? (to highlight rigidity and not just flexibility.)}.
%
\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}
%
As a consequence, the sentiment arose that this sort of flexibility is still rather exceptional, not only among combinatorial types of polytopes, but also among~realizations of a fixed type.
%Only few classes of flexible polytopes are known, constructed from a handful of techniques such as Minkowski sums and affine transformations.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that~in~dimension at least three, a \textit{generic} convex polytope of a given combinatorial type~is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

%\mwsays{Add picture with Dod, TDod, TIco}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
%     \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically. \mhsays{Suggestion: Move to Conclusion and replace image by truncated dodecahedron, dodecahedron and truncated icosahedron, since they are special.}}
%     \label{fig:TDod_flex}
% \end{figure}

%\todo{\mhsays{I do not think anymore that the first page is a good place for a flex, for which we have strong evidence against being a true polyhedral flex. This may generate false expectations. I would prefer putting it in the conclusion/outlook as future work and focusing on the examples that we can actually solve.}}
Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
%The previous exploration therefore focused on first-order and generic rigidity.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques. %, such as a naive Gröbner basis approach. %, and so it remains unknown whether they are rigid or admit continuous deformations.
This already holds for polytopes with relatively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes a suitable second-order theory as~well as an effective algorithm for testing second-order rigidity of concrete examples.
For a demonstration we analyze the rigidity properties of the Platonic, Archimedean and Catalan solids (see \cref{tab:comparison} and \cref{tab:catalan-comparison}). 
In particular, we decide the previously unknown rigidity properties of the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left).
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be determined by our techniques, but seems to require techniques of even higher order. It will thus serve as a simple test case for future theoretical and computational developments.
%
We found it remarkable that such variety of rigidity behaviors can already be observed among classical examples.
%This is not for lack of computations resources, but rather 
%In particular the truncated dodecahedron can serve a surprisingly simple test case for future theoretical and computational developments.
%Merely the \emph{truncated dodecahedron} (see \cref{fig:TDod_flex}, left) evades our approaches. The reason though is interesting, and is of a technical nature rather than from computational limitations.


% \mwsays{The first article develops first- and generic theory. In this article we address notions of rigidity skipped over in the first part: second-order, continuous and global.}

This article divides into theoretical, methodological and experimental results,
of which we give an overview below.
%
\todo{\mwsays{Albert, what do you think about the roadmap.}}
%
%\todo{\mhsays{We can also leave the introduction out or replace it by Table 1/2. The structure of our paper may be slightly confusing and this is an attempt at making the structure clearer. I am \textit{very} open to suggestions here on how to organize the roadmap.}\mwsays{Let's decide this at the end.}}

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (10.25,-2) {Chapter 5};

\node[fill=white] (c6) at (12,2)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,2)  {Chapter 7};

\node[fill=white] (c9) at (20.2,0) {Chapter 9};
% Nodes
\node[
    draw=blue!30,
    fill=blue!20,
    rounded corners,
    fit=(c3)(c6)(c5),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=red!30,
    fill=red!20,
    rounded corners,
    fit=(c7)(c8),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=green!30,
    fill=green!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (intro) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{appendix:comp-data-dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (10.25,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,2)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,2)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.2,0) {\Cref{sec:dodecahedron}};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (c9);

\draw[->,dashed] (c10) to[bend left=-5] (intro);
\draw[->,dashed] (app) -- (c9);
\draw[->,dashed] (c9) -- (intro);
\end{tikzpicture}
\end{figure}
\vspace*{-1.65em}
}

\subsection{Theoretical results}
\label{sec:intro-theory}

% The main theoretical contributions are a careful deve\-lop\-ment of the first- and second-order theory of polytope rigidity, as well as %an~application of the former to so-called 
% the creation of dual certificates based on which perturbations of a 3-dimensional polytope's edge lengths can be realized.
% %edge length perturbations for 3-dimensional polytopes.

In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions/flexes,\nls and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory}~we develop the second-order theory for polytope rigidity.
We provide analogues~for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
%including notions of second-order motions and flexes.
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cf\ \cref{res:sotest}).
%This allows us to define prestress stability for polytopes.
%
%\notodo{\mwsays{We need results to reference on the arrows.}}

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated from the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to rigidity and first-order rigidity.


% In \cref{section:edge-length-perturbations} we apply first-order theory to study polytope realization spaces, motivated from the following train of thought:
% the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo rigid motions is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
% This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.
% If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same edge lengths. 
% This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}.
%In \cref{section:edge-length-perturbations} we provide an interpretation of these degrees of freedom for first-order rigid polytopes by perturbing their edge lengths.



\iffalse % old text, maybe still useful

We subsequently apply the first-order theory to questions of realizability:
given a combinatorial type $\mathcal P$, one may ask whether there exists a realization $P\subset\RR^d$ with prescribed edge lengths $\ell_e$, $e\in E$.
In general, this question is very hard.
In \cref{section:edge-length-perturbations} we explore the connection between rigidity and the existence of so-called \emph{local edge length perturbations} (see \cref{prop:inf-rigidity-edge-perturbations} and
\cref{thm:rigidity-and-edge-length-perturbations}).\nls
In~\cref{sec:dodecahedron-global-rigidity} we use the results to show that some polytopes are \textit{not} generically globally rigid.

\mwsays{
Using this language, we demonstrate that the dodecahedron exhibits a highly interesting algebraic and topological behavior in \Cref{section:dodec-edge-length-perturbations}. We also compute deformation paths associated with perturbing a single edge length using techniques from \Cref{sec:approx_continuous_motions}.}

\mhsays{Add pictures for this section as well}

% We analyze the full realization space of a few examples where this is possible. This includes cubical zonotopes and generic Minkowski sums.

\fi



% We explore the connection between first-order rigidity and the existence of local edge-length perturbations for polytope realizations.


\subsection{Methodological results}
\label{sec:intro-methods}
%\mwsays{More details: numerical, symbolic, ...}
In \cref{section:second-order-rigidity-check}, we provide a concrete method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
%Our newly developed tools allow us to answer questions that have previously been intractable.
%The Archimedean and Catalan solids provided a convenient benchmark. 
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.

In \cref{sec:dodecahedron} we give a step-by-step account of how to apply our second-order~rigidity certificate to the regular dodecahedron. We thereby verify that it is indeed rigid (\cf\ \cref{dodecahedronrig}), answering a question posed in \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

Analogous computations are performed for the other test polytopes and are~documented in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
We highlight two results: We show that, besides the dodecahedron, also the \textit{truncated icosahedron} (\cref{fig:Dod_TIco_TDod}, center) is not first- but second-order rigid. We also show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and thus its rigidity status remains open.
A detailed explanation of the tables and discussion of the results follows in \cref{sec:experimental_results}.
Further theoretical background on the observed flexes and flex space dimensions is given in \cref{sec:dimension_estimates}.
All code and additional animations of the flexible polytopes are included in the Supplementary Material~\cite{zenodo_suppMaterial}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to~another case study of the regular dodecahedron.
%We demonstrate how to apply our second-order rigidity certificate.
We investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations and deformation paths using tools from Riemannian geometry and homotopy continuation (with more details given in \cref{sec:approx_continuous_motions}).
We also conclude that the dodecahedron is not generically globally rigid.

\iffalse  % old Appendix B intro

\todo{\mwsays{This needs rephrasing so that it is clear that we just recall this theory. Or we move to appendix. \mhsays{I guess the novel part is that we can apply it to edge length perturbations. However, it holds in greater generality, which is why I describe it like that. I could make that more explicit in the section?}}\mwsays{This is now appendix. Incorporate it into the introduction differently.}}
%
{\color{lightgray}
In \cref{sec:approx_continuous_motions} we describe an algorithm for approximating continuous motions of flexible polytopes based on Riemannian geometry and homotopy continuation. It relies on numerically tracking the solution to the 
optimization problem that searches for the Euclidean closest point to the realization space. We can also apply this method to investigate edge length perturbations of polytopes. %(see \Cref{section:edge-length-perturbations}).% \mwsays{A bit more details?} 
%\mhsays{Mention generalization to realization spaces?}
}

\fi


\iffalse % old computational results introduction

\tempnewpage

Doing so already enables us to answer questions that were previously intractable.


The results for the five Platonic, 13 Archimedean and 13 Catalan solids are shown in \Cref{sec:archimedean} and reveal a wide range of interesting behaviors.
%The 13 Catalan solids have less surprising rigidity properties and can be found in \cref{tab:catalan-comparison} in \cref{appendix:catalan}.
%The structure of the tables cells is explained in \cref{sec:explain_table}.
We highlight the most noteworthy finding from these experiments here: 
\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and \Def{truncated icosahedron} have identical rigidity properties: they are neither first-order rigid (both have a 5-dimensional~space of first-order flexes), nor prestress stable; yet, \emph{both are second order rigid}.\nls 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct~concepts.
    Previous examples were comparatively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} (\Cref{fig:Dod_TIco_TDod}, right) is not first-order rigid (it has a 4-dimensional space of first-order flexes), not prestress stable and \emph{not second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order,\nls we do not know whether it is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system that demonstrates that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}
\mwsays{Maybe also list the cool fact that most of our lower bounds match the actual flex space dimensions?}\\
%
%\todo{\mwsays{Maybe I move this to dedicated section. Outlook maybe?}}
%\todo{\mhsays{Shorten Introduction to 3 pages?} \mwsays{I will try. Is there a specific reason? Is it bad if it is 3.2 pages?}\mhsays{Not necessarily, but ``in der K\"urze liegt die W\"urze. Just add whatever now you want now and then we shorten during editing.}}
{
\color{lightgray}
%Numerical experiments reveal that all these properties are very sensitive to small changes in the polytope's geometry.
%First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
%Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
%At this time it is unclear why exactly the realizations with uniform edge lengths show low-order flexibility. 
%In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.



%In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
%The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}}
%By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
%We find bifurcating deformation paths and construct from this a counterexample to generic global rigidity for polytopes.

}

\fi



\tempnewpage

\iffalse
{
\color{gray}

Some polytopes turned out first-order rigid without us having an a priori explanation for this.
More remarkable however we found the rigidity properties of the three polytopes marked in \textcolor{orange}{orange} that are \emph{not} first-order rigid:
%
\begin{itemize}
    % \item For all but three Archimedean solids the first-order theory decides the rigidity.
    % If a polytope is first-order rigid, then it is rigid (see \cref{thm:first_order}. All Archimedean solids that were identified as flexible are so via a Minkowski flex and the dimension of the first-order flex space is as expected from this construction. 
    \item
    The \textit{regular dodecahedron} is rigid. This was previously unknown since it is first-order flexible. The second order tools developed in this article allowed to identify the dodecahedron as second-order rigid \emph{but not} prestress stable.
    The regular dodecahedron furthermore becomes first-order rigid after a generic linear transformation. This suggests that the regular realization of the dodecahedron is a singularity in the realization space.
    By computing deformation paths that shrink/extend a single edge of the regular dodecahedron, we probe the neighborhood of this singularity. We find that bifurcating deformation paths and thereby a counterexample to generic global rigidity for polytopes.
    \item 
    The truncated icosahedron (the football) is also first-order flexible yet second-order rigid.
    \item 
    The truncated dodecahedron is flexible in both first- and second order. At this time it is unknown whether it admits a deformation. If it admits a deformation it is the first example of a polytope flex that is no of Minkowski sum type. If it is rigid then it is the first example of a naturally occurring rigidity of order greater than two.
\end{itemize}


\hrulefill

\mwsays{I write ...}

We develop the second-order rigidity theory for polytopes with edge length and coplanarity constraints. 
In addition, we develop computational tools for checking the rigidity of polyhedral surfaces and for approximating continuous motions. 

\mwsays{Regarding caption \cref{tab:comparison}: we should write first-/second-order rigidity instead of the numeric variants, but if I change it the table vanishes completely. Not sure what is going on. Maybe the figure becomes too long for the page?}


% \footnotetext[1]{As a triangulated sphere, this polytope is first-order rigid by Cauchy's rigidity theorem \cite{cauchy1813}.}
% \footnotetext[2]{As a zonotope, this polytope is flexible according to Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.}
% \footnotetext[3]{As a ``generic'' Minkowski sum, this polytope is flexible (\cf\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}).}

\begin{enumerate}[label=\arabic*)]
    \item All Archimedean zonotopes (except for the cube) have 5 inf flexes because they are projectively unique as zonotopes and hence their only transformations come from the 9-dim general linear group minus rotations and global scale. The cube also loses scaling along axis, hence 3 less (but global scale is already contained in here).
    \item The first-order flex spaces of Rhombicuboctahedron and Rhombicosidodecahedron can be explained as the sum of the first-order flex spaces of their constituents + 3-dim rotations. 
\end{enumerate}

\subsection{Dodecahedron and Truncated Icosahedron}
\label{sec:dodecahedron}

The regular dodecahedron and the truncated icosahedron are interesting case studies. They are both first-order flexible and possess a 5-dimensional space of first-order flexes. Nevertheless, using techniques from computational algebra (\cf\ \Cref{section:second-order-rigidity-check}) we show that for each first-order flex there exists an equilibrium stress that \emph{blocks} the first-order flex from extending to a continuous motion. In other words, both polytopes are second-order rigid (see \Cref{section:rigidity-of-the-regdod}).

\mwsays{First-order rigid once we apply affine trafo or change the height of truncation.}

\subsection{Truncated Dodecahedron}
\label{sec:truncated_dodecahedron}

The truncated dodecahedron is both first-order and second-order flexible.
More precisely, it has a 4-dimensional space of first-order flexes, which is surprisingly different from the five dimensions that we usually associate with icosahedral symmetry (see \cref{sec:dodecahedron}). % that we found for both dodecahedron and truncated icosahedron.
For second-order rigidity it turns out that none of the first-order flexes is blocked by any stress, so all of them are potentially real. \mhsays{``real'' is not a good word in this context.}
%
Remarkably, we were able to construct a flex numerically!
So far we are not aware of an analytic way to obtain this flex.
Thus, whether this flex is actually real or not remains a mystery. 
In particular, if no such flex is real, there are currently no feasible techniques to prove the rigidity of this polytope.

Interestingly, all first-order flexes of the truncated dodecahedron vanish either on affine transformation or when changing the size of the triangles (keeping it vertex transitive).

The facts listed above suggest that the \emph{uniform} truncated dodecahedron is quite special.
In particular, it seems unlikely that the existence of its flex is a mere coincidence.
More likely, there exists a yet unknown construction, similar to Minkowski sums, that generates this flex.

If flexible, the truncated dodecahedron has some remarkable properties:
%
\begin{itemize}
    \item its flex is not reducible to a Minkowski sum
    \item its affine transformations are not (first-order) flexible.
\end{itemize}
%
In contrast, if it were rigid, this would be remarkable as well. 
It would then be the first example of a polyhedron that is second-order flexible, yet rigid.
The general consensus seems to be that rigidity beyond the second order only appears in contrived constructions specifically made for this purpose.
The truncated dodecahedron, being very natural, would then be an interesting counterexample.

\subsection{Outline}
This article is divided into three main parts: The theoretical foundation in \Cref{sec:combinatorics-of-polytopes,section:edge-length-perturbations}, followed by methods in \ref{section:second-order-rigidity-check,sec:approx_continuous_motions} and a case study on the regular dodecahedron in \Cref{sec:dodecahedron}.

}

\fi










\iffalse % paper roadmap

\tempnewpage

{\color{lightgray}

\begin{itemize}
    \item Introduction (Martin)
    \item Theory part (Martin, fix notation and terminology, stay close to first paper)
    \begin{itemize}
        \item first-order theory
        \item second order theory (prestress stability) 
        \color{lightgray}
        \item construction of flexible polytopes (continuous motions)
        \begin{itemize}
            \item theorem for generic zonotopes
            \item counterexample for general zonotopes (hex prism)
            \item questio for generic Minkowski sums
        \end{itemize}
        \item Edge length perturbation (Matthias)
    \end{itemize}
    \item Methods part
    \begin{itemize}
        \item second-order rigidity check (Gröbner bases, ...) (Albert)
        \item Computing deformation paths (also works for changing edge lengths but we don't mention this here maybe???)  (Matthias)
    \end{itemize}
    \item Case studies (results)
    \begin{itemize}
        \item Dodecahedron
        \begin{itemize}
            \item not first-order rigid (five dim space)
            \item proof of second-order rigid (not prestress stable)
            \item numerical experiments on edge length perturbations and what they might entail (Matthias) 
            \item no global rigidity (Matthias)
        \end{itemize}
        \item Truncated Icosahedron (Matthias + Martin)
        \begin{itemize}
            \item Five first-order flexes
            \item Still second-order rigid
        \end{itemize}
        \item Truncated dodecahedron (Matthias + Martin)
        \begin{itemize}
            \item unclear rigidity
            \item NOT second-order rigid (evidence?)
            \item we believe it is flexible ???
            \item have potential deformation paths
        \end{itemize}
    \end{itemize}
    \item Outlook (Martin)
    \begin{itemize}
        \item (questions about edge-length perturbations -- maybe already in theory part)
        \item is there specific structure in the TDod that helps us to see it is rigid/flexible and construct the flex
        \item Are there general stronger methods for deciding rigidity and constructing deformations
    \end{itemize}
    \item Supplementary material
    \begin{itemize}
        \item computational output (Gröbner bases etc)
        \item Code, algorithms
        \item Animations
    \end{itemize}
\end{itemize}

\tempnewpage % temporary new page

Main results:
\begin{itemize}
    \item carefully define first- and second-order rigidity and prestress stability for this setting.
    \item this gives a strong test for rigidity (resolves previously open cases).
    \begin{itemize}
        \item dodecahedron
        \item truncated icosahedron
        \item checked all Archimedean solids and duals (resolved all but one) 
    \end{itemize}
    \item very interesting special case: truncated dodecahedron (TDod)
    \begin{itemize}
        \item we believe it is flexible (for now)
    \end{itemize}
    \item something about edge length perturbation?
    \item edge length perturbations of the dodecahedron: we find there is a singularity in the ``dual space'' (rigidity transition region is algebraically singular)
    \item dodecahedron is an example that we don't have global rigidity
    \item maybe something about zonotope flexes
\end{itemize}

\hrulefill

\begin{itemize}
    \item many examples of rigidity
    \begin{itemize}
        \item short edges make rigid
        \item higher dimensions + first-order rigidity in higher dimensions
    \end{itemize}
    \item second-order rigidity
    \begin{itemize}
        \item second order rigid implies rigid
        \item Q: does second-order flexibility imply proper flexibility?
        \item $\#stresses=\#flexes$ trivial or worth mentioning?
    \end{itemize}
    \item the dodecahedron example
    \begin{itemize}
        \item affine trafos do not preserve first-order rigidity
        \item there is no global rigidity for polytopes in 3D
    \end{itemize}
    \item many other open questions
    \begin{itemize}
        \item Q: does flexibility need parallel edges?
    \end{itemize}
\end{itemize}

Notes on Archimedean solids:
\begin{itemize}
    \item the only Archimedean solids that are inf-flexible but not generic Minkowski sums are the dodecahedron, truncated dodecahedrona (4 flexes) and truncated icosahedron (5 flexes). Where do we lose the flex on the way from truncated dodecahedron to dodecahedron?
    \item Are they second-order rigid? Can the dimension of their flex spaces and their second-order rigidity be explained in some way using the known properties of the dodecahedron? (Limit argument?)
    \item Are there continuous motions between Archimedean/Catalan/Platonic solids thats preserve the planarity of facets and the edge lengths?
\end{itemize}

Other notes
\begin{itemize}
    \item A zonotope is highly flexible, but is there a zonotope that can flex in more ways than just deforming into other zonotopes, either real or infinitesimally?
    \item If $P$ and $Q$ have first-order flexes, then does $P+Q$ inherit them in some way?
\end{itemize}
\tempnewpage % temporary new page


}

\fi








\tempnewpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is~a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and~a~\Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
%Evidently, every convex polytope $P$ gives rise to such a structure, which we call the combinatorial type of $P$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
%If $\mathcal P$ is the combinatorial type of a convex polytope $P$, this notion agrees with the usual edge graph of $P$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
Convenient for computations, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}
%
% \begin{align*}
% \realSp(\mathcal P)
% %=\realSp(V,F,\sim)
% &:=\left\{\!\!
% \begin{array}{l}
%     \bs p\:V\to\RR^d
%     \\
%     \bs a\:F\to\RR^d
% \end{array}
% \Big\vert
%     \begin{array}{rcl}
%     % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
%     \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,
%     \end{array}
% \!\right\}.
% \end{align*}
%
%Analogously, the \Def{convex realization space} is defined as%\todo{\mhsays{Do we need the convex realization space?}}
%
%\todo{\mwsays{Do we really need both notations? I would like to ditch the one with the subscript c.}\mhsays{We should keep the convex realizations in our assumption right? Or do we build a second-order theory for arbitrary point-hyperplane structures?}\mwsays{I will keep the convex ones and delete the subscript-c.}\mhsays{Do we need convexity for anything in this article?}}
%
\begin{align*}
%\begin{align*}
\real(\mathcal P)
%=\realSp_{\mathrm c}(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
%
%We shall write $P\in\real(\mathcal P)$
%\notodo{\mhsays{What does this sentence add?} \mwsays{Nothing. Removed it.}}
Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ does not allow facet hyperplane to pass~though the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

%\mwsays{Maybe move the below to edge length perturbation section? I think this is the first (and only?) place it is used.}\mhsays{Sure, we can do that. Might even call it configuration space?}

% and the \Def{reduced convex realization space} is defined as
% \begin{align*}
% \realRCvx(\mathcal P)
% :=\realCvx(\mathcal{P})\,/\,\mathrm{Iso}
% \end{align*}
%
%where $\mathrm{Iso}$ is the Lie group of Euclidean isometries of $\mathbb{R}^d$.

%\mwsays{Define $\realR(P)$ reduced realization space?}

%As we show in \Cref{sec:first_order},
%\todo{\mhsays{This is absolutely not clear and we spend quite some time to show that.}\mwsays{I am not sure what you mean. This statement is either trivial or false by \cref{res:new_notion}}\mhsays{How the group action works on $\mathbf{a}$ is only explained in Section 4 and was subtle, so using ``clearly'' here is somewhat dishonest. I would suggest writing something like ``As we show in \Cref{sec:first_order}, the Lie group...}}
The \Def{Lie group of Euclidean isometries} (\ie\ rotations and translations), denoted $\Iso$, acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
%\qquad 
%\realRCvx(\mathcal P)
    %:=\realCvx(\mathcal%{P})\,/\,\mathrm{Iso}
\end{align*}

\iffalse % edge-length measurement map

\todo{\mwsays{This here is not the place for metric stuff. This is what the next section is for. I will move this later}}
\todo{\mhsays{If you want, we can call $\realR$ $\conf$ (the configuration space) instead and use something like $\textsc{M}\conf$ for $\mreal^*$, the metric configuration space.}}
Since in this article we are considering polytopes whose edge lengths are fixed, we also define the \Def{edge-length measurement map} as
\[m_E:\mathbb{R}^{dV}\rightarrow \mathbb{R}^E,\quad m_E(\bs p) = \left(\|p_i-p_j\|^2\right)_{ij\in E},\]
which lets us define the \Def{edge-length realization space}
\[\mreal(\mathcal{P},P)\,=\,\real(\mathcal{P})\,\cap\, m_E^{-1}\left(m_E(\bs p)\right),\]
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are fixed according to the realization $P$. The preimage of a given edge length vector is a real algebraic set, as its given by all realizations which satisfy a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}). \todo{\mhsays{Briefly talk about relation to $I$-rigidity?}}

\fi










% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

%\notodo{\mhsays{Maybe have this as section 2.1 instead? This section is quite short.}\mwsays{Yes, maybe. I think about it.}}
We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.


% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
% \label{def:continuous-rigidity}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
%\todo{\mhsays{Use $\mreal{\mathcal P}$ instead of ``equivalent'' to help distinguish the concepts?} \mwsays{This feels the wrong way around.}}
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, the Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
% \end{definition}
%
%\mwsays{Define configuration space $\conf$ and reduced configuration space $\conv^*$.}
%\mwsays{Define the \Def{metric realization space} $\mreal(P)$ (and reduced $\mreal^*(P)$) and replace below occurrences of $\conf(P)$ by it.}
%
For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks.
Consequently, much of what we say here applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}
%This also applies to the subsequent section, which develop a first- and second-order theory for polytopes, but are applicable more generally.

% Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% %
% A \Def{motion} of $(\bs p,\bs a)$ is a curve $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$;
% the motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% A non-trivial motion is called a \Def{flex}.
% If a realization $(\bs p,\bs a)$ has a flex, then we call it \Def{flexible}, and \Def{rigid} otherwise.

% {\color{lightgray}

% \begin{remark}
%     \mwsays{?? Simulating polytope rigidity via stacking prisms on faces.}
%     \mhsays{I'd say we leave it out.}
% \end{remark}

% }








\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a geometric constraint system studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence~provides heuristics and criteria that can be efficiently checked in practice.
%Investigating the first-order properties of a system comes down to the study of its \emph{rigidity matrix}.
%The first-order theory for polytopes is analogous to point-hyperplane frameworks, so the theory developed in this section applies verbatim to the more general case.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
    %\label{fig:placeholder}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from the rigidity~matrix.
%$p_i$ should be thought of as the coordinate of vertex $i$, and $a_\sigma$ the corresponding vertex of facet $\sigma$ in the polar dual of $P$.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    % \label{eq:flex_at_face}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    % \\
    % \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    % \label{eq:flex_at_face}
\end{align}
%
%\todo{\mwsays{Here we could say that $\bsdot a$ is determined by $\bsdot p$. Then it becomes clearer why trivial only needs to be specified on the $p$-part. This is however only true for our polytope setting and not general point-hyperplane frameworks. So we should be cautious claiming generality.}}
%
Similar to the framework setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also, that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).

%\todo{\mwsays{Turn the lemma into a short remark, maybe without proof and point to the proof below.}}

\iffalse % lemma that adot determined by pdot

{\color{lightgray}\small
\begin{lemma}
    \label{res:p_determines_a}
    The $\bsdot p$ uniquely determine the $\bsdot a$.
\end{lemma}
%
\begin{proof}
    For fixed $\sigma$ choose a basis $p_{i_1},..., p_{i_d}$ among the $p_i,i\sim \sigma$ (we can always do this in our setup).
    Then $\dot a_\sigma$ is the unique solution of the linear system $\<\dot a_\sigma,p_{i_k}\>=-\<\dot p_{i_k},a_\sigma\>$ for all $k\in\{1,...,d\}$.
\end{proof}
}

\fi % lemma that adot determined by pdot

First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any vertex $i\in V$ and facet $\sigma\in F$}.
    % \label{eq:trivial_motion_facet}
    %\\
    %\<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any $i\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    %\\
    %\<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%\mhsays{Potentially we will need $i\sim \sigma$ in $(4.4)$ as well (analogous to (4.2)). The possible trivial inf motions are already restricted to the Lie algebra of the Euclidean isometries (i.e. infinitesimal rotations and translations) by $(4.3)$ and the normals move automatically in first order alongside the vertices. By restricting the flexes further, we may make the equation impossible to satisfy (see computation below). It should be sufficient to have a complete graph as the 1-skeleton and the normals are immediately determined in first order. I don't mind $(4.5)$, but I don't think it adds much. Also, I don't quite understand where (4.5) comes from.}
%\mwsays{Let's delete (4.4) and (4.5).}
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    %The trivial first-order motions of a $d$-dimensional polytope $P$ form a vector space $\mathcal T_P$ of dimension $\binom{d+1}{2}$. 
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    %By assumption $P$ has non-empty interior, so we can assume that $\bs p$ is affinely spanning.
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    % \mhsays{I think it is necessary to at least show that 4.4 and 4.5 are satisfied to complete the proof. For a trivial motion, it holds that \[\langle S p_i+t,a_\sigma\rangle+\langle p_i,S a_\sigma\rangle= \langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle + \langle a_\sigma,Sp_i\rangle=\langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle - \langle p_i, Sa_\sigma\rangle=\langle t,a_\sigma\rangle\]
    % (for (4.5) this works). Of course, this is an issue, because in general this is $\neq 0$. Instead, we take a diagonal matrix $F(t)\in \mathbb{R}^3$ with positive eigenvalues, which is responsible for scaling ${\bs a}$. We require $\bsdot{a}=F(t)\cdot S \cdot {\bs a}$ and compute according to $(4.4)$
    % \begin{eqnarray*}
    % &~&\langle S p_i+t,a_\sigma\rangle+\langle p_i,F(t)\cdot S\cdot a_\sigma\rangle= \langle t, a_\sigma\rangle + \langle p_i,(F(t)-I)\cdot S \cdot a_\sigma\rangle \overset{!}{=}0\\
    % &\Rightarrow & \left(t+(F(t)-I)\cdot S \cdot p_i\right)\T \cdot a_\sigma=0 \quad\left(\Rightarrow t+(F(t)-I)\cdot S \cdot p_i \perp a_\sigma \right)
    % \end{eqnarray*}
    % for arbitrary choices of $t$ and normals $a_\sigma$; since $P$ is affinely spanning, the normals $a_\sigma$ generate $\mathbb{R}^3$ as a vector space. Therefore, 
    % \begin{eqnarray*}
    % S\cdot F(t)\cdot p_i=S\cdot p_i+t~\Rightarrow ~\underbrace{(F(t)-I)}_{=G(t)}\cdot \left( S\cdot p_i \right) = t
    % \end{eqnarray*}
    % for each $i$, since $S$ is not invertible in odd dimensions. This equation essentially needs to be solved for all points $p$ on the hyperplane $\mathcal{H}_\sigma$ with normal $a_\sigma$ which is spanned by the points $p_i$ with $i\sim \sigma$ (here is the exact point where problems occur when we take into account $(4.4)$, since the hyperplane is not defined and we compute on $\mathbb{R}^3$ instead). This equation is overdetermined. The main question is: why does the result for a specific point on $\mathcal{H}_\sigma$ generalize to all points on $\mathcal{H}_\sigma$??? \\[2mm]
    % For $(4.5)$ it holds that 
    % \[\langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle + \langle a_\tau, F(t)\cdot S \cdot a_\sigma\rangle = \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle - \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle = 0\]
    % due to the skew-symmetry of $S$ and diagonality of $F(t)$.}
        %Hence, $\mathcal T\simeq\mathcal T_F$ and the claim follows.
    %\mhsays{Also, I think we should give an argument that this is indeed a linear space and not an affine-linear space or a union of such spaces; contrary to the bar-joint equations, (4.2) vaguely resembles $Ax=b$. Nevertheless, we now have variables $\dot{a}$ and $\dot{p}$, so we can rewrite Equation (4.2) as $\langle \dot{p}_i\times \dot{a}_\sigma,  a_\sigma\times p_i\rangle=0$, which implies that the space is indeed linear.} \mwsays{I don't understand. The equations are linear so the solution spaces are linear.}
    %\mwsays{We should choose $\dot a_\sigma$ as the solution of $\<\dot a_\sigma, p_i\> = \<Sp_i+t,a_\sigma\> = \<p_i, S a_\sigma\> + \<t,a_\sigma\>$ over all $i\sim\sigma$. Choose a basis among the $p_i,i\sim\sigma$ to get a candidate solution. Then use that all other $p_i$ are in the affine span of this basis and that the equations are affinely covariant and hence do indeed have a solution that works for all $i\sim\sigma$. Then it satisfies (4.2), and we delete (4.4) and (4.5).}
    %
    %It suffices to show that each $\bsdot p\in\mathcal T_F$ extends to a polytopal first-order motion $(\bsdot p,\bsdot a)$.
    %
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}

\iffalse

\todo{\mhsays{Prove that trivial flexes have the correct dimension? Clearly, space of inf flexes is contained in framework inf flexes by construction. Apply Asimow-Roth $\Rightarrow$ ``$\leq$''. Construct Inf flexes: skew-symmetric $Q$, translation $T$; on vertices: $Qp(i)+T$, on normals $Qa(\sigma)$.}}

{\color{lightgray}

\begin{observation}
    If a facet $\sigma\in F$ is a simplex, then the left hand side of \eqref{eq:stress_at_face} is a linear combination of $d$ linearly independent vectors in $\RR^d$. 
    This can be zero only if all coefficients are zero.
    Hence, $\eta_{i\sigma}=0$ for all $i\sim\sigma$.

    Thus, if the polytope is simplicial, then all facet stresses are zero and the stress is a pure classical framework stress. Due to a theorem of Dehn, convex simplicial polytopes cannot have a non-zero framework stress. \mwsays{True in $d\ge 4$?}\asays{the 16-cell (cross-polytope) has 8 vertices and 24 edges and hence has two self-stresses. In general, there are many stresses, I think}
\end{observation}
}

\fi

%Since $\mathcal T_P\subset\ker \mathcal R(P)$, it 

\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    %\asays{below we use infinitesimal rigidity. Let's choose one throughout} 
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
    %\mwsays{I prefer ``first-order rigid'' because it is more consistent with ``second-order rigid''. Using ``first-order rigid'' and ``corank'' would be consistent with the other paper.}
\end{corollary}
%
%\todo{\mhsays{First prove inf rigid $\Rightarrow$ regular point in realization space. Then use Riemannian geometry. (see also Asimow-Roth)}\mwsays{Why did we need this complicated stuff again?} \mhsays{Yeah, I agree that it doesn't seem to be necessary anymore. I think the ``complexity'' happens in 4.1.}}
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
    %
    %\qedhere
    
    %By \cref{res:trivial_dim} $\corank \mathcal (P)\ge \binom{d+1}{2}$.
    % If $P$ is first-order rigid, all its first-order flexes are trivial, that is, $\ker \mathcal R(P) \subseteq\mathcal T$. Hence $\ker \mathcal R(P)=\mahcal T$ and the claim follows from \cref{res:trivial_dim}.

    % \TODO\ \mwsays{Maybe not true if $P$ is not affinely spanning. But we are always spanning. Cite a paper by Bernd, Bill, Tony, ... for this}\asays{it's not formally proved there, but I think we can still reference it. I do agree we need spanning. If the joints are spanning, then this statement is pretty clear I think. We have a non-trivial first-order flex iff kernel has dimension larger than ${d+1}\choose 2$}
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:

% \mwsays{In the theorem below, should we go for the differential geometry proof?}
% \mhsays{I think it's fine. The proof technique is pretty standard in rigidity theory.}
% \mwsays{I try to formulate the differential geometry argument. See Matthias' paper.}

% \begin{theorem}
%     % \label{res:second-order-implies-rigid}
%     % \label{res:first_order}
%     If a polytope is first-order rigid, then it is rigid.
% \end{theorem}
% %
% \begin{proof}
%     Observe that $\mathcal R(P)$ is the Jacobi matrix of the constraint system. %If its rank is maximal, then this implies that $\real(\mathcal P)$ is smooth at $P$.
%     \mwsays{We currently have no name for the space of all realizations with prescribed edge lengths.}
% \end{proof}

\begin{theorem}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}

%\notodo{\mhsays{I would say we refer to the Corollary 6.6.}\mwsays{I added a reference. Though I also see educational value in seeing the first- and second-order theory proofs side by side and observing that they are so similar. I know I found this interesting.}}

This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends in $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms~of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a maximal~number $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    The converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}



% {\color{gray}
% \todo{\mwsays{I think this text would fit better in \cref{sec:selected_results}}\mhsays{I agree. Can you move it?}\mwsays{Okay, I will}}

% Dehn's theorem \cite{dehnstheorem} proves that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
% Later, we encounter plenty of non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
% Currently no theoretical tools are available that would identify these as rigid a priorily.
% We therefore formulate the following question:

% \begin{question}
%     %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
%     Can we extend Dehn's theorem to some classes of non-simplicial polytopes? 
%     That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
% \end{question}

% Natural candidates are polytopes whose faces are triangles and 4-gons.
% See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

% }



\iffalse % Albert's proof

{\color{lightgray}

\begin{proof}
    %\textcolor{red}{Add proof here}
    We prove the contrapositive: if $P$ is flexible, then it is first-order flexible. 
    Let $P^t$ be a flex. \todo{\mwsays{I think we need to invoke curve selection to get an analytic flex}} 
    Since $P^t$ is non-trivial, there is some minimal order $k$ for which truncating the Taylor expansion of $P^t$ at this order does not look like the truncation of a trivial motion.
    %we can truncate the Taylor expansion of $P^t$ at some order, say $k$, after which it cannot be completed to a trivial motion by adding higher order terms. 

    We expand the $k$-th derivative of the constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}\!(p_i^t-p_j^t)\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}\!(p_i^t-p_j^t)=0.
    \end{equation*}
    %
    For the coplanarity constraint \eqref{eq:flex_at_vertex_face} at $i\sim\sigma$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell} \!p_i^t\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell} \!\!a_\sigma^t=0.
    \end{equation*}

    Since $k$ was chosen minimal, we can add a suitable trivial motion to cancel all terms of order up to $k-1$. The two equations above become the following. 
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!(p_i^t-p_j^t)=0
    \end{equation*}
    and 
    \begin{equation*}
        p_i^t \cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!a_\sigma^t+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!p_i^t \cdot a_\sigma^t=0
    \end{equation*}
    The $k$-th derivative satisfies the same equation as a first-order flex does.\todo{\mwsays{I don't think this is clear from what we know so far.}} Therefore, $P$ is first-order flexible. 
\end{proof}

}

\fi

\iftrue % polyhedra rigidity stresses first-order theory

%\tempnewpage

\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second, and equally important, first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
%(recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a Hookean spring with a spring constant given by the stress $\omega_{ij}$ at $ij\in E$. The spring constant determines the magnitude of the force with which the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

% Stresses have no counterpart to ``trivial'' motions

Like first-order flexes, stresses form a linear space -- the \Def{stress space}.
Stresses~are particularly relevant in second-order theory (see \cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).

%One fact that makes 3-dimensional polytope rigidity tractable as compared to dimension $d\ge 4$ is that first-order rigidity can be expressed purely in terms of stresses.

\begin{proposition}
    \label{res:flex_eq_stress}
    If $P \subset\RR^3$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%
%\notodo{\mhsays{I think it would be cleaner to simply move this comment after the proof.} \mwsays{I like to comment on results before everybody got drained out by the proof. I consider the proof as a nice addendum but nothing crucial for reading. Matter of taste I guess.} \mhsays{This is not important to me. The way I read a paper is I usually skip the proof and read the comments first, but like you said, matter of taste. Why I wanted to move the text is so that before section 4 there is not such a weird gap anymore after the $\square$.}}

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]
    %We first show that for $\mathcal R(P)$ holds $(*)$ $\text{$\#$rows}=\text{$\#$columns}-6$.

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}

% \begin{corollary}
%     \label{res:rigid_eq_stress_free}
%     A polyhedron is first-order rigid if and only if it has no non-zero stress.
% \end{corollary}


The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.


\fi


\iffalse

\hrulefill

\begin{lemma}
    For $\mathcal R(P)$ holds $\text{$\#$columns}=\text{$\#$rows}+6$.
\end{lemma}
%
\begin{proof}
    Let $v,e$ and $f$ be the number of vertices, edges and faces of $P$ respectively.
    
    For each vertex, the number of incident faces equals the number of incident~edges. Thus, the total number of vertex-face incidences in $P$ is equal to the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we arrive at
    %
    \begin{align*}
        \text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
\end{proof}

\mhsays{Add the property that $\# flexes = \# stresses$ for polytopes?} \mwsays{Only true for $d=3$, and yes we should mention this.}

\fi


% \subsection{Flex space dimensions}
% \label{sec:flex_space_dim}

% \mwsays{Delete this section.}















% \tempnewpage % temporary new page

\section{Second-order theory}
% \section{Second-order rigidity and prestress stability}
\label{sec:second_order}
\label{sec:second-order-theory}

%\notodo{\mhsays{Segue from previous section. We now consider arbitrary polytopes again? Or exchange Sections 5 and 6.}}
Second-order rigidity theory investigates deformations that preserve constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
%Sometimes, the polyhedron can still be rigid even if it is not first-order rigid. 
%Rigidity beyond first order is often difficult to test even for bar frameworks. 
%
For that, we follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if $(\bsdot p,\bsdot a)$ form a first-order motion and additionally it holds 
%
%\notodo{\mhsays{Don't we also need that $\dot{P}$ is a first-order flex?}\mwsays{Thanks! Fixed.}}
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$}
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
%Analogous to what was observed in \Cref{sec:first-order-theory}, the $\bsddot a$ are automatically determined by the $\bsddot p$ in this setting
%\todo{\mwsays{Is the sentence about $\bsddot a$ being determined by $\bsddot p$ necessary?}\mhsays{Not really. We can remove it.}}.
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

%\todo{\asays{I think we deleted what it means to be non-trivial in this case. An issue is that $(0,\bsdot p)$ would be non-trivial for a non-trivial first-order $\bsdot p$ if you are not careful, but it doesn't tell us anything other than the first order motion being non-trivial. A clear definition would be a second-order motion with nontrivial first-order terms.}\mwsays{Oops, true, this got deleted. Will fix.}}
%\mwsays{I previously introduced commands to render $\bs p, \bsdot p, \bsddot p$ (see TeX code for commands) in place of $\mathbf{\ddot{p}}$; again, this would be consistent with the first paper. In any way, I recommend to use the command, we can change its appearance later if desired.}

% Let $\dot P,\ddot{P}$ be the vectors $(\dot{p}_1,...,\dot{p}_{|V|},\dot{a}_1,...,\dot{a}_{|F|})$, $(\ddot{p}_1,...,\ddot{p}_{|V|}$ and $\ddot{a}_1,...,\ddot{a}_{|F|})$ correspondingly. We can now define the second-order flex:
%\mhsays{I suggest using textit and a pale color (\eg\ blue) for definitions instead of bold font. That makes it distinguishable from Definitions/Theorems} \mwsays{I imported the command \texttt{\textbackslash Def} for this. It renders \Def{like this}. Feel free to modify.} \mhsays{Looks good!}

% \begin{definition}\label{sorigid}
%     The pair $(\dot{P},\ddot{P})$ is a \Def{second-order flex} if equations \eqref{eq1} and \eqref{eq2} are satisfied. A second-order flex is \Def{non-trivial} if $\dot{P}$ is not a trivial first-order flex. The polyhedron $P$ is \Def{second order flexible} if there exists a non-trivial second-order flex. Otherwise, we say that it is \Def{second-order rigid}.
%     %\mwsays{Use eqref for referencing equations. Use cref for everything else.}
% \end{definition}

% \begin{remark}
%     Notice that we are not defining trivial second-order flexes as the first and second derivatives of trivial flexes. The reason is that while it is possible to build a non-trivial flex with a trivial first derivative, it is not interesting because $\ddot P$ is simply identical to a non-trivial first-order flex, as the proof of \cref{res:second-order-implies-rigid} shows. Therefore, we only need to look at the case where $\dot{p}$ is non-trivial. 
%     \todo{\mwsays{Not really clear}}
% \end{remark}

% \mhsays{We should fix a notation about the realization ${\bs p}, P, ({\bs p},{\bs a})...$ and keep it consistent throughout the article.}
% \asays{Since we defined $P=(\mathbf p,\mathbf a)$, I defined $\dot P$ and $\ddot P$ analogously.} \mwsays{I am fine with using $P$ and $(\bs p,\bs a)$ (and the dotted variants) almost interchangeably. But I also find it weird to use $\dot P$ as a vector.}

%\mhsays{Are the $\ddot{a}$ automatically determined by the $\ddot{p}$? $\Rightarrow$ write a lemma about it?} \mwsays{They are. We have no lemma for this in the first-order case, just a sentence. If it is not needed, let's keep it at the one-sentence-level, no?}\mhsays{ok.}

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    \label{res:second-order-implies-rigid}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking the curve selection lemma \cite[Lemma 18.3]{algebraicapproximationcurves}, we obtain an analytic flex $P^t$.
    There is then a maximal number $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \,\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j),\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i,\, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,\,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:second-order-implies-rigid}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system.
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently whether $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.

\iffalse % stresses

% \subsection{Equilibrium Stresses}
% \label{sec:stresses}

%The test is based on the notion of equilibrium stresses, which we introduce next.

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system. 
We denote them by pairs $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$ (recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ sake of brevity and call it a \Def{polytope stress}.

\mwsays{Remark: first-order rigid iff no stress. (and then make this its own equilibrium stress subsection). Maybe move stresses to first-order theory.}\mhsays{Maybe as Proposition?}

%\begin{remark}
%\label{res:stress_eq_flex}    
%\end{remark}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

\fi





% Equations \eqref{eq1} and \eqref{eq2} can be compactly written as a single equation:
% % \begin{equation*}
% %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
% % \end{equation*}
% %
% \begin{equation}\label{eq:compact}
%     \mathcal R(P)\cdot \ddot{P}+\mathcal R(\dot{P})\cdot \dot{P}=0
%     % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
% \end{equation}
% %
% Recall that we use $P$ interchangeably with $(\bs p,\bs a)\in \RR^{dV}\oplus\RR^{dF}$, and analogously~with $\dot P$ and $\ddot P$.
% %
% Now, given a second-order motion $(\dot P,\ddot P)$ and any stress ${\bs \xi}$, we obtain
% %
% \begin{equation}
%     \label{eq:with_stress}
%     {\bs \xi}\T \left(\mathcal R(P)\cdot \ddot P+ \mathcal R(\dot P)\cdot \dot P\right)=0.
% \end{equation}
% %
% %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
% Since ${\bs \xi} \in \ker \mathcal R(P)\T$ by definition of stress, we have ${\bs \xi}\T \mathcal  R(P)\ddot P=0$.
% Equation \eqref{eq:with_stress} then becomes ${\bs \xi}\T \mathcal  R(\dot P)\dot P=0$. We say that a stress $\bs\xi$ \Def{blocks} a first-order motion $\bs P$ if
% %
% $${\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0$$
% %Next, we move on to the second-order duality which can be useful when we want to prove $\ddot{P}$ does not exist. 


\iffalse 
Before that, we first introduce the following equality form of Farkas' lemma:
    \begin{lemma}\label{farkaseq}
        \mwsays{Maybe just use it in the proof and don't list it as a separate lemmas.}\mhsays{I don't mind the Lemma here tbh. }
        Either $Ax=b$ has a solution, or $A^Ty=0$ has a solution with $b^T y\not =0$.
    \end{lemma}
    Intuitively, this Lemma says that either $b$ is in $A$'s column space, or there exists a hyperplane containing the column space of $A$ and $b$ is not in it. 

\begin{lemma}\label{lem2}
    Given a first-order flex $\dot P$, if and only if there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
        {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
    \end{equation}
    then there cannot be a $\ddot P$ such that $(\dot P,\ddot P)$ is a second-order flex. 
    ${\bs \xi}$ is called a \Def{blocking stress} for $\dot P$ if Inequality $\eqref{block}$ holds. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
\end{lemma}
\begin{proof}
    The ``if'' direction is already given in the discussion above. To show ``only if'', we use \cref{farkaseq}.
    %\mhsays{I don't like using the theorem environment in a proof} 
    Let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$. Then \cref{farkaseq} says that either there exists a $\ddot P$ or you can find a blocking stress. 
\end{proof}
\fi

%The following test is an elegant application of Farkas' lemma:

\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

% \begin{lemma}\label{lem2}
%     Let $\dot P$ denote a first-order flex of a polytope $P$. Then there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
%         {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
%     \end{equation}
%     if and only if there is no $\ddot P$ for which $(\dot P,\ddot P)$ is a second-order flex. If $\eqref{block}$ holds,
%     ${\bs \xi}$ is said to \Def{block} $\dot P$. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
% \end{lemma}
\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    % \begin{equation*}
    %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
    % \end{equation*}
    %
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

    
    % This system has the form $A\ddot P=b$ for $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$.
    % By Farkas' lemma, the non-existence of a solution for $\ddot P$ (and hence, second-order rigidity of $P$) is equivalent to the existence of a solution of the system $A\T \bs \xi=0$ for some $\bs\xi$ with $\bs\xi\T b=0$, that is,
    % %
    % $$\mathcal R(P)\T \xi=0,\qquad \bs\xi\T\mathcal R(\sot P)\dot P\not=0.$$
    
    % For an arbitrary stress ${\bs \xi}$ therefore holds
    % %
    % \begin{equation}
    %     \label{eq:with_stress}
    %     0 = {\bs \xi}\T \left(\mathcal R(P) \ddot P+ \mathcal R(\dot P) \dot P\right) = 
    %    \underbrace{ {\bs \xi}\T \mathcal R(P)}_{=0} \ddot P+ 
    %     {\bs \xi}\T\mathcal R(\dot P) \dot P={\bs \xi}\T\mathcal R(\dot P) \dot P.
    % \end{equation}
    % %
    % %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
    % where ${\bs \xi}\T \mathcal  R(P)=0$ follows from the definition of a stress as an element of $\ker \mathcal R(P)\T$.
    % We see that $\dot P$ cannot be blocked by any $\bs \xi$.
    
    % To show ``only if'', let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$ and consider the two linear systems $Ax=b$ and $A\T y = 0$. We apply a linearized version of Farkas' Lemma, which implies that either $Ax=b$ has a solution, or $A\T y=0$ has a solution with $b\T y\not =0$.
    % In other words, there either exists a second-order flex $\ddot P$ or it is possible to find a blocking stress. 
\end{proof}

    % By combining the definition of second-order rigidity and \cref{lem2}, we can obtain the following result:
    % \begin{theorem}\label{res:sotest}
    %     $P$ is second-order rigid if and only if every non-trivial first-order flex has a blocking stress. 
    % \end{theorem}%\mhsays{Formulate as a theorem? This seems to be what people are usually doing in second-order rigidity papers, right?} 

In following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 

% The following notion is often more convenient to use:

%\todo{\mhsays{Expand on the relevance of prestress stability and that it is connected to second-order rigidity by swapping quantifiers?}}

% \begin{definition}
% \label{def:prestress-stable}
%     If there exists a stress that blocks every non-trivial first-order flex, we say the polyhedron is \Def{prestress stable}.
% \end{definition}

\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}

\iffalse

{\color{lightgray}

\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    
    Let $k$ be the smallest integer such that the first $k$ derivatives of $P^t$ do not come from a trivial flex at $t=0$. The $2k$-th derivative of the constraints can be expanded as:
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(a_k^t)=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $k$ is the smallest integer, the first, second, all the way up to $k-1^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to the $k-1^{th}$ are all zeros. The two equations above become the following. 
    %
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t-p_j^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    and 
    %
    \begin{equation*}
        (p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(a_k)+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t)\cdot (a_k^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t)\cdot\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(a_k)=0
    \end{equation*}
    %
    Set $\dot P= \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}P^t\big|_{t=0}$ and $\ddot P=2/\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}P^t\big|_{t=0}$. The two above equations become Equations \eqref{eq1} and \eqref{eq2}. Therefore, if $P$ is flexible, it has a non-trivial second-order flex. 
    \mwsays{It remains to show that the motion is non-trivial.}
\end{proof}

}

\fi














\iffalse % previous first-order section

\tempnewpage

\subsection{First-order theory}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.


A \Def{first-order motion} $(\bsdot p,\bsdot a)$ of $P$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$, %=(\dot p_i\in\RR^3:i \in V;\, \dot a_\sigma\in\RR^3 : \sigma \in F)$.
that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    %\label{eq:flex_at_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    %\label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    %\label{eq:flex_at_face}
\end{align}

A first-order motion is \Def{trivial} if in addition it satisfies
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    %\label{eq:trivial_motion_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
A non-trivial first-order motion is called a \Def{first-order flex}.
A framework is \Def{first-order rigid} if it has no first-order flexes; it is \Def{first-order flexible} otherwise.
Many results from the bar-joint framework setting transfer in the expected way. In particular, if a polytope is first-order rigid, then it is rigid. 

The first-order flex conditions \eqref{eq:flex_at_vertex} -- \eqref{eq:flex_at_face} can be collected in a corresponding \Def{rigidity matrix} $\mathcal R(P)$ % with dimensions $(E+\VF)\times(dV+dF)$. 
which satisfies $\mathcal R(P)(\dotbs p,\dotbs a)=0$ if and only if $(\dotbs p,\dotbs a)$ is a first-order motion.
%
Since we only consider polytopes with non-empty interior, they are in particular affinely spanning and
the rank condition of first-order rigidity applies: 

\begin{lemma}
    \label{res:rank_condition}
    We have
    %
    $$\corank \mathcal R(P) \ge \binom{d+1}{2},$$
    %
    with equality if and only if $P$ is first-order rigid.
\end{lemma}

\hrulefill

%\begin{definition}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
We write
%
\begin{align*}
    \realP{\mathcal P}P &= \realpa{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \real(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
    \\
    \realPCvx{\mathcal P}P &= \realpaCvx{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \realCvx(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
\end{align*}
%
for the (\Def{convex}) \Def{configuration space}, \ie\ the space of all (convex) realizations equivalent to a given (convex) realization $P=(\bs p,\bs a)$.

A \Def{motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\realpa{\mathcal P}{\bs p}{\bs a}$ for which $(\bs p^0,\bs a^0)=(\bs p,\bs a)$.
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all~$t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, we call it \Def{flexible}, and \Def{rigid} otherwise.
%\end{definition}

In general, understanding the full configuration space is intractable in all but the simplest cases. 
We mention here a few situations in which such a full understanding is possible due to various genericity assumptions.
In our language, Cauchy's classical rigidity theorem \cite{cauchy1813} states that $\realPCvx{\mathcal P}P$ is a single point whenever $\mathcal P$ is a simplicial polytope.
As a consequence of the main result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} we also obtain the following:

\begin{theorem}
    Let $\mathcal P$ be the combinatorial type of a 3-dimensional polytopes (\ie\ a polyhedral graph).
    Then for almost all convex (in fact, Zariski convex) realizations $P$ of $\mathcal P$ holds: $\realP{\mathcal P}P$ consists of finitely many isolated points.
\end{theorem}
%
Here, \emph{almost all} means that a dense open subset of the (Zariski closure of) the convex realization space has this property.
%
\begin{proof}
    \TODO \mhsays{$\real(\mathcal{P})$ may be irreducible, but that does not mean that $\real(\mathcal{P},P)$ is. The geometry of $\real(\mathcal{P},P)$ may be pretty complicated. We know that $P$ has generic coordinates; however, it seems like what we need to do is show that $P$ also has generic edge lengths. By going back to the edge length perturbation space and proving a stronger result than Proposition 5.2, we then may be able to prove this. The main issue is that we don't really understand the edge length measurement variety and much less the intersection of that variety with $\real(\mathcal{P})$. So I guess to conclude: I don't really have an easy idea how to approach this. You?} \mwsays{I cannot prove this at this moment. Maybe delete theorem?}
\end{proof}

We conjecture the same to be the case in higher dimensions.

Lastly, recall that a \Def{zonotope} is a polytope obtained as the Minkowski sum of finitely many line segments. A \Def{cubic zonotope} is a zonotope with all faces being combinatorial cubes. Cubical zonotopes are the zonotopal equivalent of simplicial polytopes, in the sense that they are generic in the class of zonotopes: they are generated from line segments in general position:

\begin{theorem}
If $P\subset\RR^d$ is a cubic zonotope generated from $k$ line segments, then %
$$\realP{\mathcal P}P = (\RR P^{d-1})^k.$$
\end{theorem}
%
\begin{proof}
    \TODO
\end{proof}

\fi








\iffalse % old flexible polytopes section by Martin

\tempnewpage % temporary new page

{\color{lightgray}

\section{Constructing flexible polytopes}
\label{sec:flexible_polytopes}

% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
%     Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% A \Def{continuous motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that
% \begin{itemize}
% \item $(\bs p^t(0),\bs a^t(0))=(\bs p,\bs a)$ and 
% \item $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% \end{itemize}
% The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% If a realization $(\bs p,\bs a)$ has a motion, then we call it \Def{flexible}, and \Def{rigid} otherwise.
% \end{definition}
As defined in \Cref{sec:rigidity}, a polytopal realization is flexible if it admits a non-trivial continuous motion.

\subsection{Zonotopes}

A zonotope is \Def{generic} if all its faces are combinatorial cubes. We call it generic because it generated from line segments in generic position. Generic zonotopes are the zonotopal equivalent of simplicial polytopes. For the latter the rigidity theory is classical -- they are rigid, both in first order and globally (Chauchy's and Dehn's theorem).
Likewise, for generic zonotopes a complete theory can be given.

\begin{theorem}
    Let $P\subset\RR^d$ be a rhombic zonotope with $n$ generators. Then
    %
    \begin{myenumerate}
        \item 
        $\realR(P)$ is a connected smooth variety of dimension $(d-1)n-\binom{d}{2}$.
        In particular, each polytope $Q$ combinatorially equivalent to $P$ with the same edge lengths can be deformed into $P$.
        \item if $Q\in\real(P)$ then $Q$ is a zonotope.
        \item The first-order flex space of $P$ has dimension $(d-1)n-\binom{d}{2}$.
        \item Each first-order flex of $P$ corresponds to a real flex.
    \end{myenumerate}
\end{theorem}
%
\begin{proof} \mwsays{Work in progress, these are just ``mental'' notes.}
    Consider the space of all deformations of a zonotope that preserves only coplanarity and central symmetry of the facets (the latter is in combinatorial cubes also implied by edge length constraints).
    Note that for $n$ generators there are $2\binom{n}{d-1}$ facets, and that the central symmetry of each is guaranteed by $d(d-2)$ equations: each pair of opposite vertices (of which there are $d-1$) must have a centroid identical to the centroid of the first pair; this is a vector identity with $d$ components.
    Note that this preserves coplanarity automatically.
    Likewise for an first-order flex -- there $dV$ DOFs and $2d(d-2)\binom{n}{d-1}$ constraints. Removing translations but not rotations, we obtain $dV-2d(d-2)\binom{n}{d-1}-d$ final first-order DOFs.
    Observe that the realization space is a manifold of dimension $nd$, or $n(d-1)$ if we want to preserve lengths. It is also well known that $V=2\sum_{k=0}^{d-1} \binom{n-1}{k}$.
    It remains to check
    %
    $$dV-2d(d-2)\binom{n}{d-1}-d = nd.$$
    %
    This seems to yield too few remaining DOFs ($< dn$) and so some of the constraints are redundant. Which and how many is unclear?
    
    \mwsays{Check that the fact that all inf flexes extend follows already from some general theory about realization spaces of polytopes when the realization spaces are smooth manifolds.}
\end{proof}

\begin{remark}
    More general zonotopes have non-zonotopal flexes. 
    As soon as some face of a zonotope is not a rhombus, then it is the Minkowski sum of this face with the other generators. But a polygon with more than four sides has a non-trivial (\ie\ not symmetry preserving) flex. Hence the Minowski sum of this flex with the other generators yields a non-zonotope.
\end{remark}

\begin{question}
    Is the first-order flex space of zonotopes exactly the tangent space to the finite flexes?
\end{question}

We can ask analogous questions for general Minkowski sums.

\begin{question}
    Is it true that the generic Minkowski sum (where no two faces, edge or higher, share an affine span) of rigid polytopes only has Minkowski flexes? Same first-order. More generally Is the first-order flex space of a Minkowski sum just the sum of the first-order flex spaces of the individual polytopes?
\end{question}

\subsection{Minkowski sums}

% We previously explained how \emph{generic} Minkowski sums become flexible polytopes.
% We can be more precise here.

% \begin{theorem}
%     Given polytopes $P,Q$, let
%     Let $\mathcal U$ be the set of linear subspaces of 
% \end{theorem}

Let $\mathfrak F(P)$ be the first-order flex space of $P$.

\begin{theorem}
    For a generic Minkowski sum of dimension $d\ge 3$ holds $\mathfrak F(P+Q) = \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$.
\end{theorem}
%
\begin{proof}
    \mwsays{This theorem is wishful thinking. It could be that a Minkowski sum has more (first-order) flexes than the ones that come from the summands. I think we know enough to show that $\mathfrak F(P+Q) \subseteq \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$. Maybe the other direction can be proven using some limit argument.}
\end{proof}

\mwsays{Not true in $d=2$ or for non-generic Minkowski sums, consider two triangles that add up to a hexagon, or prisms over those.}

\subsection{Truncation}

If two frameworks on the same graph have the same edge directions, then they have the same first-order theory since the rows in the rigidity matrix are just multiples of each other.
The following would be a generalization to polytopes:

\begin{theorem}
    If $P$ and $Q$ are normally equivalent, then $\mathfrak F(P)\simeq \mathfrak F(Q)$.
\end{theorem}
%
\begin{proof}
    \TODO
    \mwsays{True?} \mwsays{WRONG! TIco and TDod}
\end{proof}

\mhsays{We lose all flexes when changing the truncation of the truncated dodecahedron. Therefore, the flexes are not a result of the polytopes' symmetry, but rather of the coordinates. }

\subsection{Truncation}
Questions:
\begin{itemize}
    \item Does there exist a truncation in (0,1) preserving the flexes of either of the truncated ends?
    \item Is rigidity/flexibility preserved under certain assumptions on the truncation? 
\end{itemize}

}

\fi













\tempnewpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

%The convex realization space $\realCvx({\mathcal{P}})$ of 3-dimensional polytopes of combinatorial type $\mathcal{P}$ is a smooth $(E+6)$-dimensional manifold, on which the 6-dimensional Lie group of rigid motions acts smoothly. %In fact, the reduced realization space $\realRCvx(\mathcal{P})$ is homeomorphic to an open ball (\cf\ \cite[Thm.\ 13.3]{richter2006realization}). Intuitively, this claim \emph{has} to be true, simply by subtracting the appropriate dimensions. However, proving it is %\todo{\mwsays{Not only ``slightly more subtle'', but this is a big deal :D}}
%significantly more difficult than it seems, as we are working with manifolds and associated Lie groups instead of Euclidean space.

%\mwsays{We should start with emphasizing very clearly that this section will be $d=3$ only. This is the first place in the paper where we are not general-$d$.}
%\todo{\mhsays{I reference second-order rigidity in this section. Honestly, I would prefer to switch this section with the second-order rigidity; also, because we restrict ourselves to 3D here and later relax that assumption again.}\mwsays{I am torn. The current transition from ``second-order theory'' straight to ``certifying second-order theory'' is also nice. Where do you mention 2nd-order? Only in the question? Maybe move the question?} \mhsays{I don't think there is a place for the question other than here. I could write ``rigid, but not fo rigid'', which would fix the problem. However, my main issue is that we restrict to $\mathbb{R}^3$ and then revert the restriction in the coming section. That feels confusing and unnatural. But I also understand that second-order rigidity$\Rightarrow$ certifying is a nice order. Let's discuss!}}
%\notodo{\mwsays{Use polyhedron for 3-dim polytope. Also, convex is implicit everywhere.}}
For this section, we restrict ourselves to polyhedra, \ie\ 3-dimensional polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
%\notodo{\mwsays{I still think it is a bad idea to say we study the complement. We don't really. The complement is a terrible object. It is not a variety. I would say we study $\real(\mathcal P)$ locally.}}
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polyhedra, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to %\notodo{\mwsays{I am not sure I understand ``first-order flexes which only preserve the coplanarity constraints'', or if I do, I think this is misuse of terminology because flex has a well-defined meaning always fixing edge lengths. Otherwise it is a deformation, or a curve in $\real(\mathcal P)$, but not a flex. First-order terminology we don't have for this at all.}} 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization the trivial first-order motions form a 6-dimensional subspace of the space of first-order motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$. %For that reason, $\Iso$ acts smoothly on $\real({\mathcal{P}})$ and since $\realR(\mathcal{P})$ is given by a quotient manifold of the form $\real(\mathcal{P})/\mathrm{Iso}$, 
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension%\todo{\mwsays{$\real^*$ is a smooth manifold, but the reason given here is incorrect:quotients by smooth actions can fail to be smooth.}\mhsays{Not if the group acts smoothly, freely, and properly (see citation). Feel free to rewrite the paragraph though.}} (\cf\ \cite[Thm.\ 21.10]{lee-smooth-manifolds})
%
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
%\notodo{\mwsays{You want to pin a vertex, constrain an edge to a 1-dim subspace and a face to a 2-dim subspace. Pinning the edge sounds like restricting its length.}\mhsays{Adjusted.}}%
In other words, all polyhedra have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). %\todo{\mwsays{Not enough pinning. Maybe use Louis' paper? Or just pin an edge and an constraint a vertex to a plane that is in the same face as this edge.}} 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
%\todo{\mwsays{I would not call it a coincidence that $E$ is the number of edges}}
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. %\notodo{\mwsays{\emph{``This line of thought would imply that we can locally freely perturb the edge lengths around rigid realizations''} I think it is not clear why you mention ``rigid realizations'' in this sentence.} \mhsays{Changed the sentence.}} 
Since rigid realizations correspond to isolated points in $\mreal^*(\mathcal{P},P)$, the degrees of freedom in $\realR(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.

%\notodo{\mwsays{Can't we just define existence of edge-length perturbations as that ``the map from realizations to edge length vectors is locally surjective at $P$?} \mhsays{I do not believe this avoids the invariance of domain theorem. ``continuous'' plus ``locally surjective'' just rewords what is already there and abstracts the meaning. I am not necessarily against this change, I just don't believe it is going to be impactful.}}
    
\begin{definition}
\label{def:edge-length-perturbations}
%Fix an ordering of the edges $E$ for a polytope $P$. We denote 
The
 %\todo{\mwsays{maybe ``edge length vector'', since then perturbations are a more natural thing?}}
 \Def{edge length vector} of $P$ is given by
 %\notodo{\mwsays{Should we use $(a|b)$ instead of $(a : b)$ for consistency with the other text? Or are vectors significantly different to justify different notation from sets?}}
 %
% \notodo{\mwsays{I want to suggest notation: $\bs\ell(P)$ for the edge length vector, since consistent with other indexed families like $\bs p$. Also I think it is not good to have both $\ell(e)$ and $\ell_e$. I think we should use only $\ell_e$ since we call it a vector, and $\bs\ell'$ or so if we need another vector like in the paragraph below. Next, $\mathcal L(\mathcal P)$ can now be used for the space of edge lengths vectors. Or something like $\text{\textsc{Len}}(\mathcal P)$, but I think it would be useful to have notation since we write the phrase so often}}
 %
 %\notodo{\mwsays{Why not just $\|p_i-p_j\|$?} \mhsays{So that the Jacobian is actually the rigidity matrix and we do not need the weird shenanigans with scaling.}\mwsays{A bit weird to call it the ``edge length'' vector then, but this was already weird because of the square ... so I guess this is fine :)}\mhsays{I get where you're coming from. At least it is heavily related to edge lengths. Unfortunately, I don't have a better name in mind (which does not completely ignore brevity).}}
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
% \ie\ if there are edge length perturbations arbitrarily close to ${\bs\ell}(P)$ that can not be realized as a polytope $Q$ sufficiently close to $P$, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

\iffalse 
More precisely, $P$ has all edge length perturbations if for some $C>0$ and every $\varepsilon\in (0,C]$ there exists a $\delta>0$ such that every edge length vector $\bs\ell'$ with 
%
\[\text{dist}({\bs\ell}(P),\,\bs\ell')<\delta\] 
%
there exists a polytope $Q=\psi(\bs\ell')$ of the same combinatorial type as $P$ that satisfies
%
\[\text{dist}(P,\,Q)<\varepsilon\] 
%
in the Euclidean metric on $\mathbb{R}^{d(V+F)}$. This definition implies that the edge length map $\bs\ell:\real(\mathcal{P})\rightarrow\mathbb{R}^E$ is locally surjective around $P$. \fi

%\todo{\mhsays{Add the following? Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, the Legendre-Steinitz theorem is necessary to state the following results, justifying this restriction.}\mwsays{My suggestion: ``... however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.''}} 
%
Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.

Let us first consider an example of the first-order rigid regular tetrahedron. For this polyhedron, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    As a polytope, it is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polyhedron is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$, as a bar-joint framework, meaning that the removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the corresponding value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polyhedron's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polyhedra concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid polyhedron $P$ has all edge length perturbations.
    \iffalse
    \begin{proof}
    %\notodo{\mwsays{I find this confusing: we start talking about reduced non-metric realization space, but then continue with the Jacobian, which is the tangent space of the non-reduced metric realization space}}
    %The reduced realization space of a convex polytope $\realR(\mathcal{P})$ is a smooth $E$-dimensional manifold, where $E$ denotes the number of edges of $P$. 
    Assuming that $P$ is %\todo{\mwsays{First-order rigid}}
        first-order rigid, the rigidity matrix $\mathcal{R}(P)$ has the minimal corank $6$ (\cf\ \cref{res:corank_rigid}), so its rank is $dV+dF-6$. 
        %In particular, $P$ is a regular point of $\mreal(\mathcal P, P)$. 
        %This implies that all sufficiently close realizations of $P$ are also first-order rigid: the Jacobian matrix of a polynomial system drops rank in a proper algebraic subset of lower dimension, implying that around every \todo{\mwsays{Let's not talk abut regular points --  we did not introduce the relation between regular points and first-order rigidity (via generic rigidity). Since we only care about the rigidity, let's just reference \cref{res:corank_rigid}}\mhsays{But this doesn't give us that all sufficiently close realizations are first-order rigid, does it? We need something algebraic here.}}regular point of an algebraic variety there is an open neighborhood of regular points \cite[Thm.\ 5.3]{hartshorne}.
%This implies that $\mreal({\mathcal{P},P})$ locally forms a 6-dimensional manifold around the realization $P$ which is locally parametrized by $\mathrm{Iso}$.
Moreover, the realization space $\real(\mathcal{P})$ is a $(E+6)$-dimensional manifold according to the Legendre-Steinitz theorem, which implies that its tangent space $T_P(\real(\mathcal{P}))$ at the realization $P$ also has dimension $(E+6)$. Moreover $\real(\mathcal{P})\subset\mathbb{R}^{dV+dF}$, so that the dimension of the normal space of the realization space $\real(\mathcal{P})$ is equal to $dV+dF-(E+6)$. Since the rows of the rigidity matrix $\mathcal{R}(\mathcal{P})$ are exactly given by a basis of the normal space of $\real(\mathcal{P})$ (\cf\ \cite[Proposition 5.38 and Section 6]{lee-smooth-manifolds}) and the Jacobian %\todo{\mwsays{$d\bs\ell$? Not $J\bs\ell$? If you insist on $d$, can we do $\mathrm d\bs \ell$ or $\partial \bs \ell$ or $\delta\bs\ell$? $d$ is already the variable for the dimension.}}
$d\bs\ell$ of the edge length map $\bs\ell: \real(\mathcal{P})\rightarrow \mathbb{R}^E$, the rank of the rigidity matrix satisfies the inequality
%
\begin{eqnarray*}
    dF+dV-6=\rank(\mathcal{R}(P))&\leq& \rank(J\bs\ell(P))+\dim(T_P(\real(\mathcal{P}))^\perp)\\
    &=&\rank(J\bs\ell(P))+dV+dF-(E+6)\\[3mm]
    &\Rightarrow& \rank(J\bs\ell(P))\geq E
\end{eqnarray*}
%
    On the other hand, $\rank(J\bs\ell(P))\leq E$ by construction, which implies that the rank of $J\bs\ell(P))$ is equal to $E$. Thus, the Jacobian $J\bs\ell(P)$ has full rank. Consequently, $\bs\ell$ is locally a submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}), which implies that $\bs\ell$ is locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). Therefore, all sufficiently small edge length perturbations are realizable.
    \end{proof}
\fi
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    %\notodo{\mwsays{In the rest of the section your write $E$ instead of $E$ for cardinalities.}\mhsays{I reckon you prefer using $E$ for cardinalities? How do we call the set of edges then?}\mwsays{I prefer $E$ for the set and the number. I reckon you are not okay with this abuse of notation. And since we already do it differently everywhere else, lets just use $|E|$, no?}\mhsays{No, I am fine with it. We should just be consistent and say it once in Section 2 that we use them interchangeably.}}
    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). %\todo{\mhsays{There is a gap in the proof here, since the definition requires the existence of $\ell^{-1}$ (sort of), so we need to construct a continuous map from $\mathbb{R}^E\rightarrow \real(\mathcal{P})$} \mwsays{This is easy enough by quotienting by the Iso-action. But let's not touch this before we have figured out the definition problem}}
    %Therefore, all sufficiently small edge length perturbations of $P$ are realizable.
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of polyhedra are first-order rigid.  
This result requires a suitable definition of \emph{genericity}, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polyhedra to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 

%\mwsays{``For a suitable definition of generic, see \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}:''. Random Coordinates}


\begin{corollary}
    Generic realizations of polyhedra have all edge length perturbations.
    \begin{proof}
        Take any polyhedron $P$. In \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polyhedron is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polyhedron in the following example. This example highlights that not all realizations of a polyhedron have all edge length perturbation.

%\notodo{\mwsays{Proposal: we bring the two examples as motivation; we take the locally surjective definition; we prove fo-rigid implies all perturbation exist; we discuss whether the cube example can be generalized; we give Theorem 5.6 as a question; we discuss the $z^2$ problem; we prove flexible implies not all perturbations exist under the additional example of continuous inverse (maybe constant fiber?).}}

\begin{example}
\label{ex:cube-edge-length-perturbations}
    %\todo{\mwsays{I think this example is very educational and should, together with a positive example, come in the beginning of this section}}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polyhedron, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    %\notodo{\mwsays{``antipodal edges'' better?} \mhsays{Sure}}
    antipodal edges. 
\end{example}

We can turn the observation from this example, that not all polyhedra admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polyhedron's edge length vector to distinct polyhedra sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the polyhedron $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        Assume now that all of $P$'s edge length perturbations are realizable via 
        % Then, in particular, we can locally extend and contract each of $P$'s edges individually. In fact, we can arbitrarily combine these edge length perturbations, %\todo{\mwsays{``Since we factored out Euclidean isometries'': how does this imply the second half of the sentence?}}Since we factored out Euclidean isometries, 
        %so that each combination of edges that we perturb gives rise to a \emph{distinct} continuous deformation of $P$. This implies that there is an open ${E}$-dimensional ball of realizable edge length perturbations containing ${\bs\ell}(P)$. Therefore, the map 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. As a consequence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi=\varphi^{-1}\circ(\varphi\circ \psi)$ and $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        
        Consequently, there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ through the realization $P$ which preserves the edge lengths ${\bs\ell}(P)$, so $P$ is rigid. 
    \end{proof}
\end{theorem}
%
The assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. This restricts the family of admissible polyhedra.

Since \Cref{thm:rigidity-and-edge-length-perturbations} provides a sufficient condition for the rigidity of polyhedra, its contrapositive yields information about the reduced realization space $\realR(\mathcal{P})$. This observation is sufficiently useful to state explicitly as a corollary. Albeit, it is currently unclear whether checking the theorems preconditions offers any advantage over directly verifying a polyhedron's rigidity or flexibility.

\begin{corollary}
    If a polyhedron $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}
%
Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample. 
\begin{remark}
\label{res:square_root_branching}
Consider $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.
\end{remark}

However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 

The correspondence between the edge length realization space of a polyhedron and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polyhedron is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

%\notodo{\mwsays{Can we make the first two questions into one with (i) and (ii) since they are just inverses of each other?} \mhsays{I was contemplating that, too. Fixed.}}

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polyhedron $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization of a polyhedron have all edge length perturbations?
\end{question}

%\notodo{\mwsays{In the question below, do you also want to ask that it is not first-order rigid? Otherwise the tetrahedron is a counterexample. And maybe move this question to the end of the so-theory section? Depends on if we move this section of course.} \mhsays{True. Thanks for pointing out this oversight. I chose to replace it by ``rigid, but not fo-rigid''.}}

% \begin{question}
% Assuming a convex polytope $P$ is rigid, but not first-order rigid, is ${\bs\ell}(P)$ then singular in the edge length realization space $\mathcal{L}(P)$ (see \cref{fig:edge-contraction-deformation-space})?
% \end{question}

%\todo{\mhsays{I might delete this question, since I find it confusing in the context of Legendre-Steinitz and it is not formulated precisely, since we only change the length of a single edge.}}

%While we do not understand the edge length realization space of polytopes nearly enough to provide answers to these questions, they provide interesting observations that should be investigated in future research.\todo{\mwsays{You essentially repeat the last sentence before the questions}}

%\todo{\mhsays{Technically, we could also move this section to the appendix if need be. Without \Cref{thm:rigidity-and-edge-length-perturbations}, this section is not what it used to be.}}


















\tempnewpage
\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}
\label{sec:so_certificate}

%\todo{\mwsays{Use $\mathcal{R}$ for rigidity matrix}}

As laid out in \Cref{sec:second-order-theory}, any first-order flex of a polytope 
%in the edge-length realization space \mbox{$\mreal(\mathcal{P},P)$} 
that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. 
%This provides a convenient heuristic for finding non-blocked first-order flexes: 
That is, according to \Cref{res:sotest}, there exits a first-order flex $\dot P$ so that for all equilibrium stresses $\bs \xi$ we have $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$.
Conversely, if for each $\dot{P}$ there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$, then the polytope is 
%\notodo{\mwsays{In fact, PSS. Is this the proper converse that you want to state here?} \mhsays{Good catch, thanks.}}
second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the first-order flex space via a basis ${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ and variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ and variables $\mu=(\mu_1, \dots, \mu_s)$. %\notodo{\mwsays{refer to \eqref{res:sotest} explicitly}\mhsays{done}}
This turns the second-order condition \eqref{block} into a cubic polynomial of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, the homogeneous polynomial $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.

By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is non-zero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. 
Therefore, the first-order flexes that are not blocked by any stresses can be parametrized by the solutions of the polynomial system $Q_1=\dots= Q_s=0$, which form an algebraic set. %\todo{\mwsays{Is this clear?}}
This system can also be represented by the gradient of $E_{\dot{P},{\bs\xi}}$ with respect to $\mu$ to obtain $\nabla_\mu E_{\dot{P},{\bs\xi}}(\lambda)=0$.

%\todo{\mwsays{Why does this suffice? Finitely many solutions are still solutions. Further below you explain that finite implies empty due to homogeneity. This should come here, no?} \mhsays{We are in projective space, so finitely many solutions implies positive-dimensional solution space.}\mwsays{I know. This is mentioned below because it is necessary for the argument. But it must be mentioned here because the argument is already used here.} \mhsays{Potentially I can just remove/replace this sentence here, since I explain it in the next paragraph anyway.}\mwsays{That is possible. Just without a comment this sentence is confusing}}
We will later see that the zero-dimensionality of the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$ is sufficient for second-order rigidity. As a criterion for that, we formulate the following. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field %\todo{\mwsays{Can we use $\Bbbk$ for the field?}}
        $\Bbbk$. Given an ideal $\mathcal{I}=\langle f_1,...,f_s\rangle$, where $f_i\in \Bbbk[x_1,..,x_r]$, and a Gröbner basis $\mathcal{G}$ of $\mathcal{I}$. Then, $\mathcal{I}$ is zero dimensional if and only if for every $i\in\{1,...,r\}$ some power of $x_i$ is the leading monomial of an element of $\mathcal{G}$.%\mhsays{Only for algebraically closed $k$? If so, replace $k$ by $\mathbb{C}$. Else, define what $k$ can be. }
    \end{lemma}

Of course, there are also other methods based on Gröbner bases to verify that an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic set $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homogeneous, it holds that \[\left(Q_1(c\cdot \lambda^*),\,\dots,\,Q_s(c\cdot \lambda^*)\right)=\left(c^2\cdot Q_1(\lambda^*),\,\dots,\,c^2\cdot Q_s(\lambda^*)\right)= 0\] 
for any $c\in \mathbb{C}$ and any $\lambda^*\in \mathcal{V}(\mathcal{I})$. In other words, all scalar multiples $c\cdot\lambda^*$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\{0\}$.
%\notodo{\mwsays{for Matthias: Projective comment.}}
In our context, this translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system %\notodo{\mwsays{Since this proposition tries to be self-contained, one should repeat what is the \emph{finite} system. As written down I don't see a system but only one equations. What do we quantify over? Alternatively, refer to (6.1), but also name what finitely many indices we quantify over.}}
    %\notodo{\mwsays{I was confused for the wrong reasons, but I am still confused: where does nabla come from?} \mhsays{It's the gradient. This is standard notation. I added a line above to explain this.}\mwsays{My question should have been: where does the gradient come from? I agree the notation is standard. But I think I found the sentence where this is explained.}}
    $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ defined in \eqref{eqn:stress_polynomial_Qi} only has $\lambda_1=\dots=\lambda_r = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)=0$.
\end{proposition}

%\mhsays{Describe Test for prestress stability: Albert's code.}

%\notodo{\mwsays{This paragraph reads to me like: we were lucky that our technique worked for the polytopes we tested it on, but there was no guarantee. If true, this is new to me and this is not how we sell it in other parts of the paper.} \mhsays{Why would there be a guarantee? I don't see how we could prove something like that. We use an established sufficient condition, which works over $\mathbb{C}$ and lets us certify second-order rigidity in the cases we consider. I don't believe it is necessary. We can easily tweak it though in case we ever need it by using the Euclidean distance degree, which has a significantly higher complexity, so I wouldn't worry too much about that (last sentence). }\mwsays{I think I understand now: even if the algorithm says ``no'', it might still be so-rigid.}}
The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all polytopes tested in \cref{sec:experimental_results} (\cf\ \Cref{tab:comparison} and \ref{tab:catalan-comparison}). Still, %\notodo{\mwsays{I am stumbling with the sentence structure here: what is not necessary for what?} \mhsays{elaborated.}}
our result using Gröbner bases is clearly not necessary for second-order rigidity, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})=\{0\}$ over the real numbers, even when we find non-trivial solutions over $\mathbb{C}$. A simple counterexample is given by the equation $x^2+y^2=0$, which only has $x=y=0$ as a real solution, yet the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solution on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}). By appending the equation $\sum_{i=1}^r\lambda_i^2-1$ to the ideal $\mathcal{I}$ which describes the unit hypersphere, we guarantee that this approach only finds non-trivial solutions. We also do not lose any solutions due to the invariance of solutions under scalar multiplication.

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a $\mu\in \mathbb{R}^s$ defining a %\notodo{\mwsays{Why ``linear combination of stresses $\mu$'' instead of ``stress $\mu$?}}
stress ${\bs\xi}=\sum_{j=1}^s \mu_j\cdot {\bs\xi}_j$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu_j$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix
%
$$\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_j\lambda_k}Q_j(\lambda)\right)_{j,k=1}^r$$
%
is positive definite for some choice of $\mu$. 






\tempnewpage

\section{Second-order rigidity of the regular dodecahedron}
\label{sec:so_rigidity_dod}

Among the Platonic solids, there is only one for which the question of rigidity is not answered immediately.
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid by Dehn's theorem \cite{dehnstheorem}. 
The cube is the classical example of~a~flexible polytope.
Solely the regular dodecahedron remains to be understood and initially eluded direct computation.

Symbolic computations reveal a 5-dimensional space of first-order flexes and a~5-dimensional space of stresses.\footnote{The specific embedding and orderings of vertices, edges and faces are provided in \cref{appendix:comp-data-dodecahedron}.}
%
Note that these dimensions must be identical~due~to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
%
It is tempting to somehow relate the dimensions of the flex and stress spaces to the 5-fold symmetries of the dodecahedron.
We have no evidence~for such a relation, and rather mild counter-evidence in the case of the truncated~dode\-cahedron (see \cref{sec:selected_rigidity}).


\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

% By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
% \footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
% Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
% %\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
% Consequently, the regular dodecahedron is not first-order rigid.

%We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. 

Since the regular dodecahedron is not first-order rigid, it is a promising test case for the second-order certificate from \cref{sec:so_certificate}.
Concretely, \cref{prop:stress-energy-condition} asserts that it suffices to compute the zeros of a certain polynomial system. 
We~proceed~as follows:
%
\begin{enumerate}
    \setlength{\itemsep}{0.7ex}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. 
    Using the~bases, we parametrize the spaces by variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$.
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadric forms $Q_i$. % (see \cref{section:second-order-rigidity-check}).
    
    \item Use the equivalence in \cref{gbasis} to determine whether the system~has~fi\-nitely many (real) zeros.
    This is the case for the regular dodecahedron.
    
    \item Use \Cref{prop:stress-energy-condition} to infer second-order rigidity.
\end{enumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. Then, $\mathcal{I}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}.
    For more specifics on the relevant \textsc{Mathematica} files, see \cref{appendix:comp-data-dodecahedron}.
    With the help of this Gröbner basis, we obtain the following results:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        The monomials $\lambda_1^2$, $\lambda_2^3$, $\lambda_3^3$, $\lambda_4^5$,  $\lambda_5^6$, appear as leading monomials in the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$.
        \Cref{gbasis} therefore implies that $\mathcal{I}$ is zero-dimensional. 
        %By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). 
        Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. 
        By \cref{prop:stress-energy-condition}, for any non-zero linear combination of the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. 
        By \Cref{res:sotest}, $P$ is second-order rigid. 
        By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

Having understood the rigidity properties of the Platonic solids, a natural move is to extend the search to the next best well-documented class of polytopes -- the Archimedean and Catalan solids.
A detailed account of the findings is given~in~\cref{sec:archimedean} (see also \cref{tab:comparison} and \cref{tab:catalan-comparison}).

Among the 31 polytopes checked, only three are not first-order rigid, but also not predictably flexible (\cf\ \cref{sec:dimension_estimates}): the regular dodecahedron, the truncated icosahedron and the truncated dodecahedron (\cf\ \cref{fig:Dod_TIco_TDod}).
The procedure above was applied to all of them, and our findings are documented in \cref{sec:selected_results}.


% \begin{remark}
%     Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid}). The contraposition of \Cref{gbasis} can be used to show that the truncated dodecahedron is \emph{not} second-order rigid (see \Cref{res:TDod_not_Second_order_rigid} for details).
%     % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
% \end{remark}\todo{\mwsays{Incorporate TIco and TDod into Remark}\mhsays{I made an attempt. Feel free to change.}}











\tempnewpage

\section{Computational results: Platonic, Archimedean and Catalan solids}
\label{sec:experimental_results}
\label{sec:archimedean}

% \todo{\mwsays{Note to myself: add this footnote somewhere: The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}\mhsays{Is this footnote now part of Section 7?}}


We apply our techniques to the Platonic, Archimedean, and Catalan~solids.\nls
For these classes combinatorial data and algebraic vertex and normal coordinates are readily available.%
%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}
%
The results are shown in \cref{tab:comparison} (for the Platonic and Archime\-dean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation for the content of the tables is given in \cref{sec:explain_table}.
%
%A more detailed step-by-step~expla\-nation for how the second-order rigidity results were obtained is given in \cref{section:rigidity-of-the-regdod} on the example of the regular dodecahedron.
%
A key takeaway is that already simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
See \cref{sec:selected_results}, \ref{sec:selected_rigidity} and \ref{sec:selected_flexibility}~for a discussion of the results.


\newpage
\vspace*{6mm}
\input{sec/table1}
\newpage

\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{1ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    %{\color{gray} 
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semi-definite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
    A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate for our setting.
    
%\mwsays{Something about how the numerical computations are sufficiently stable and the results away from zero or whatever so that we can trust them.}\mhsays{Replace ``We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.'' by: The numerical results are based on an eigenvalue computation, for which \noBut\ indicates the existence of an eigenvalue close to machine precision ($\approx 0$), whereas \yesBut\ indicates the existence of an eigenvalue whose absolute value lies above $10^{-6}$, which is sufficiently far away from zero. We observe no intermediate eigenvalues. Since eigenvalue computation is numerically stable and the thresholds have been chosen conservatively, we have a high degree of confidence in these results.}\mwsays{Then we should probably only explain \noBut, because \yesBut\ is never used. And also: do we ever explain this eigenvalue stuff in the paper? I don't remember having done anything with eigenvalues in Mathematica when I checked prestress stability.}\mhsays{I guess you solved an SDP of the form $C=\lambda_1\cdot A_1+\dots+\lambda_4\cdot A_4$ to find an assignment of $\lambda_i$ that makes $C$ positive definite. However, we always found a zero eigenvalue I guess? I don't exactly recall.}
    %}\mwsays{Okay, let's look into Albert's code to see what can be said.}
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flexe space} as introduced in \cref{sec:first_order}.
    %\nls Heu\-ristically, it is the expected number of independent ways in which the polytope can deform in first order. 
    %If the number is zero, the polytope~is first-order rigid. 
    %If the polytope is a generic Minkowski sum, the dimension~decomposes as explained in \cref{sec:generic_Msum} (see also \SymThree\ below).
    In some cases we have a good understanding for how~the~dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension. 
    If further explanations are available, this is indicated by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and more theoretical background given in \cref{sec:dimension_estimates}.
    %
    %\todo{\mhsays{Maybe only refer to \SymTwo\ and \SymThree\ here? \ie\, ``see \SymTwo\ and \SymThree\ for an explanation of the number''? Otherwise we write it twice.}}
\end{enumerate}
%
The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{1ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension for the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
    %If~the zonotope is generic (\ie\ all faces are rhombi), the dimension of the first-order flex space is precisely $2\times\#\text{generators}-3$ (see \cref{res:generic_zonotope}).
    %For~general zonotopes a lower bound is given~by $\dim\GL(\RR^3)-4=5$ (with a few exceptions, see \cref{res:bound_zonotopes}).
    
    % The dimension of the flex space of a generic Minkowski sum is at least the sum of the dimensions of the flex spaces of the summands, plus the dimension of the Lie group that parametrizes the relative orientations of the summands.
    % For this class we write the flex space dimension in the table as a sum of these two contributions.
    
    % %show how this dimension decomposes into flexes coming from flexes of the Minkowski summands (left term) and flexes coming from the relative orientation changes of the Minkowski summands (right term). 
    % For example, the \emph{rhombicuboctahedron} (\cf\ \cref{tab:comparison}) is a Minkowski sum of a cube and an octahedron. The cube provides itself three dimensions~for the flex space, whereas the octahedron provides none. The remaining three dimensions come from $\mathrm{SO}(\RR^3)$, which encodes the relative orientation of~the cube and octahedron. We denote this by 3+3.
\end{itemize}
%
%These considerations are elaborated in \cref{sec:dimension_estimates}.
Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
Again,\nls details are given in \cref{sec:dimension_estimates}.

% \mwsays{In all cases our heuristic lower bounds match the actual dimension of the flex space. In some cases (permutahedra) this is especially remarkable since it suggests that the combinatorics and edge lengths constrains enforce a zonotopal realization.}


\iffalse
Numerical experiments reveal that all these properties are sensitive to small changes in the polytope's geometry.
First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
At this time it is unclear why exactly the realizations with uniform edge lengths are flexible in first- and second-order. 
In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.
\fi

\pagebreak

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding table cells are marked with \Star):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} have identical~rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes), nor prestress stable; yet, \emph{both are second \mbox{order} rigid}. 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    %In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct concepts.
    Previous examples of this distinction were compa\-ratively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
    %
    In fact, we verified symbolically that $Q_i=0$ for all quadratic forms in~\eqref{eqn:stress_polynomial_Qi}. Second-order flexibility then followed via \cref{prop:stress-energy-condition}.
    %
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order, we do not know whether the truncated dodecahedron is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above are sensitive to small changes in the their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.

\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priorily.
We therefore formulate the following question:

\begin{question}
    %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps polytopes whose faces are triangles and 4-gons are simple enough for a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.


% \mwsays{Here would be a good place to put Question 3.5} \mhsays{I agree}

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained from actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} match the values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.





\input{sec/table2}









% \tempnewpage

\pagebreak

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}

Due to its previous status as the guiding example,
%
we single out the dodecahedron once again for a closer inspection.
%
Exploring its realization space close to the regular dodecahedron helps us better understand the source of its exceptional behavior.
%
From that, we draw conclusions about the global rigidity of the polytope.






\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

\iffalse % old rigidity section

\subsection{Rigidity} 
\label{section:rigidity-of-the-regdod}

By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
Consequently, the regular dodecahedron is not first-order rigid.

We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. \Cref{prop:stress-energy-condition} asserts that computing the zeros of a certain polynomial system lets us certify this property. For that reason, we employ the following strategy:

\begin{myenumerate}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. We parametrize these bases via variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$, respectively. 
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadrics $Q_i$ (see \cref{section:second-order-rigidity-check}).
    
    \item Employ \Cref{gbasis} to show that this system has finitely many zeros.
    
    \item According to \Cref{prop:stress-energy-condition}, this implies that the regular dodecahedron is second-order rigid.
\end{myenumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. $\mathcal{G}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}. With the help of this Gröbner basis, we can prove the following theorem:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. As a result, for any non-zero $\dot P$ generated by the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. By \Cref{res:sotest}, $P$ is second-order rigid. By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

\begin{remark}
    Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid} for details).
    % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
\end{remark}

\fi







\subsection{Deformation paths}
\label{section:dodec-edge-length-perturbations}


%\todo{\mwsays{Potentially incorporate: ``By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. We find bifurcating deformation paths and from this, we construct  a counterexample to generic global rigidity for polytopes.''}\mhsays{Done}}
%
By the Legendre-Steinitz theorem the reduced realization space $\realR(\mathcal{P})$ of the dodecahedron is a smooth $30$-dimensional manifold. 
%\notodo{\mwsays{What has Sec 5 to do with this}\mhsays{I guess I am talking about the introduction, where I derive $\dim(\realR(\mathcal{P}))=|E|$. Feel free to rephrase.}}
%\Cref{section:edge-length-perturbations} we can say more: its reduced realization space $\realR(\mathcal{P})$ is a smooth $30$-dimensional manifold. 
The dodecahedron is rigid by \Cref{dodecahedronrig}, suggesting that these 30 degrees of freedom translate directly into changes in the lengths of its 30 edges.
Although we formulate the hope that all edge length perturbations of rigid polytopes are realizable in \Cref{conj:edge_length_perturbations}, even for the regular dodecahedron it is completely unclear whether this statement true.

Due to dodecahedron's high symmetry (all edges are the same), one might suggest to deform a single edge and, if this is possible, to conclude that arbitrary perturbations are possible.
In this section, we investigate the deformations of the regular dodecahedron induced by shrinking or extending a single edge. 
By approximating such deformation paths using methods explained in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of $P$ this polytope in $\realR(\mathcal P)$. 
However, whether this implies that all edge length perturbations are possible, must remain open.
%With this approach, we describe bifurcating deformation paths, which lets us construct a counterexample to generic global rigidity for polytopes.

%Due to dodecahedron's high symmetry, all edges are combinatorially identical. It does not matter which edge is chosen. 
For this experiment, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert~ < 1$. 
Sampling from the realization space intersected with the real algebraic set of prescribed edge lengths reveals \textit{six} distinct arcs starting in the regular dodecahedron corresponding to the shrinking of a single edge and \textit{two} corresponding to its expansion (see also \cite{deformationpaths}). 

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by perturbing a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge constractions, whereas gray curves correspond to edge expansions. On these curves, the eight corresponding realizations at $\ell^*(\pm 0.25)$ are depicted. Four realizations are connected by a nodal cubic (dark blue dashes).}
            %Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
 
%
%\notodo{\mwsays{Is this sentence just repeating what we said before? Or should it come much earlier? Also what is the ``also'' doing here?}\mhsays{Good point. I moved it.}}
%
In \Cref{fig:edge-contraction-deformation-space}, we depict a random projection of the deformations induced by edge contractions 
%\notodo{\mwsays{I am not sure this dashed line will be universally understood to be blue} \mhsays{Like this?}\mwsays{Much better!}}
(blue) and expansions (gray), alongside eight realizations at $\ell^{\star}(\pm 0.25)$.
Remarkably, it appears that some of these arcs rejoin smoothly. 
For instance, the gray arcs corresponding to an edge expansion have the same tangent in the regular dodecahedron, and so do suitable pairs of arcs of the blue curves. 
Moreover, the arcs corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (dark blue dashed curve).
%todo{\mwsays{Give a different color to nodal cubic so it is easier to refer to.}} %In particular, the regular dodecahedron is a singularity in the deformation space induced by all possible modifications of a single edge. 
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron since there are multiple realizations with the same edge lengths arbitrarily close to the regular dodecahedron. Hence, it is possible that there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$ in this case (\cf\ \Cref{res:square_root_branching}). 
%
%\notodo{\mwsays{We could refer here to your example with squaring a complex number in Sec 5, if it would be a numbered remark or so.}}

In total, three curves are passing through the regular dodecahedron that are induced by length changes of a single edge. 
Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective sum of the tangent vectors is sufficiently close to zero. 
We attach an animation of the smooth deformation passing through the regular dodecahedron on the solid blue path from $\ell^*(-0.25)$ via $\ell^*(0)$ to $\ell^*(-0.25)$ in the Supplementary Material \cite{zenodo_suppMaterial} of this article.%\todo{\mwsays{How is this possible? Expansions and contractions don't match smoothly. Or do you decelerate to speed 0. Maybe clarify?}}

Additionally, we find that in the case of edge contractions there are two types of deformations: those that react to the edge contraction by flattening horizontally (see \Cref{fig:edge-contraction-deformation-space}, top) and those that flatten vertically (see \Cref{fig:edge-contraction-deformation-space}, bottom). Both types contain one realization with two reflection symmetries, and two realizations with only one reflection symmetry that are mutual mirror images of each other. 
        Intriguingly, not all dodecahedra persist until the edge collapses to lenght zero. 
        The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations below this particular edge length. 
        %
        %\notodo{\mwsays{Discuss the fact that the orange branches meet again: the two branches of the loop have opposite symmetries, and must therefore pass through a common symmetrization to connect to each other}\mwsays{Nah, its fine, I dont need this.}} 
        %
        All of them persist until $\ell^*(-1)=0$. 


        Conversely, expanding an edge only produces two realizations with distinct reflection axes. 
        They are depicted on the left and right of \Cref{fig:edge-contraction-deformation-space}. 
        %
        %\notodo{\mwsays{Surely there is a maximal length!}\mhsays{I mean, yes, there has to be one. However, it could be a highly degenerate limit (everything collapses to a plane), which numerical methods would struggle with. In my experiments, I did not find a maximal length. I removed the sentence}}
        %
        %There is no indication that there exists a maximal edge length beyond which no realizations exist. 
        Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.

        %What remains is a qualitative analysis of the eight deformation paths that emerge from contracting any of the dodecahedron's edges. By considering projections of the eight deformation paths onto random 2-dimensional subspaces and approximating the curves' derivatives, an understanding of the curves' tangents in the regular dodecahedron can be obtained. \Cref{fig:edge-contraction-deformation-space} visualizes these curves' behavior. 

        %\mhsays{Mention how the graphic was formed (see above text)}

        % \begin{figure}[h!]
        %     \centering
        %     %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation.jpg}
        %     %\hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom.jpg}
        %     %\\[4mm]
        %      %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation2.jpg}
        %     \hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom2.jpg}
        %     \addtocounter{equation}{1}
        %     \caption{Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths (\cf\ \Cref{fig:dodecahedron-configurations-contraction}) have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
        %     \label{fig:edge-contraction-deformation-space}
        % \end{figure}

         %\todo[inline]{\mwsays{Put little pictures of the deformations at the branches of the graphics.}}

%Two symmetric deformations remain, which also share the same tangent in the regular dodecahedron. 




\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytopes is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore~globally rigid.
%
This leaves open the possibility of generic global rigidity. 

A polytope is called \Def{generically globally rigid} if every generic %\todo{\mwsays{Generic undefined. We mention it already earlier, but never define it I think.} \mhsays{We define it \emph{intuitively} on page 15}}\textit{generic} 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
%Let us consider a small generic perturbation $P'$ of one of the realizations shown in \cref{fig:edge-contraction-deformation-space}.
First, we confirmed numerically that all of the equivalent realizations which are %\notodo{\mwsays{What highlights?}\mhsays{depicted?}}
depicted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. 
Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently close generic realization of the dodecahedron.
Hence, generic realizations are also not necessarily globally rigid.
%
Notably, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}

%\notodo{\mhsays{This is the opposite of global rigidity :D}}

It would be surprising, though also not absurd, that other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{13mm}
    \begin{minipage}[c]{0.32\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edge have the same lengths (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}

\iffalse
\todo{\mwsays{Something bothers me about the discussion below. Lets talk.}}
For bar-joint frameworks, generic global rigidity is often checked by computing the rank of a \Def{stress matrix} for a random equilibrium stress (\cf\ \cite{gortler-healy-thurston}). Since we demonstrate in this article, that many concepts from bar-joint framework rigidity theory carry over to the polytopal setting, it is possible that we can formulate a similar criterion for the generic global rigidity of polytopes. This provides an exciting direction for future research.

\begin{question}
    Can the rank of the stress matrix be used as a criterion for generic global rigidity?
\end{question}
\fi

% Still, that argument does not resolve whether the regular dodecahedron with combinatorial type $\mathcal{D}$ is globally rigid. Nevertheless, we know that there exists a realization of the dodecahedral graph in $\mathbb{R}^2$ that has equal edge lengths (\cf\ \Cref{fig:planar-dodec}). While this realization is not affinely spanning, it clearly has planar facets. If $0$ lies in the relative interior of this polytope, it is impossible to satisfy the equation $\langle p_i, a_\sigma\rangle=1$ for $i\sim \sigma$, as each facet normal must necessarily be normal to the embedded plane $\mathbb{R}^2$, so that $\langle p_i, a_\sigma\rangle=0$. For that reason, we put the plane at height $1$ so that each face has the same normal vector. With this modification, we find that the realization of $\mathcal{D}$ lies in $\real(\mathcal{D})$, implying that the regular dodecahedron is not globally rigid.






%\tempnewpage % temporary new page

%\section{Case study: The truncated dodecahedron}
%\label{sec:truncated_dodecahedron}
%\label{sec:TDod}





\tempnewpage % temporary new page

\section{Conclusion}
\label{sec:outlook}

%\notodo{\mwsays{I am not a fan of a conclusions section that just repeats introduction and main body for the third time. I liked the outlook we had in the last paper because it was just full of questions. If I see correctly, then the only new bit here is the TDod discussion, which might as well go into the results section. This section would be an easy place to shorten the paper.}
%\mhsays{A conclusion/outlook is a formal requirement for any scientific paper. In it, the main arguments/results should be restated and it gives room for open problems and future research. Ideally, one uses the three questions ``what?'', ``so what?'' and ``now what?'' to guide the writing. The conclusion is an important place in the paper to state and summarize our most significant findings and results, why they are useful and what should happen next. We can keep it to 1 page, but it is an essential section.}}


% \todo{\mwsays{Like for title and abstract, I don't think we should reduce this article to second-order theory} \mhsays{Better? }}%

In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 

%\notodo{\mwsays{I see ``a careful development of first- and second-order theory'' as a main result.}\mhsays{First-order theory was in the first paper, right? Added this sentence to Main Results.}\mwsays{First paper only contains claims, no development of the actual first-order theory. Developing first-order theory properly was one of the selling point of this paper here that we declared back then.}\mhsays{This was a question that a reviewer might ask. I have no problem adding this to the Conclusion (which I now did).}}

\subsection{Main results}

We carefully develop a first-order and second-order theory for the rigidity of polytopes in \Cref{sec:first_order,sec:second-order-theory}. %\notodo{\mwsays{Without some background knowledge ``so-rigid implies rigid'' always sounds underwhelming. I wonder whether we should mention somewhere that this is not true for naive higher-order rigidity} \mhsays{Good idea. I'll give it a try.}\mwsays{I reworded a bit. okay?}}
Using these tools, we demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. 
Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 
A well-developed second-order theory is important since it is right at the boundary of what is practically possible: analogous statements are no longer true for naive higher-order rigidity criteria (see \Cref{sec:higher_order_rigidity}). 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves induced by edge length modifications.

\iffalse\textcolor{gray}{
\todo{\mwsays{Saying this makes only sense if it would be in the main body, but it is in the appendix} \mhsays{The conclusion was written when this was not the case.} Feel free to remove.}%
Moreover, we extend our analysis to flexible polytopes. For zonotopes and generic Minkowski sums, we provide a lower bound on the dimension of the flex space. As of now, all flexible convex polytopes that we are able to find arise as zonotopes or generic Minkowski sums. To approximate the flexes of polytopes, we develop an algorithm in \Cref{sec:approx_continuous_motions}, which relies on Riemannian geometry and homotopy continuation, alongside several useful heuristics.}
\fi

Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. 
%\notodo{\mwsays{Sec 9 has changed}\mhsays{Done.}}
In \Cref{sec:so_rigidity_dod}, we explicitly demonstrate a strategy for proving the second-order rigidity of the regular dodecahedron as a test case. Moreover, we investigate deformations induced by modifying the length of a single edge in \Cref{sec:dodecahedron}, which reveals a highly interesting local geometry and also serves as a counterexample for the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}

\iffalse
\begin{remark}
For the truncated dodecahedron, the system of homogeneous quadratic \todo{\mwsays{Reference these equations by number rather than words}}equations introduced in \Cref{section:second-order-rigidity-check} has a non-trivial solution. According to \Cref{res:sotest}, this implies that the truncated dodecahedron is not second-order rigid. In fact, we find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
\end{remark}
\fi

Among the 31 polytopes we considered, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is 4-dimensional, so it is not first-order rigid.
We also determine that it is not second-order rigid, since the associated system of homogeneous quadratic equations $Q_1=\dots=Q_4=0$ arising from \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. 
In fact, we 
%\notodo{\mwsays{Say that we find this only numerically.}\mhsays{Apparently we know this symbolically! (Y)}}
find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.

In \Cref{fig:TDod_flex_conc}, we depict samples from a numerically generated deformation of the truncated dodecahedron.
It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances.
%which is \todo{\mwsays{``It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances''}} constructed using gradient descent with reasonable numerical tolerance.
%
%\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}
%
However, when we apply a more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
\label{sec:higher_order_rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
%\todo{\mhsays{Discuss energy interpretation}}
This result would help explain why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which %\notodo{\mwsays{This sounds technically wrong. The deformation has low tolerance?}\mhsays{You're right. I added ``satisfies the constraints with reasonably...''}}
satisfies the edge length and facet planarity constraints with reasonably low numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, they observe that the energy landscape around an $N$-th order rigid realization locally looks like the %\notodo{\mwsays{Is this really called a parabola}\mhsays{After coordinate change it is. I replaced the term. }}
polynomial curve $y=x^{2N}$. This implies that for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

Unfortunately, if the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 

%\mhsays{Develop higher-order rigidity techniques.}

% \notodo{\mwsays{I would say we don't need this section. Move the problems to their sections or mention them in the introduction.} 
% \mhsays{Open problems only belong into the introduction if (a) we solve them or (b) they are guiding problems that motivate our article. Neither is the case. We should move them to the respective sections instead (which I did). }}

%\mhsays{Theoretical results for why some polytopes in special position are inf rigid, even though Cauchy-Dehn does not say this.}

%\mhsays{More constructions for flexible polytopes OR proof that Minkowski flexes are all.}

%\mhsays{Dodecahedron and truncated icosahedron have the same numer of first-order flexes; does this come from the symmetries? Counter point: the truncated dodecahedron only has 4 dimensions of first-order flexes even though it has the same symmetry. Where is the lost dimension? Is there a general way of predicting the first-order flexes from the symmetry group?}

%\mwsays{Is there special structure in the TDod that helps deciding the rigidity question?}

%\mhsays{Point out many interesting questions from \Cref{sec:dodecahedron}}



==> sec/introduction_-_copy_-_2026-06-20.tex <==

%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}

%\notodo{\mhsays{Abstract: Replace at least one of the ``we'' alliterations by a different beginning. Fix overful. \mwsays{Will do.} }}

\vspace*{-1em}

\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities.
If such deformations exist, the polytopes is said to be flexible, otherwise rigid.
%. The major difference to the classical setting of polyhedral rigidity is that these deformations are explicitly 
%
Classical results in polyhedral rigidity (such as the rigidity theorems by Cauchy \cite{cauchy1813} or Dehn \cite{dehnstheorem}) enforce the stronger constraint of fixed face shapes, and then find that convexity generally implies rigidity.
This is in contrast to our setting, in which flexible convex polytopes do exist.
Still, only few techniques are known to construct such.

%
%These assumptions are weak in comparison to classical polyhedral rigidity, which also enforces fixed face shapes. 
%
%\todo{\mhsays{I don't understand this sentence.}\mwsays{Sorry, what exactly is unclear?}\mhsays{I understand what you want to say here, but ``weak'' is always slightly confusing to me as a non-logician. Maybe ``are more restrictive'' or ``are implied by the flexibility in classical polyhedral rigidity''?}}%\todo{\mhsays{Should we highlight rigidity in the first sentence of the introduction, too? Currently it is only about flexibility.}}
% \notodo{\mwsays{This sentence sounds like we are in the classical setting}}
%
%Due to In contrast to the classical setting, our setting admits flexibility, even when the polytopes are convex.
%
%While~in~our~setting~even~convex polytopes may be flexible
%Still, only few techniques are known to construct such. %polytopes that admit such deformations.%\mhsays{and which polytopes do not admit continuous deformations? (to highlight rigidity and not just flexibility.)}.
%
\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}
%
As a consequence, the sentiment arose that this sort of flexibility is still rather exceptional, not only among combinatorial types of polytopes, but also among~realizations of a fixed type.
%Only few classes of flexible polytopes are known, constructed from a handful of techniques such as Minkowski sums and affine transformations.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that~in~dimension at least three, a \textit{generic} convex polytope of a given combinatorial type~is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

%\mwsays{Add picture with Dod, TDod, TIco}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
%     \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically. \mhsays{Suggestion: Move to Conclusion and replace image by truncated dodecahedron, dodecahedron and truncated icosahedron, since they are special.}}
%     \label{fig:TDod_flex}
% \end{figure}

%\todo{\mhsays{I do not think anymore that the first page is a good place for a flex, for which we have strong evidence against being a true polyhedral flex. This may generate false expectations. I would prefer putting it in the conclusion/outlook as future work and focusing on the examples that we can actually solve.}}
Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
%The previous exploration therefore focused on first-order and generic rigidity.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques. %, such as a naive Gröbner basis approach. %, and so it remains unknown whether they are rigid or admit continuous deformations.
This already holds for polytopes with relatively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes a suitable second-order theory as~well as an effective algorithm for testing second-order rigidity of concrete examples.
For a demonstration we analyze the rigidity properties of the Platonic, Archimedean and Catalan solids (see \cref{tab:comparison} and \cref{tab:catalan-comparison}). 
In particular, we decide the previously unknown rigidity properties of the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left).
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be determined by our techniques, but seems to require techniques of even higher order. It will thus serve as a simple test case for future theoretical and computational developments.
%
We found it remarkable that such variety of rigidity behaviors can already be observed among classical examples.
%This is not for lack of computations resources, but rather 
%In particular the truncated dodecahedron can serve a surprisingly simple test case for future theoretical and computational developments.
%Merely the \emph{truncated dodecahedron} (see \cref{fig:TDod_flex}, left) evades our approaches. The reason though is interesting, and is of a technical nature rather than from computational limitations.


% \mwsays{The first article develops first- and generic theory. In this article we address notions of rigidity skipped over in the first part: second-order, continuous and global.}

This article divides into theoretical, methodological and experimental results,
of which we give an overview below.
%
\todo{\mwsays{Albert, what do you think about the roadmap.}}
%
%\todo{\mhsays{We can also leave the introduction out or replace it by Table 1/2. The structure of our paper may be slightly confusing and this is an attempt at making the structure clearer. I am \textit{very} open to suggestions here on how to organize the roadmap.}\mwsays{Let's decide this at the end.}}

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (10.25,-2) {Chapter 5};

\node[fill=white] (c6) at (12,2)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,2)  {Chapter 7};

\node[fill=white] (c9) at (20.2,0) {Chapter 9};
% Nodes
\node[
    draw=blue!30,
    fill=blue!20,
    rounded corners,
    fit=(c3)(c6)(c5),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=red!30,
    fill=red!20,
    rounded corners,
    fit=(c7)(c8),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=green!30,
    fill=green!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (intro) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,0) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{appendix:comp-data-dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (10.25,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,2)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,2)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.2,0) {\Cref{sec:dodecahedron}};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (c9);

\draw[->,dashed] (c10) to[bend left=-5] (intro);
\draw[->,dashed] (app) -- (c9);
\draw[->,dashed] (c9) -- (intro);
\end{tikzpicture}
\end{figure}
\vspace*{-1.65em}
}

\subsection{Theoretical results}
\label{sec:intro-theory}

% The main theoretical contributions are a careful deve\-lop\-ment of the first- and second-order theory of polytope rigidity, as well as %an~application of the former to so-called 
% the creation of dual certificates based on which perturbations of a 3-dimensional polytope's edge lengths can be realized.
% %edge length perturbations for 3-dimensional polytopes.

In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions/flexes,\nls and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory}~we develop the second-order theory for polytope rigidity.
We provide analogues~for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
%including notions of second-order motions and flexes.
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cf\ \cref{res:sotest}).
%This allows us to define prestress stability for polytopes.
%
%\notodo{\mwsays{We need results to reference on the arrows.}}

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated from the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to rigidity and first-order rigidity.


% In \cref{section:edge-length-perturbations} we apply first-order theory to study polytope realization spaces, motivated from the following train of thought:
% the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo rigid motions is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
% This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.
% If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same edge lengths. 
% This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}.
%In \cref{section:edge-length-perturbations} we provide an interpretation of these degrees of freedom for first-order rigid polytopes by perturbing their edge lengths.



\iffalse % old text, maybe still useful

We subsequently apply the first-order theory to questions of realizability:
given a combinatorial type $\mathcal P$, one may ask whether there exists a realization $P\subset\RR^d$ with prescribed edge lengths $\ell_e$, $e\in E$.
In general, this question is very hard.
In \cref{section:edge-length-perturbations} we explore the connection between rigidity and the existence of so-called \emph{local edge length perturbations} (see \cref{prop:inf-rigidity-edge-perturbations} and
\cref{thm:rigidity-and-edge-length-perturbations}).\nls
In~\cref{sec:dodecahedron-global-rigidity} we use the results to show that some polytopes are \textit{not} generically globally rigid.

\mwsays{
Using this language, we demonstrate that the dodecahedron exhibits a highly interesting algebraic and topological behavior in \Cref{section:dodec-edge-length-perturbations}. We also compute deformation paths associated with perturbing a single edge length using techniques from \Cref{sec:approx_continuous_motions}.}

\mhsays{Add pictures for this section as well}

% We analyze the full realization space of a few examples where this is possible. This includes cubical zonotopes and generic Minkowski sums.

\fi



% We explore the connection between first-order rigidity and the existence of local edge-length perturbations for polytope realizations.


\subsection{Methodological results}
\label{sec:intro-methods}
%\mwsays{More details: numerical, symbolic, ...}
In \cref{section:second-order-rigidity-check}, we provide a concrete method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
%Our newly developed tools allow us to answer questions that have previously been intractable.
%The Archimedean and Catalan solids provided a convenient benchmark. 
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.

In \cref{sec:dodecahedron} we give a step-by-step account of how to apply our second-order~rigidity certificate to the regular dodecahedron. We thereby verify that it is indeed rigid (\cf\ \cref{dodecahedronrig}), answering a question posed in \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

Analogous computations are performed for the other test polytopes and are~documented in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
We highlight two results: We show that, besides the dodecahedron, also the \textit{truncated icosahedron} (\cref{fig:Dod_TIco_TDod}, center) is not first- but second-order rigid. We also show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and thus its rigidity status remains open.
A detailed explanation of the tables and discussion of the results follows in \cref{sec:experimental_results}.
Further theoretical background on the observed flexes and flex space dimensions is given in \cref{sec:dimension_estimates}.
All code and additional animations of the flexible polytopes are included in the Supplementary Material~\cite{zenodo_suppMaterial}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to~another case study of the regular dodecahedron.
%We demonstrate how to apply our second-order rigidity certificate.
We investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations and deformation paths using tools from Riemannian geometry and homotopy continuation (with more details given in \cref{sec:approx_continuous_motions}).
We also conclude that the dodecahedron is not generically globally rigid.

\iffalse  % old Appendix B intro

\todo{\mwsays{This needs rephrasing so that it is clear that we just recall this theory. Or we move to appendix. \mhsays{I guess the novel part is that we can apply it to edge length perturbations. However, it holds in greater generality, which is why I describe it like that. I could make that more explicit in the section?}}\mwsays{This is now appendix. Incorporate it into the introduction differently.}}
%
{\color{lightgray}
In \cref{sec:approx_continuous_motions} we describe an algorithm for approximating continuous motions of flexible polytopes based on Riemannian geometry and homotopy continuation. It relies on numerically tracking the solution to the 
optimization problem that searches for the Euclidean closest point to the realization space. We can also apply this method to investigate edge length perturbations of polytopes. %(see \Cref{section:edge-length-perturbations}).% \mwsays{A bit more details?} 
%\mhsays{Mention generalization to realization spaces?}
}

\fi


\iffalse % old computational results introduction

\tempnewpage

Doing so already enables us to answer questions that were previously intractable.


The results for the five Platonic, 13 Archimedean and 13 Catalan solids are shown in \Cref{sec:archimedean} and reveal a wide range of interesting behaviors.
%The 13 Catalan solids have less surprising rigidity properties and can be found in \cref{tab:catalan-comparison} in \cref{appendix:catalan}.
%The structure of the tables cells is explained in \cref{sec:explain_table}.
We highlight the most noteworthy finding from these experiments here: 
\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and \Def{truncated icosahedron} have identical rigidity properties: they are neither first-order rigid (both have a 5-dimensional~space of first-order flexes), nor prestress stable; yet, \emph{both are second order rigid}.\nls 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct~concepts.
    Previous examples were comparatively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} (\Cref{fig:Dod_TIco_TDod}, right) is not first-order rigid (it has a 4-dimensional space of first-order flexes), not prestress stable and \emph{not second-order rigid}.
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order,\nls we do not know whether it is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system that demonstrates that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}
\mwsays{Maybe also list the cool fact that most of our lower bounds match the actual flex space dimensions?}\\
%
%\todo{\mwsays{Maybe I move this to dedicated section. Outlook maybe?}}
%\todo{\mhsays{Shorten Introduction to 3 pages?} \mwsays{I will try. Is there a specific reason? Is it bad if it is 3.2 pages?}\mhsays{Not necessarily, but ``in der K\"urze liegt die W\"urze. Just add whatever now you want now and then we shorten during editing.}}
{
\color{lightgray}
%Numerical experiments reveal that all these properties are very sensitive to small changes in the polytope's geometry.
%First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
%Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
%At this time it is unclear why exactly the realizations with uniform edge lengths show low-order flexibility. 
%In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.



%In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
%The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}}
%By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. 
%We find bifurcating deformation paths and construct from this a counterexample to generic global rigidity for polytopes.

}

\fi



\tempnewpage

\iffalse
{
\color{gray}

Some polytopes turned out first-order rigid without us having an a priori explanation for this.
More remarkable however we found the rigidity properties of the three polytopes marked in \textcolor{orange}{orange} that are \emph{not} first-order rigid:
%
\begin{itemize}
    % \item For all but three Archimedean solids the first-order theory decides the rigidity.
    % If a polytope is first-order rigid, then it is rigid (see \cref{thm:first_order}. All Archimedean solids that were identified as flexible are so via a Minkowski flex and the dimension of the first-order flex space is as expected from this construction. 
    \item
    The \textit{regular dodecahedron} is rigid. This was previously unknown since it is first-order flexible. The second order tools developed in this article allowed to identify the dodecahedron as second-order rigid \emph{but not} prestress stable.
    The regular dodecahedron furthermore becomes first-order rigid after a generic linear transformation. This suggests that the regular realization of the dodecahedron is a singularity in the realization space.
    By computing deformation paths that shrink/extend a single edge of the regular dodecahedron, we probe the neighborhood of this singularity. We find that bifurcating deformation paths and thereby a counterexample to generic global rigidity for polytopes.
    \item 
    The truncated icosahedron (the football) is also first-order flexible yet second-order rigid.
    \item 
    The truncated dodecahedron is flexible in both first- and second order. At this time it is unknown whether it admits a deformation. If it admits a deformation it is the first example of a polytope flex that is no of Minkowski sum type. If it is rigid then it is the first example of a naturally occurring rigidity of order greater than two.
\end{itemize}


\hrulefill

\mwsays{I write ...}

We develop the second-order rigidity theory for polytopes with edge length and coplanarity constraints. 
In addition, we develop computational tools for checking the rigidity of polyhedral surfaces and for approximating continuous motions. 

\mwsays{Regarding caption \cref{tab:comparison}: we should write first-/second-order rigidity instead of the numeric variants, but if I change it the table vanishes completely. Not sure what is going on. Maybe the figure becomes too long for the page?}


% \footnotetext[1]{As a triangulated sphere, this polytope is first-order rigid by Cauchy's rigidity theorem \cite{cauchy1813}.}
% \footnotetext[2]{As a zonotope, this polytope is flexible according to Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.}
% \footnotetext[3]{As a ``generic'' Minkowski sum, this polytope is flexible (\cf\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}).}

\begin{enumerate}[label=\arabic*)]
    \item All Archimedean zonotopes (except for the cube) have 5 inf flexes because they are projectively unique as zonotopes and hence their only transformations come from the 9-dim general linear group minus rotations and global scale. The cube also loses scaling along axis, hence 3 less (but global scale is already contained in here).
    \item The first-order flex spaces of Rhombicuboctahedron and Rhombicosidodecahedron can be explained as the sum of the first-order flex spaces of their constituents + 3-dim rotations. 
\end{enumerate}

\subsection{Dodecahedron and Truncated Icosahedron}
\label{sec:dodecahedron}

The regular dodecahedron and the truncated icosahedron are interesting case studies. They are both first-order flexible and possess a 5-dimensional space of first-order flexes. Nevertheless, using techniques from computational algebra (\cf\ \Cref{section:second-order-rigidity-check}) we show that for each first-order flex there exists an equilibrium stress that \emph{blocks} the first-order flex from extending to a continuous motion. In other words, both polytopes are second-order rigid (see \Cref{section:rigidity-of-the-regdod}).

\mwsays{First-order rigid once we apply affine trafo or change the height of truncation.}

\subsection{Truncated Dodecahedron}
\label{sec:truncated_dodecahedron}

The truncated dodecahedron is both first-order and second-order flexible.
More precisely, it has a 4-dimensional space of first-order flexes, which is surprisingly different from the five dimensions that we usually associate with icosahedral symmetry (see \cref{sec:dodecahedron}). % that we found for both dodecahedron and truncated icosahedron.
For second-order rigidity it turns out that none of the first-order flexes is blocked by any stress, so all of them are potentially real. \mhsays{``real'' is not a good word in this context.}
%
Remarkably, we were able to construct a flex numerically!
So far we are not aware of an analytic way to obtain this flex.
Thus, whether this flex is actually real or not remains a mystery. 
In particular, if no such flex is real, there are currently no feasible techniques to prove the rigidity of this polytope.

Interestingly, all first-order flexes of the truncated dodecahedron vanish either on affine transformation or when changing the size of the triangles (keeping it vertex transitive).

The facts listed above suggest that the \emph{uniform} truncated dodecahedron is quite special.
In particular, it seems unlikely that the existence of its flex is a mere coincidence.
More likely, there exists a yet unknown construction, similar to Minkowski sums, that generates this flex.

If flexible, the truncated dodecahedron has some remarkable properties:
%
\begin{itemize}
    \item its flex is not reducible to a Minkowski sum
    \item its affine transformations are not (first-order) flexible.
\end{itemize}
%
In contrast, if it were rigid, this would be remarkable as well. 
It would then be the first example of a polyhedron that is second-order flexible, yet rigid.
The general consensus seems to be that rigidity beyond the second order only appears in contrived constructions specifically made for this purpose.
The truncated dodecahedron, being very natural, would then be an interesting counterexample.

\subsection{Outline}
This article is divided into three main parts: The theoretical foundation in \Cref{sec:combinatorics-of-polytopes,section:edge-length-perturbations}, followed by methods in \ref{section:second-order-rigidity-check,sec:approx_continuous_motions} and a case study on the regular dodecahedron in \Cref{sec:dodecahedron}.

}

\fi










\iffalse % paper roadmap

\tempnewpage

{\color{lightgray}

\begin{itemize}
    \item Introduction (Martin)
    \item Theory part (Martin, fix notation and terminology, stay close to first paper)
    \begin{itemize}
        \item first-order theory
        \item second order theory (prestress stability) 
        \color{lightgray}
        \item construction of flexible polytopes (continuous motions)
        \begin{itemize}
            \item theorem for generic zonotopes
            \item counterexample for general zonotopes (hex prism)
            \item questio for generic Minkowski sums
        \end{itemize}
        \item Edge length perturbation (Matthias)
    \end{itemize}
    \item Methods part
    \begin{itemize}
        \item second-order rigidity check (Gröbner bases, ...) (Albert)
        \item Computing deformation paths (also works for changing edge lengths but we don't mention this here maybe???)  (Matthias)
    \end{itemize}
    \item Case studies (results)
    \begin{itemize}
        \item Dodecahedron
        \begin{itemize}
            \item not first-order rigid (five dim space)
            \item proof of second-order rigid (not prestress stable)
            \item numerical experiments on edge length perturbations and what they might entail (Matthias) 
            \item no global rigidity (Matthias)
        \end{itemize}
        \item Truncated Icosahedron (Matthias + Martin)
        \begin{itemize}
            \item Five first-order flexes
            \item Still second-order rigid
        \end{itemize}
        \item Truncated dodecahedron (Matthias + Martin)
        \begin{itemize}
            \item unclear rigidity
            \item NOT second-order rigid (evidence?)
            \item we believe it is flexible ???
            \item have potential deformation paths
        \end{itemize}
    \end{itemize}
    \item Outlook (Martin)
    \begin{itemize}
        \item (questions about edge-length perturbations -- maybe already in theory part)
        \item is there specific structure in the TDod that helps us to see it is rigid/flexible and construct the flex
        \item Are there general stronger methods for deciding rigidity and constructing deformations
    \end{itemize}
    \item Supplementary material
    \begin{itemize}
        \item computational output (Gröbner bases etc)
        \item Code, algorithms
        \item Animations
    \end{itemize}
\end{itemize}

\tempnewpage % temporary new page

Main results:
\begin{itemize}
    \item carefully define first- and second-order rigidity and prestress stability for this setting.
    \item this gives a strong test for rigidity (resolves previously open cases).
    \begin{itemize}
        \item dodecahedron
        \item truncated icosahedron
        \item checked all Archimedean solids and duals (resolved all but one) 
    \end{itemize}
    \item very interesting special case: truncated dodecahedron (TDod)
    \begin{itemize}
        \item we believe it is flexible (for now)
    \end{itemize}
    \item something about edge length perturbation?
    \item edge length perturbations of the dodecahedron: we find there is a singularity in the ``dual space'' (rigidity transition region is algebraically singular)
    \item dodecahedron is an example that we don't have global rigidity
    \item maybe something about zonotope flexes
\end{itemize}

\hrulefill

\begin{itemize}
    \item many examples of rigidity
    \begin{itemize}
        \item short edges make rigid
        \item higher dimensions + first-order rigidity in higher dimensions
    \end{itemize}
    \item second-order rigidity
    \begin{itemize}
        \item second order rigid implies rigid
        \item Q: does second-order flexibility imply proper flexibility?
        \item $\#stresses=\#flexes$ trivial or worth mentioning?
    \end{itemize}
    \item the dodecahedron example
    \begin{itemize}
        \item affine trafos do not preserve first-order rigidity
        \item there is no global rigidity for polytopes in 3D
    \end{itemize}
    \item many other open questions
    \begin{itemize}
        \item Q: does flexibility need parallel edges?
    \end{itemize}
\end{itemize}

Notes on Archimedean solids:
\begin{itemize}
    \item the only Archimedean solids that are inf-flexible but not generic Minkowski sums are the dodecahedron, truncated dodecahedrona (4 flexes) and truncated icosahedron (5 flexes). Where do we lose the flex on the way from truncated dodecahedron to dodecahedron?
    \item Are they second-order rigid? Can the dimension of their flex spaces and their second-order rigidity be explained in some way using the known properties of the dodecahedron? (Limit argument?)
    \item Are there continuous motions between Archimedean/Catalan/Platonic solids thats preserve the planarity of facets and the edge lengths?
\end{itemize}

Other notes
\begin{itemize}
    \item A zonotope is highly flexible, but is there a zonotope that can flex in more ways than just deforming into other zonotopes, either real or infinitesimally?
    \item If $P$ and $Q$ have first-order flexes, then does $P+Q$ inherit them in some way?
\end{itemize}
\tempnewpage % temporary new page


}

\fi








\tempnewpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is~a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and~a~\Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
%Evidently, every convex polytope $P$ gives rise to such a structure, which we call the combinatorial type of $P$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
%If $\mathcal P$ is the combinatorial type of a convex polytope $P$, this notion agrees with the usual edge graph of $P$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
Convenient for computations, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}
%
% \begin{align*}
% \realSp(\mathcal P)
% %=\realSp(V,F,\sim)
% &:=\left\{\!\!
% \begin{array}{l}
%     \bs p\:V\to\RR^d
%     \\
%     \bs a\:F\to\RR^d
% \end{array}
% \Big\vert
%     \begin{array}{rcl}
%     % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
%     \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,
%     \end{array}
% \!\right\}.
% \end{align*}
%
%Analogously, the \Def{convex realization space} is defined as%\todo{\mhsays{Do we need the convex realization space?}}
%
%\todo{\mwsays{Do we really need both notations? I would like to ditch the one with the subscript c.}\mhsays{We should keep the convex realizations in our assumption right? Or do we build a second-order theory for arbitrary point-hyperplane structures?}\mwsays{I will keep the convex ones and delete the subscript-c.}\mhsays{Do we need convexity for anything in this article?}}
%
\begin{align*}
%\begin{align*}
\real(\mathcal P)
%=\realSp_{\mathrm c}(V,F,\sim)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
%
%We shall write $P\in\real(\mathcal P)$
%\notodo{\mhsays{What does this sentence add?} \mwsays{Nothing. Removed it.}}
Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ does not allow facet hyperplane to pass~though the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

%\mwsays{Maybe move the below to edge length perturbation section? I think this is the first (and only?) place it is used.}\mhsays{Sure, we can do that. Might even call it configuration space?}

% and the \Def{reduced convex realization space} is defined as
% \begin{align*}
% \realRCvx(\mathcal P)
% :=\realCvx(\mathcal{P})\,/\,\mathrm{Iso}
% \end{align*}
%
%where $\mathrm{Iso}$ is the Lie group of Euclidean isometries of $\mathbb{R}^d$.

%\mwsays{Define $\realR(P)$ reduced realization space?}

%As we show in \Cref{sec:first_order},
%\todo{\mhsays{This is absolutely not clear and we spend quite some time to show that.}\mwsays{I am not sure what you mean. This statement is either trivial or false by \cref{res:new_notion}}\mhsays{How the group action works on $\mathbf{a}$ is only explained in Section 4 and was subtle, so using ``clearly'' here is somewhat dishonest. I would suggest writing something like ``As we show in \Cref{sec:first_order}, the Lie group...}}
The \Def{Lie group of Euclidean isometries} (\ie\ rotations and translations), denoted $\Iso$, acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
%\qquad 
%\realRCvx(\mathcal P)
    %:=\realCvx(\mathcal%{P})\,/\,\mathrm{Iso}
\end{align*}

\iffalse % edge-length measurement map

\todo{\mwsays{This here is not the place for metric stuff. This is what the next section is for. I will move this later}}
\todo{\mhsays{If you want, we can call $\realR$ $\conf$ (the configuration space) instead and use something like $\textsc{M}\conf$ for $\mreal^*$, the metric configuration space.}}
Since in this article we are considering polytopes whose edge lengths are fixed, we also define the \Def{edge-length measurement map} as
\[m_E:\mathbb{R}^{dV}\rightarrow \mathbb{R}^E,\quad m_E(\bs p) = \left(\|p_i-p_j\|^2\right)_{ij\in E},\]
which lets us define the \Def{edge-length realization space}
\[\mreal(\mathcal{P},P)\,=\,\real(\mathcal{P})\,\cap\, m_E^{-1}\left(m_E(\bs p)\right),\]
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are fixed according to the realization $P$. The preimage of a given edge length vector is a real algebraic set, as its given by all realizations which satisfy a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}). \todo{\mhsays{Briefly talk about relation to $I$-rigidity?}}

\fi










% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

%\notodo{\mhsays{Maybe have this as section 2.1 instead? This section is quite short.}\mwsays{Yes, maybe. I think about it.}}
We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.


% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
% \label{def:continuous-rigidity}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
%\todo{\mhsays{Use $\mreal{\mathcal P}$ instead of ``equivalent'' to help distinguish the concepts?} \mwsays{This feels the wrong way around.}}
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, the Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
% \end{definition}
%
%\mwsays{Define configuration space $\conf$ and reduced configuration space $\conv^*$.}
%\mwsays{Define the \Def{metric realization space} $\mreal(P)$ (and reduced $\mreal^*(P)$) and replace below occurrences of $\conf(P)$ by it.}
%
For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks.
Consequently, much of what we say here applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}
%This also applies to the subsequent section, which develop a first- and second-order theory for polytopes, but are applicable more generally.

% Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% %
% A \Def{motion} of $(\bs p,\bs a)$ is a curve $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$;
% the motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% A non-trivial motion is called a \Def{flex}.
% If a realization $(\bs p,\bs a)$ has a flex, then we call it \Def{flexible}, and \Def{rigid} otherwise.

% {\color{lightgray}

% \begin{remark}
%     \mwsays{?? Simulating polytope rigidity via stacking prisms on faces.}
%     \mhsays{I'd say we leave it out.}
% \end{remark}

% }








\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a geometric constraint system studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence~provides heuristics and criteria that can be efficiently checked in practice.
%Investigating the first-order properties of a system comes down to the study of its \emph{rigidity matrix}.
%The first-order theory for polytopes is analogous to point-hyperplane frameworks, so the theory developed in this section applies verbatim to the more general case.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
    %\label{fig:placeholder}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from the rigidity~matrix.
%$p_i$ should be thought of as the coordinate of vertex $i$, and $a_\sigma$ the corresponding vertex of facet $\sigma$ in the polar dual of $P$.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    % \label{eq:flex_at_face}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
    % \\
    % \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    % \label{eq:flex_at_face}
\end{align}
%
%\todo{\mwsays{Here we could say that $\bsdot a$ is determined by $\bsdot p$. Then it becomes clearer why trivial only needs to be specified on the $p$-part. This is however only true for our polytope setting and not general point-hyperplane frameworks. So we should be cautious claiming generality.}}
%
Similar to the framework setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also, that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).

%\todo{\mwsays{Turn the lemma into a short remark, maybe without proof and point to the proof below.}}

\iffalse % lemma that adot determined by pdot

{\color{lightgray}\small
\begin{lemma}
    \label{res:p_determines_a}
    The $\bsdot p$ uniquely determine the $\bsdot a$.
\end{lemma}
%
\begin{proof}
    For fixed $\sigma$ choose a basis $p_{i_1},..., p_{i_d}$ among the $p_i,i\sim \sigma$ (we can always do this in our setup).
    Then $\dot a_\sigma$ is the unique solution of the linear system $\<\dot a_\sigma,p_{i_k}\>=-\<\dot p_{i_k},a_\sigma\>$ for all $k\in\{1,...,d\}$.
\end{proof}
}

\fi % lemma that adot determined by pdot

First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
    % \\
    % \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any vertex $i\in V$ and facet $\sigma\in F$}.
    % \label{eq:trivial_motion_facet}
    %\\
    %\<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{for any $i\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    %\\
    %\<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%\mhsays{Potentially we will need $i\sim \sigma$ in $(4.4)$ as well (analogous to (4.2)). The possible trivial inf motions are already restricted to the Lie algebra of the Euclidean isometries (i.e. infinitesimal rotations and translations) by $(4.3)$ and the normals move automatically in first order alongside the vertices. By restricting the flexes further, we may make the equation impossible to satisfy (see computation below). It should be sufficient to have a complete graph as the 1-skeleton and the normals are immediately determined in first order. I don't mind $(4.5)$, but I don't think it adds much. Also, I don't quite understand where (4.5) comes from.}
%\mwsays{Let's delete (4.4) and (4.5).}
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    %The trivial first-order motions of a $d$-dimensional polytope $P$ form a vector space $\mathcal T_P$ of dimension $\binom{d+1}{2}$. 
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    %By assumption $P$ has non-empty interior, so we can assume that $\bs p$ is affinely spanning.
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    % \mhsays{I think it is necessary to at least show that 4.4 and 4.5 are satisfied to complete the proof. For a trivial motion, it holds that \[\langle S p_i+t,a_\sigma\rangle+\langle p_i,S a_\sigma\rangle= \langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle + \langle a_\sigma,Sp_i\rangle=\langle t,a_\sigma\rangle+\langle p_i, Sa_\sigma\rangle - \langle p_i, Sa_\sigma\rangle=\langle t,a_\sigma\rangle\]
    % (for (4.5) this works). Of course, this is an issue, because in general this is $\neq 0$. Instead, we take a diagonal matrix $F(t)\in \mathbb{R}^3$ with positive eigenvalues, which is responsible for scaling ${\bs a}$. We require $\bsdot{a}=F(t)\cdot S \cdot {\bs a}$ and compute according to $(4.4)$
    % \begin{eqnarray*}
    % &~&\langle S p_i+t,a_\sigma\rangle+\langle p_i,F(t)\cdot S\cdot a_\sigma\rangle= \langle t, a_\sigma\rangle + \langle p_i,(F(t)-I)\cdot S \cdot a_\sigma\rangle \overset{!}{=}0\\
    % &\Rightarrow & \left(t+(F(t)-I)\cdot S \cdot p_i\right)\T \cdot a_\sigma=0 \quad\left(\Rightarrow t+(F(t)-I)\cdot S \cdot p_i \perp a_\sigma \right)
    % \end{eqnarray*}
    % for arbitrary choices of $t$ and normals $a_\sigma$; since $P$ is affinely spanning, the normals $a_\sigma$ generate $\mathbb{R}^3$ as a vector space. Therefore, 
    % \begin{eqnarray*}
    % S\cdot F(t)\cdot p_i=S\cdot p_i+t~\Rightarrow ~\underbrace{(F(t)-I)}_{=G(t)}\cdot \left( S\cdot p_i \right) = t
    % \end{eqnarray*}
    % for each $i$, since $S$ is not invertible in odd dimensions. This equation essentially needs to be solved for all points $p$ on the hyperplane $\mathcal{H}_\sigma$ with normal $a_\sigma$ which is spanned by the points $p_i$ with $i\sim \sigma$ (here is the exact point where problems occur when we take into account $(4.4)$, since the hyperplane is not defined and we compute on $\mathbb{R}^3$ instead). This equation is overdetermined. The main question is: why does the result for a specific point on $\mathcal{H}_\sigma$ generalize to all points on $\mathcal{H}_\sigma$??? \\[2mm]
    % For $(4.5)$ it holds that 
    % \[\langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle + \langle a_\tau, F(t)\cdot S \cdot a_\sigma\rangle = \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle - \langle a_\sigma, F(t)\cdot S \cdot a_\tau\rangle = 0\]
    % due to the skew-symmetry of $S$ and diagonality of $F(t)$.}
        %Hence, $\mathcal T\simeq\mathcal T_F$ and the claim follows.
    %\mhsays{Also, I think we should give an argument that this is indeed a linear space and not an affine-linear space or a union of such spaces; contrary to the bar-joint equations, (4.2) vaguely resembles $Ax=b$. Nevertheless, we now have variables $\dot{a}$ and $\dot{p}$, so we can rewrite Equation (4.2) as $\langle \dot{p}_i\times \dot{a}_\sigma,  a_\sigma\times p_i\rangle=0$, which implies that the space is indeed linear.} \mwsays{I don't understand. The equations are linear so the solution spaces are linear.}
    %\mwsays{We should choose $\dot a_\sigma$ as the solution of $\<\dot a_\sigma, p_i\> = \<Sp_i+t,a_\sigma\> = \<p_i, S a_\sigma\> + \<t,a_\sigma\>$ over all $i\sim\sigma$. Choose a basis among the $p_i,i\sim\sigma$ to get a candidate solution. Then use that all other $p_i$ are in the affine span of this basis and that the equations are affinely covariant and hence do indeed have a solution that works for all $i\sim\sigma$. Then it satisfies (4.2), and we delete (4.4) and (4.5).}
    %
    %It suffices to show that each $\bsdot p\in\mathcal T_F$ extends to a polytopal first-order motion $(\bsdot p,\bsdot a)$.
    %
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}

\iffalse

\todo{\mhsays{Prove that trivial flexes have the correct dimension? Clearly, space of inf flexes is contained in framework inf flexes by construction. Apply Asimow-Roth $\Rightarrow$ ``$\leq$''. Construct Inf flexes: skew-symmetric $Q$, translation $T$; on vertices: $Qp(i)+T$, on normals $Qa(\sigma)$.}}

{\color{lightgray}

\begin{observation}
    If a facet $\sigma\in F$ is a simplex, then the left hand side of \eqref{eq:stress_at_face} is a linear combination of $d$ linearly independent vectors in $\RR^d$. 
    This can be zero only if all coefficients are zero.
    Hence, $\eta_{i\sigma}=0$ for all $i\sim\sigma$.

    Thus, if the polytope is simplicial, then all facet stresses are zero and the stress is a pure classical framework stress. Due to a theorem of Dehn, convex simplicial polytopes cannot have a non-zero framework stress. \mwsays{True in $d\ge 4$?}\asays{the 16-cell (cross-polytope) has 8 vertices and 24 edges and hence has two self-stresses. In general, there are many stresses, I think}
\end{observation}
}

\fi

%Since $\mathcal T_P\subset\ker \mathcal R(P)$, it 

\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    %\asays{below we use infinitesimal rigidity. Let's choose one throughout} 
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
    %\mwsays{I prefer ``first-order rigid'' because it is more consistent with ``second-order rigid''. Using ``first-order rigid'' and ``corank'' would be consistent with the other paper.}
\end{corollary}
%
%\todo{\mhsays{First prove inf rigid $\Rightarrow$ regular point in realization space. Then use Riemannian geometry. (see also Asimow-Roth)}\mwsays{Why did we need this complicated stuff again?} \mhsays{Yeah, I agree that it doesn't seem to be necessary anymore. I think the ``complexity'' happens in 4.1.}}
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
    %
    %\qedhere
    
    %By \cref{res:trivial_dim} $\corank \mathcal (P)\ge \binom{d+1}{2}$.
    % If $P$ is first-order rigid, all its first-order flexes are trivial, that is, $\ker \mathcal R(P) \subseteq\mathcal T$. Hence $\ker \mathcal R(P)=\mahcal T$ and the claim follows from \cref{res:trivial_dim}.

    % \TODO\ \mwsays{Maybe not true if $P$ is not affinely spanning. But we are always spanning. Cite a paper by Bernd, Bill, Tony, ... for this}\asays{it's not formally proved there, but I think we can still reference it. I do agree we need spanning. If the joints are spanning, then this statement is pretty clear I think. We have a non-trivial first-order flex iff kernel has dimension larger than ${d+1}\choose 2$}
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:

% \mwsays{In the theorem below, should we go for the differential geometry proof?}
% \mhsays{I think it's fine. The proof technique is pretty standard in rigidity theory.}
% \mwsays{I try to formulate the differential geometry argument. See Matthias' paper.}

% \begin{theorem}
%     % \label{res:second-order-implies-rigid}
%     % \label{res:first_order}
%     If a polytope is first-order rigid, then it is rigid.
% \end{theorem}
% %
% \begin{proof}
%     Observe that $\mathcal R(P)$ is the Jacobi matrix of the constraint system. %If its rank is maximal, then this implies that $\real(\mathcal P)$ is smooth at $P$.
%     \mwsays{We currently have no name for the space of all realizations with prescribed edge lengths.}
% \end{proof}

\begin{theorem}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}

%\notodo{\mhsays{I would say we refer to the Corollary 6.6.}\mwsays{I added a reference. Though I also see educational value in seeing the first- and second-order theory proofs side by side and observing that they are so similar. I know I found this interesting.}}

This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends in $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms~of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a maximal~number $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    The converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}



% {\color{gray}
% \todo{\mwsays{I think this text would fit better in \cref{sec:selected_results}}\mhsays{I agree. Can you move it?}\mwsays{Okay, I will}}

% Dehn's theorem \cite{dehnstheorem} proves that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
% Later, we encounter plenty of non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
% Currently no theoretical tools are available that would identify these as rigid a priorily.
% We therefore formulate the following question:

% \begin{question}
%     %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
%     Can we extend Dehn's theorem to some classes of non-simplicial polytopes? 
%     That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
% \end{question}

% Natural candidates are polytopes whose faces are triangles and 4-gons.
% See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

% }



\iffalse % Albert's proof

{\color{lightgray}

\begin{proof}
    %\textcolor{red}{Add proof here}
    We prove the contrapositive: if $P$ is flexible, then it is first-order flexible. 
    Let $P^t$ be a flex. \todo{\mwsays{I think we need to invoke curve selection to get an analytic flex}} 
    Since $P^t$ is non-trivial, there is some minimal order $k$ for which truncating the Taylor expansion of $P^t$ at this order does not look like the truncation of a trivial motion.
    %we can truncate the Taylor expansion of $P^t$ at some order, say $k$, after which it cannot be completed to a trivial motion by adding higher order terms. 

    We expand the $k$-th derivative of the constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}\!(p_i^t-p_j^t)\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}\!(p_i^t-p_j^t)=0.
    \end{equation*}
    %
    For the coplanarity constraint \eqref{eq:flex_at_vertex_face} at $i\sim\sigma$ we obtain
    %
    \begin{equation*}
        \sum_{\ell=0}^k\binom{k}{\ell}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell} \!p_i^t\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell} \!\!a_\sigma^t=0.
    \end{equation*}

    Since $k$ was chosen minimal, we can add a suitable trivial motion to cancel all terms of order up to $k-1$. The two equations above become the following. 
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!(p_i^t-p_j^t)=0
    \end{equation*}
    and 
    \begin{equation*}
        p_i^t \cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!a_\sigma^t+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}\!\!p_i^t \cdot a_\sigma^t=0
    \end{equation*}
    The $k$-th derivative satisfies the same equation as a first-order flex does.\todo{\mwsays{I don't think this is clear from what we know so far.}} Therefore, $P$ is first-order flexible. 
\end{proof}

}

\fi

\iftrue % polyhedra rigidity stresses first-order theory

%\tempnewpage

\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second, and equally important, first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
%(recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a Hookean spring with a spring constant given by the stress $\omega_{ij}$ at $ij\in E$. The spring constant determines the magnitude of the force with which the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

% Stresses have no counterpart to ``trivial'' motions

Like first-order flexes, stresses form a linear space -- the \Def{stress space}.
Stresses~are particularly relevant in second-order theory (see \cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).

%One fact that makes 3-dimensional polytope rigidity tractable as compared to dimension $d\ge 4$ is that first-order rigidity can be expressed purely in terms of stresses.

\begin{proposition}
    \label{res:flex_eq_stress}
    If $P \subset\RR^3$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%
%\notodo{\mhsays{I think it would be cleaner to simply move this comment after the proof.} \mwsays{I like to comment on results before everybody got drained out by the proof. I consider the proof as a nice addendum but nothing crucial for reading. Matter of taste I guess.} \mhsays{This is not important to me. The way I read a paper is I usually skip the proof and read the comments first, but like you said, matter of taste. Why I wanted to move the text is so that before section 4 there is not such a weird gap anymore after the $\square$.}}

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]
    %We first show that for $\mathcal R(P)$ holds $(*)$ $\text{$\#$rows}=\text{$\#$columns}-6$.

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}

% \begin{corollary}
%     \label{res:rigid_eq_stress_free}
%     A polyhedron is first-order rigid if and only if it has no non-zero stress.
% \end{corollary}


The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.


\fi


\iffalse

\hrulefill

\begin{lemma}
    For $\mathcal R(P)$ holds $\text{$\#$columns}=\text{$\#$rows}+6$.
\end{lemma}
%
\begin{proof}
    Let $v,e$ and $f$ be the number of vertices, edges and faces of $P$ respectively.
    
    For each vertex, the number of incident faces equals the number of incident~edges. Thus, the total number of vertex-face incidences in $P$ is equal to the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we arrive at
    %
    \begin{align*}
        \text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
\end{proof}

\mhsays{Add the property that $\# flexes = \# stresses$ for polytopes?} \mwsays{Only true for $d=3$, and yes we should mention this.}

\fi


% \subsection{Flex space dimensions}
% \label{sec:flex_space_dim}

% \mwsays{Delete this section.}















% \tempnewpage % temporary new page

\section{Second-order theory}
% \section{Second-order rigidity and prestress stability}
\label{sec:second_order}
\label{sec:second-order-theory}

%\notodo{\mhsays{Segue from previous section. We now consider arbitrary polytopes again? Or exchange Sections 5 and 6.}}
Second-order rigidity theory investigates deformations that preserve constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
%Sometimes, the polyhedron can still be rigid even if it is not first-order rigid. 
%Rigidity beyond first order is often difficult to test even for bar frameworks. 
%
For that, we follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if $(\bsdot p,\bsdot a)$ form a first-order motion and additionally it holds 
%
%\notodo{\mhsays{Don't we also need that $\dot{P}$ is a first-order flex?}\mwsays{Thanks! Fixed.}}
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$}
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
%Analogous to what was observed in \Cref{sec:first-order-theory}, the $\bsddot a$ are automatically determined by the $\bsddot p$ in this setting
%\todo{\mwsays{Is the sentence about $\bsddot a$ being determined by $\bsddot p$ necessary?}\mhsays{Not really. We can remove it.}}.
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

%\todo{\asays{I think we deleted what it means to be non-trivial in this case. An issue is that $(0,\bsdot p)$ would be non-trivial for a non-trivial first-order $\bsdot p$ if you are not careful, but it doesn't tell us anything other than the first order motion being non-trivial. A clear definition would be a second-order motion with nontrivial first-order terms.}\mwsays{Oops, true, this got deleted. Will fix.}}
%\mwsays{I previously introduced commands to render $\bs p, \bsdot p, \bsddot p$ (see TeX code for commands) in place of $\mathbf{\ddot{p}}$; again, this would be consistent with the first paper. In any way, I recommend to use the command, we can change its appearance later if desired.}

% Let $\dot P,\ddot{P}$ be the vectors $(\dot{p}_1,...,\dot{p}_{|V|},\dot{a}_1,...,\dot{a}_{|F|})$, $(\ddot{p}_1,...,\ddot{p}_{|V|}$ and $\ddot{a}_1,...,\ddot{a}_{|F|})$ correspondingly. We can now define the second-order flex:
%\mhsays{I suggest using textit and a pale color (\eg\ blue) for definitions instead of bold font. That makes it distinguishable from Definitions/Theorems} \mwsays{I imported the command \texttt{\textbackslash Def} for this. It renders \Def{like this}. Feel free to modify.} \mhsays{Looks good!}

% \begin{definition}\label{sorigid}
%     The pair $(\dot{P},\ddot{P})$ is a \Def{second-order flex} if equations \eqref{eq1} and \eqref{eq2} are satisfied. A second-order flex is \Def{non-trivial} if $\dot{P}$ is not a trivial first-order flex. The polyhedron $P$ is \Def{second order flexible} if there exists a non-trivial second-order flex. Otherwise, we say that it is \Def{second-order rigid}.
%     %\mwsays{Use eqref for referencing equations. Use cref for everything else.}
% \end{definition}

% \begin{remark}
%     Notice that we are not defining trivial second-order flexes as the first and second derivatives of trivial flexes. The reason is that while it is possible to build a non-trivial flex with a trivial first derivative, it is not interesting because $\ddot P$ is simply identical to a non-trivial first-order flex, as the proof of \cref{res:second-order-implies-rigid} shows. Therefore, we only need to look at the case where $\dot{p}$ is non-trivial. 
%     \todo{\mwsays{Not really clear}}
% \end{remark}

% \mhsays{We should fix a notation about the realization ${\bs p}, P, ({\bs p},{\bs a})...$ and keep it consistent throughout the article.}
% \asays{Since we defined $P=(\mathbf p,\mathbf a)$, I defined $\dot P$ and $\ddot P$ analogously.} \mwsays{I am fine with using $P$ and $(\bs p,\bs a)$ (and the dotted variants) almost interchangeably. But I also find it weird to use $\dot P$ as a vector.}

%\mhsays{Are the $\ddot{a}$ automatically determined by the $\ddot{p}$? $\Rightarrow$ write a lemma about it?} \mwsays{They are. We have no lemma for this in the first-order case, just a sentence. If it is not needed, let's keep it at the one-sentence-level, no?}\mhsays{ok.}

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    \label{res:second-order-implies-rigid}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking the curve selection lemma \cite[Lemma 18.3]{algebraicapproximationcurves}, we obtain an analytic flex $P^t$.
    There is then a maximal number $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \,\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j),\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i,\, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,\,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:second-order-implies-rigid}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system.
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently whether $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.

\iffalse % stresses

% \subsection{Equilibrium Stresses}
% \label{sec:stresses}

%The test is based on the notion of equilibrium stresses, which we introduce next.

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system. 
We denote them by pairs $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$ (recall that $\VF$ denotes the set of incident vertex-facet pairs). % $(\omega_{ij}\in\RR:ij\in E;\, \alpha_{ik}\in\RR:i\in F_k)$.
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ sake of brevity and call it a \Def{polytope stress}.

\mwsays{Remark: first-order rigid iff no stress. (and then make this its own equilibrium stress subsection). Maybe move stresses to first-order theory.}\mhsays{Maybe as Proposition?}

%\begin{remark}
%\label{res:stress_eq_flex}    
%\end{remark}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a spring with a strength given by the stress $\omega_{ij}$ at $ij\in E$. The strength determines how strongly the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign on $\omega_{ij}$. The stress equilibrium condition (the first term of \eqref{eq:stress_at_vertex}) states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be though of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying sign from facet to facet.
    %Equation \eqref{eq:stress_at_vertex} states that the ``spring'' forces of incident edges and ``pressure'' forces of incident facets cancel out.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}

\fi





% Equations \eqref{eq1} and \eqref{eq2} can be compactly written as a single equation:
% % \begin{equation*}
% %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
% % \end{equation*}
% %
% \begin{equation}\label{eq:compact}
%     \mathcal R(P)\cdot \ddot{P}+\mathcal R(\dot{P})\cdot \dot{P}=0
%     % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
% \end{equation}
% %
% Recall that we use $P$ interchangeably with $(\bs p,\bs a)\in \RR^{dV}\oplus\RR^{dF}$, and analogously~with $\dot P$ and $\ddot P$.
% %
% Now, given a second-order motion $(\dot P,\ddot P)$ and any stress ${\bs \xi}$, we obtain
% %
% \begin{equation}
%     \label{eq:with_stress}
%     {\bs \xi}\T \left(\mathcal R(P)\cdot \ddot P+ \mathcal R(\dot P)\cdot \dot P\right)=0.
% \end{equation}
% %
% %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
% Since ${\bs \xi} \in \ker \mathcal R(P)\T$ by definition of stress, we have ${\bs \xi}\T \mathcal  R(P)\ddot P=0$.
% Equation \eqref{eq:with_stress} then becomes ${\bs \xi}\T \mathcal  R(\dot P)\dot P=0$. We say that a stress $\bs\xi$ \Def{blocks} a first-order motion $\bs P$ if
% %
% $${\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0$$
% %Next, we move on to the second-order duality which can be useful when we want to prove $\ddot{P}$ does not exist. 


\iffalse 
Before that, we first introduce the following equality form of Farkas' lemma:
    \begin{lemma}\label{farkaseq}
        \mwsays{Maybe just use it in the proof and don't list it as a separate lemmas.}\mhsays{I don't mind the Lemma here tbh. }
        Either $Ax=b$ has a solution, or $A^Ty=0$ has a solution with $b^T y\not =0$.
    \end{lemma}
    Intuitively, this Lemma says that either $b$ is in $A$'s column space, or there exists a hyperplane containing the column space of $A$ and $b$ is not in it. 

\begin{lemma}\label{lem2}
    Given a first-order flex $\dot P$, if and only if there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
        {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
    \end{equation}
    then there cannot be a $\ddot P$ such that $(\dot P,\ddot P)$ is a second-order flex. 
    ${\bs \xi}$ is called a \Def{blocking stress} for $\dot P$ if Inequality $\eqref{block}$ holds. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
\end{lemma}
\begin{proof}
    The ``if'' direction is already given in the discussion above. To show ``only if'', we use \cref{farkaseq}.
    %\mhsays{I don't like using the theorem environment in a proof} 
    Let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$. Then \cref{farkaseq} says that either there exists a $\ddot P$ or you can find a blocking stress. 
\end{proof}
\fi

%The following test is an elegant application of Farkas' lemma:

\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

% \begin{lemma}\label{lem2}
%     Let $\dot P$ denote a first-order flex of a polytope $P$. Then there exists a stress ${\bs \xi}$ such that \begin{equation}\label{block}
%         {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0
%     \end{equation}
%     if and only if there is no $\ddot P$ for which $(\dot P,\ddot P)$ is a second-order flex. If $\eqref{block}$ holds,
%     ${\bs \xi}$ is said to \Def{block} $\dot P$. %\mhsays{Does the space of blocking stresses/blocked flexes have structure? I think it is clear that the space of non-blocking stresses for $\mathbf{\dot p}$ is linear (since they satisfy linear equalities). Same holds for the space of flexes blocked not by $\omega$. Can we say something about the combination of $\omega$ and $\mathbf{\dot p}$?  }\asays{I'm actually not sure about this. In the dodecahedron example, almost all stresses block all motions.} \mwsays{Wait what? This would mean the dodecahedron is prestress-stable. I thought it is not?}
% \end{lemma}
\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    % \begin{equation*}
    %     \mathcal R(P)\ddot{P}+\mathcal R(\dot P)\dot P=0
    % \end{equation*}
    %
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

    
    % This system has the form $A\ddot P=b$ for $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$.
    % By Farkas' lemma, the non-existence of a solution for $\ddot P$ (and hence, second-order rigidity of $P$) is equivalent to the existence of a solution of the system $A\T \bs \xi=0$ for some $\bs\xi$ with $\bs\xi\T b=0$, that is,
    % %
    % $$\mathcal R(P)\T \xi=0,\qquad \bs\xi\T\mathcal R(\sot P)\dot P\not=0.$$
    
    % For an arbitrary stress ${\bs \xi}$ therefore holds
    % %
    % \begin{equation}
    %     \label{eq:with_stress}
    %     0 = {\bs \xi}\T \left(\mathcal R(P) \ddot P+ \mathcal R(\dot P) \dot P\right) = 
    %    \underbrace{ {\bs \xi}\T \mathcal R(P)}_{=0} \ddot P+ 
    %     {\bs \xi}\T\mathcal R(\dot P) \dot P={\bs \xi}\T\mathcal R(\dot P) \dot P.
    % \end{equation}
    % %
    % %\mhsays{Use a different symbol for the all-zeros vector? \eg\, $\overrightarrow{\rm 0}$ or $0$.} 
    % where ${\bs \xi}\T \mathcal  R(P)=0$ follows from the definition of a stress as an element of $\ker \mathcal R(P)\T$.
    % We see that $\dot P$ cannot be blocked by any $\bs \xi$.
    
    % To show ``only if'', let $A=\mathcal  R(P)$, $b=-\mathcal  R(\dot P)\dot P$, $x=\ddot P$, and $y={\bs \xi}$ and consider the two linear systems $Ax=b$ and $A\T y = 0$. We apply a linearized version of Farkas' Lemma, which implies that either $Ax=b$ has a solution, or $A\T y=0$ has a solution with $b\T y\not =0$.
    % In other words, there either exists a second-order flex $\ddot P$ or it is possible to find a blocking stress. 
\end{proof}

    % By combining the definition of second-order rigidity and \cref{lem2}, we can obtain the following result:
    % \begin{theorem}\label{res:sotest}
    %     $P$ is second-order rigid if and only if every non-trivial first-order flex has a blocking stress. 
    % \end{theorem}%\mhsays{Formulate as a theorem? This seems to be what people are usually doing in second-order rigidity papers, right?} 

In following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 

% The following notion is often more convenient to use:

%\todo{\mhsays{Expand on the relevance of prestress stability and that it is connected to second-order rigidity by swapping quantifiers?}}

% \begin{definition}
% \label{def:prestress-stable}
%     If there exists a stress that blocks every non-trivial first-order flex, we say the polyhedron is \Def{prestress stable}.
% \end{definition}

\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}

\iffalse

{\color{lightgray}

\begin{proof}
    The proof is largely analogous to the proof of \cref{res:second-order-implies-rigid}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible; and show that it is second-order flexible.
    
    Let $k$ be the smallest integer such that the first $k$ derivatives of $P^t$ do not come from a trivial flex at $t=0$. The $2k$-th derivative of the constraints can be expanded as:
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    for edge $e_{ij}$, and
    %
    \begin{equation*}
        \sum_{i=0}^{2k}\binom{2k}{i}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^i(p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k-i}(a_k^t)=0
    \end{equation*}
    %
    for vertex $v_i$ in facet $f_k$.

    Since $k$ is the smallest integer, the first, second, all the way up to $k-1^{th}$ derivative come from a trivial flex. Therefore, by adding a trivial flex to cancel these terms, we may assume that all derivatives up to the $k-1^{th}$ are all zeros. The two equations above become the following. 
    %
    \begin{equation*}
        2(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t-p_j^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t-p_j^t)=0
    \end{equation*}
    %
    and 
    %
    \begin{equation*}
        (p_i^t)\cdot \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(a_k)+\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}(p_i^t)\cdot (a_k^t)+\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(p_i^t)\cdot\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}(a_k)=0
    \end{equation*}
    %
    Set $\dot P= \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{k}P^t\big|_{t=0}$ and $\ddot P=2/\binom{2k}{k}\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{2k}P^t\big|_{t=0}$. The two above equations become Equations \eqref{eq1} and \eqref{eq2}. Therefore, if $P$ is flexible, it has a non-trivial second-order flex. 
    \mwsays{It remains to show that the motion is non-trivial.}
\end{proof}

}

\fi














\iffalse % previous first-order section

\tempnewpage

\subsection{First-order theory}

The first-order theory of polytope rigidity is the same as for point-hyperplane~frameworks.
We recall the essentials.


A \Def{first-order motion} $(\bsdot p,\bsdot a)$ of $P$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$, %=(\dot p_i\in\RR^3:i \in V;\, \dot a_\sigma\in\RR^3 : \sigma \in F)$.
that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    %\label{eq:flex_at_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{whenever $i,j\sim\sigma$}.
    %\label{eq:flex_at_vertex_face}
    \\
    \<a_\sigma,\dot a_\sigma\> &= 0,\quad\text{whenever $\sigma\in F$}.
    %\label{eq:flex_at_face}
\end{align}

A first-order motion is \Def{trivial} if in addition it satisfies
%
\begin{align}
    \<p_i-p_j,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    %\label{eq:trivial_motion_vertex}
    \\
    \<p_i-p_j,\dot a_\sigma\> + \<\dot p_i-\dot p_j, a_\sigma\> &= 0 ,\quad\text{for any $i,j\in V$ and $\sigma\in F$}.
    %\label{eq:trivial_motion_vertex_facet}
    \\
    \<a_\sigma,\dot a_\tau\> + \<\dot a_\sigma, a_\tau\> &= 0 ,\quad\text{for any $\sigma,\tau\in F$}.
    %\label{eq:trivial_motion_facet}
\end{align}
%
A non-trivial first-order motion is called a \Def{first-order flex}.
A framework is \Def{first-order rigid} if it has no first-order flexes; it is \Def{first-order flexible} otherwise.
Many results from the bar-joint framework setting transfer in the expected way. In particular, if a polytope is first-order rigid, then it is rigid. 

The first-order flex conditions \eqref{eq:flex_at_vertex} -- \eqref{eq:flex_at_face} can be collected in a corresponding \Def{rigidity matrix} $\mathcal R(P)$ % with dimensions $(E+\VF)\times(dV+dF)$. 
which satisfies $\mathcal R(P)(\dotbs p,\dotbs a)=0$ if and only if $(\dotbs p,\dotbs a)$ is a first-order motion.
%
Since we only consider polytopes with non-empty interior, they are in particular affinely spanning and
the rank condition of first-order rigidity applies: 

\begin{lemma}
    \label{res:rank_condition}
    We have
    %
    $$\corank \mathcal R(P) \ge \binom{d+1}{2},$$
    %
    with equality if and only if $P$ is first-order rigid.
\end{lemma}

\hrulefill

%\begin{definition}
    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
We write
%
\begin{align*}
    \realP{\mathcal P}P &= \realpa{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \real(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
    \\
    \realPCvx{\mathcal P}P &= \realpaCvx{\mathcal P}{\bs p}{\bs a} \\&\!:= \{(\tilbs p,\tilbs a)\in \realCvx(\mathcal P)\mid \text{$(\tilbs p,\tilbs a)$ is equivalent to $(\bs p,\bs a)$} \}
\end{align*}
%
for the (\Def{convex}) \Def{configuration space}, \ie\ the space of all (convex) realizations equivalent to a given (convex) realization $P=(\bs p,\bs a)$.

A \Def{motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\realpa{\mathcal P}{\bs p}{\bs a}$ for which $(\bs p^0,\bs a^0)=(\bs p,\bs a)$.
The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all~$t\in[0,1]$.
A non-trivial motion is called a \Def{flex}.
If a realization $(\bs p,\bs a)$ has a flex, we call it \Def{flexible}, and \Def{rigid} otherwise.
%\end{definition}

In general, understanding the full configuration space is intractable in all but the simplest cases. 
We mention here a few situations in which such a full understanding is possible due to various genericity assumptions.
In our language, Cauchy's classical rigidity theorem \cite{cauchy1813} states that $\realPCvx{\mathcal P}P$ is a single point whenever $\mathcal P$ is a simplicial polytope.
As a consequence of the main result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} we also obtain the following:

\begin{theorem}
    Let $\mathcal P$ be the combinatorial type of a 3-dimensional polytopes (\ie\ a polyhedral graph).
    Then for almost all convex (in fact, Zariski convex) realizations $P$ of $\mathcal P$ holds: $\realP{\mathcal P}P$ consists of finitely many isolated points.
\end{theorem}
%
Here, \emph{almost all} means that a dense open subset of the (Zariski closure of) the convex realization space has this property.
%
\begin{proof}
    \TODO \mhsays{$\real(\mathcal{P})$ may be irreducible, but that does not mean that $\real(\mathcal{P},P)$ is. The geometry of $\real(\mathcal{P},P)$ may be pretty complicated. We know that $P$ has generic coordinates; however, it seems like what we need to do is show that $P$ also has generic edge lengths. By going back to the edge length perturbation space and proving a stronger result than Proposition 5.2, we then may be able to prove this. The main issue is that we don't really understand the edge length measurement variety and much less the intersection of that variety with $\real(\mathcal{P})$. So I guess to conclude: I don't really have an easy idea how to approach this. You?} \mwsays{I cannot prove this at this moment. Maybe delete theorem?}
\end{proof}

We conjecture the same to be the case in higher dimensions.

Lastly, recall that a \Def{zonotope} is a polytope obtained as the Minkowski sum of finitely many line segments. A \Def{cubic zonotope} is a zonotope with all faces being combinatorial cubes. Cubical zonotopes are the zonotopal equivalent of simplicial polytopes, in the sense that they are generic in the class of zonotopes: they are generated from line segments in general position:

\begin{theorem}
If $P\subset\RR^d$ is a cubic zonotope generated from $k$ line segments, then %
$$\realP{\mathcal P}P = (\RR P^{d-1})^k.$$
\end{theorem}
%
\begin{proof}
    \TODO
\end{proof}

\fi








\iffalse % old flexible polytopes section by Martin

\tempnewpage % temporary new page

{\color{lightgray}

\section{Constructing flexible polytopes}
\label{sec:flexible_polytopes}

% To determine whether a given realization of a polytope is flexible or rigid, we need to specify what it means to continuously deform it. In Himmelmann, Schulze and Winter \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}, continuous motions are defined in terms of a notion of when two realizations of the same combinatorial type are equivalent. 

% \begin{definition}
%     Formally, we say that two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
% %
% \begin{align*}
%     \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
%     \\
%     \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
% \end{align*}
% A \Def{continuous motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$ so that
% \begin{itemize}
% \item $(\bs p^t(0),\bs a^t(0))=(\bs p,\bs a)$ and 
% \item $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% \end{itemize}
% The motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
% If a realization $(\bs p,\bs a)$ has a motion, then we call it \Def{flexible}, and \Def{rigid} otherwise.
% \end{definition}
As defined in \Cref{sec:rigidity}, a polytopal realization is flexible if it admits a non-trivial continuous motion.

\subsection{Zonotopes}

A zonotope is \Def{generic} if all its faces are combinatorial cubes. We call it generic because it generated from line segments in generic position. Generic zonotopes are the zonotopal equivalent of simplicial polytopes. For the latter the rigidity theory is classical -- they are rigid, both in first order and globally (Chauchy's and Dehn's theorem).
Likewise, for generic zonotopes a complete theory can be given.

\begin{theorem}
    Let $P\subset\RR^d$ be a rhombic zonotope with $n$ generators. Then
    %
    \begin{myenumerate}
        \item 
        $\realR(P)$ is a connected smooth variety of dimension $(d-1)n-\binom{d}{2}$.
        In particular, each polytope $Q$ combinatorially equivalent to $P$ with the same edge lengths can be deformed into $P$.
        \item if $Q\in\real(P)$ then $Q$ is a zonotope.
        \item The first-order flex space of $P$ has dimension $(d-1)n-\binom{d}{2}$.
        \item Each first-order flex of $P$ corresponds to a real flex.
    \end{myenumerate}
\end{theorem}
%
\begin{proof} \mwsays{Work in progress, these are just ``mental'' notes.}
    Consider the space of all deformations of a zonotope that preserves only coplanarity and central symmetry of the facets (the latter is in combinatorial cubes also implied by edge length constraints).
    Note that for $n$ generators there are $2\binom{n}{d-1}$ facets, and that the central symmetry of each is guaranteed by $d(d-2)$ equations: each pair of opposite vertices (of which there are $d-1$) must have a centroid identical to the centroid of the first pair; this is a vector identity with $d$ components.
    Note that this preserves coplanarity automatically.
    Likewise for an first-order flex -- there $dV$ DOFs and $2d(d-2)\binom{n}{d-1}$ constraints. Removing translations but not rotations, we obtain $dV-2d(d-2)\binom{n}{d-1}-d$ final first-order DOFs.
    Observe that the realization space is a manifold of dimension $nd$, or $n(d-1)$ if we want to preserve lengths. It is also well known that $V=2\sum_{k=0}^{d-1} \binom{n-1}{k}$.
    It remains to check
    %
    $$dV-2d(d-2)\binom{n}{d-1}-d = nd.$$
    %
    This seems to yield too few remaining DOFs ($< dn$) and so some of the constraints are redundant. Which and how many is unclear?
    
    \mwsays{Check that the fact that all inf flexes extend follows already from some general theory about realization spaces of polytopes when the realization spaces are smooth manifolds.}
\end{proof}

\begin{remark}
    More general zonotopes have non-zonotopal flexes. 
    As soon as some face of a zonotope is not a rhombus, then it is the Minkowski sum of this face with the other generators. But a polygon with more than four sides has a non-trivial (\ie\ not symmetry preserving) flex. Hence the Minowski sum of this flex with the other generators yields a non-zonotope.
\end{remark}

\begin{question}
    Is the first-order flex space of zonotopes exactly the tangent space to the finite flexes?
\end{question}

We can ask analogous questions for general Minkowski sums.

\begin{question}
    Is it true that the generic Minkowski sum (where no two faces, edge or higher, share an affine span) of rigid polytopes only has Minkowski flexes? Same first-order. More generally Is the first-order flex space of a Minkowski sum just the sum of the first-order flex spaces of the individual polytopes?
\end{question}

\subsection{Minkowski sums}

% We previously explained how \emph{generic} Minkowski sums become flexible polytopes.
% We can be more precise here.

% \begin{theorem}
%     Given polytopes $P,Q$, let
%     Let $\mathcal U$ be the set of linear subspaces of 
% \end{theorem}

Let $\mathfrak F(P)$ be the first-order flex space of $P$.

\begin{theorem}
    For a generic Minkowski sum of dimension $d\ge 3$ holds $\mathfrak F(P+Q) = \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$.
\end{theorem}
%
\begin{proof}
    \mwsays{This theorem is wishful thinking. It could be that a Minkowski sum has more (first-order) flexes than the ones that come from the summands. I think we know enough to show that $\mathfrak F(P+Q) \subseteq \mathfrak F(P)\oplus\mathfrak F(Q)\oplus \mathfrak{so}(d)$. Maybe the other direction can be proven using some limit argument.}
\end{proof}

\mwsays{Not true in $d=2$ or for non-generic Minkowski sums, consider two triangles that add up to a hexagon, or prisms over those.}

\subsection{Truncation}

If two frameworks on the same graph have the same edge directions, then they have the same first-order theory since the rows in the rigidity matrix are just multiples of each other.
The following would be a generalization to polytopes:

\begin{theorem}
    If $P$ and $Q$ are normally equivalent, then $\mathfrak F(P)\simeq \mathfrak F(Q)$.
\end{theorem}
%
\begin{proof}
    \TODO
    \mwsays{True?} \mwsays{WRONG! TIco and TDod}
\end{proof}

\mhsays{We lose all flexes when changing the truncation of the truncated dodecahedron. Therefore, the flexes are not a result of the polytopes' symmetry, but rather of the coordinates. }

\subsection{Truncation}
Questions:
\begin{itemize}
    \item Does there exist a truncation in (0,1) preserving the flexes of either of the truncated ends?
    \item Is rigidity/flexibility preserved under certain assumptions on the truncation? 
\end{itemize}

}

\fi













\tempnewpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

%The convex realization space $\realCvx({\mathcal{P}})$ of 3-dimensional polytopes of combinatorial type $\mathcal{P}$ is a smooth $(E+6)$-dimensional manifold, on which the 6-dimensional Lie group of rigid motions acts smoothly. %In fact, the reduced realization space $\realRCvx(\mathcal{P})$ is homeomorphic to an open ball (\cf\ \cite[Thm.\ 13.3]{richter2006realization}). Intuitively, this claim \emph{has} to be true, simply by subtracting the appropriate dimensions. However, proving it is %\todo{\mwsays{Not only ``slightly more subtle'', but this is a big deal :D}}
%significantly more difficult than it seems, as we are working with manifolds and associated Lie groups instead of Euclidean space.

%\mwsays{We should start with emphasizing very clearly that this section will be $d=3$ only. This is the first place in the paper where we are not general-$d$.}
%\todo{\mhsays{I reference second-order rigidity in this section. Honestly, I would prefer to switch this section with the second-order rigidity; also, because we restrict ourselves to 3D here and later relax that assumption again.}\mwsays{I am torn. The current transition from ``second-order theory'' straight to ``certifying second-order theory'' is also nice. Where do you mention 2nd-order? Only in the question? Maybe move the question?} \mhsays{I don't think there is a place for the question other than here. I could write ``rigid, but not fo rigid'', which would fix the problem. However, my main issue is that we restrict to $\mathbb{R}^3$ and then revert the restriction in the coming section. That feels confusing and unnatural. But I also understand that second-order rigidity$\Rightarrow$ certifying is a nice order. Let's discuss!}}
%\notodo{\mwsays{Use polyhedron for 3-dim polytope. Also, convex is implicit everywhere.}}
For this section, we restrict ourselves to polyhedra, \ie\ 3-dimensional polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
%\notodo{\mwsays{I still think it is a bad idea to say we study the complement. We don't really. The complement is a terrible object. It is not a variety. I would say we study $\real(\mathcal P)$ locally.}}
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polyhedra, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to %\notodo{\mwsays{I am not sure I understand ``first-order flexes which only preserve the coplanarity constraints'', or if I do, I think this is misuse of terminology because flex has a well-defined meaning always fixing edge lengths. Otherwise it is a deformation, or a curve in $\real(\mathcal P)$, but not a flex. First-order terminology we don't have for this at all.}} 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization the trivial first-order motions form a 6-dimensional subspace of the space of first-order motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$. %For that reason, $\Iso$ acts smoothly on $\real({\mathcal{P}})$ and since $\realR(\mathcal{P})$ is given by a quotient manifold of the form $\real(\mathcal{P})/\mathrm{Iso}$, 
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension%\todo{\mwsays{$\real^*$ is a smooth manifold, but the reason given here is incorrect:quotients by smooth actions can fail to be smooth.}\mhsays{Not if the group acts smoothly, freely, and properly (see citation). Feel free to rewrite the paragraph though.}} (\cf\ \cite[Thm.\ 21.10]{lee-smooth-manifolds})
%
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
%\notodo{\mwsays{You want to pin a vertex, constrain an edge to a 1-dim subspace and a face to a 2-dim subspace. Pinning the edge sounds like restricting its length.}\mhsays{Adjusted.}}%
In other words, all polyhedra have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). %\todo{\mwsays{Not enough pinning. Maybe use Louis' paper? Or just pin an edge and an constraint a vertex to a plane that is in the same face as this edge.}} 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
%\todo{\mwsays{I would not call it a coincidence that $E$ is the number of edges}}
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. %\notodo{\mwsays{\emph{``This line of thought would imply that we can locally freely perturb the edge lengths around rigid realizations''} I think it is not clear why you mention ``rigid realizations'' in this sentence.} \mhsays{Changed the sentence.}} 
Since rigid realizations correspond to isolated points in $\mreal^*(\mathcal{P},P)$, the degrees of freedom in $\realR(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.

%\notodo{\mwsays{Can't we just define existence of edge-length perturbations as that ``the map from realizations to edge length vectors is locally surjective at $P$?} \mhsays{I do not believe this avoids the invariance of domain theorem. ``continuous'' plus ``locally surjective'' just rewords what is already there and abstracts the meaning. I am not necessarily against this change, I just don't believe it is going to be impactful.}}
    
\begin{definition}
\label{def:edge-length-perturbations}
%Fix an ordering of the edges $E$ for a polytope $P$. We denote 
The
 %\todo{\mwsays{maybe ``edge length vector'', since then perturbations are a more natural thing?}}
 \Def{edge length vector} of $P$ is given by
 %\notodo{\mwsays{Should we use $(a|b)$ instead of $(a : b)$ for consistency with the other text? Or are vectors significantly different to justify different notation from sets?}}
 %
% \notodo{\mwsays{I want to suggest notation: $\bs\ell(P)$ for the edge length vector, since consistent with other indexed families like $\bs p$. Also I think it is not good to have both $\ell(e)$ and $\ell_e$. I think we should use only $\ell_e$ since we call it a vector, and $\bs\ell'$ or so if we need another vector like in the paragraph below. Next, $\mathcal L(\mathcal P)$ can now be used for the space of edge lengths vectors. Or something like $\text{\textsc{Len}}(\mathcal P)$, but I think it would be useful to have notation since we write the phrase so often}}
 %
 %\notodo{\mwsays{Why not just $\|p_i-p_j\|$?} \mhsays{So that the Jacobian is actually the rigidity matrix and we do not need the weird shenanigans with scaling.}\mwsays{A bit weird to call it the ``edge length'' vector then, but this was already weird because of the square ... so I guess this is fine :)}\mhsays{I get where you're coming from. At least it is heavily related to edge lengths. Unfortunately, I don't have a better name in mind (which does not completely ignore brevity).}}
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
% \ie\ if there are edge length perturbations arbitrarily close to ${\bs\ell}(P)$ that can not be realized as a polytope $Q$ sufficiently close to $P$, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

\iffalse 
More precisely, $P$ has all edge length perturbations if for some $C>0$ and every $\varepsilon\in (0,C]$ there exists a $\delta>0$ such that every edge length vector $\bs\ell'$ with 
%
\[\text{dist}({\bs\ell}(P),\,\bs\ell')<\delta\] 
%
there exists a polytope $Q=\psi(\bs\ell')$ of the same combinatorial type as $P$ that satisfies
%
\[\text{dist}(P,\,Q)<\varepsilon\] 
%
in the Euclidean metric on $\mathbb{R}^{d(V+F)}$. This definition implies that the edge length map $\bs\ell:\real(\mathcal{P})\rightarrow\mathbb{R}^E$ is locally surjective around $P$. \fi

%\todo{\mhsays{Add the following? Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, the Legendre-Steinitz theorem is necessary to state the following results, justifying this restriction.}\mwsays{My suggestion: ``... however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.''}} 
%
Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.

Let us first consider an example of the first-order rigid regular tetrahedron. For this polyhedron, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    As a polytope, it is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polyhedron is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$, as a bar-joint framework, meaning that the removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the corresponding value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polyhedron's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polyhedra concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid polyhedron $P$ has all edge length perturbations.
    \iffalse
    \begin{proof}
    %\notodo{\mwsays{I find this confusing: we start talking about reduced non-metric realization space, but then continue with the Jacobian, which is the tangent space of the non-reduced metric realization space}}
    %The reduced realization space of a convex polytope $\realR(\mathcal{P})$ is a smooth $E$-dimensional manifold, where $E$ denotes the number of edges of $P$. 
    Assuming that $P$ is %\todo{\mwsays{First-order rigid}}
        first-order rigid, the rigidity matrix $\mathcal{R}(P)$ has the minimal corank $6$ (\cf\ \cref{res:corank_rigid}), so its rank is $dV+dF-6$. 
        %In particular, $P$ is a regular point of $\mreal(\mathcal P, P)$. 
        %This implies that all sufficiently close realizations of $P$ are also first-order rigid: the Jacobian matrix of a polynomial system drops rank in a proper algebraic subset of lower dimension, implying that around every \todo{\mwsays{Let's not talk abut regular points --  we did not introduce the relation between regular points and first-order rigidity (via generic rigidity). Since we only care about the rigidity, let's just reference \cref{res:corank_rigid}}\mhsays{But this doesn't give us that all sufficiently close realizations are first-order rigid, does it? We need something algebraic here.}}regular point of an algebraic variety there is an open neighborhood of regular points \cite[Thm.\ 5.3]{hartshorne}.
%This implies that $\mreal({\mathcal{P},P})$ locally forms a 6-dimensional manifold around the realization $P$ which is locally parametrized by $\mathrm{Iso}$.
Moreover, the realization space $\real(\mathcal{P})$ is a $(E+6)$-dimensional manifold according to the Legendre-Steinitz theorem, which implies that its tangent space $T_P(\real(\mathcal{P}))$ at the realization $P$ also has dimension $(E+6)$. Moreover $\real(\mathcal{P})\subset\mathbb{R}^{dV+dF}$, so that the dimension of the normal space of the realization space $\real(\mathcal{P})$ is equal to $dV+dF-(E+6)$. Since the rows of the rigidity matrix $\mathcal{R}(\mathcal{P})$ are exactly given by a basis of the normal space of $\real(\mathcal{P})$ (\cf\ \cite[Proposition 5.38 and Section 6]{lee-smooth-manifolds}) and the Jacobian %\todo{\mwsays{$d\bs\ell$? Not $J\bs\ell$? If you insist on $d$, can we do $\mathrm d\bs \ell$ or $\partial \bs \ell$ or $\delta\bs\ell$? $d$ is already the variable for the dimension.}}
$d\bs\ell$ of the edge length map $\bs\ell: \real(\mathcal{P})\rightarrow \mathbb{R}^E$, the rank of the rigidity matrix satisfies the inequality
%
\begin{eqnarray*}
    dF+dV-6=\rank(\mathcal{R}(P))&\leq& \rank(J\bs\ell(P))+\dim(T_P(\real(\mathcal{P}))^\perp)\\
    &=&\rank(J\bs\ell(P))+dV+dF-(E+6)\\[3mm]
    &\Rightarrow& \rank(J\bs\ell(P))\geq E
\end{eqnarray*}
%
    On the other hand, $\rank(J\bs\ell(P))\leq E$ by construction, which implies that the rank of $J\bs\ell(P))$ is equal to $E$. Thus, the Jacobian $J\bs\ell(P)$ has full rank. Consequently, $\bs\ell$ is locally a submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}), which implies that $\bs\ell$ is locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). Therefore, all sufficiently small edge length perturbations are realizable.
    \end{proof}
\fi
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    %\notodo{\mwsays{In the rest of the section your write $E$ instead of $E$ for cardinalities.}\mhsays{I reckon you prefer using $E$ for cardinalities? How do we call the set of edges then?}\mwsays{I prefer $E$ for the set and the number. I reckon you are not okay with this abuse of notation. And since we already do it differently everywhere else, lets just use $|E|$, no?}\mhsays{No, I am fine with it. We should just be consistent and say it once in Section 2 that we use them interchangeably.}}
    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). %\todo{\mhsays{There is a gap in the proof here, since the definition requires the existence of $\ell^{-1}$ (sort of), so we need to construct a continuous map from $\mathbb{R}^E\rightarrow \real(\mathcal{P})$} \mwsays{This is easy enough by quotienting by the Iso-action. But let's not touch this before we have figured out the definition problem}}
    %Therefore, all sufficiently small edge length perturbations of $P$ are realizable.
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of polyhedra are first-order rigid.  
This result requires a suitable definition of \emph{genericity}, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polyhedra to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 

%\mwsays{``For a suitable definition of generic, see \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}:''. Random Coordinates}


\begin{corollary}
    Generic realizations of polyhedra have all edge length perturbations.
    \begin{proof}
        Take any polyhedron $P$. In \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} it is shown that any generic realization of a polyhedron is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polyhedron in the following example. This example highlights that not all realizations of a polyhedron have all edge length perturbation.

%\notodo{\mwsays{Proposal: we bring the two examples as motivation; we take the locally surjective definition; we prove fo-rigid implies all perturbation exist; we discuss whether the cube example can be generalized; we give Theorem 5.6 as a question; we discuss the $z^2$ problem; we prove flexible implies not all perturbations exist under the additional example of continuous inverse (maybe constant fiber?).}}

\begin{example}
\label{ex:cube-edge-length-perturbations}
    %\todo{\mwsays{I think this example is very educational and should, together with a positive example, come in the beginning of this section}}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polyhedron, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    %\notodo{\mwsays{``antipodal edges'' better?} \mhsays{Sure}}
    antipodal edges. 
\end{example}

We can turn the observation from this example, that not all polyhedra admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polyhedron's edge length vector to distinct polyhedra sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the polyhedron $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        Assume now that all of $P$'s edge length perturbations are realizable via 
        % Then, in particular, we can locally extend and contract each of $P$'s edges individually. In fact, we can arbitrarily combine these edge length perturbations, %\todo{\mwsays{``Since we factored out Euclidean isometries'': how does this imply the second half of the sentence?}}Since we factored out Euclidean isometries, 
        %so that each combination of edges that we perturb gives rise to a \emph{distinct} continuous deformation of $P$. This implies that there is an open ${E}$-dimensional ball of realizable edge length perturbations containing ${\bs\ell}(P)$. Therefore, the map 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. As a consequence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi=\varphi^{-1}\circ(\varphi\circ \psi)$ and $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        
        Consequently, there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ through the realization $P$ which preserves the edge lengths ${\bs\ell}(P)$, so $P$ is rigid. 
    \end{proof}
\end{theorem}
%
The assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. This restricts the family of admissible polyhedra.

Since \Cref{thm:rigidity-and-edge-length-perturbations} provides a sufficient condition for the rigidity of polyhedra, its contrapositive yields information about the reduced realization space $\realR(\mathcal{P})$. This observation is sufficiently useful to state explicitly as a corollary. Albeit, it is currently unclear whether checking the theorems preconditions offers any advantage over directly verifying a polyhedron's rigidity or flexibility.

\begin{corollary}
    If a polyhedron $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}
%
Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample. 
\begin{remark}
\label{res:square_root_branching}
Consider $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.
\end{remark}

However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 

The correspondence between the edge length realization space of a polyhedron and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polyhedron is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

%\notodo{\mwsays{Can we make the first two questions into one with (i) and (ii) since they are just inverses of each other?} \mhsays{I was contemplating that, too. Fixed.}}

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polyhedron $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization~of a polyhedron have all edge length perturbations?
\end{question}

%\notodo{\mwsays{In the question below, do you also want to ask that it is not first-order rigid? Otherwise the tetrahedron is a counterexample. And maybe move this question to the end of the so-theory section? Depends on if we move this section of course.} \mhsays{True. Thanks for pointing out this oversight. I chose to replace it by ``rigid, but not fo-rigid''.}}

% \begin{question}
% Assuming a convex polytope $P$ is rigid, but not first-order rigid, is ${\bs\ell}(P)$ then singular in the edge length realization space $\mathcal{L}(P)$ (see \cref{fig:edge-contraction-deformation-space})?
% \end{question}

%\todo{\mhsays{I might delete this question, since I find it confusing in the context of Legendre-Steinitz and it is not formulated precisely, since we only change the length of a single edge.}}

%While we do not understand the edge length realization space of polytopes nearly enough to provide answers to these questions, they provide interesting observations that should be investigated in future research.\todo{\mwsays{You essentially repeat the last sentence before the questions}}

%\todo{\mhsays{Technically, we could also move this section to the appendix if need be. Without \Cref{thm:rigidity-and-edge-length-perturbations}, this section is not what it used to be.}}















\pagebreak

\tempnewpage

\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}
\label{sec:so_certificate}
%\notodo{\mhsays{Add page break?}\mwsays{Not great, but looks okay enough.}}

%\todo{\mwsays{Use $\mathcal{R}$ for rigidity matrix}}

As laid out in \Cref{sec:second-order-theory}, any first-order flex of a polytope 
%in the edge-length realization space \mbox{$\mreal(\mathcal{P},P)$} 
that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. 
%This provides a convenient heuristic for finding non-blocked first-order flexes: 
That is, according to \Cref{res:sotest}, there exits a first-order flex $\dot P$ so that for all equilibrium stresses $\bs \xi$ we have $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$.
Conversely, if for each $\dot{P}$ there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$, then the polytope is 
%\notodo{\mwsays{In fact, PSS. Is this the proper converse that you want to state here?} \mhsays{Good catch, thanks.}}
second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the first-order flex space via a basis ${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ with variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ with variables $\mu=(\mu_1, \dots, \mu_s)$. %\mhsays{According to \Cref{res:flex_eq_stress}, it even holds that $r=s$.} 
%\todo{\mhsays{Potentially rename the indices $r,s$? Or keep them? Normally, I would use $n,m$, but we already use those names.}}
%\todo{\mhsays{Mention $s=r$ according to \Cref{res:flex_eq_stress}; also mention below that the system $\nabla _\mu E_{\dot{P},\bs\xi}(\lambda)=0$ further below}}
%\notodo{\mwsays{refer to \eqref{res:sotest} explicitly}\mhsays{done}}
This turns the second-order condition \eqref{block} into the cubic polynomial% of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, the homogeneous polynomial $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding $\mu$ for each $\lambda$ so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.
%
%\notodo{\mhsays{Remove this line break?}}
%
By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is non-zero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. 
Therefore, the first-order flexes that are not blocked by any stresses can be parametrized by the solutions of the %\mhsays{square}
polynomial system $Q_1=\dots= Q_s=0$, which form an algebraic set. %\todo{\mwsays{Is this clear?}}
This system can also be represented by the gradient of $E_{\dot{P},{\bs\xi}}$ with respect to $\mu$ to obtain $\nabla_\mu E_{\dot{P},{\bs\xi}}(\lambda)=0$.

%\todo{\mwsays{Why does this suffice? Finitely many solutions are still solutions. Further below you explain that finite implies empty due to homogeneity. This should come here, no?} \mhsays{We are in projective space, so finitely many solutions implies positive-dimensional solution space.}\mwsays{I know. This is mentioned below because it is necessary for the argument. But it must be mentioned here because the argument is already used here.} \mhsays{Potentially I can just remove/replace this sentence here, since I explain it in the next paragraph anyway.}\mwsays{That is possible. Just without a comment this sentence is confusing}}
We will later see that the zero-dimensionality of the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$ is sufficient for second-order rigidity. As a criterion for that, we formulate the following. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field %\todo{\mwsays{Can we use $\Bbbk$ for the field?}}
        $\Bbbk$. Given an ideal $\mathcal{I}=\langle f_1,...,f_s\rangle$, where $f_i\in \Bbbk[x_1,..,x_r]$, and a Gröbner basis $\mathcal{G}$ of $\mathcal{I}$. Then, $\mathcal{I}$ is zero dimensional if and only if for every $i\in\{1,...,r\}$ some power of $x_i$ is the leading monomial of an element of $\mathcal{G}$.%\mhsays{Only for algebraically closed $k$? If so, replace $k$ by $\mathbb{C}$. Else, define what $k$ can be. }
    \end{lemma}

Of course, there are also other methods based on Gröbner bases to verify that an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic set $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homogeneous, it holds that \[\left(Q_1(c\cdot \lambda^*),\,\dots,\,Q_s(c\cdot \lambda^*)\right)=\left(c^2\cdot Q_1(\lambda^*),\,\dots,\,c^2\cdot Q_s(\lambda^*)\right)= 0\] 
for any $c\in \mathbb{C}$ and any $\lambda^*\in \mathcal{V}(\mathcal{I})$. In other words, all scalar multiples $c\cdot\lambda^*$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\{0\}$.
%\notodo{\mwsays{for Matthias: Projective comment.}}
In our context, this translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system %\notodo{\mwsays{Since this proposition tries to be self-contained, one should repeat what is the \emph{finite} system. As written down I don't see a system but only one equations. What do we quantify over? Alternatively, refer to (6.1), but also name what finitely many indices we quantify over.}}
    %\notodo{\mwsays{I was confused for the wrong reasons, but I am still confused: where does nabla come from?} \mhsays{It's the gradient. This is standard notation. I added a line above to explain this.}\mwsays{My question should have been: where does the gradient come from? I agree the notation is standard. But I think I found the sentence where this is explained.}}
    $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ defined in \eqref{eqn:stress_polynomial_Qi} only has $\lambda_1=\dots=\lambda_r = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)=0$.
\end{proposition}

%\mhsays{Describe Test for prestress stability: Albert's code.}

%\notodo{\mwsays{This paragraph reads to me like: we were lucky that our technique worked for the polytopes we tested it on, but there was no guarantee. If true, this is new to me and this is not how we sell it in other parts of the paper.} \mhsays{Why would there be a guarantee? I don't see how we could prove something like that. We use an established sufficient condition, which works over $\mathbb{C}$ and lets us certify second-order rigidity in the cases we consider. I don't believe it is necessary. We can easily tweak it though in case we ever need it by using the Euclidean distance degree, which has a significantly higher complexity, so I wouldn't worry too much about that (last sentence). }\mwsays{I think I understand now: even if the algorithm says ``no'', it might still be so-rigid.}}
The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all polytopes tested in \cref{sec:experimental_results} (\cf\ \Cref{tab:comparison} and \ref{tab:catalan-comparison}). Still, %\notodo{\mwsays{I am stumbling with the sentence structure here: what is not necessary for what?} \mhsays{elaborated.}}
our result using Gröbner bases is clearly not necessary for second-order rigidity, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})=\{0\}$ over the real numbers, even when we find non-trivial solutions over $\mathbb{C}$. A simple counterexample is given by the equation $x^2+y^2=0$, which only has $x=y=0$ as a real solution, yet the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solution on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}). By appending the equation $\sum_{i=1}^r\lambda_i^2-1$ to the ideal $\mathcal{I}$ which describes the unit hypersphere, we guarantee that this approach only finds non-trivial solutions. We also do not lose any solutions beyond the origin due to the invariance of solutions under scalar multiplication.

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a $\mu\in \mathbb{R}^s$ defining a %\notodo{\mwsays{Why ``linear combination of stresses $\mu$'' instead of ``stress $\mu$?}}
stress ${\bs\xi}=\sum_{j=1}^s \mu_j\cdot {\bs\xi}_j$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu_j$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix
%
$$\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_j\lambda_k}Q_j(\lambda)\right)_{j,k=1}^r$$
%
is positive definite for some choice of $\mu$. 






\tempnewpage

\section{Second-order rigidity of the regular dodecahedron}
\label{sec:so_rigidity_dod}

Among the Platonic solids, there is only one for which the question of rigidity is not answered immediately.
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid by Dehn's theorem \cite{dehnstheorem}. 
The cube is the classical example of~a~flexible polytope.
Solely the regular dodecahedron remains to be understood and initially eluded direct computation.

Symbolic computations reveal a 5-dimensional space of first-order flexes and a~5-dimensional space of stresses.\footnote{The specific embedding and orderings of vertices, edges and faces are provided in \cref{appendix:comp-data-dodecahedron}.}
%
Note that these dimensions must be identical~due~to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
%
It is tempting to somehow relate the dimensions of the flex and stress spaces to the 5-fold symmetries of the dodecahedron.
We have no evidence~for such a relation, and rather mild counter-evidence in the case of the truncated~dode\-cahedron (see \cref{sec:selected_rigidity}).


\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

% By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
% \footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
% Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
% %\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
% Consequently, the regular dodecahedron is not first-order rigid.

%We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. 

Since the regular dodecahedron is not first-order rigid, it is a promising test case for the second-order certificate from \cref{sec:so_certificate}.
Concretely, \cref{prop:stress-energy-condition} asserts that it suffices to compute the zeros of a certain polynomial system. 
We~proceed~as follows:
%
\begin{enumerate}
    \setlength{\itemsep}{0.7ex}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. 
    Using the~bases, we parametrize the spaces by variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$.
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadric forms $Q_i$. % (see \cref{section:second-order-rigidity-check}).
    
    \item Use the equivalence in \cref{gbasis} to determine whether the system~has~fi\-nitely many (real) zeros.
    This is the case for the regular dodecahedron.
    
    \item Use \Cref{prop:stress-energy-condition} to infer second-order rigidity.
\end{enumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. Then, $\mathcal{I}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}.
    For more specifics on the relevant \textsc{Mathematica} files, see \cref{appendix:comp-data-dodecahedron}.
    With the help of this Gröbner basis, we obtain the following results:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        The monomials $\lambda_1^2$, $\lambda_2^3$, $\lambda_3^3$, $\lambda_4^5$,  $\lambda_5^6$, appear as leading monomials in the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$.
        \Cref{gbasis} therefore implies that $\mathcal{I}$ is zero-dimensional. 
        %By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). 
        Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. 
        By \cref{prop:stress-energy-condition}, for any non-zero linear combination of the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. 
        By \Cref{res:sotest}, $P$ is second-order rigid. 
        By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

Having understood the rigidity properties of the Platonic solids, a natural move is to extend the search to the next best well-documented class of polytopes -- the Archimedean and Catalan solids.
A detailed account of the findings is given~in~\cref{sec:archimedean} (see also \cref{tab:comparison} and \cref{tab:catalan-comparison}).

Among the 31 polytopes checked, only three are not first-order rigid, but also not predictably flexible (\cf\ \cref{sec:dimension_estimates}): the regular dodecahedron, the truncated icosahedron and the truncated dodecahedron (\cf\ \cref{fig:Dod_TIco_TDod}).
The procedure above was applied to all of them, and our findings are documented in \cref{sec:selected_results}.


% \begin{remark}
%     Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid}). The contraposition of \Cref{gbasis} can be used to show that the truncated dodecahedron is \emph{not} second-order rigid (see \Cref{res:TDod_not_Second_order_rigid} for details).
%     % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
% \end{remark}\todo{\mwsays{Incorporate TIco and TDod into Remark}\mhsays{I made an attempt. Feel free to change.}}











\tempnewpage

\section{Computational results: Platonic, Archimedean and Catalan solids}
\label{sec:experimental_results}
\label{sec:archimedean}

% \todo{\mwsays{Note to myself: add this footnote somewhere: The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}\mhsays{Is this footnote now part of Section 7?}}


We apply our techniques to the Platonic, Archimedean, and Catalan~solids.\nls
For these classes combinatorial data and algebraic vertex and normal coordinates are readily available.%
%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}}
%
The results are shown in \cref{tab:comparison} (for the Platonic and Archime\-dean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation for the content of the tables is given in \cref{sec:explain_table}.
%
%A more detailed step-by-step~expla\-nation for how the second-order rigidity results were obtained is given in \cref{section:rigidity-of-the-regdod} on the example of the regular dodecahedron.
%
A key takeaway is that already simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
See \cref{sec:selected_results}, \ref{sec:selected_rigidity} and \ref{sec:selected_flexibility}~for a discussion of the results.


\newpage
\vspace*{6mm}
\input{sec/table1}
\newpage

\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{1ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    %{\color{gray} 
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semi-definite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
    A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate for our setting.
    
%\mwsays{Something about how the numerical computations are sufficiently stable and the results away from zero or whatever so that we can trust them.}\mhsays{Replace ``We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.'' by: The numerical results are based on an eigenvalue computation, for which \noBut\ indicates the existence of an eigenvalue close to machine precision ($\approx 0$), whereas \yesBut\ indicates the existence of an eigenvalue whose absolute value lies above $10^{-6}$, which is sufficiently far away from zero. We observe no intermediate eigenvalues. Since eigenvalue computation is numerically stable and the thresholds have been chosen conservatively, we have a high degree of confidence in these results.}\mwsays{Then we should probably only explain \noBut, because \yesBut\ is never used. And also: do we ever explain this eigenvalue stuff in the paper? I don't remember having done anything with eigenvalues in Mathematica when I checked prestress stability.}\mhsays{I guess you solved an SDP of the form $C=\lambda_1\cdot A_1+\dots+\lambda_4\cdot A_4$ to find an assignment of $\lambda_i$ that makes $C$ positive definite. However, we always found a zero eigenvalue I guess? I don't exactly recall.}
    %}\mwsays{Okay, let's look into Albert's code to see what can be said.}
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flexe space} as introduced in \cref{sec:first_order}.
    %\nls Heu\-ristically, it is the expected number of independent ways in which the polytope can deform in first order. 
    %If the number is zero, the polytope~is first-order rigid. 
    %If the polytope is a generic Minkowski sum, the dimension~decomposes as explained in \cref{sec:generic_Msum} (see also \SymThree\ below).
    In some cases we have a good understanding for how~the~dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension. 
    If further explanations are available, this is indicated by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and more theoretical background given in \cref{sec:dimension_estimates}.
    %
    %\todo{\mhsays{Maybe only refer to \SymTwo\ and \SymThree\ here? \ie\, ``see \SymTwo\ and \SymThree\ for an explanation of the number''? Otherwise we write it twice.}}
\end{enumerate}
%
The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{1ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension for the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
    %If~the zonotope is generic (\ie\ all faces are rhombi), the dimension of the first-order flex space is precisely $2\times\#\text{generators}-3$ (see \cref{res:generic_zonotope}).
    %For~general zonotopes a lower bound is given~by $\dim\GL(\RR^3)-4=5$ (with a few exceptions, see \cref{res:bound_zonotopes}).
    
    % The dimension of the flex space of a generic Minkowski sum is at least the sum of the dimensions of the flex spaces of the summands, plus the dimension of the Lie group that parametrizes the relative orientations of the summands.
    % For this class we write the flex space dimension in the table as a sum of these two contributions.
    
    % %show how this dimension decomposes into flexes coming from flexes of the Minkowski summands (left term) and flexes coming from the relative orientation changes of the Minkowski summands (right term). 
    % For example, the \emph{rhombicuboctahedron} (\cf\ \cref{tab:comparison}) is a Minkowski sum of a cube and an octahedron. The cube provides itself three dimensions~for the flex space, whereas the octahedron provides none. The remaining three dimensions come from $\mathrm{SO}(\RR^3)$, which encodes the relative orientation of~the cube and octahedron. We denote this by 3+3.
\end{itemize}
%
%These considerations are elaborated in \cref{sec:dimension_estimates}.
Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
Again,\nls details are given in \cref{sec:dimension_estimates}.

% \mwsays{In all cases our heuristic lower bounds match the actual dimension of the flex space. In some cases (permutahedra) this is especially remarkable since it suggests that the combinatorics and edge lengths constrains enforce a zonotopal realization.}


\iffalse
Numerical experiments reveal that all these properties are sensitive to small changes in the polytope's geometry.
First, applying a generic linear transformation resulted in a first-order rigid polytope. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants resulted in a first-order rigid polytope. 
At this time it is unclear why exactly the realizations with uniform edge lengths are flexible in first- and second-order. 
In particular, we see that these properties are not a consequence of the polytope's symmetry alone. %, since symmetries are preserved by changing truncation height.
\fi

\pagebreak

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding table cells are marked with \Star):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} have identical~rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes), nor prestress stable; yet, \emph{both are second \mbox{order} rigid}. 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    %In \Cref{sec:dodecahedron}, we therefore provide a detailed case study about the regular dodecahedron.
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct concepts.
    Previous examples of this distinction were compa\-ratively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
    %
    In fact, we verified symbolically that $Q_i=0$ for all quadratic forms in~\eqref{eqn:stress_polynomial_Qi}. Second-order flexibility then followed via \cref{prop:stress-energy-condition}.
    %
    Since at this time no 
        %\notodo{\mwsays{Is it correct to say that there are none? Or just that we are not ready to apply them?}\mhsays{methods/algorithms}}
    methods exist to test rigidity beyond the second order, we do not know whether the truncated dodecahedron is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. %\notodo{\mhsays{??? But it does ??? Also, for higher-order rigidity, this sentence makes no sense. Just remove?} Maybe ``that the second-order rigidity theory is not sufficient''?\mwsays{Implication was the wrong way around, fixed it.}}. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). % or the \emph{cusp mechanism} \cite[Figure 3]{higher-order-rigidity}).
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
    %Some potential flexes that preserve many symmetries have been computed numerically (see \cref{fig:TDod_flex}).\todo{\mhsays{This sentence again raises hope that the truncDod is flexible (and that we have evidence for that). I suggest removing it, since the discussion on what the flex looks like is too lengthy. Would fit the outlook nicely though.\mwsays{We can remove it here. But it would be good to mention somewhere in the introduction what the figure is about. Any idea where?}\mhsays{I would like to move the figure, too.}}}
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above are sensitive to small changes in the their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.

\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty non-simplicial polytopes that are first-order rigid, for example, the truncated tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theoretical tools are available that would identify these as rigid a priorily.
We therefore formulate the following question:

\begin{question}
    %It is not possible to certify the first-order rigidity of all polytopes from \cref{tab:comparison} and \cref{tab:catalan-comparison} by only using Dehn's theorem \cite{dehnstheorem}. For instance, the truncated tetrahedron and the \notodo{\mwsays{You probably don't mean the rhombic dodecahedron, because it is a generic zonotope and hence fo-flexible}.\mhsays{Fixed}}deltoidal icositetrahedron are first-order rigid, even though they are not simplicial. 
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps polytopes whose faces are triangles and 4-gons are simple enough for a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.


% \mwsays{Here would be a good place to put Question 3.5} \mhsays{I agree}

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained from actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} match the values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.





\input{sec/table2}









% \tempnewpage

\pagebreak

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}

Due to its previous status as the guiding example,
%
we single out the dodecahedron once again for a closer inspection.
%
Exploring its realization space close to the regular dodecahedron helps us better understand the source of its exceptional behavior.
%
From that, we draw conclusions about the global rigidity of the polytope.






\iffalse

{\color{gray}
In \cref{sec:dodecahedron} we follow up with a detailed case study of the regular dodecahedron.
The experiments suggest that the regular (\ie\ maximally~symmetric) realization of the dodecahedron is a singularity in its realization space.
%
\todo{\mhsays{This is impossible according to Legendre-Steinitz. Rephrase!}\mwsays{True}}
%
}


    \begin{itemize}
    \item First-order flexible, that is lost under affine trafo
    \item not prestress stable
    \item Second-order rigid
    \item single edge length perturbable
    \item perturbations are not globally rigid
\end{itemize}
\fi

\iffalse % old rigidity section

\subsection{Rigidity} 
\label{section:rigidity-of-the-regdod}

By symbolically computing the space of first-order flexes and stresses associated with the regular dodecahedron, we find that their dimensions are five.%
\footnote{The specific embedding, computations, and orderings of vertices, edges, and facets are all provided as \textsc{Mathematica} code in the Supplementary Material \cite{zenodo_suppMaterial}. For the regular dodecahedron, see also \cref{appendix:comp-data-dodecahedron}.}
Note that these dimensions must be identical due to \cref{res:flex_eq_stress}.
%\todo{\mwsays{Ordering of sentences is weird. Put the sentence about Mathematica etc in a footnote?}}
Consequently, the regular dodecahedron is not first-order rigid.

We still intend to show that the regular dodecahedron is rigid through an algebraic computation reliant on Gröbner bases. In \Cref{sec:second-order-theory}, we introduce a sufficient condition for the rigidity of a polytope called second-order rigidity. \Cref{prop:stress-energy-condition} asserts that computing the zeros of a certain polynomial system lets us certify this property. For that reason, we employ the following strategy:

\begin{myenumerate}
    \item 
    %\todo{\mwsays{Here it becomes visible that there are equally many fo-flexes and stresses. Do we want to leave this uncommented? Because the section that explained this was just removed.}\mhsays{Do we comment on this in the last paper? I think this is a nice property. I don't think this is the place to mention it though.}\mwsays{The last paper did not mention stresses, so no. I could mention it in the stress section, but here is the first time we observe/use it.}\mhsays{Thanks for clarifying. I think the correspondence is sufficiently nice to be mentioned. If it was up to me, you can move it to the stress section.}}
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. We parametrize these bases via variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$, respectively. 
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadrics $Q_i$ (see \cref{section:second-order-rigidity-check}).
    
    \item Employ \Cref{gbasis} to show that this system has finitely many zeros.
    
    \item According to \Cref{prop:stress-energy-condition}, this implies that the regular dodecahedron is second-order rigid.
\end{myenumerate}

\iffalse

    Expand $\omega \mathcal{R}(\dot P)\dot P$ in terms of $y_i$, we have $$\omega\T \mathcal{R}(\dot P)\dot P=\sum_{i=1}^5 x_i Q_i(y_1,...,y_5)$$ where $Q_i$ are quadratic forms in terms of $y_i$, with specific values given in the Appendix. 

    If any of the $Q_i$ is non-zero for a given $y$, then we can find an $x$ such that $\omega$ blocks $\dot P$. Therefore, the first-order flexes corresponding to a $y$ that are not blocked by any stresses must live in the algebraic set that is the intersection of the zeros of $Q_1,...,Q_5$. Since the polynomials $Q_1,...,Q_5$ are homogeneous, it is sufficient to show that there are only finitely many elements in the algebraic set. 

    The following lemma is a standard result in computational algebraic geometry that can be found in textbooks such as \cite{Basu_Pollack_Coste-Roy_2010}. 
    \begin{lemma}\label{gbasis}
        Given an ideal $I=(f_1,...,f_n)$, where $f_i\in k[y_1,..,y_m]$, and a set of Gröbner bases $\mathcal{G}$. $\mathcal{G}$ is zero dimensional if and only if some power of $y_i$ is the leading monomial of an element of $\mathcal{G}$ for every $i\in\{1,...,m\}$
    \end{lemma}
\fi
    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}. With the help of this Gröbner basis, we can prove the following theorem:
   % \Cref{gbasis} implies that $\mathcal{V}(\mathcal{I})$ has only finitely many complex roots and, therefore, finitely many real roots. 
%The ideal is generated by homogeneous polynomials, so the only real solution is $\lambda_1=\lambda_2=\dots=\lambda_5=0$. As a result, every possible non-zero linear combination of the generators $\dot{P}_1,\dots, \dot{P}_5$ has a blocking stress. Consequently, the regular dodecahedron is second-order rigid and therefore rigid. We have proved the following theorem:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. As a result, for any non-zero $\dot P$ generated by the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. By \Cref{res:sotest}, $P$ is second-order rigid. By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

\begin{remark}
    Second-order rigidity of the truncated icosahedron is obtained analogously (see \Cref{res:TIco_Second_order_rigid} for details).
    % Using analogous techniques to \Cref{dodecahedronrig}, we can show that the truncated icosahedron is also second-order rigid (\cf\ \cref{tab:comparison}).
\end{remark}

\fi







\subsection{Deformation paths}
\label{section:dodec-edge-length-perturbations}


%\todo{\mwsays{Potentially incorporate: ``By computing deformation paths that shrink or extend a single edge of the regular dodecahedron we probe the neighborhood of this singularity. We find bifurcating deformation paths and from this, we construct  a counterexample to generic global rigidity for polytopes.''}\mhsays{Done}}
%
By the Legendre-Steinitz theorem the reduced realization space $\realR(\mathcal{P})$ of the dodecahedron is a smooth $30$-dimensional manifold. 
%\notodo{\mwsays{What has Sec 5 to do with this}\mhsays{I guess I am talking about the introduction, where I derive $\dim(\realR(\mathcal{P}))=|E|$. Feel free to rephrase.}}
%\Cref{section:edge-length-perturbations} we can say more: its reduced realization space $\realR(\mathcal{P})$ is a smooth $30$-dimensional manifold. 
The dodecahedron is rigid by \Cref{dodecahedronrig}, suggesting that these 30 degrees of freedom translate directly into changes in the lengths of its 30 edges.
Although we formulate the hope that all edge length perturbations of rigid polytopes are realizable in \Cref{conj:edge_length_perturbations}, even for the regular dodecahedron it is completely unclear whether this statement true.

Due to dodecahedron's high symmetry (all edges are the same), one might suggest to deform a single edge and, if this is possible, to conclude that arbitrary perturbations are possible.
In this section, we investigate the deformations of the regular dodecahedron induced by shrinking or extending a single edge. 
By approximating such deformation paths using methods explained in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of $P$ this polytope in $\realR(\mathcal P)$. 
However, whether this implies that all edge length perturbations are possible, must remain open.
%With this approach, we describe bifurcating deformation paths, which lets us construct a counterexample to generic global rigidity for polytopes.

%Due to dodecahedron's high symmetry, all edges are combinatorially identical. It does not matter which edge is chosen. 
For this experiment, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert~ < 1$. 
Sampling from the realization space intersected with the real algebraic set of prescribed edge lengths reveals \textit{six} distinct arcs starting in the regular dodecahedron corresponding to the shrinking of a single edge and \textit{two} corresponding to its expansion (see also \cite{deformationpaths}). 

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by perturbing a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge constractions, whereas gray curves correspond to edge expansions. On these curves, the eight corresponding realizations at $\ell^*(\pm 0.25)$ are depicted. Four realizations are connected by a nodal cubic (dark blue dashes).}
            %Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
 
%
%\notodo{\mwsays{Is this sentence just repeating what we said before? Or should it come much earlier? Also what is the ``also'' doing here?}\mhsays{Good point. I moved it.}}
%
In \Cref{fig:edge-contraction-deformation-space}, we depict a random projection of the deformations induced by edge contractions 
%\notodo{\mwsays{I am not sure this dashed line will be universally understood to be blue} \mhsays{Like this?}\mwsays{Much better!}}
(blue) and expansions (gray), alongside eight realizations at $\ell^{\star}(\pm 0.25)$.
Remarkably, it appears that some of these arcs rejoin smoothly. 
For instance, the gray arcs corresponding to an edge expansion have the same tangent in the regular dodecahedron, and so do suitable pairs of arcs of the blue curves. 
Moreover, the arcs corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (dark blue dashed curve).
%todo{\mwsays{Give a different color to nodal cubic so it is easier to refer to.}} %In particular, the regular dodecahedron is a singularity in the deformation space induced by all possible modifications of a single edge. 
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron since there are multiple realizations with the same edge lengths arbitrarily close to the regular dodecahedron. Hence, it is possible that there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$ in this case (\cf\ \Cref{res:square_root_branching}). 
%
%\notodo{\mwsays{We could refer here to your example with squaring a complex number in Sec 5, if it would be a numbered remark or so.}}

In total, three curves are passing through the regular dodecahedron that are induced by length changes of a single edge. 
Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective sum of the tangent vectors is sufficiently close to zero. 
We attach an animation of the smooth deformation passing through the regular dodecahedron on the solid blue path from $\ell^*(-0.25)$ via $\ell^*(0)$ to $\ell^*(-0.25)$ in the Supplementary Material \cite{zenodo_suppMaterial} of this article.%\todo{\mwsays{How is this possible? Expansions and contractions don't match smoothly. Or do you decelerate to speed 0. Maybe clarify?}}

Additionally, we find that in the case of edge contractions there are two types of deformations: those that react to the edge contraction by flattening horizontally (see \Cref{fig:edge-contraction-deformation-space}, top) and those that flatten vertically (see \Cref{fig:edge-contraction-deformation-space}, bottom). Both types contain one realization with two reflection symmetries, and two realizations with only one reflection symmetry that are mutual mirror images of each other. 
        Intriguingly, not all dodecahedra persist until the edge collapses to lenght zero. 
        The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations below this particular edge length. 
        %
        %\notodo{\mwsays{Discuss the fact that the orange branches meet again: the two branches of the loop have opposite symmetries, and must therefore pass through a common symmetrization to connect to each other}\mwsays{Nah, its fine, I dont need this.}} 
        %
        All of them persist until $\ell^*(-1)=0$. 


        Conversely, expanding an edge only produces two realizations with distinct reflection axes. 
        They are depicted on the left and right of \Cref{fig:edge-contraction-deformation-space}. 
        %
        %\notodo{\mwsays{Surely there is a maximal length!}\mhsays{I mean, yes, there has to be one. However, it could be a highly degenerate limit (everything collapses to a plane), which numerical methods would struggle with. In my experiments, I did not find a maximal length. I removed the sentence}}
        %
        %There is no indication that there exists a maximal edge length beyond which no realizations exist. 
        Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.

        %What remains is a qualitative analysis of the eight deformation paths that emerge from contracting any of the dodecahedron's edges. By considering projections of the eight deformation paths onto random 2-dimensional subspaces and approximating the curves' derivatives, an understanding of the curves' tangents in the regular dodecahedron can be obtained. \Cref{fig:edge-contraction-deformation-space} visualizes these curves' behavior. 

        %\mhsays{Mention how the graphic was formed (see above text)}

        % \begin{figure}[h!]
        %     \centering
        %     %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation.jpg}
        %     %\hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom.jpg}
        %     %\\[4mm]
        %      %\includegraphics[width=0.35\linewidth]{Images/Edge_length_deformation2.jpg}
        %     \hspace*{7mm}
        %     \includegraphics[width=0.38\linewidth]{Images/Edge_length_deformation_zoom2.jpg}
        %     \addtocounter{equation}{1}
        %     \caption{Both figures depict distinct random projections of the eight deformation paths parametrized by the expansion (gray) or contraction (green, red) of a single edge in the regular dodecahedron (blue pentagon). The two types of edge contraction paths (\cf\ \Cref{fig:dodecahedron-configurations-contraction}) have distinct colors. }%The top and bottom row depict two different random projections and the pictures in the right column are zoomed-in versions of the left plot.}
        %     \label{fig:edge-contraction-deformation-space}
        % \end{figure}

         %\todo[inline]{\mwsays{Put little pictures of the deformations at the branches of the graphics.}}

%Two symmetric deformations remain, which also share the same tangent in the regular dodecahedron. 




\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytopes is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore~globally rigid.
%
This leaves open the possibility of generic global rigidity. 

A polytope is called \Def{generically globally rigid} if every generic %\todo{\mwsays{Generic undefined. We mention it already earlier, but never define it I think.} \mhsays{We define it \emph{intuitively} on page 15}}\textit{generic} 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
%Let us consider a small generic perturbation $P'$ of one of the realizations shown in \cref{fig:edge-contraction-deformation-space}.
First, we confirmed numerically that all of the equivalent realizations which are %\notodo{\mwsays{What highlights?}\mhsays{depicted?}}
depicted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. 
Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently close generic realization of the dodecahedron.
Hence, generic realizations are also not necessarily globally rigid.
%
Notably, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}

%\notodo{\mhsays{This is the opposite of global rigidity :D}}

It would be surprising, though also not absurd, that other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{13mm}
    \begin{minipage}[c]{0.32\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edge have the same lengths (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}

\iffalse
\todo{\mwsays{Something bothers me about the discussion below. Lets talk.}}
For bar-joint frameworks, generic global rigidity is often checked by computing the rank of a \Def{stress matrix} for a random equilibrium stress (\cf\ \cite{gortler-healy-thurston}). Since we demonstrate in this article, that many concepts from bar-joint framework rigidity theory carry over to the polytopal setting, it is possible that we can formulate a similar criterion for the generic global rigidity of polytopes. This provides an exciting direction for future research.

\begin{question}
    Can the rank of the stress matrix be used as a criterion for generic global rigidity?
\end{question}
\fi

% Still, that argument does not resolve whether the regular dodecahedron with combinatorial type $\mathcal{D}$ is globally rigid. Nevertheless, we know that there exists a realization of the dodecahedral graph in $\mathbb{R}^2$ that has equal edge lengths (\cf\ \Cref{fig:planar-dodec}). While this realization is not affinely spanning, it clearly has planar facets. If $0$ lies in the relative interior of this polytope, it is impossible to satisfy the equation $\langle p_i, a_\sigma\rangle=1$ for $i\sim \sigma$, as each facet normal must necessarily be normal to the embedded plane $\mathbb{R}^2$, so that $\langle p_i, a_\sigma\rangle=0$. For that reason, we put the plane at height $1$ so that each face has the same normal vector. With this modification, we find that the realization of $\mathcal{D}$ lies in $\real(\mathcal{D})$, implying that the regular dodecahedron is not globally rigid.






%\tempnewpage % temporary new page

%\section{Case study: The truncated dodecahedron}
%\label{sec:truncated_dodecahedron}
%\label{sec:TDod}





\tempnewpage % temporary new page

\section{Conclusion}
\label{sec:outlook}

%\notodo{\mwsays{I am not a fan of a conclusions section that just repeats introduction and main body for the third time. I liked the outlook we had in the last paper because it was just full of questions. If I see correctly, then the only new bit here is the TDod discussion, which might as well go into the results section. This section would be an easy place to shorten the paper.}
%\mhsays{A conclusion/outlook is a formal requirement for any scientific paper. In it, the main arguments/results should be restated and it gives room for open problems and future research. Ideally, one uses the three questions ``what?'', ``so what?'' and ``now what?'' to guide the writing. The conclusion is an important place in the paper to state and summarize our most significant findings and results, why they are useful and what should happen next. We can keep it to 1 page, but it is an essential section.}}


% \todo{\mwsays{Like for title and abstract, I don't think we should reduce this article to second-order theory} \mhsays{Better? }}%

In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 

%\notodo{\mwsays{I see ``a careful development of first- and second-order theory'' as a main result.}\mhsays{First-order theory was in the first paper, right? Added this sentence to Main Results.}\mwsays{First paper only contains claims, no development of the actual first-order theory. Developing first-order theory properly was one of the selling point of this paper here that we declared back then.}\mhsays{This was a question that a reviewer might ask. I have no problem adding this to the Conclusion (which I now did).}}

\subsection{Main results}

We carefully develop a first-order and second-order theory for the rigidity of polytopes in \Cref{sec:first_order,sec:second-order-theory}. %\notodo{\mwsays{Without some background knowledge ``so-rigid implies rigid'' always sounds underwhelming. I wonder whether we should mention somewhere that this is not true for naive higher-order rigidity} \mhsays{Good idea. I'll give it a try.}\mwsays{I reworded a bit. okay?}}
Using these tools, we demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. 
Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 
A well-developed second-order theory is important since it is right at the boundary of what is practically possible: analogous statements are no longer true for naive higher-order rigidity criteria (see \Cref{sec:higher_order_rigidity}). 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves induced by edge length modifications.

\iffalse\textcolor{gray}{
\todo{\mwsays{Saying this makes only sense if it would be in the main body, but it is in the appendix} \mhsays{The conclusion was written when this was not the case.} Feel free to remove.}%
Moreover, we extend our analysis to flexible polytopes. For zonotopes and generic Minkowski sums, we provide a lower bound on the dimension of the flex space. As of now, all flexible convex polytopes that we are able to find arise as zonotopes or generic Minkowski sums. To approximate the flexes of polytopes, we develop an algorithm in \Cref{sec:approx_continuous_motions}, which relies on Riemannian geometry and homotopy continuation, alongside several useful heuristics.}
\fi

Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. 
%\notodo{\mwsays{Sec 9 has changed}\mhsays{Done.}}
In \Cref{sec:so_rigidity_dod}, we explicitly demonstrate a strategy for proving the second-order rigidity of the regular dodecahedron as a test case. Moreover, we investigate deformations induced by modifying the length of a single edge in \Cref{sec:dodecahedron}, which reveals a highly interesting local geometry and also serves as a counterexample for the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}

\iffalse
\begin{remark}
For the truncated dodecahedron, the system of homogeneous quadratic \todo{\mwsays{Reference these equations by number rather than words}}equations introduced in \Cref{section:second-order-rigidity-check} has a non-trivial solution. According to \Cref{res:sotest}, this implies that the truncated dodecahedron is not second-order rigid. In fact, we find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.
\end{remark}
\fi

Among the 31 polytopes we considered, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is 4-dimensional, so it is not first-order rigid.
We also determine that it is not second-order rigid, since the associated system of homogeneous quadratic equations $Q_1=\dots=Q_4=0$ arising from \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. 
In fact, we 
%\notodo{\mwsays{Say that we find this only numerically.}\mhsays{Apparently we know this symbolically! (Y)}}
find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish, whether it is flexible or rigid.

In \Cref{fig:TDod_flex_conc}, we depict samples from a numerically generated deformation of the truncated dodecahedron.
It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances.
%which is \todo{\mwsays{``It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances''}} constructed using gradient descent with reasonable numerical tolerance.
%
%\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}
%
However, when we apply a more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
\label{sec:higher_order_rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
%\todo{\mhsays{Discuss energy interpretation}}
This result would help explain why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which %\notodo{\mwsays{This sounds technically wrong. The deformation has low tolerance?}\mhsays{You're right. I added ``satisfies the constraints with reasonably...''}}
satisfies the edge length and facet planarity constraints with reasonably low numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, they observe that the energy landscape around an $N$-th order rigid realization locally looks like the %\notodo{\mwsays{Is this really called a parabola}\mhsays{After coordinate change it is. I replaced the term. }}
polynomial curve $y=x^{2N}$. This implies that for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

Unfortunately, if the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 

%\mhsays{Develop higher-order rigidity techniques.}

% \notodo{\mwsays{I would say we don't need this section. Move the problems to their sections or mention them in the introduction.} 
% \mhsays{Open problems only belong into the introduction if (a) we solve them or (b) they are guiding problems that motivate our article. Neither is the case. We should move them to the respective sections instead (which I did). }}

%\mhsays{Theoretical results for why some polytopes in special position are inf rigid, even though Cauchy-Dehn does not say this.}

%\mhsays{More constructions for flexible polytopes OR proof that Minkowski flexes are all.}

%\mhsays{Dodecahedron and truncated icosahedron have the same numer of first-order flexes; does this come from the symmetries? Counter point: the truncated dodecahedron only has 4 dimensions of first-order flexes even though it has the same symmetry. Where is the lost dimension? Is there a general way of predicting the first-order flexes from the symmetry group?}

%\mwsays{Is there special structure in the TDod that helps deciding the rigidity question?}

%\mhsays{Point out many interesting questions from \Cref{sec:dodecahedron}}



==> sec/introduction_-_copy_-_2026-06-27.tex <==
%For comments: \mhsrealRays{\texttt{\textbackslash mhsays}}
%\mwsays{\texttt{\textbackslash mwsays}}
%\asays{\texttt{\textbackslash asays}}


\vspace*{-1em}
\section{Introduction}
\label{sec:introduction}

In \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors initiated the study of convex polytopes as point-hyperplane frameworks and asked under what conditions a polytope admits a continuous deformation that preserves both its edge lengths and face coplanarities.
If such deformations exist, the polytope is said to be flexible, otherwise rigid.
Classical results in polyhedral rigidity (such as the rigidity theorems by Cauchy \cite{cauchy1813} or Dehn \cite{dehnstheorem}) enforce the stronger constraint of fixed face shapes, 
%\todo{\mhsays{``and then find'' $\Rightarrow$ ``to then conclude''.}}
and then find that convexity generally implies rigidity.
This is in contrast to our setting, in which flexible convex polytopes do exist.
Still, only
few techniques for
their construction are
known.


\begin{figure}[h!] %[H]
    \centering
\includegraphics[width=0.235\linewidth]{Images/dodecahedron.png}
\hspace{0.75em}
\includegraphics[width=0.235\linewidth]{Images/truncatedIcosahedron.png}
\hspace{0.75em}
\includegraphics[width=0.2425\linewidth]{Images/truncatedDodecahedron.png}
    \caption{The regular dodecahedron (left), the truncated icosahedron (center) and the truncated dodecahedron (right) provide simple examples of polytopes with fascinating rigidity properties.
}
    \label{fig:Dod_TIco_TDod}
\end{figure}
%
As a consequence, the sentiment arose that this sort of flexibility is still rather exceptional, not only among combinatorial types of polytopes, but also among~realizations of a fixed type.
In \cite[Conjecture 1.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors conjecture that~in~dimension at least three, a \textit{generic} convex polytope of a given combinatorial type~is rigid. This claim was shown to hold %true
in dimension three \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}, but remains open for higher dimensions.

Analogous to the classical setting of bar-joint frameworks, deciding rigidity for a given polytope is computationally hard.
Once a polytope is not first-order rigid, the question of rigidity is often out of reach for direct techniques.
This already holds for polytopes with relatively few vertices and faces.
For example, in \cite[Section~6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} the authors singled out the \textit{regular dodecahedron} (\Cref{fig:Dod_TIco_TDod}, left) as a primary example of a relatively small polytope with unclear rigidity status.

In this article, we develop novel tools for the analysis of realization spaces and rigidity properties of polytopes. 
This includes a suitable second-order theory as~well as an effective algorithm for testing second-order rigidity of concrete examples.
For a demonstration, we analyze the rigidity properties of the Platonic, Archimedean and Catalan solids (see \cref{tab:comparison} and \cref{tab:catalan-comparison}). 
In particular, we decide the previously unknown rigidity properties of the \textit{regular dodecahedron} (\cref{fig:Dod_TIco_TDod}, left).
Solely the rigidity of the \emph{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) cannot be determined by~our techniques, but seems to require techniques of even higher order. It will thus~serve as a simple test case for future theoretical and computational developments.
%
We find it remarkable that such varied rigidity behaviors can already be observed in classical examples.

This article is divided into theoretical, methodological, and experimental results,
of which we give an overview below (also refer to the roadmap in \Cref{roadmap}).
\notodo{\mhsays{Added reference to roadmap}}

\subsection{Theoretical results}
\label{sec:intro-theory}


In \cref{sec:combinatorics-of-polytopes} we recall the basics of polytope geometry, combinatorics, and rigidity from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
In \cref{sec:first_order} we present the first-order theory. This includes definitions for the rigidity matrix, first-order motions and~flexes,
%
%\notodo{\mhsays{I don't like the ``/''. Can we write ``first-order motions and flexes'' instead? In continuous text, one should avoid ``/'', as it it bad writing style (according to ChatGPT).}}
%
and equilibrium stresses.
We prove that first-order rigidity implies rigidity.
%
In \cref{sec:second-order-theory} we develop the second-order theory for polytope rigidity.
We provide analogues for the following notions and implications from framework rigidity:
%
$$\text{first-order rigid} \;\xRightarrow{\ref{res:prestress}}\; \text{prestress stable} \;\xRightarrow{\ref{res:prestress}}\; \text{second-order rigid} \;\xRightarrow{\ref{res:second_order}}\;
\text{rigid}.$$
%
We generalize the second-order stress test by Connelly and Whiteley \cite{connelly1996second} to~the~polytope setting (\cf\ \cref{res:sotest}).

\cref{section:edge-length-perturbations} conducts a local study of polyhedral realization spaces motivated by the following train of thought:
the classical Legendre-Steinitz theorem states that the realization space of a 3-dimensional polytope modulo isometries is homeomorphic to $\RR^{E}$, where $E$ is the number of edges \cite{rastanawi2021dimensions}.
This suggests that the shape of a 3-polytope can be controlled by one free and independent parameter per edge.\nls
If the polytope is flexible, however, these parameters cannot map to edge lengths directly, since there are different realizations with the same lengths. 
This suggests that the geometric freedoms somehow distribute between flexes and other deformations that do change edge length. The latter we call \emph{edge length perturbations}, and we explore their relations to the various notions of rigidity. % and first-order rigidity.




\subsection{Methodological results}
\label{sec:intro-methods}
In \cref{section:second-order-rigidity-check}, we provide a concrete method based on real algebraic geometry for certifying second-order rigidity of polytopes. It relies on transforming the condition for second-order rigidity into a polynomial system of homogeneous equations, which can be symbolically solved using Gröbner bases. If this system has no non-trivial solutions, then the polytope is second-order rigid.


\subsection{Computational results}
\label{sec:intro-results}

Our newly developed first- and second-order rigidity certificates apply to any polytope.
For demonstration purposes, we benchmark them on the Platonic, Archimedean and Catalan solids for which combinatorial~data and exact vertex and normal coordinates are readily available.

In \cref{sec:so_rigidity_dod} we give a step-by-step account of how to apply our second-order~rigidity certificate to the regular dodecahedron. We thereby verify that it is indeed rigid (\cf\ \cref{dodecahedronrig}), answering a question posed in \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

Analogous computations are performed for the other test polytopes and are~documented in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
We highlight two results: We show that, besides the dodecahedron, also the \textit{truncated icosahedron} (\cref{fig:Dod_TIco_TDod}, center) is not first- but second-order rigid. We also show that the \textit{truncated dodecahedron} (\cref{fig:Dod_TIco_TDod}, right) is \emph{not} second-order rigid, and thus its rigidity status remains open.
A detailed explanation of the tables and a discussion of the results follow in \cref{sec:experimental_results}.
Further theoretical background on the observed flexes and flex space dimensions is given in \cref{sec:dimension_estimates}.
All code and additional animations of the flexible polytopes are included in the Supplementary Material~\cite{zenodo_suppMaterial}.

Due to its previous status as the guiding example, we dedicate \cref{sec:dodecahedron} to~another case study of the regular dodecahedron.
We investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
We investigate edge length perturbations and deformation paths using tools from Riemannian geometry and homotopy continuation (with more details given in \cref{sec:approx_continuous_motions}).
We also conclude that the dodecahedron is not generically globally rigid.

%\todo{\mhsays{Removed clutter text (first half sentence) from the next paragraph to correct the layout.}}
% \cref{sec:dodecahedron} is dedicated to~another case study of the regular dodecahedron.
% We investigate the local behavior of its realization space with the goal of understanding the (potentially singular) nature of its very special configuration.
% Using tools from Riemannian geometry and homotopy continuation (with details given in \cref{sec:approx_continuous_motions}), we compute edge length perturbations and deformation paths.
% We also conclude that the dodecahedron is not generically globally rigid.

\todo{\mwsays{Sec 5 needs Sec 3. App A needs Sec 8. Why does App B need Sec 5?}}

{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,1.65) {Intro};

\node[fill=white] (app) at (21.5,-1.65) {Appendix};

\node[fill=white] (c10) at (12,-0.7) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,1.65)  {Chapter 4};
\node[fill=white] (c5) at (8.5,-1.65) {Chapter 5};

\node[fill=white] (c6) at (12,1)  {Chapter 6};
\node[fill=white] (c8) at (16,-0.7) {Chapter 8};
\node[fill=white] (c7) at (16,1)  {Chapter 7};
\node[draw=none] (anchor1) at (16,1.65) {};
\node[draw=none] (anchor2) at (16,-1.65) {};

\node[fill=none] (c9) at (20.9,0) {\Cref{sec:so_rigidity_dod} (\cf\ App.\ \ref{appendix:comp-data-dodecahedron})};
% Nodes
\node[
    draw=NiceBlue!40,
    fill=NiceBlue!20,
    rounded corners,
    fit=(c3)(c4)(c5)(c6),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=DarkRed!40,
    fill=DarkRed!20,
    rounded corners,
    fit=(anchor1)(anchor2),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=DarkGreen!40,
    fill=DarkGreen!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (tables) at (21.5,1.65) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,-0.7) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-1.65) {\Cref{sec:dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,1.65)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (8.5,-1.65) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,1)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-0.7) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,1)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.9,0) {\Cref{sec:so_rigidity_dod} (\cf\ App.\ \ref{appendix:comp-data-dodecahedron})};

% Edges
\draw[over] ([yshift=1.5mm]c10) -| (13.855,2.05);
\draw[over2] ([yshift=1.5mm]c8) -| (18.25,1.875);

\draw[myarrow] (13.855,2.05) to[bend left=3] ([yshift=0.2mm,xshift=-12.6mm]tables);

\draw[myarrow] (c3) -- (c10);
\draw[myarrow] (c3) -- (c4);
\draw[myarrow] (c3) -- (c5);
%\draw[->] (c3) -- (c8);

\draw[myarrow] (c4) -- (c6);
\draw[-] (c4) to[bend left=3] (13.855,2.05);
\draw[-] (c6) to[bend left=20] (13.855,2.05);

\draw[myarrow] (c6) -- (c7);

\draw[myarrow] (c5) -| (c8);

\draw[myarrow] (c7) -- (c9);
\draw[myarrow] (c8) |- (app);
\draw[myarrow] (c8) -- (app);

%\draw[->] (c10) to[bend left=20] (intro);
%\draw[->,dashed] (app) -- (c9);
\draw[-, color=white, line width=2mm] (13.9,2.05) -- (14.02,2.05);
\draw[-, color=white, line width=2mm] (18.275,1.875) -- (18.415,1.863);
\draw[myarrow] (c9) -- (tables);
\draw[myarrow] (13.855,2.05) -- (14.01,2.05);
\draw[myarrow] (18.25,1.8625) -- (18.405,1.8625);

\end{tikzpicture}
\vspace*{-2.2em}
\caption{Roadmap for this article's overall structure. Necessary results and logical dependencies are indicated by arrows.}
\label{roadmap}

\vspace*{-1.15em}
\end{figure}
}
\iffalse
{
\hypersetup{hidelinks}
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[
    scale=0.675,
    transform shape,
    every node/.style={
        draw,
        rounded corners,
        minimum width=2.5cm,
        minimum height=0.9cm,
        align=center
    },
    >=stealth
]

\node[fill=white] (intro) at (21.5,2) {Intro};

\node[fill=white] (app) at (21.5,-2) {Appendix};

\node[fill=white] (c10) at (12,-1) {\Cref{sec:dimension_estimates}};


\node[fill=white] (c3) at (6,0) {Chapter 3};

\node[fill=white] (c4) at (8.5,2)  {Chapter 4};
\node[fill=white] (c5) at (8.5,-2) {Chapter 5};

\node[fill=white] (c6) at (12,1.3333)  {Chapter 6};
\node[fill=white] (c8) at (16,-2) {Chapter 8};
\node[fill=white] (c7) at (16,0.6667)  {Chapter 7};
\node[draw=none] (anchor1) at (16,2) {};
\node[draw=none] (anchor2) at (16,-2) {};

\node[fill=none] (c9) at (20.8,0) {\Cref{sec:so_rigidity_dod} (\cf\ App.\ \ref{appendix:comp-data-dodecahedron})};
% Nodes
\node[
    draw=NiceBlue!40,
    fill=NiceBlue!20,
    rounded corners,
    fit=(c3)(c4)(c5)(c6),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Theory (\cf\ \Cref{sec:intro-theory})}
] {};
\node[
    draw=DarkRed!40,
    fill=DarkRed!20,
    rounded corners,
    fit=(anchor1)(anchor2),
    inner sep=0.2cm,
    fill opacity=0.15,
    label=below:{Methods (\cf\ \Cref{sec:intro-methods})}
] {};
\node[
    draw=DarkGreen!40,
    fill=DarkGreen!20,
    rounded corners,
    fit=(app)(intro)(c9),
    inner xsep=0.3cm,
    inner ysep=0.2cm,
    fill opacity=0.15,
    label=below:{Results (\cf\ \Cref{sec:intro-results})}
] {};

\node[fill=white] (tables) at (21.5,2) {\Cref{sec:archimedean}};

\node[fill=white] (c10) at (12,-1) {\Cref{sec:dimension_estimates}};

\node[fill=white] (app) at (21.5,-2) {\Cref{sec:dodecahedron}};

\node[fill=white] (c3) at (6,0) {\Cref{sec:notation}};

\node[fill=white] (c4) at (8.5,2)  {\Cref{sec:first_order}};
\node[fill=white] (c5) at (8.5,-2) {\Cref{section:edge-length-perturbations}};

\node[fill=white] (c6) at (12,1.3333)  {\Cref{sec:second_order}};
\node[fill=white] (c8) at (16,-2) {\Cref{sec:approx_continuous_motions}};
\node[fill=white] (c7) at (16,0.6667)  {\Cref{section:second-order-rigidity-check}};

\node[fill=white] (c9) at (20.8,0) {\Cref{sec:so_rigidity_dod} (\cf\ App.\ \ref{appendix:comp-data-dodecahedron})};

% Edges
\draw[->] (c3) -- (c10);
\draw[->] (c3) -- (c4);
\draw[->] (c3) -- (c5);
%\draw[->] (c3) -- (c8);

\draw[->] (c4) -- (c6);
\draw[->, dashed] (c4) to[bend left=5] ([yshift=2.7mm,xshift=-12.5mm]tables);
\draw[->, dashed] (c6) to[bend left=4] ([yshift=-0.6mm,xshift=-12.5mm]tables);

\draw[->] (c6) -- (c7);

\draw[->] (c5) -- (c8);

\draw[->] (c7) -- (c9);
\draw[->] (c8) -- (app);
\draw[->,dashed] (c10) to[bend right=13] ([yshift=-4mm,xshift=-11.875mm]tables);

%\draw[->] (c10) to[bend left=20] (intro);
%\draw[->,dashed] (app) -- (c9);
\draw[->, dashed] (c9) -- (tables);
\end{tikzpicture}
%\vspace*{-2.2em}
%\caption*{\footnotesize\textbf{Roadmap:} Solid lines indicate requirements and dashed lines indicate utilization.}
\vspace*{-1.65em}
\end{figure}
}
\fi


\tempnewpage

\section{Basic notions}
\label{sec:notation}
\label{sec:combinatorics-of-polytopes}

Throughout %the paper
this article, let $P\subset\RR^d$ denote a $d$-dimensional \textit{convex}
polytope with non-empty interior and \Def{vertices} $p_1,...,p_n$, \ie\ $P$ is the~convex hull $\conv\{p_1,...,p_n\}$.
%
We often focus on polytopes in dimension three, which we call \Def{polyhedra}. 
Below~we recall the relevant facts about polytopes; for a general introduction we refer to \cite{ziegler2012lectures}.

\subsection{Combinatorial types}

The combinatorics of a polytope can be described using its vertex-facet incidence structure: a \Def{combinatorial type}
$\mathcal P=(V,F,\sim)$ is~a triple consisting of an (abstract) \Def{vertex set} $V$, an (abstract) \Def{facet set} $F$ and~a~\Def{vertex-facet incidence relation} ${\sim}\subseteq V\times F$.
To each convex polytope $P\subset\RR^d$ we can assign such a combinatorial type in the obvious way.
Note that the edge graph is encoded within $\mathcal P$ too: we say that vertices $i,j\in V$ are \Def{adjacent} in $\mathcal P$, and denote this by $i\sim j$, if there are facets $\sigma_1,...,\sigma_r\in F$ so that $i$ and $j$ are the only two vertices incident to all of them.\nls
This defines a graph structure on $V$ which we call the \Def{edge graph} $G_{\mathcal P}=(V,E)$.
To emphasize the presence of this graph structure we shall denote a combinatorial type also as the quadruple $\mathcal P = (V,E,F,\sim)$.


\subsection{Polytopal realizations}

The polytopes that share a combinatorial type $\mathcal P$ form the \emph{polytopal realizations} of $\mathcal P$.
For computational convenience, a $d$-dimensional \Def{polytopal realization} of $\mathcal P$ will be given as a pair $(\bs p,\bs a)$ consisting of a \Def{vertex map} $\bs p\: V\to\RR^d$ and a \Def{facet normal map} $\bs a\: F\to\RR^d$, so that for each $\sigma\in F$ the points (or \Def{vertices}) $\{p_i\mid i\sim\sigma\}$ lie on a common affine hyperplane (the \Def{facet hyperplane}) with normal vector $a_\sigma$ (the \Def{facet normal}).
This can be expressed as
%
$$\<p_i,a_\sigma\>=1,\quad\text{whenever $i\sim \sigma$}.$$
We say that a realization is \Def{strictly convex} (or just \Def{convex} for short) if additionally
%
$$\<p_i,a_\sigma\><1,\quad\text{whenever $i\not\sim\sigma$}.$$
%
Each convex polytope $P$ with combinatorial type $\mathcal P$ and $0\in\Int(P)$ gives rise~to~a convex realization in this sense with the facet normals pointing outwards.
We~often identify a polytope with the corresponding realization and use $P$ and $(\bs p,\bs a)$~interchangeably.



All convex realizations of $\mathcal P$ taken together form its \Def{(convex) realization space}

\begin{align*}
\real(\mathcal P)
&:=\left\{\!\!
\begin{array}{l}
    \bs p\:V\to\RR^d
    \\
    \bs a\:F\to\RR^d
\end{array}
\Bigg\vert
    \begin{array}{rcl}
    % \|a_\sigma\| &\!\!\!\!=\!\!\!\!\!& 1 \text{ for all $\sigma\in F$} \\
    \<p_i,a_\sigma\> &\!\!\!\!=\!\!\!\!\!& 1\text{ whenever $i\sim \sigma$}\,\\
    \<p_i,a_\sigma\> &\!\!\!\!<\!\!\!\!\!& 1\text{ whenever $i\not\sim\sigma$}\,
    \end{array}
\!\right\},
\end{align*}
%
With these definitions, $\real(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$\!. %, and $\realCvx(\mathcal P)$ is a semi-algebraic set in $\RR^{dV}\oplus\RR^{dF}$.
%Note that~we may use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.
Note 
%\todo{\mhsays{Moved position of ``also'' so that this sentence fits on two lines.}}
that~we use certain set variables, such as $V$, $E$ and $F$, to also stand in for their~cardinalities.

\begin{remark}\label{res:new_notion}
    The realization spaces defined in \cite[Section 2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} are slightly different from the ones used here.
    Our constraint $\<p_i,a_\sigma\>=1$ for $i\sim \sigma$ prevents facet~hyperplanes from passing through the origin.
    This formulation is more convenient for our purpose.
    The corresponding constraint from \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is $\<p_i-p_j,a_\sigma\> = 0$ for $i,j\sim\sigma$ and does not entail this restriction.
    Both definitions lead to spaces that are birationally equivalent in a neighborhood of each convex realization that has the origin in its interior.
    Since our analysis will be primarily local and since every affinely-spanning convex polytope can be translated so that it contains the origin in its interior, this distinction can be ignored.
\end{remark}

The \Def{Lie group of Euclidean isometries $\Iso$} 
(\ie\ rotations, translations and reflec\-tions) acts on $\real(\mathcal P)$.
Factoring it out yields the \Def{reduced~realization space}:
%
\begin{align*}
\realR(\mathcal P)
    :=\realSp(\mathcal{P})\,/\,\Iso . 
\end{align*}











% \tempnewpage

\subsection{Polytope rigidity}
\label{sec:rigidity}

We examine continuous deformations of $P$ that preserve edge lengths, analogous to bar-joint framework rigidity. Unlike in the framework setting, these motions~must also preserve the polytope's structure, that is, facet planarities and the combinatorial type.
Below we make this precise.



    Two realizations $(\bs p,\bs a),(\tilbs p,\tilbs a)\in\real(\mathcal P)$ are 
%
\begin{align*}
    \text{\Def{equivalent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\| \text{ for each edge $ij\in E$},
    \\
    \text{\Def{congruent} if } \|p_j-p_i\|&=\|\tilde p_j-\tilde p_i\|\text{  for each pair $i,j\in V$}.
\end{align*}
%
A \Def{(continuous) motion} of $(\bs p,\bs a)$ is a continuous map $(\bs p^t,\bs a^t)\:[0,1]\to\real(\mathcal P)$~so that $(\bs p^0,\bs a^0)=(\bs p,\bs a)$ and $(\bs p^t,\bs a^t)$ is equivalent to $(\bs p,\bs a)$ for all $t\in[0,1]$.

We define the \Def{metric realization space}
%
$$\mreal(\mathcal P, P) := \big\{(\bs p, \bs a) \in \real(\mathcal P)\mid \text{$(\bs p,\bs a)$ is equivalent to $P$}\big\},$$
%
which contains all realizations of the polytope $\mathcal{P}$, whose edge lengths are prescribed according to the realization $P$. 
The equivalence of edge lengths can be expressed as $\smash{\|p_i-p_j\|^2=\|\tilde p_i-\tilde p_j\|^2}$, that is, by a system of quadratic polynomial equations. Therefore, $\mreal(\mathcal{P},P)$ also is a semi-algebraic set in $\mathbb{R}^{dV}\oplus \mathbb{R}^{dF}$. %, on which a natural group action of $\Iso$ is induced (\cf\ \cite{Asimow1978TheRO}).
A motion can~also be understood as a continuous curve $\bs p^t\:[0,1]\to\mreal(\mathcal P,P)$.

A motion is \Def{trivial} if $(\bs p^t,\bs a^t)$ is congruent to $(\bs p,\bs a)$ for all $t\in[0,1]$.
If non-trivial, we call it a \Def{flex} of $P$.
If a polytope has a flex, we call it \Def{flexible}, otherwise \Def{rigid}.
As before, the Lie group of Euclidean isometries $\Iso$ acts on $\mreal(\mathcal P, P)$ and can be factored out to obtain the \Def{reduced metric realization space}
%
$$\mreal^*(\mathcal P, P) = \mreal(\mathcal P,P)/\Iso.$$
%
A flex can be understood as a non-constant curve $\bs p^t:[0,1]\to\mreal^*(\mathcal P,P)$.
%
%
For constructions of flexible polytopes, see \cref{sec:flexible_polytopes} or \cite[Section 4]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.

\begin{remark}
Evidently, these definitions apply verbatim to the more general class of point-hyperplane frameworks \cite{EJNSTW}.
%\notodo{\mhsays{Add citation for point-hyperplane frameworks here? I don't think we currently cite any point-hyperplane literature, though we should and here would be a good point for it. }}
Consequently, much of what we say~here applies more generally.
Caution is necessary when we assume certain sub-configurations to be affinely spanning, which is natural in the polytope setting, but does not apply to general point-hyperplane frameworks.    
\end{remark}







\tempnewpage % temporary new page

\section{First-order theory of polytope rigidity}
\label{sec:first_order}

The first-order theory of a geometric constraint system studies the deformations that preserve the constraints up to first order. 
It is a linear theory and hence~provides heuristics and criteria that can be efficiently checked in practice.

Given a polytope $P=(\bs p,\bs a)\subset\RR^d$, its \Def{rigidity matrix} $\mathcal R(P)=\mathcal R(\bs p,\bs a)$ has the following structure:

\begin{figure}[h!]
    \centering \includegraphics[width=0.97\textwidth]{Images/rigidity_matrix.pdf}
\end{figure}

\noindent
All displayed entries are to be interpreted as $1\times d$ sub-matrices. 
The dimensions~of $\mathcal R(P)$ are therefore $(E+\VF)\times(dV+dF)$, where \Def{$\VF$} denotes the set of incident vertex-facet pairs. The rigidity matrix can be interpreted as (a scaled~version~of)~the Jacobian corresponding to the polynomial system of equations that define the metric realization space $\mreal(\mathcal{P},P)$.

The first-order theory of rigidity is essentially the study of the linear algebra~pro\-perties of $\mathcal R(P)$.
All first-order notions can be derived from the rigidity~matrix.

\subsection{First-order rigidity}
\label{sec:first-order-theory}

The elements of the kernel of $\mathcal R(P)$ are called \Def{first-order motions} of $P$. We denote them as pairs $\smash{\dot P=(\bsdot p,\bsdot a)}$ consisting of maps $\bsdot p\:V\to\RR^d$ and $\bsdot a\:F\to\RR^d$ that satisfy the following equations:
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{whenever $ij\in E$},
    \label{eq:flex_at_vertex}
    \\
    \<p_i,\dot a_\sigma\> + \<\dot p_i, a_\sigma\> &= 0 ,\quad\text{whenever $i\sim\sigma$}.
    \label{eq:flex_at_vertex_face}
\end{align}
%
%
Similar to the framework setting, the interpretation is that $\bsdot p$ and $\bsdot a$ are infinitesimal changes in the values of $\bs p$ and $\bs a$. In particular, \eqref{eq:flex_at_vertex} and \eqref{eq:flex_at_vertex_face} can be obtained~by differentiating the equations for edge length and coplanarity constraints.
Note~also that $\bsdot a$ is already determined by $\bsdot p$ via \eqref{eq:flex_at_vertex_face} (for details see the proof of \cref{res:trivial_dim}).


First-order motions are called \Def{trivial} if they satisfy
%
\begin{align}
    \<p_i-p_j,\,\dot p_i-\dot p_j\> &= 0 ,\quad\text{for any $i,j\in V$},
    \label{eq:trivial_motion_vertex}
\end{align}
%
Separate constraints on $\bsdot a$ are not necessary since they are already~determined via \eqref{eq:flex_at_vertex_face}.
%
%
Non-trivial first-order motions are called \Def{first-order flexes}. If a \mbox{first-order flex} exists, the polytope is called \Def{first-order flexible}, otherwise \Def{first-order rigid}.

The trivial first-order motions of $P$ form a linear subspace $\mathcal T_P\subseteq\ker \mathcal R(P)$.\nls
The first-order flexes do not form a linear space, though for matters of dimension counting we can consider the quotient $\ker \mathcal R(P)/\mathcal T_P$. We shall call it the \Def{first-order flex space} of $P$.
This space is trivial if and only if $P$ is first-order rigid.
The dimensions of the first-order flex space for the Platonic, Archimedean and Catalan solids are included in \cref{tab:comparison} and \cref{tab:catalan-comparison}.

\begin{lemma}
    \label{res:trivial_dim}
    $\dim\mathcal T_P=\binom{d+1}{2}$.
    In particular, $\corank \mathcal{R}(P)\geq \binom{d+1}{2}$.
\end{lemma}
%
\begin{proof}
    Constraints \eqref{eq:trivial_motion_vertex} are precisely the constraints of trivial first-order motions for bar-joint frameworks.
    In this setting, trivial first-order motions have the form $\bsdot p = S \bs p + t$ for a \mbox{skew-sym}\-metric matrix $S\in\RR^{d\x d}$ and $t\in\RR^d$, forming a vector space $\mathcal T_P'$ of dimension $\binom{d+1}{2}$ \cite{Asimow1978TheRO}.
    Note that this assumes that $\bs p$ is affinely spanning, which follows from our assumption that $P$ has nonempty interior.
    
    It remains to verify that each $\bsdot p\in\mathcal T_P'$ extends to a polytopal first-order motion of $P$.
    For this, fix $\sigma\in F$ and choose a basis $p_{i_1},...,p_{i_k}$ among the $p_i,i\sim\sigma$.\nls
    This~is possible because the face spans a $(d-1)$-dimensional affine subspace.
    Let~$\dot a_\sigma$~be~the unique solution of the full-rank linear system $\<\dot a_\sigma, p_{i_k}\> = -\<a_\sigma,\dot p_{i_k}\>$~where $k$ ranges over $\{1,...,d\}$. This ensures \eqref{eq:flex_at_vertex_face} for the $p_{i_k}$, and it remains to verify \eqref{eq:flex_at_vertex_face} for a general $p_i,i\sim\sigma$.
    Since the $p_i,i\sim\sigma$ are coplanar, we can write $p_i = \sum_{k}\alpha_k p_{i_k}$ for coefficients $\alpha_k$ that satisfy $\sum_k \alpha_k=1$. Using $\dot p_i = S p_i + t$, we obtain
    %
    \begin{align*}
        \<\dot a_\sigma, p_i\> 
            &= \Big\< \dot a_\sigma, \sum_k \alpha_k p_{i_k}\Big\>
            = \sum_k \alpha_k \< \dot a_\sigma, p_{i_k}\>
            = -\sum_k \alpha_k \< a_\sigma, \dot p_{i_k}\>
            \\&= -\sum_k \alpha_k \< a_\sigma, Sp_{i_k}+t\>
            %= - \Big\< a_\sigma, \sum_k \alpha_k (S p_{i_k}+t)\Big\>
            = - \Big\< a_\sigma, S\sum_k \alpha_k p_{i_k} + t\sum_k \alpha_k\Big\>
            \\&= - \< a_\sigma, Sp_i + t\>
            = - \< a_\sigma, \dot p_i\>.
    \end{align*}
    %
    We conclude $\mathcal T_P\simeq\mathcal T_P'$, and the claim follows.
\end{proof}
%\notodo{\mhsays{Weird equation break :(}\mwsays{Accidentally resolved :)}}

\begin{corollary}
    \label{res:corank_rigid}
    A polytope is first-order
    rigid if and only if $\corank \mathcal R(P) = \binom{d+1}{2}$
\end{corollary}
%
%
\begin{proof}
    Let $\mathcal T_P\subseteq\ker\mathcal R(P)$ be the space of trivial first-order motions of $P$.
    Then
    %
    \[ \text{$P$ is first-order rigid}\; \overset{\text{def}}\Longleftrightarrow\; \ker\mathcal R(P)=\mathcal T_P \;\overset{\ref{res:trivial_dim}}\Longleftrightarrow\; \corank \mathcal R(P)=\textstyle\binom{d+1}{2}.\]
    
    \vspace{-1.6em}
    \qedhere
\end{proof}

%A major reason to care about 
First-order rigidity provides an efficiently computable certificate for rigidity:


\begin{theorem}
    \label{res:first_order}
    If a polytope is first-order rigid, then it is rigid.
\end{theorem}


This is a consequence of the second-order results \cref{res:second_order} and \cref{res:prestress}.
Below we give an independent proof to highlight the similarities between the first- and second-order theory (in particular, compare to the proof of \cref{res:second_order}).

\begin{proof}[Proof of \cref{res:first_order}]
    We prove the contrapositive: we assume that $P$ is flexible, and show that it is first-order flexible.
    For this, consider the algebraic subset $M\subseteq \mreal(\mathcal P,P)$ where we restrict sufficiently many vertices of $P$ to subspaces so as to precisely cancel the trivial motions. 
    If $P$ is flexible, then $P$ is not an isolated point of $M$.
    Hence, using the \emph{curve selection lemma} (see \eg\ \cite[Lemma 18.3]{algebraicapproximationcurves}) we obtain a non-constant analytic path $P^t$ in $M$ that ends at $P$.
    In other words, $P^t$ is a flex of $P$ that has a Taylor series expansion that converges to $P^t$.

    By adding trivial motions to $P^t$ we can cancel some of the lower order terms~of the series expansion.
    Since $P^t$ is non-trivial and analytic, there is a largest~integer $k$ so that we can simultaneously cancel all orders $1,...,k-1$.

    We now consider the $k$-th derivatives of the first-order motion constraints. We write $(\frac{\mathrm d}{\mathrm dt})^m_{t=0}$ for the operator that takes the $m$-th derivative and evaluates at $t=0$.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0}\, \|p_i-p_j\|^2 &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=
        2\Big\<p_i-p_j, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>,
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero by the choice of $k$.
    Analogously, for the vertex-facet incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        = 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!k}_{\!t=0} \<p_i,a_\sigma\>
        &= 
        \sum_{\ell=0}^k\binom{k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}\, p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big\<p_i, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}a_\sigma\Big\>+\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}\,p_i, a_\sigma\Big\>.
    \end{align*}
    %
    Observe that these two identities precisely express that $\dot P := (\tfrac{\mathrm d}{\mathrm dt})^k_{t=0} P$ satisfies the equations of a first-order motion.
    It remains to show that $\smash{\dot P}$ is non-trivial. %, which concludes that $P$ is first-order flexible.
    In fact, if $\dot P$ were trivial, then $\dot P= \tfrac{\mathrm d}{\mathrm dt} Q$ for some trivial motion $Q^t$.
    One can check that then the reparameterization $\hat Q^t:= Q^{t^k/k!}$ is still trivial and cancels the $k$-th order term of $P^t$, in contradiction to the choice of $k$.
\end{proof}

\begin{remark}
    \label{res:first_order_no_reverse}
    The converse of \cref{res:first_order} does not hold in general.
    For example, the regular dodecahedron is first-order flexible (it has a 5-dimensional space of~first-order flexes), but is second-order rigid, and hence rigid (\cf\ \cref{tab:comparison}).    
\end{remark}



\subsection{Equilibrium stresses}

The elements of the cokernel of the  rigidity matrix $\mathcal R(P)$ (\ie\ the kernel of $\mathcal R(P)\T$) are called the \Def{equilibrium stresses} (or just \Def{stresses}) of a system.
Stresses form the second, and equally important, first-order notion of rigidity theory.
We denote a stress by a pair $(\bs\omega,\bs\eta)$ consisting of maps $\bs\omega\:E\to\RR$ and $\bs\eta\:\VF\to\RR$. 
They satisfy the following two \Def{stress equilibrium conditions}:
%
\begin{align}
    \sum_{\mathclap{j:ij\in E}} \omega_{ij}(p_i-p_j) + \sum_{\mathclap{\sigma:i\sim\sigma}} \eta_{i\sigma} a_
    \sigma&= 0,\quad\text{for all $i\in V$}, 
    \label{eq:stress_at_vertex}
    \\
    \sum_{\mathclap{i:i\sim\sigma}} \eta_{i\sigma} p_i &= 0,\quad\text{for all $\sigma\in F$}.
    \label{eq:stress_at_face}
\end{align}
%
We write $\bs\xi=({\bs \omega}, {\bs \eta})$ for sake of brevity and call it a \Def{polytope stress}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/stress_on_face.pdf}
    \caption{Visualization of a polytope stress $(\bs\omega,\bs\eta)$.}
    \label{fig:stress_on_face}
\end{figure}

\begin{remark}
\label{remark:stresses}
    Stresses in frameworks can be given a physical interpretation: each edge of a framework is thought of as a Hookean spring with a spring constant given
    %\todo{\mhsays{``with a spring constant given by'' $\Rightarrow$ ``whose spring constant is given by''}\mwsays{I think my wording is fine.}}
    by the stress $\omega_{ij}$ at $ij\in E$. The spring constant determines the magnitude of the force with which the edge pushes or pulls on its end vertices along the direction of the edge. Whether it pulls or pushes is determined by the sign of $\omega_{ij}$. The stress equilibrium condition (\ie\ \eqref{eq:stress_at_vertex} with second term removed)
    %\notodo{\mhsays{``(the first term of \eqref{eq:stress_at_vertex})'' is not technically correct. Maybe ``by setting $\bs\eta=0$ in \eqref{eq:stress_at_vertex}''?}\mwsays{I don't see a problem with ``first term''. I think your suggestion adds avoidable complexity.} \mhsays{The first term is \textbf{not} the stress equilibrium condition. First term equal to 0 is the equilibrium condition. ``setting the first term of (3.4) to 0'' would be techically correct, but also adds complexity. I think we need to be precise here.} \mwsays{Gotcha. Better?}}
    states that the forces that act on a vertex $i\in V$ cancel each other out.

    The spring constant interpretation persists for the $\bs\omega$-part of the polytope stress $(\bs\omega,\bs\eta)$, but now they do not need to cancel out at the vertices on their own.
    Instead, they need to add up to be equal and opposite to the second term -- the $\bs\eta$-part of the stress.
    This is complicated by the fact that $\bs\eta$ contributes to two equilibrium conditions, \eqref{eq:stress_at_vertex} and \eqref{eq:stress_at_face}, for which we try to provide interpretations below.
     
    First, the right term in \eqref{eq:stress_at_vertex} can be thought of as forces pushing a vertex along the normals of its incident facets (see \cref{fig:stress_on_face}, left).
    One may think of this term as a force resulting from pressure from within the polytope, though this analogy is mostly non-physical: the forces are not proportional to the volumes of the facets and may even have varying signs from facet to facet.

    Second, the stress condition \eqref{eq:stress_at_face} for a facet $\sigma\in F$ can be interpreted as a force equilibrium at the origin: each vertex $i\sim\sigma$ pushes or pulls the origin along their connecting line (\cf\ \cref{fig:stress_on_face}, right).
\end{remark}


Like first-order motions, stresses form a linear space -- the \Def{stress space}.
Stresses are particularly relevant in second-order theory (see \cref{sec:second_order}), but also play a special role in the first-order study of polyhedra (\ie\ 3-dimensional polytopes).


\begin{proposition}
    \label{res:flex_eq_stress}
    If $P \subset\RR^3$ is a polyhedron, then the dimension of its first-order flex space equals the dimension of the space of equilibrium stresses.
    In particular, a polyhedron is first-order rigid if and only if it has no non-zero stress.
\end{proposition}
%

\begin{proof}%[Proof of \cref{res:flex_eq_stress}]

    For each vertex, the number of incident faces equals the number of~incident edges. Thus, the total number of vertex-face incidences in $P$ (denoted by $\VF$)~equals the total number of vertex-edge incidences, which (by the handshaking lemma) is equal to $2E$.
    % In equations, $\VF=2E$.
    Using Euler's polyhedral formula $V-E+F=2$, we find the following relation between the number of rows and columns of the rigidity matrix $\mathcal{R}(P)$:
    %
    \begin{align*}
        (*)\quad\text{\#rows}=\VF+E=2E+E=3E&=3(V+F-2)
        \\&=3V+3F-6=\text{\#columns}-6.
    \end{align*}
%
    The claim now follows from
    %
    \begin{align*}
        \dim(\text{first-order flexes}) \overset{\ref{res:trivial_dim}}= \corank\mathcal R(P) - 6 \overset{(*)}= \corank \mathcal R(P)\T = \dim(\text{stresses}).
    \end{align*}
\end{proof}



The advantage of checking first-order rigidity via stresses is that stresses have~no analogue of the trivial first-order flexes that have to be treated separately.
This~fact is important in Dehn's proof of first-order rigidity for simplicial polytopes \cite{dehnstheorem}, and with \cref{res:flex_eq_stress} we highlight that it holds for non-simplicial polytopes as well.



\section{Second-order theory}
\label{sec:second_order}
\label{sec:second-order-theory}

Second-order rigidity theory investigates deformations that preserve constraints up to second order.
It is mainly employed for the analysis of systems that fail the first-order rigidity test.
%
For that, we follow the work of Connelly and Whiteley \cite{connelly1996second}. 

\subsection{Second-order rigidity}

A tuple $(\dot P,\ddot P) = (\bsdot p,\bsdot a;\bsddot p,\bsddot a)$ of maps $\bsdot p,\bsddot p\:V\to\RR^d$ and $\bsdot a,\bsddot a\:F\to\RR^d$ is called a \Def{second-order motion} of $P$ if $(\bsdot p,\bsdot a)$ forms a first-order motion and additionally the following equations hold:
%
%
\begin{align}
    \label{eq1}
    \<p_i-p_j,\,\ddot{p}_i-\ddot{p}_j\>+\<\dot{p}_i-\dot{p}_j,\,\dot{p}_i-\dot{p}_j\> & =0, \quad\text{whenever $ij\in E$},
    \\
    \label{eq2}
    \<p_i,\ddot{a}_\sigma\>+2\< \dot{p}_i,\dot{a}_\sigma\>+\<\ddot p_i,a_\sigma\> &= 0,\quad\text{whenever $i\sim \sigma$}.
\end{align}
%
We call a second-order motion \Def{trivial} if $(\bsdot p,\bsdot a)$ is trivial as a first-order motion. 
A non-trivial second-order motion is called a \Def{second-order flex}.
If $P$ has some second-order flex, then it is called \Def{second-order flexible}, and \Def{second-order rigid} otherwise.

Second-order rigidity provides a certificate for rigidity:

\begin{theorem}         \label{res:second_order_rigid_impl_rigid}
    \label{res:second_order}
    \label{res:second-order-implies-rigid}
    If a polytope is second-order rigid, then it is rigid. 
\end{theorem}
%
\begin{proof}
    The proof is largely analogous to the proof of \cref{res:first_order}. 
    As before, we prove the contrapositive: we assume that $P$ is flexible and show that it is second-order flexible.
    Through restricting vertices to suitable subspaces and invoking the curve selection lemma \cite[Lemma 18.3]{algebraicapproximationcurves}, we obtain an analytic flex $P^t$.
    There is then a largest integer $k$ so that adding a suitably chosen trivial motion simultaneously cancels all terms of order $1,...,k-1$ in the Taylor expansion of $P^t$.

    This time we consider the $2k$-th derivatives of the first-order motion constraints.
    For the edge length constraint \eqref{eq:flex_at_vertex} at $ij\in E$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \|p_i-p_j\|^2 
        = %\\& = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0}(p_i-p_j), \,\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0}(p_i-p_j)\Big\>
        \\&\overset{\mathclap{(*)}}=\;
        2\Big\<p_i-p_j,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0}(p_i-p_j)\Big>
            + \binom{2k}{k} \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j),\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0}(p_i-p_j)\Big\>
    \end{align*}
    %
    where in $(*)$ we use that most terms are zero.
    Analogously, for the vertex-facet~incidence constraint \eqref{eq:flex_at_vertex_face} at $i\sim \sigma$ we obtain
    %
    \begin{align*}
        0 
        &= 
        \Big(\frac{\mathrm d}{\mathrm dt}\Big)^{\!2k}_{\!t=0} \<p_i,a_\sigma\>
        = 
        \sum_{\ell=0}^{2k}\binom{2k}{\ell} \Big\< \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!\ell}_{\!t=0} \,p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k-\ell}_{\!t=0} a_\sigma\Big\>
        \\&=
        \Big<p_i,\, \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}\!\!a_k\Big\>
            + \Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!2k}_{\!t=0} \,p_i,\, a_k\Big\>
            + \binom{2k}{k}\Big\<\Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} \,p_i,\,
                \Bigl(\frac{\mathrm d}{\mathrm dt}\Bigr)^{\!k}_{\!t=0} a_k\Big\>.
    \end{align*}
    %
    Observe that these two identities express that
    %
    $$\dot P := \Big(\frac{\mathrm d}{\mathrm dt}\Big)^k_{t=0} P
    \quad\text{and}\quad
    \ddot P := 2 \binom{2k}{k}^{-1}\Big(\frac{\mathrm d}{\mathrm dt}\Big)^{2k}_{t=0} P$$ 
    %
    together form a second-order motion of $P$.
    It remains to show that $\dot P$ is non-trivial.
    Analogously to the proof of \cref{res:first_order}, this follows from the choice of $k$.
\end{proof}

The notion of a second-order flex is not easy to apply directly.
In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} are quadratic rather than linear in the unknowns $(\bsdot p,\bsddot p;\bsdot a,\bsddot a)$.
%
%\notodo{\mhsays{Should we expand on this comment slightly? The system is quadratic in the flexes...}\mwsays{Can you write something?}\mhsays{Maybe ``In contrast~to~first-order theory, the defining equations \eqref{eq1} and \eqref{eq2} form a quadratic rather than linear system in terms of a second-order flex $(\dot{P},\ddot{P})$.'' will do?}\mwsays{Ha, I completely missed which sentence you are talking about. Got it now. Is it okay what I did? I prefer to use these variables here.}}
%
Given a candidate first-order flex $(\bsdot p,\bsdot a)$, the system becomes linear in $(\bsddot p,\bsddot a)$ and we can check efficiently if $(\bsdot p,\bsdot a)$ extends to a second-order flex.
This allows us to check second-order rigidity at least for systems whose space of first-order flexes is 1-dimensional.
If the dimension is higher, there is no obvious way to choose the candidate first-order flexes from which to start.

\subsection{The second-order stress test}
\label{sec:stress_test}

In \cite[Section 1.4]{connelly1996second} Connelly and Whiteley developed a second-order rigidity test that reinterprets second-order rigidity as the study of the bilinear pairing between first-order motions and equilibrium stresses. We adapt this technique to our setting.




\begin{theorem}[Stress test] \label{res:sotest}
    A polytope is second-order rigid if and only if for every first-order flex $\dot P$ there is a \Def{blocking} stress, that is, a stress $\bs\xi$ with
    %
    \begin{eqnarray}
    \label{block}
    {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.\end{eqnarray}
\end{theorem}

\begin{proof}
    Fix a first-order flex $\dot P=(\bsdot p,\bsdot a)$. We shall show that it can be extended~to~a second-order flex if and only if there is no blocking stress.

    Recall that, after fixing $\dot P$, the equations \eqref{eq1} and \eqref{eq2} become linear in $\ddot P=(\bsddot p,\bsddot a)$.
    The linear system can be compactly expressed as
    \begin{equation}\label{eq:compact}
        \mathcal R(P) \ddot{P}= -\mathcal R(\dot{P}) \dot{P}.
        % \mathcal R(P)\cdot (\bsddot p,\bsddot a)+\mathcal R(\dot{P})\cdot (\bsdot p,\bsdot a)=0
    \end{equation}
    %
    This system has a solution in $\ddot P$ if and only if $\dot P$ extends to a second-order flex.

    The existence of a blocking stress $\bs\xi$ for $\dot P$ can be expressed by the system
    %
    \begin{equation}\label{eq:blocking_system}
        \mathcal R(P)\T\bs\xi = 0,\qquad {\bs \xi}\T \mathcal  R(\dot P)\dot P\not=0.
    \end{equation}

    It remains to observe that the systems \eqref{eq:compact} and \eqref{eq:blocking_system} are dual in the sense of Farkas' lemma: if we set $A:=\mathcal R(P)$ and $b:=-\mathcal R(\dot P)\dot P$, then either there is~a~$\ddot P$~with $A\ddot P = b$, or there is a $\bs\xi$ with $A\T\bs\xi=0$ and $\bs\xi\T b\not=0$.
    %
    \qedhere

\end{proof}


Following \cite{connelly1996second}, we also introduce the notion of prestress stability: a polytope is \Def{prestress stable} if there is a single stress $\bs\xi$ that blocks every first-order flex $\dot P$. By reversing the quantifiers from the criterion for second-order rigidity in \Cref{res:sotest}, this creates a stronger sufficient condition for rigidity. 
%In \Cref{remark:stresses}, we provide an interpretation of the stresses that gives rise to a nonlinear optimization problem, whose strict equilibria correspond to prestress stable realizations. 
%
%\notodo{\mhsays{Previous sentence is difficult to read and I am not entirely sure whether it is grammatically correct.}\mwsays{I am fine with just deleteing the sentence.} \mhsays{I commented the sentence out.}}

\notodo{\mhsays{Added a pagebreak here so that the entire Corollary appears on the same page. Fortunately, there is a pagebreak before section 6, so the layout does not change overall.}}

%\pagebreak

\begin{corollary}
    \label{res:prestress}
    first-order rigid $\implies$ prestress stable $\implies$ second-order rigid.
\end{corollary}
%
\begin{proof}
    If $P$ is first-order rigid, then there are no first-order flexes, and the condition of prestress stability is trivially satisfied.
    The second implication is clear~from~\cref{res:sotest} and the definition of prestress stability.
\end{proof}



\tempnewpage

\section{Edge Length Perturbations}
\label{section:edge-length-perturbations}

For this section, we restrict ourselves to polyhedra, \ie\ 3-dimensional polytopes, which come with various theoretical advantages over the general case (see \eg\ \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength}). Here, we investigate 
$\real(\mathcal{P})$ locally by considering the space of all realizations that arise from perturbing some of the edge lengths of $P$. We establish topological techniques that provide novel conditions for the rigidity and flexibility of polyhedra, but also provide insights into the geometry of $\mreal(\mathcal{P},P)$ by providing an intuition for how first-order flexes are related to 
curves in $\real({\mathcal{P}})$.

According to the Legendre-Steinitz theorem \cite{rastanawi2021dimensions}, the realization space $\real({\mathcal{P}})$ is a $(E+6)$-dimensional manifold. At every polytopal realization, the trivial first-order motions form a 6-dimensional subspace of the space of first-order motions (\cf\ \Cref{res:trivial_dim}) which is completely determined by the 6-dimensional Lie group of Euclidean isometries $\Iso$.  
This turns $\realR(\mathcal{P})$ into a smooth manifold of dimension
\[\dim\left(\realR(\mathcal{P})\right)=\dim(\real(\mathcal{P}))-\dim(\mathrm{Iso})=(E+6)-6=E.
\]
%
In other words, all polyhedra have $E$ degrees of freedom when pinning a vertex, constraining an edge to a line and a face to a plane (\cf\ \cite{gortler2025higherorderrigidityenergy}). 
This modification factors out the trivial motions from $\real(\mathcal{P})$. 
The fact that $\dim(\real(\mathcal{P}))$ is exactly equal to the number of edges of $\mathcal{P}$ suggests that the degrees of freedom exactly correspond to perturbations of edge lengths. 
Since rigid realizations correspond to isolated points in $\mreal^*(\mathcal{P},P)$, the degrees of freedom in $\realR(\mathcal{P})$ must concentrate on the deformations that change the edge lengths. This line of thought would imply that we can freely perturb the edge lengths locally around rigid realizations (see \Cref{conj:edge_length_perturbations}). We formalize this intuition in the following definition.
    
\begin{definition}
\label{def:edge-length-perturbations}
The
 \Def{edge length vector} of $P$ is given by
 \[{\bs\ell}(P)\,:=\,\left(\,\frac{1}{2}\|p_i-p_j\|^2 ~\bigg\lvert~ij\in E\right).\]
 %
This gives rise to the \Def{edge length map} $\bs\ell:\real(\mathcal{P})\rightarrow \mathbb{R}^E$. We say that a vector ${\bs\ell}'\in \mathbb{R}^{E}$ is \Def{realized} by $P$ if ${\bs\ell}'={\bs\ell}(P)$. The \Def{edge length realization space} $\mathcal{L(P)}$ of $P$ consists of all possible vectors of edge lengths corresponding to convex realizations of $\mathcal P$.
Moreover, $P$ \Def{has all edge length perturbations} if the edge length map $\bs\ell$ is locally surjective in a neighborhood of $P$. %\mwsays{Which space?}
If that is not the case, 
we say that \Def{some of $P$'s edge length perturbations are not realizable}.
\end{definition}

%
Note that \Cref{def:edge-length-perturbations} can analogously be stated for $d$-dimensional polytopes; however, our focus on 3-dimensional polytopes is justified in that most results of this section use the Legendre-Steinitz theorem in an essential way.

Let us first consider an example of the first-order rigid regular tetrahedron. For this polyhedron, all edge length perturbations are realizable.

\begin{example}
    \label{ex:tetrahedron-edge-length-perturbations}
    Consider the regular tetrahedron with realization $P$.
    As a polytope, it is first-order rigid according to Dehn's theorem \cite{dehnstheorem}. The facet planarity constraints are superfluous in this case, as all facets are triangles. As the edge graph of the tetrahedron is the complete graph $K_4$, this polyhedron is first-order rigid, in fact, even minimally first-order rigid in $\mathbb{R}^3$, as a bar-joint framework, meaning that the removal of any edge renders it flexible. Given any sufficiently small perturbation ${\bs\ell}'\in \mathbb{R}^{E}$ of ${\bs\ell}(P)$, we can thus remove the length constraint from any edge to make the tetrahedron flexible, and then deform it until the particular edge length attains the corresponding value in $\bs\ell'$.
    We can iteratively repeat this process until we find a tetrahedral realization $Q$ sufficiently close to $P$ which satisfies ${\bs\ell}'={\bs\ell}(Q)$.
\end{example}

\Cref{def:edge-length-perturbations} can be used to formulate a relationship between a polyhedron's rigidity and the topological properties of its metric realization space $\mreal(\mathcal{P},P)$. With this language, we can show that first-order rigid polyhedra concentrate their degrees of freedom on deformations induced by edge length perturbations.

\begin{proposition}
    \label{prop:inf-rigidity-edge-perturbations}
    A first-order rigid polyhedron $P$ has all edge length perturbations.
\begin{proof}
    Consider the following commutative diagram:
    %
    \[\begin{tikzcd}
    	{\RR^{dV}\oplus\RR^{dF}} && {\RR^E\oplus \RR^{V\!F}} \\
    	\\
    	{\real(\mathcal P)} && {\RR^E}
    	\arrow["f", from=1-1, to=1-3]
    	\arrow["\imath", hook, from=3-1, to=1-1]
    	\arrow["{\boldsymbol{\ell}}", from=3-1, to=3-3]
    	\arrow[hook, from=3-3, to=1-3, "\jmath"]
    \end{tikzcd}\]
    %
    %The arrows in the diagram are as follows.
    The vertical arrows $\imath$ and $\jmath$ are the canonical embeddings.
    The arrow $\bs \ell$ is the edge length map. The arrow $f$ maps an arbitrary pair $(\bs p,\bs a)$ to the vector of lengths $\frac{1}{2}\|p_i-p_j\|^2$ for $ij\in E$ and coplanarity-defects $\<p_i,a_\sigma\>$ for $i\sim \sigma$.

    We observe that the Jacobian of $f$ at the realization $P$ is equal to the rigidity matrix $\mathcal R(P)$, and since $P$ is first-order rigid, \cref{res:corank_rigid} yields that
    \[\rank f = \rank\mathcal R(P)=dV+dF-\corank\mathcal R(P)=dV+dF-6,\]
    where the rank of a map is given by the rank of its Jacobian at the realization $P$.
    The map $\imath$ has rank $E+6$ by the Legendre-Steinitz theorem. 
    From the commutative diagram and basic results about the rank of matrix products, we obtain    
    %
    \begin{align*}
        \rank(\bs\ell)\ge \rank(\jmath\circ \bs\ell) &= \rank(f\circ\imath)
        \\
        &\ge \rank(f) + \rank(\imath) - \dim(\RR^{dV}\oplus\RR^{dF})
        \\
        &= (dV+dF-6) + (E+6) - (dV+dF) 
        \\ &= E.
    \end{align*}
    %
    Since $\bs\ell$ maps into $\RR^E$, it follows that the map has the maximal $\rank(\bs\ell)= E$. Finally, $\bs\ell$ is smooth, so
    we conclude that $\bs \ell$ is a local submersion (\cf\ \cite[Proposition 4.1]{lee-smooth-manifolds}) and hence locally surjective (\cf\ \cite[Proposition 2.2]{lang1999}). 
\end{proof}
\end{proposition}


A major result of \cite{himmelmannschulzewinter2025rigiditypolytopesedgelength} is that almost all realizations of polyhedra are first-order rigid.  
This result requires a suitable definition of \emph{genericity}, which is omitted here for the sake of brevity (see \cite[Definition 5.3.]{himmelmannschulzewinter2025rigiditypolytopesedgelength} for details). Intuitively, we can obtain a generic realization by drawing a random convex realization from $\real(\mathcal{P})$. We can apply the statement on the generic rigidity of polyhedra to \Cref{prop:inf-rigidity-edge-perturbations} in order to obtain a genericity result on the edge length perturbation space. 
\notodo{\mhsays{Also added a pagebreak here. Fortunately, there is a pagebreak before section 6, so the layout does not change overall.}}

%\pagebreak

\begin{corollary}
    Generic polyhedral realizations have all edge length perturbations.
    \begin{proof}
        Take any generic polyhedral realization $P$ of a combinatorial type $\mathcal P$.
        %
        Accor\-ding to \cite[Theorem 1.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength} $P$ is first-order rigid. Hence, \Cref{prop:inf-rigidity-edge-perturbations} is applicable, showing that $P$ has all edge length perturbations.
    \end{proof}
\end{corollary}


In contrast to \Cref{ex:tetrahedron-edge-length-perturbations}, we now consider a flexible polyhedron in the following example. This example highlights that not all realizations of a polyhedron have all edge length perturbations.

\begin{example}
\label{ex:cube-edge-length-perturbations}
    Consider the regular cube, whose vertices are realized by the points in $\{1,-1\}^3$. This is a flexible polyhedron, as it is a zonotope (see \Cref{sec:dimension_estimates}). It is not possible to continuously perturb a single edge without violating the planarity of the facets; the minimum requirement for realizing an edge length perturbation is to simultaneously adjust two 
    antipodal edges. 
\end{example}

We can turn the observation from this example, that not all polyhedra admit all edge length perturbations, into a general statement about the edge length perturbation space. 
However, we need to assert a slightly stronger condition than the local surjectivity of the edge length map $\bs\ell$, which is that we can construct a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \real(\mathcal{P})$ that maps vectors in $\mathbb{R}^E$ sufficiently close to the polyhedron's edge length vector to distinct polyhedra sufficiently close to $P$ of the same combinatorial type such that $\psi(\bs\ell(P))=P$. If that is the case, we say that \Def{all edge length perturbations of $P$ are realizable via a continuous, locally injective map}.

\begin{theorem}
\label{thm:rigidity-and-edge-length-perturbations}
    If all edge length perturbations of $P$ are realizable via a continuous, locally injective map, then $P$ is rigid. 
    \begin{proof}
        Let $\mathcal P$ denote the combinatorial type of the polyhedron $P$. By a previous observation, the reduced realization space $\realR(\mathcal{P})$ of $\mathcal{P}$ is a smooth $E$-dimensional manifold with the local homeomorphism $\varphi:U_P\rightarrow \mathbb{R}^{E}$, which is defined in an open neighborhood $U_P\subset \realR(\mathcal{P})$ of $P$. 

        Assume now that all of $P$'s edge length perturbations are realizable via 
        the continuous map $\psi:\mathbb{R}^{E}\rightarrow \realR(\mathcal{P})$. This map takes a list of edge lengths and produces a realization of $\mathcal{P}$ with $\psi(\bs\ell(P))=P$ and it is injective in a sufficiently small open neighborhood $U_{{\bs\ell}(P)}\subset\mathbb{R}^{E}$ of ${\bs\ell}(P)$. After sufficiently shrinking $U_{\bs\ell(P)}$, we can assume that $\psi: U_{\bs\ell(P)}\rightarrow U_P$ is continuous and injective.
        
	\begin{figure}[h!]
		\centering
		\begin{tikzpicture}[node distance=3.5cm, auto]
			
			% --- Nodes ---
			\node (R1) { $\mathbb{R}^{E}$};
            \node (UR) [right=-0.1cm of R1] { $\supset U_{{\bs\ell}(P)}$};
			\node (L) [below=-0.075cm of UR] { \rotatebox[origin=c]{90}{$\in$}};
			\node (L2) [below=-0.075cm of L] { 
			\small${\bs\ell}(P)$};
			\node (CP) [right=of R1] {~\small$U_P$~};
            \node (L3) [below=-0.075cm of CP] { \rotatebox[origin=c]{90}{$\supset$}};
			\node (L4) [below=-0.075cm of L3] { 
			\small$\realR(\mathcal{P})$};
			\node (R2) [right=of CP] {$\mathbb{R}^{E}$};
			
			% --- Straight arrows ---
			\draw[->, thick] (UR) to node[above]{ $\psi$} (CP);
			\draw[->, thick] (CP) to node[above]{ $\varphi$} node[below]{\small $\mathrm{Legendre}$-$\mathrm{Steinitz}$} (R2);
			
			% --- Long curved arrow from first to last with label ---
			\draw[->, thick, bend left=20] ([xshift=0.1cm,yshift=0.035cm]UR.north) to node[above=0.1cm] {\small $\mathrm{Invariance}$ $\mathrm{of}$ $\mathrm{Domain}$} ([xshift=-0.1cm,yshift=0.035cm]R2.north);
			
		\end{tikzpicture}
        \caption{A diagram for the topological argument used in this proof}
        \label{fig:proofhelper-invariance-of-domain}
	\end{figure}
    
        We visualize the following topological arguments in \Cref{fig:proofhelper-invariance-of-domain}. By the Invariance of Domain Theorem \cite{invariance-of-domain}, the continuous injection $\varphi\circ \psi: U_{{\bs\ell}(P)}\rightarrow V\subset \mathbb{R}^{E}$ for \mbox{$V=\varphi\circ \psi (U_{{\bs\ell}(P)})$} is a homeomorphism on its domain and $V$ is open. This lets us pull back the open set $V$ to the open set $\varphi^{-1}(V)$ in $\realR(\mathcal{P})$, since $\varphi$ is a local homeomorphism. %Consequently,
        Hence, $\psi:U_{{\bs\ell}(P)}\rightarrow \varphi^{-1}(V)$ is a homeomorphism, since $\psi$ can be expressed as $\varphi^{-1}\circ(\varphi\circ \psi)$ and since $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.
        %\todo{\mhsays{Double ``and'' is weird. Rewrite this sentence. Suggestion: ``...is a homeomorphism, since $\psi$ can be expressed as $\varphi^{-1}\circ(\varphi\circ \psi)$ and since $\varphi^{-1}$ and $\varphi\circ \psi$ are both homeomorphisms.''}\mwsays{Don't get the sentence at all. Probably due to a missing closing parenthesis.} \mhsays{Added closing parenthesis. I intend to say ``$\psi$ is a homeomorphism because $\psi$ can be expressed as $\varphi^{-1}\circ (\varphi \circ \psi)$ and we know that $\varphi^{-1}$ is a homeomorphism, as well as $\varphi \circ \psi$.'' Does the sentence I suggest above convey this? If so, feel free to replace the sentence and delete this comment.}\mwsays{Replaced it, but I am almost sure you don't like the linebreak.} \mhsays{Replaces ``As a consequence, ...'' by ``Hence, ...''. Does this work for you? If so, you can delete this comment.}}
        
        Consequently, there exists an open neighborhood around $P$ in the manifold $\realR(\mathcal{P})$, in which all realizations come from edge length perturbations. In other words, there is no curve in $\realR(\mathcal{P})$ through the realization $P$ which preserves the edge lengths ${\bs\ell}(P)$, so $P$ is rigid. 
    \end{proof}
\end{theorem}
%
The assumption that $\psi$ is continuous is equivalent to the local continuity of $\psi$ in the neighborhood $U_{\bs\ell(P)}$: We can find a sufficiently small ball around $\bs\ell(P)$ inside the open set $U_{\bs\ell(P)}$, which lets us continuously extend $\psi$ to all of $\mathbb{R}^E$ since an open ball is homeomorphic to $\mathbb{R}^E$. Moreover, we show in the proof of \Cref{thm:rigidity-and-edge-length-perturbations} that $\psi$ must be a local homeomorphism under these assumptions. 
%This restricts the family of admissible polyhedra.
%\todo{\mhsays{Last sentence is weird. Maybe rewrite? I don't have an idea though.} \mhsays{We can also keep the sentence the way if is if you don't mind. You decide. Just remove the comment after you decided.}\mwsays{Removed it}}

Since \Cref{thm:rigidity-and-edge-length-perturbations} provides a sufficient condition for the rigidity of polyhedra, its contrapositive yields information about the reduced realization space $\realR(\mathcal{P})$. This observation is sufficiently useful to state explicitly as a corollary. Albeit, it is currently unclear whether checking the theorem's preconditions offers any advantage over directly verifying a polyhedron's rigidity or flexibility.

\begin{corollary}
    If a polyhedron $P$ of combinatorial type $\mathcal{P}$ is flexible, then there exists no continuous map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ that is locally injective around $\bs\ell(P)$ with $\psi(\bs\ell(P))=P$.
\end{corollary}
%
Note that the local surjectivity of $\bs\ell$ is a strictly weaker condition than the existence of a locally continuous map $\psi$ that is asserted in \Cref{thm:rigidity-and-edge-length-perturbations}. 
To explain that the condition is strictly weaker, let us consider a counterexample. 
\begin{remark}
\label{res:square_root_branching}
Consider $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ with $(x,y)\mapsto (x^2-y^2,\,2xy)$. This mimics the holomorphic function $\mathbb{C}\rightarrow \mathbb{C}$ that maps $z\mapsto z^2$ with values over $\mathbb{R}$. The map $f$ is continuous and, since over $\mathbb{C}$ square roots do exist, it is also locally surjective at the point $(0,0)$. 
However, the square root function is set-valued, so there exists no (locally) continuous square root function over $\mathbb{C}$ due to the branching at $(0,0)$.
\end{remark}

However, it may still be possible that the local surjectivity of $\bs\ell$ is sufficient for the statement of \Cref{thm:rigidity-and-edge-length-perturbations}. With the example of the square root in mind, we may need to show that the fiber size of $\bs\ell$ is constant outside of the realization $P$. 

The correspondence between the edge length realization space of a polyhedron and its rigidity properties is fascinating. Even though \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations} almost paint a complete picture of this correspondence, we were unable to resolve the case where the polyhedron is rigid, but not first-order rigid. In our experiments (\cf\ \Cref{section:dodec-edge-length-perturbations}), we find that this case seems to have particularly interesting algebraic and topological properties. For that reason, we formulate the following two questions, which we hope will inspire future research in this topic. 

\begin{question}
\label{conj:edge_length_perturbations_implies_rigid}
\label{conj:edge_length_perturbations}
    If all edge length perturbations of a convex polyhedron $P$ are realizable, is $P$ then necessarily rigid? Conversely, does every rigid realization~of a polyhedron have all edge length perturbations?
\end{question}







%\pagebreak

\tempnewpage

\section{Certifying Second-order rigidity}
\label{section:second-order-rigidity-check}
\label{sec:so_certificate}

As laid out in \Cref{sec:second-order-theory}, any first-order flex of a polytope 
that has the chance to extend to a continuous motion must necessarily not be blocked by an equilibrium stress. 
That is, according to \Cref{res:sotest}, there exists a first-order flex $\dot P$ so that for all equilibrium stresses $\bs \xi$ we have $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}=0$.
Conversely, if for each $\dot{P}$ there exists a $\bs \xi$ such that $\bs \xi\T
\mathcal{R}(\dot{P}) \dot{P}\neq 0$, then the polytope is 
%\notodo{\mwsays{In fact, PSS. Is this the proper converse that you want to state here?} \mhsays{Good catch, thanks.}}
second-order rigid, which guarantees that it is rigid (\cf\ \Cref{res:second_order_rigid_impl_rigid} and \ref{res:sotest}). This criterion can be checked by parameterizing the first-order flex space via a basis
%\notodo{\mhsays{We say before that the first-order flex space is not a linear space and now it is. Maybe we should explain this detail slightly more?}\mwsays{No no, we say that the first order flexes do not form a linear space, but then we define a stand-in that we call first-order flex space, and we already discuss exactly this point!}}
${\dot{P}}=({\dot{P}}_1,\dots,{\dot{P}}_r)$ with variables $\lambda=(\lambda_1,\dots, \lambda_r)$ and the equilibrium stress space via a basis $\bs\xi=({\bs \xi}_1,\dots,{\bs \xi}_s)$ with variables $\mu=(\mu_1, \dots, \mu_s)$. 
This turns the second-order condition \eqref{block} into the cubic polynomial% of the form 

\[E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\left(\sum_{j=1}^s \mu_j{\bs \xi}_j\right) \cdot \mathcal{R}\left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right)\cdot \left(\sum_{i=1}^r \lambda_i{\dot{P}}_i\right).\]

More precisely, the homogeneous polynomial $E_{\dot{P},\,\bs\xi}$ is linear in the variables $\mu$ and quadratic in the variables $\lambda$. For asserting second-order rigidity, it suffices to show that every first-order flex has a blocking stress according to \Cref{res:sotest}. In other words, second-order rigidity can be checked by finding a $\mu$ for each $\lambda$ 
so that $E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\neq 0$.
%
%
By expanding $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)$ in terms of $\mu_j$, we obtain 
%
\begin{eqnarray}
\label{eqn:stress_polynomial_Qi}
E_{{\dot{P}},\,\bs \xi}(\lambda,\mu)\,=\,\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)
\end{eqnarray}
%
for quadratic forms $Q_j\in \mathbb{R}_2[\lambda_1,\dots,\lambda_r]$.

The crucial observation is the following: If any of the $Q_j$ is non-zero for a given $\lambda$, then we can find $\mu$ such that $\sum_{j=1}^s\mu_j\cdot {\bs\xi}_j$ blocks $\sum_{i=1}^r\lambda_i\cdot{\dot{P}}_i$. 
Therefore, the first-order flexes that are not blocked by any stresses can be parametrized by the solutions of the %\mhsays{square}
polynomial system $Q_1=\dots= Q_s=0$, which form an algebraic set. %\todo{\mwsays{Is this clear?}}
This system can also be represented by the gradient of $E_{\dot{P},{\bs\xi}}$ with respect to $\mu$ to obtain $\nabla_\mu E_{\dot{P},{\bs\xi}}(\lambda)=0$.

We will later see that the zero-dimensionality of the algebraic set $\mathcal{V}(Q_1,\dots,Q_s)$ is sufficient for second-order rigidity. As a criterion for that, we formulate the following. It is a standard result in computational algebraic geometry and can be found in textbooks such as \cite[Theorem 5.3.6]{cox-little-oshea}. 
    \begin{lemma}\label{gbasis}
        Fix a field 
        $\Bbbk$ and let $\mathcal{I}=\langle f_1,...,f_s\rangle$ be an ideal in $\Bbbk[x_1,..,x_r]$. Let $\mathcal{G}$ be a Gröbner basis of $\mathcal{I}$. Then, $\mathcal{I}$ is zero dimensional if and only if for every $i\in\{1,...,r\}$ some power of $x_i$ is the leading monomial of an element of $\mathcal{G}$.
    \end{lemma}

Of course, there are also other methods based on Gröbner bases to verify that an ideal is zero-dimensional; however, for our purposes, \Cref{gbasis} proves to be sufficient. If the ideal $\mathcal{I}=\langle Q_1,\dots,Q_s \rangle$ is zero-dimensional, then the algebraic set $\mathcal{V}(\mathcal{I})$ contains only finitely many points \cite[Proposition 1.7]{hartshorne}. Since the quadratic forms $Q_i$ are homogeneous, it holds that \[\left(Q_1(c\cdot \lambda^*),\,\dots,\,Q_s(c\cdot \lambda^*)\right)=\left(c^2\cdot Q_1(\lambda^*),\,\dots,\,c^2\cdot Q_s(\lambda^*)\right)= 0\] 
for any $c\in \mathbb{C}$ and any $\lambda^*\in \mathcal{V}(\mathcal{I})$. In other words, all scalar multiples $c\cdot\lambda^*$ must also lie in $\mathcal{V}(\mathcal{I})$. The zero-dimensionality of $\mathcal{V}(\mathcal{I})$ is therefore equivalent to $\mathcal{V}(\mathcal{I})=\{0\}$.
In our context, this translates to the non-existence of non-blocked flexes. We summarize our observations in the following:
\begin{proposition}
\label{prop:stress-energy-condition}
    If the homogeneous polynomial system 
    $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda) = 0$ defined in \eqref{eqn:stress_polynomial_Qi} only has $\lambda_1=\dots=\lambda_r = 0$ as a real solution, then all first-order flexes are blocked by equilibrium stresses. Conversely, any flex that is not blocked by an equilibrium stress corresponds to a non-trivial, real zero of $\nabla_\mu E_{\dot{P}, \bs \xi} (\lambda)=0$.
\end{proposition}

The approach based on Gröbner bases described in this section is sufficient to decide the second-order rigidity of all polytopes tested in \cref{sec:experimental_results} (\cf\ \Cref{tab:comparison} and \cref{tab:catalan-comparison}). 
%\notodo{\mhsays{``Table 1 and Table 2'' for consistency.}}
Still, 
our result using Gröbner bases is clearly not necessary for second-order rigidity, as we only determine the emptiness of $\mathcal{V}(\mathcal{I})$ over $\mathbb{C}$. Therefore, it is possible that $\mathcal{V}(\mathcal{I})=\{0\}$ over the real numbers, even when we find non-trivial solutions over $\mathbb{C}$. A simple counterexample is given by the equation $x^2+y^2=0$, which only has $x=y=0$ as a real solution, but has the line $x=iy$ as a complex solution. A weaker certificate is given by the \Def{Euclidean distance degree problem} \cite{euclideandistancedegree} for a generic point $p\in \mathbb{R}^r$, which guarantees finitely many solutions on all connected components of $\mathcal{V}_\mathbb{R}(\mathcal{I})$ (\cf\ \cite{deformationpaths}). By appending the equation $\sum_{i=1}^r\lambda_i^2-1$ to the ideal $\mathcal{I}$ which describes the unit hypersphere, we guarantee that this approach only finds non-trivial solutions. We also do not lose any solutions beyond the origin due to the invariance of solutions under scalar multiplication.

Analogous to second-order rigidity, we can decide prestress stability (\cf\ \Cref{res:prestress}). For that, we need to decide if there exists a $\mu\in \mathbb{R}^s$ defining a 
stress ${\bs\xi}=\sum_{j=1}^s \mu_j\cdot {\bs\xi}_j$ such that $E_{\dot{P},\,{\bs\xi}}(\lambda,\mu)\not= 0$ for all $\lambda$. This is a standard semidefinite programming (SDP) problem: we need to show that $\sum_{j=1}^s \mu_j \cdot Q_j(\lambda)$ is positive definite for some choice of $\mu$. As this is a homogeneous quadratic form, we can alternatively check whether the matrix
%
$$\sum_{j=1}^s \mu_j \cdot \left(\frac{\partial^2}{\partial \lambda_k\lambda_\ell}Q_j(\lambda)\right)_{k,\ell=1}^r$$
%
is positive definite for some choice of $\mu$. 
%\todo{\mhsays{We say ``for some choice of $\mu$'' twice in this paragraph. Maybe we can use synonyms for one to make the reading more varied?}\mwsays{Personally I am not bothered, but I also don't mind changing this.}}






\tempnewpage

\section{Second-order rigidity of the regular dodecahedron}
\label{sec:so_rigidity_dod}

Among the Platonic solids, there is only one for which the question of rigidity is not answered immediately.
The regular tetrahedron, octahedron and icosahedron are simplicial, hence rigid by Dehn's theorem \cite{dehnstheorem}. 
The cube is the classical example of~a~flexible polytope.
Solely the regular dodecahedron remains to be understood and initially eluded direct computation.

Symbolic computations reveal a 5-dimensional space of first-order flexes and a~5-dimensional space of stresses.\footnote{The specific embedding and orderings of vertices, edges and faces are provided in \cref{appendix:comp-data-dodecahedron}.}
%
Note that these dimensions must be identical~due~to \cref{res:flex_eq_stress}.
%
It is tempting to somehow relate the dimensions of the flex and stress spaces to the 5-fold symmetries of the dodecahedron.
We have no evidence~for such a relation, and instead found rather mild counter-evidence in the case of the truncated~dode\-cahedron (see \cref{sec:selected_rigidity}).


Since the regular dodecahedron is not first-order rigid, it is a promising test case for the second-order certificate from \cref{sec:so_certificate}.
Concretely, \cref{prop:stress-energy-condition} asserts that it suffices to compute the zeros of a certain polynomial system. 
We~proceed~as follows:
%
\begin{enumerate}
    \setlength{\itemsep}{0.7ex}
    \item 
    Symbolically compute a basis of the space of first-order flexes $(\dot{P}_1,\dots,\dot{P}_5)$ and a basis of the space of equilibrium stresses $(\bs \xi_1,\dots, \bs\xi_5)$. 
    Using the~bases, we parametrize the spaces by variables $\lambda_1,\dots,\lambda_5$ and $\mu_1,\dots,\mu_5$.
    
    \item From the stress energy $E_{\dot{P},\bs\xi}(\lambda, \mu)$, we extract the polynomial system $$\nabla_\mu E_{\dot{P},\bs\xi}(\lambda)=(Q_1(\lambda),\,\dots,\, Q_5(\lambda))=0$$ consisting of quadratic forms $Q_i$. % (see \cref{section:second-order-rigidity-check}).
    
    \item Use the equivalence in \cref{gbasis} to determine whether the system~has~fi\-nitely many (real) zeros.
    This is the case for the regular dodecahedron.
    
    \item Use \Cref{prop:stress-energy-condition} to infer second-order rigidity.
\end{enumerate}

    The Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\,Q_5\rangle$ in the lexicographic ordering consists of 31 polynomials and is provided in the Supplementary Material \cite{zenodo_suppMaterial}.
    For more specifics on the relevant \textsc{Mathematica} files, see \cref{appendix:comp-data-dodecahedron}.
    With the help of this Gröbner basis, we obtain the following results:

    \begin{theorem}\label{dodecahedronrig}
        The regular dodecahedron is rigid. 
    \end{theorem}
    \begin{proof}
        The monomials $\lambda_1^2$, $\lambda_2^3$, $\lambda_3^3$, $\lambda_4^5$,  $\lambda_5^6$, appear as leading monomials in the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$.
        \Cref{gbasis} therefore implies that $\mathcal{I}$ is zero-dimensional. 
        %By \cref{gbasis}, the Gröbner basis $\mathcal{G}$ for the ideal $\mathcal{I}=\langle Q_1,\,\dots,\, Q_5\rangle$ only has finitely many common zeros, as it contains some power of $\lambda_i$ as a leading monomial for $i\in\{1,...,5\}$ (see \Cref{appendix:comp-data-dodecahedron}). 
        Since $\mathcal{I}$ is a homogeneous ideal, the only solution is $\lambda_1=\lambda_2=\cdots=\lambda_5=0$. 
        By \cref{prop:stress-energy-condition}, for any non-zero linear combination of the five first-order flexes, we can find a stress so that inequality \eqref{block} holds. 
        By \Cref{res:sotest}, $P$ is second-order rigid. 
        By \cref{res:second-order-implies-rigid}, $P$ then is rigid. 
    \end{proof}

Having understood the rigidity properties of the Platonic solids, a natural move is to extend the search to the next best well-documented classes of polytopes -- the Archimedean and Catalan solids.
A detailed account of the findings is given~in~\cref{sec:archimedean} (see also \cref{tab:comparison} and \cref{tab:catalan-comparison}).

Among the 31 polytopes checked, only three are not first-order rigid, but also not predictably flexible (\cf\ \cref{sec:dimension_estimates}): the regular dodecahedron, the truncated icosahedron and the truncated dodecahedron (\cf\ \cref{fig:Dod_TIco_TDod}).
The procedure above was applied to all of them, and our findings are documented in \cref{sec:selected_results}.
%\todo{\mhsays{Should we also refer to Appendix C for the truncIco and truncDod?}}








\tempnewpage

\section{Computational results: Platonic, Archimedean and Catalan solids}
\label{sec:experimental_results}
\label{sec:archimedean}


We apply our techniques to the Platonic, Archimedean, and Catalan~solids.\nls
For these classes, combinatorial data and algebraic vertex and normal coordinates are readily available.%
%
%\notodo{\mhsays{Also, I don't think the footnote is correct. The coordinates, orderings of vertices, edges and facets are provided via the \textsc{Mathematica} database. The computations are provided in the Supplementary Material.}\mwsays{We should still write that they are taken from the mathematica database.}\mhsays{Absolutely, but we should precisely distinguish what we do and what \textsc{Mathematica} does. I would suggest changing the footnote to ``The coordinates, orderings of vertices, edges and facets are extracted from the \textsc{Mathematica} polyhedral database. The computations are provided in the Supplementary Material \cite{zenodo_suppMaterial}.''.}}%
%
\footnote{The coordinates, orderings of vertices, edges and facets are taken from the \textsc{Mathematica} polyhedral database. The computations are provided in the Supplementary Material \cite{zenodo_suppMaterial}.}
%
The results are shown in \cref{tab:comparison} (for the Platonic and Archime\-dean solids) and \cref{tab:catalan-comparison} (for the Catalan solids).
%
An explanation of the content of the tables is given in \cref{sec:explain_table}.
%
%
A key takeaway is that even simple examples can show a wide range of rigidity behaviors.


We were able to decide the rigidity of the tested polytopes in all but one case. 
In particular, we determined the previously unknown rigidity properties of the \textit{regular dodecahedron}.
Solely the rigidity of the \emph{truncated dodecahedron} cannot be decided by our techniques (marked with \Ques\ in \cref{tab:comparison}). 
Solving this question appears to~re\-quire techniques of even higher order and can thus serve as a simple test case for future theoretical and computational developments.
See \cref{sec:selected_results,sec:rigidity_comments,sec:selected_flexibility}~for a discussion of the results.
%\notodo{\mhsays{``See Section``s'' ...''}}


\subsection{Explanation of table contents}
\label{sec:explain_table}

Each table cell contains the name and~a~visualization of the polytope in question.
The parentheses contain the following data from left to right:

\begin{enumerate}
\setlength{\itemsep}{1ex}

    \item Whether the polytope is \textit{first-order rigid} (\yes) or \textit{first-order flexible} (\no). This is computed \textit{symbolically} based on the description in \cref{sec:first_order}.
    
    
    \item Whether the polytope is \textit{prestress stable} (\yes) or \textit{not} (\no). If not implied~by other symbolic first- or second-order computations, this is computed \textit{numerically} based on the description in \cref{sec:second_order} and using our novel techniques developed in \cref{section:second-order-rigidity-check}, in this case reducing to a semidefinite program.\nls
    We use \yesBut\kern-1pt/\kern1pt\noBut\ to indicate numerical results.
    A dual symbolic approach is described in \cite[Lemma 6.3.2]{Lovasz2003SDP}, but we do not currently have a way to produce such a certificate for our setting.
    
    \item Whether the polytope is \textit{second-order rigid} (\yes) or \textit{second-order flexible}~(\no). This is computed \textit{symbolically} based on the description in \cref{sec:second_order} and using our new techniques developed in \cref{section:second-order-rigidity-check}.
    
    \item Whether the polytope is \textit{rigid} (\yes) or \textit{flexible}~(\no). This is inferred from the previous symbolic computations, from the polytope's combinatorial data (see \Cref{sec:dimension_estimates}) or indicated as unknown (\Ques).
    
    \item The \textit{dimension of the first-order flex space} as introduced in \cref{sec:first_order}, which we compute \emph{symbolically}.
    In some cases we have a good theoretical understanding of how the dimension of the flex space comes about. 
    In other cases we can derive theoretical lower bounds on the dimension.
    %
    %\notodo{\mhsays{This sounds like for some polytopes, we only have a lower bound on the dimension which is displayed in the table. Instead, we have the exact values, but can explain a lower bound for them using theoretical arguments.}\mwsays{I can't see this interpretation of the sentence.} \mhsays{We never say that we actually compute the dimension of the flex space right? I guess to me, it sounds as though we don't actually compute the dimension, but \textit{only} have the theoretical lower bounds, which are \textit{insufficient} in some cases. I think for me an easy fix would be the change `` we have a good understanding of how'' $\Rightarrow$ `` we have a good theoretical understanding of how''}\mwsays{Also added ``symbolically''.}}
    %
    If further explanations are available, this is indicated~by a symbol \SymOne, \SymTwo, \SymThree\ (see below), and further theoretical background is provided in \cref{sec:dimension_estimates}.
\end{enumerate}

The following symbols in the table indicate further explanations regarding their rigidity properties and flex space dimensions:
%
\begin{itemize}
\setlength{\itemsep}{1ex}

    \item[\SymTwo] This is a \textit{simplicial polytope} (\ie\ all faces are triangles). 
    Hence the polytope is first-order rigid by Dehn's rigidity theorem, as well as globally rigid by Cauchy's rigidity theorem (for details on the classical rigidity theorems see \cite[Remark 1.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength} or \cite[Chapter 26+]{pak2010lectures}).
    
    \item[\SymThree] This polytope is a \emph{generic Minkowski sum}, and hence flexible according~to \cite[Section 4.1]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
    The dimension of the first-order flex space decomposes~according to~the two types of flexes that exist for such polytopes~(summand flexes and reorientation flexes; see \cref{sec:generic_Msum} for details).
    
    \item[\SymOne] This is a \textit{zonotope}, and therefore flexible according to \cite[Section 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. See \cref{sec:zonotopes} for an explanation of the observed flex space dimensions.\nls If the zonotope is generic (marked by \SymOne\ \SymThree), the dimension of the first-order flex space can be computed exactly (\cf\ \cref{res:generic_zonotopes}).
\end{itemize}
%
%Remarkably, the theoretically obtained lower bounds are always matched exactly by the computationally obtained results.
%The consequence is that we have an exact understanding of the flexes that exist locally at the shown realizations.\nls
%Again,\nls details are given in \cref{sec:dimension_estimates}.






\pagebreak
\vspace*{6mm}
\input{sec/table1}
\newpage





% \pagebreak

\subsection{Selected results}
\label{sec:selected_results}
\label{sec:selected_rigidity}

We highlight the following findings from \cref{tab:comparison} (the corresponding table cells are marked with \Star):

\begin{itemize}
\setlength{\itemsep}{0.7ex}
    \item The \Def{regular dodecahedron} and the \Def{truncated icosahedron} have identical~rigidity properties: they are neither first-order rigid (both have a 5-dimensional space of first-order flexes) nor prestress stable; yet, \emph{both are second-\mbox{order} rigid}. 
    In particular, they are rigid. 
    This was previously stated as an open question for the regular dodecahedron in
    \cite[Section 6.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}. 
    With these rigidity properties, both polytopes are remarkably natural geometric constraint systems which demonstrate that prestress stability and second-order rigidity are distinct concepts.
    Previous examples of this distinction were compa\-ratively ad hoc (\eg\ \cite[Figures 9b and 17a]{connelly1996second}).
    
    \item The \Def{truncated dodecahedron} is not first-order rigid (it~has~a 4-dimensional space of first-order flexes), not prestress stable and \emph{not~second-order rigid}.
 In fact, for all quadratic forms in \eqref{eqn:stress_polynomial_Qi} we verified symbolically that $Q_i=0$. 
 Second-order flexibility then followed via \cref{prop:stress-energy-condition}.
    %
    Since at this time no 
    methods exist to test rigidity beyond the second order, we do not know whether the truncated dodecahedron is in fact rigid.
    If it is rigid, it would provide a remarkably natural geometric constraint system demonstrating that rigidity does not imply second-order rigidity. 
    Previous examples of~this distinction have been comparatively ad hoc (\eg\ \cite[Figure 22]{connelly1996second}). 
    If it is flexible, its flex would be fundamentally different from all polytope flexes encountered before (\cf\ \cite[Question 4.2]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
\end{itemize}

Numerical experiments suggest that the first-order flexibility of the three polytopes discussed above is sensitive to small changes in their geometry.
First, applying a generic linear transformation results in first-order rigid polytopes. This is in contrast to how all known flexible polytopes preserve their flexibility under linear transformations (\cf\ \cite[Question 4.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}).
Second, changing the height of truncation in the truncated variants results in first-order rigid polytopes. 
At this time, it is unclear why exactly the realizations with uniform edge lengths are the ones~that end up being first-order flexible.
In particular, these properties cannot be a consequence of the polytopes' symmetry alone.
%\todo{\mhsays{``... symmetry alone according to the discussion above''?}\mwsays{I mean, according to what else? :D} \mhsays{fair}}





\subsection{Comments on rigidity}
\label{sec:rigidity_comments}

Dehn's theorem \cite{dehnstheorem} states that simplicial polytopes (\ie\ where all faces are simplices) are first-order rigid.
\Cref{tab:comparison} and \cref{tab:catalan-comparison} contain plenty of non-simplicial polytopes that are first-order rigid, for example, the~trunca\-ted tetrahedron (\cref{tab:comparison}) or deltoidal icositetrahedron (\cref{tab:catalan-comparison}).
Currently no theo\-retical tools are available that would identify these as rigid a priori.
We therefore formulate the following question:

\begin{question}
    Can Dehn's theorem be extended to some classes of non-simplicial polytopes? 
    That is, can we formulate combinatorial/geometric
    %
    %\notodo{\mhsays{Replace ``/'' by ``or'' or ``and'' in running text (see previous comment).}\mwsays{I think the best replacement would be ``and/or'' xD.} \mhsays{I see. Let's keep it like that.}} 
    %
    criteria for the first-order rigidity of polytopes? % that extend Dehn's theorem?
\end{question}

Perhaps, polytopes whose only faces are triangles and 4-gons form a class simple enough to admit a complete characterization.
See also \cite[Question 4.4.]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%\notodo{\mhsays{The truncated tetrahedron is a counterexample for this claim. Maybe ``... triangles and 4-gons are simple enough to serve as the first step on the way to a complete characterization''?}\mwsays{Truncated tetrahedron has hexagon faces.} \mhsays{Exactly. Therefore, 4-gons and triangles \textbf{cannot} provide a complete characterization of first-order rigidity? Potentially rephrase the sentence if you mean something else.}\mwsays{Better?}}

\subsection{Comments on flexibility}
\label{sec:selected_flexibility}
\label{sec:flexibility_comments}

Save the polytopes of \cref{sec:selected_rigidity}, we have partial explanations for the first-order flex space dimensions listed in \cref{tab:comparison} and \cref{tab:catalan-comparison}.
In all cases, these first-order flexes are explained by actual flexes.
We know~this both from theoretical considerations (see \cref{sec:dimension_estimates}) and the numerically generated flexes provided in the Supplementary Material \cite{zenodo_suppMaterial}.

Remarkably, the lower bounds on the dimensions of the first-order flex spaces obtained in \cref{sec:dimension_estimates} match the computationally obtained values in the tables exactly.
We can conclude that, at least locally at their respective realizations, we have a full understanding of the flexes of these polytopes.

\input{sec/table2}





% \tempnewpage

\pagebreak

\section{Case study: the regular dodecahedron}
\label{sec:dodecahedron}
%\notodo{\mhsays{Is this table position better? Maybe we should discuss this?}\mwsays{Currently I like it}}

Due to its previous status as the guiding example,
%
we single out the dodecahedron once again for a closer inspection.
%
Exploring its realization space close to the regular dodecahedron helps us better understand the source of its exceptional behavior.
%
From that, we draw conclusions about the global rigidity of the polytope.






\subsection{Deformation paths}
\label{section:dodec-edge-length-perturbations}


%
By the Legendre-Steinitz theorem the reduced realization space $\realR(\mathcal{P})$ of the dodecahedron is a smooth $30$-dimensional manifold. 
The dodecahedron is rigid by \Cref{dodecahedronrig}, suggesting that these 30 degrees of freedom translate directly into changes in the lengths of its 30 edges.
Although we formulate the hope that all edge length perturbations of rigid polytopes are realizable in \Cref{conj:edge_length_perturbations}, even for the regular dodecahedron it is completely unclear whether this statement is true.

Due to the dodecahedron's high symmetry (all edges are the same), one might suggest to deform a single edge and, if this is possible, to conclude that arbitrary perturbations are possible.
In this section, we investigate the deformations of the regular dodecahedron induced by shrinking or extending a single edge. 
By approximating such deformation paths using methods explained in \Cref{sec:approx_continuous_motions}, we probe a neighborhood of this polytope $P$ in $\realR(\mathcal P)$. 
However, whether this implies that all edge length perturbations are possible remains unanswered.
%\notodo{\mhsays{``must remain open'' sounds weird.}}

For this experiment, we keep all but one edge length constant at $\ell=1$ throughout the deformation. Denote the non-constant edge length by $\ell^*(t) = 1+t$ with $t\in (-\delta,+\delta)$ for some $\delta>0$ such that $\lvert \delta \lvert~ < 1$. 
Sampling from the realization space intersected with the real algebraic set of prescribed edge lengths (see also \cite{deformationpaths}) reveals \textit{six} distinct arcs starting at the regular dodecahedron corresponding to the shrinking of a single edge and \textit{two} corresponding to its expansion. 

        \begin{figure}[ht]
            \centering
            \includegraphics[width=0.75\linewidth]{Images/DodecahedronCurves_blue.png}
            \caption{Realizations obtained by modifying the length of a single edge of the dodecahedron (central blue circle). Blue curves correspond to edge contractions, whereas gray curves correspond to edge expansions. On these curves, the eight depicted %corresponding 
            realizations are located at $\ell^*(\pm 0.25)$. Four realizations are connected by a nodal cubic (dark blue dashes).}
            \label{fig:edge-contraction-deformation-space}
        \end{figure}
%\notodo{\mhsays{Figure Caption: ``... by perturbing a single edge...'' $\Rightarrow$ ``... by modifying a single edge...''}}
%\notodo{\mhsays{I removed ``corresponding'' from the caption so that it fits on 5 lines. If you're ok with this change, just remove this comment.}\mwsays{Slightly reworded.}}

%
%
In \Cref{fig:edge-contraction-deformation-space}, we depict a random projection of the deformations induced by edge contractions 
(blue) and expansions (gray), alongside eight realizations at $\ell^{\star}(\pm 0.25)$.
Remarkably, it appears that some of these arcs rejoin smoothly. 
For instance, the gray arcs corresponding to an edge expansion have the same tangent in the regular dodecahedron, and so do suitable pairs of arcs of the blue curves. 
Moreover, the arcs corresponding to the four lower-symmetry realizations can be combined to form a nodal cubic curve (dark blue dashed curve).
It is conceivable that for these reasons \Cref{thm:rigidity-and-edge-length-perturbations} does not apply to the regular dodecahedron since there are multiple realizations with the same edge lengths arbitrarily close to this polytopes. 
%\notodo{\mhsays{``close to the regular dodecahedron'' $\Rightarrow$ ``close to this polytope''. Otherwise, we use ``the regular dodecahedron'' twice in the same sentence.}}
Hence, it is possible that in this case there cannot exist a continuous, locally injective map $\psi:\mathbb{R}^E\rightarrow \realR(\mathcal{P})$ such that $\psi(\bs\ell(P))=P$ (\cf\ \Cref{res:square_root_branching}). 
%

In total, three curves are passing through the regular dodecahedron that are induced by length changes of a single edge. 
Numerically computing the derivative in the regular dodecahedron confirms this observation: though naturally, we expect that our numerical calculations are not exact, the respective sum of the tangent vectors is sufficiently close to zero. 
We attach an animation of the smooth deformation passing through the regular dodecahedron on the solid blue path from $\ell^*(-0.25)$ via $\ell^*(0)$ to $\ell^*(-0.25)$ in the Supplementary Material \cite{zenodo_suppMaterial} of this article.

Additionally, we find that in the case of edge contractions there are two types of deformations: those that react to the edge contraction by flattening horizontally (see \Cref{fig:edge-contraction-deformation-space}, top) and those that flatten vertically (see \Cref{fig:edge-contraction-deformation-space}, bottom). Both types contain one realization with two reflection symmetries, and two realizations with only one reflection symmetry that are mutual mirror images of each other. 
        Intriguingly, not all dodecahedra persist until the edge collapses to length zero. 
        The configurations in the bottom left and bottom right are confluent with the configuration in the bottom center at $\approx\ell^{\star}(-0.37194\dots)$, leaving only four configurations below this particular edge length. 
        %
        %
        All of them persist until $\ell^*(-1)=0$. 


        Conversely, expanding an edge only produces two realizations with distinct reflection axes. 
        They are depicted on the left and right of \Cref{fig:edge-contraction-deformation-space}. 
        %
        Despite the dodecahedron's high level of regularity and symmetry, there are more deformation paths for contracting an edge than for expanding it. This behavior is surprising and should be the object of further investigation.



\subsection{Global rigidity}
\label{sec:dodecahedron-global-rigidity}

The results of
\Cref{section:dodec-edge-length-perturbations} provide insight into the concept of global rigidity for convex polytopes.
Recall that a polytope is called \Def{globally rigid} if there exists no other realization of the polytope with the same edge lengths.
%
Clearly, the realizations shown in \cref{fig:edge-contraction-deformation-space} (either on the blue or on the gray curve) are equivalent, that is, have identical edge lengths. None of them is therefore~globally rigid.
%
This observation
%\notodo{\mhsays{``This observation leaves open...''? Reference unclear.}}
leaves open the possibility of generic global rigidity. 

A polytope is called \Def{generically globally rigid} if every generic 
realization is globally rigid \cite{Connelly2005}. Once again, we refer to the notion of genericity introduced in \cite[Definition 5.3]{himmelmannschulzewinter2025rigiditypolytopesedgelength}.
%
First, we confirmed numerically that all of the equivalent realizations which are 
depicted in \cref{fig:edge-contraction-deformation-space} are first-order rigid. 
Using \cref{prop:inf-rigidity-edge-perturbations}, each of these realizations can therefore be perturbed to achieve the same edge lengths as a sufficiently close generic realization of the dodecahedron.
Hence, generic realizations are also not necessarily globally rigid.
%
Notably, the most concrete case remains open:

\begin{question}
    \label{q:global_rigid}
    Is the regular dodecahedron globally rigid? Conversely, does there exist a convex realization of the dodecahedron with all edges of the same length, besides the regular dodecahedron?
\end{question}


It would be surprising, though also not absurd, if other realizations with equal edge lengths exist. Consider, for example, the near miss shown in \cref{fig:dodecahedron_variation} (left, center), whose edge lengths are almost all equal.
An alternative realization, for which all edges have exactly the same length, is the ``flat dodecahedron'' shown in \cref{fig:planar-dodec} (right). It does not lie in $\real(\mathcal{P})$, since $\langle p_i,\,a_\sigma\rangle = 1$ for all $i\sim \sigma$.

\begin{figure}[h!]
    \centering
    \begin{minipage}[c]{0.575\textwidth}
    \includegraphics[width=\linewidth]{Images/dodecahedron_variation.pdf}
    \end{minipage}\hspace*{12mm}
    \begin{minipage}[c]{0.32\textwidth}
    \includegraphics[width=\linewidth]{Images/global_rigidity_dodecahedron.png}
    \end{minipage}
    \caption{The regular dodecahedron (left) and another realization, known as the ``Pyritohedron'', for which all edges have \emph{almost} the same length (center). The blue and black edges have slightly different lengths. Moreover, we depict a 2-dimensional drawing of the dodecahedral graph for which all edges have the same length (right). The flat dodecahedron is a reproduction and is courtesy to Bob Connelly and Simon Guest. }
    \label{fig:dodecahedron_variation}
    \label{fig:planar-dodec}
\end{figure}





\tempnewpage % temporary new page

\section{Conclusion}
\label{sec:outlook}


In this article, we investigate deformations and develop a second-order rigidity theory for polytopes with edge length and coplanarity constraints. 


\subsection{Main results}

We carefully develop a first-order and second-order theory for the rigidity of polytopes in \Cref{sec:first_order,sec:second-order-theory}. 
Using these tools, we demonstrate in \Cref{res:second_order} that second-order rigidity is sufficient for the rigidity of polytopes. 
Using equilibrium stresses, we subsequently develop an effective algorithm for checking second-order rigidity in \Cref{section:second-order-rigidity-check}. 
A well-developed second-order theory is important since it is right at the boundary of what is practically possible: analogous statements are no longer true for naive higher-order rigidity criteria (see \Cref{sec:higher_order_rigidity}). 

For 3-dimensional polytopes, we also investigate the topological properties of the realization space $\real(\mathcal{P})$ by considering the edge length perturbation space. This lets us generate novel conditions for rigidity (\eg\ \Cref{prop:inf-rigidity-edge-perturbations} and \Cref{thm:rigidity-and-edge-length-perturbations}). By applying the numerical curve-tracking scheme from \Cref{sec:approx_continuous_motions}, we generate animations of flexes and the curves induced by edge length modifications.


Using these tools, we characterize the rigidity properties of the five Platonic and 13 Archimedean solids in \Cref{tab:comparison}, and of the 13 Catalan solids in \Cref{tab:catalan-comparison}. Notably, we demonstrate that the regular dodecahedron and the truncated icosahedron  are second-order rigid, even though they are neither first-order rigid, nor prestress stable. Therefore, they represent examples of rigid polytopes, for which the first-order theory is insufficient. 
%\notodo{\mwsays{Sec 9 has changed}\mhsays{Done.}}
In \Cref{sec:so_rigidity_dod}, we explicitly demonstrate a strategy~for proving the second-order rigidity of the regular dodecahedron as a test case. Moreover, we investigate deformations induced by modifying the length of a single edge in \Cref{sec:dodecahedron}, which reveals a highly interesting local geometry and also serves as a counterexample to the generic global rigidity of polytopes.

\subsection{The Truncated Dodecahedron}


Among the 31 polytopes we considered, the truncated dodecahedron is the only one whose rigidity we are unable to determine. We are able to show that this polytope's space of first-order flexes is 4-dimensional, so it is not first-order rigid.
We also determine that it is not second-order rigid, since the associated system of homogeneous quadratic equations $Q_1=\dots=Q_4=0$ arising from \eqref{eqn:stress_polynomial_Qi} has a non-trivial solution. 
In fact, we 
find that all quadratic forms $Q_i$ are identically zero, and hence no first-order flex can be blocked by any stress. 
Still, with our current tools we are not able to distinguish whether it is flexible or rigid.

In \Cref{fig:TDod_flex_conc}, we depict samples from a numerically generated deformation of the truncated dodecahedron.
It is constructed from deforming along first-order flexes of high symmetry and subsequently restoring length and coplanarity constraints by gradient descent with reasonable numerical tolerances.
%
%\todo{\mwsays{The picture could also go into results section} \mhsays{It is a non-result.}}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Tdod_flex.pdf}
    \caption{The Archimedean truncated dodecahedron (left) and two of its potential flexes (middle and right) constructed numerically.}
    \label{fig:TDod_flex_conc}
\end{figure}
%
However, when we apply a more robust numerical scheme (\cf\ \Cref{sec:approx_continuous_motions}) with a tolerance close to machine precision, all of the realizations from the flex visualized in \Cref{fig:TDod_flex_conc} converge back to the maximally symmetric truncated dodecahedron. Therefore, this symmetric deformation is likely not a true flex. 

\subsection{Higher-Order Rigidity}
\label{sec:higher_order_rigidity}
Initial experiments using the energy-based approach for higher-order rigidity of Gortler, Holmes-Cerfon and Theran \cite{gortler2025higherorderrigidityenergy} suggest that the truncated dodecahedron is instead third-order rigid. 
This result would help explain why we are able to find a deformation of the truncated dodecahedron in \Cref{fig:TDod_flex_conc}, which 
satisfies the edge length and facet planarity constraints with reasonably small numerical tolerance but does not hold up to more robust numerical tests. In \cite{gortler2025higherorderrigidityenergy}, the authors observe that the energy landscape around an $N$-th order rigid realization locally looks like the 
polynomial curve $y=x^{2N}$. This implies that, for larger $N$, one would have to deviate relatively far from the original realization to see a noticeable increase in the energy.

If the dimension of the space of first-order flexes is greater than one, there currently exists no effective and conclusive algorithm for checking higher-order rigidity, and we would have to solve infinitely many polynomial optimization problems. It is a problem for future research to apply hierarchies from the polynomial optimization literature (\eg\ Lasserre hierarchy) to limit the number of cases that need to be checked. Solving this issue would lead to an algorithmic framework which would be applicable to various geometric constraint systems across rigidity theory, and not just polytopes. 

